Learning to Extract Distributed Polarization Sensing Data from Noisy Jones Matrices

We consider the problem of recovering spatially resolved polarization information from receiver Jones matrices. We introduce a physics-based learning approach, improving noise resilience compared to previous inverse scattering methods, while highlighting challenges related to model overparameterization.

==> Figs/random_phi_change/failed_case_noise_0.0001.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm, group name=column4 plots }]


%================= Fig1 ===============
\firstgplot{column3}{(d) Overparam.~($\sigma^2_z=0.0001$)}

\plotTrue
table {%
0 0.0245707776166385
1 0.0245707776166385
2 0.0245707776166385
3 0.0245707776166385
4 0.0245707776166385
5 0.0245707776166385
6 0.0245707776166385
7 0.0245707776166385
8 0.0245707776166385
9 0.0245707776166385
10 0.0245707776166385
11 0.0245707776166385
12 0.0245707776166385
13 0.0245707776166385
14 0.0245707776166385
15 0.0245707776166385
16 0.0245707776166385
17 0.0245707776166385
18 0.0245707776166385
19 0.0245707776166385
20 0.0245707776166385
21 0.0245707776166385
22 0.0245707776166385
23 0.0245707776166385
24 0.0245707776166385
25 0.0245707776166385
26 0.0245707776166385
27 0.0245707776166385
28 0.0245707776166385
29 0.0245707776166385
30 0.0245707776166385
31 0.0245707776166385
32 0.0245707776166385
33 0.0245707776166385
34 0.0245707776166385
35 0.0245707776166385
36 0.0245707776166385
37 0.0245707776166385
38 0.0245707776166385
39 0.0245707776166385
40 0.0245707776166385
41 0.0245707776166385
42 0.0245707776166385
43 0.0245707776166385
44 0.0245707776166385
45 0.0245707776166385
46 0.0245707776166385
47 0.0245707776166385
48 0.0245707776166385
49 0.0245707776166385
50 0.0245707776166385
51 0.0245707776166385
52 0.0245707776166385
53 0.0245707776166385
54 0.0245707776166385
55 0.0245707776166385
56 0.0245707776166385
57 0.0245707776166385
58 0.0245707776166385
59 0.0245707776166385
60 0.0245707776166385
61 0.0245707776166385
62 0.0245707776166385
63 0.0245707776166385
64 0.0245707776166385
65 0.0245707776166385
66 0.0245707776166385
67 0.0245707776166385
68 0.0245707776166385
69 0.0245707776166385
70 0.0245707776166385
71 0.0245707776166385
72 0.0245707776166385
73 0.0245707776166385
74 0.0245707776166385
75 0.0245707776166385
76 0.0245707776166385
77 0.0245707776166385
78 0.0245707776166385
79 0.0245707776166385
80 0.0245707776166385
81 0.0245707776166385
82 0.0245707776166385
83 0.0245707776166385
84 0.0245707776166385
85 0.0245707776166385
86 0.0245707776166385
87 0.0245707776166385
88 0.0245707776166385
89 0.0245707776166385
90 0.0245707776166385
91 0.0245707776166385
92 0.0245707776166385
93 0.0245707776166385
94 0.0245707776166385
95 0.0245707776166385
96 0.0245707776166385
97 0.0245707776166385
98 0.0245707776166385
99 0.0245707776166385
};
\plotNetwork
table {%
0 0.994391001904268
1 0.993590825410883
2 0.992023489465153
3 0.990713486320866
4 0.991419552162517
5 0.989441351270044
6 0.985967987035861
7 0.986591439748254
8 0.984670286347738
9 0.986597615414255
10 0.979080746438938
11 0.936462525974394
12 0.958460205980893
13 0.977461709767043
14 0.926143567044687
15 0.969877221779873
16 0.925972885044056
17 0.97643929816115
18 0.88611663820043
19 0.917625243931487
20 0.877145740184788
21 0.953381472009079
22 0.974847852348981
23 0.927111812334532
24 0.934531518335522
25 0.980827984776332
26 0.739449302714185
27 0.0165268251851707
28 0.0242172410413297
29 0.00721320476851423
30 0.0570705396937386
31 0.0713426995687485
32 0.117299555830363
33 0.135229538847016
34 0.063600727763936
35 0.0706248524204548
36 0.119392320335038
37 0.0381834501022485
38 0.0255290641058863
39 0.117753979288055
40 0.0117760812682947
41 0.0436763182753637
42 0.0363630434644735
43 0.0823891634208204
44 0.0360113232634925
45 0.155558850091638
46 0.269960569866067
47 0.19046165186407
48 0.20123595690344
49 0.215823860533451
50 0.214196769809024
51 0.164617758683008
52 0.136165602457356
53 0.130171659975048
54 0.170701750460507
55 0.190553967781076
56 0.0990810814671496
57 0.0853072985246207
58 0.0969155607001727
59 0.09353936753321
60 0.0349658762122373
61 0.130589459020042
62 0.398867311071014
63 0.244857360686911
64 0.00909265722371248
65 0.113311248326232
66 0.109276162333659
67 0.167700735509685
68 0.0823485802881675
69 0.0144209031988826
70 0.00617759899796809
71 0.0230910450464928
72 0.0171292712908548
73 0.000829106975726176
74 0.0708381570410189
75 0.0779399967969744
76 0.010724288558744
77 0.0133747985210881
78 0.046208956696191
79 0.0379587511395605
80 0.0289124910834945
81 0.0319568722933578
82 0.0236896821174848
83 0.0271253953733398
84 0.0228206963786261
85 0.0298576086148561
86 0.0265755521574235
87 0.0318396664205288
88 0.0255345841104967
89 0.0245550493549986
90 0.0230087042339706
91 0.0238996101735972
92 0.0257473363806445
93 0.0235924636438903
94 0.0306389142081135
95 0.0275012346579162
96 0.0202740045058776
97 0.0279627903401782
98 0.0242651126117082
99 0.0237469148287655
};
\plotInvscat
table {%
0 0.969182074069977
1 0.976240277290344
2 0.959551930427551
3 0.976244568824768
4 0.966413378715515
5 0.915303528308868
6 0.961997985839844
7 0.952916920185089
8 0.976226449012756
9 0.97721666097641
10 0.965310633182526
11 0.989404678344727
12 0.967788100242615
13 0.977948665618896
14 0.966520845890045
15 0.938928544521332
16 0.980758488178253
17 0.969111382961273
18 0.983753502368927
19 0.875054657459259
20 0.980845510959625
21 0.911844849586487
22 0.964713215827942
23 0.953747570514679
24 0.954650819301605
25 0.927320778369904
26 0.83820778131485
27 0.864595830440521
28 0.802489519119263
29 0.978740811347961
30 0.976535499095917
31 0.992749154567719
32 0.961867928504944
33 0.976606249809265
34 0.987753331661224
35 0.97024929523468
36 0.956831395626068
37 0.954851031303406
38 0.960090398788452
39 0.9508096575737
40 0.947561144828796
41 0.951627671718597
42 0.957270741462708
43 0.977704346179962
44 0.948898375034332
45 0.951896965503693
46 0.964131832122803
47 0.95647794008255
48 0.969967603683472
49 0.974561095237732
50 0.938155770301819
51 0.960932791233063
52 0.977557003498077
53 0.965994536876678
54 0.963357090950012
55 0.960285186767578
56 0.952984511852264
57 0.970089495182037
58 0.946129381656647
59 0.962903797626495
60 0.96126663684845
61 0.96542090177536
62 0.983666598796844
63 0.96205997467041
64 0.920154333114624
65 0.980610430240631
66 0.953224003314972
67 0.954712092876434
68 0.976130962371826
69 0.979389607906342
70 0.944278955459595
71 0.954823315143585
72 0.912834644317627
73 0.995994448661804
74 0.981224000453949
75 0.911551058292389
76 0.953721821308136
77 0.564257860183716
78 0.985868275165558
79 0.990012347698212
80 0.454087495803833
81 0.933582186698914
82 0.540674388408661
83 0.795141100883484
84 0.879168927669525
85 0.597076117992401
86 0.713367462158203
87 0.926122903823853
88 0.719994246959686
89 0.485396146774292
90 0.446164488792419
91 0.402833968400955
92 0.540696799755096
93 0.470048189163208
94 0.66285765171051
95 0.916391730308533
96 0.724520206451416
97 0.466566860675812
98 0.575414419174194
99 0.742052435874939
};
%================= Fig2 ===============
\nextgplot
\perturbation
\plotTrue
table {%
0 0.0796525557961304
1 0.0796525557961304
2 0.0796525557961304
3 0.0796525557961304
4 0.0796525557961304
5 0.0796525557961304
6 0.0796525557961304
7 0.0796525557961304
8 0.0796525557961304
9 0.0796525557961304
10 0.0953390684937343
11 0.15832830576006
12 0.074209401453014
13 0.0562947809910471
14 0.162434262577782
15 0.0786592992134329
16 0.153351841476454
17 0.0136003632408747
18 0.208244430342285
19 0.18081998010704
20 0.211445263738759
21 0.0754756573444908
22 0.0432501349440016
23 0.156436015696073
24 0.151514144877208
25 0.0153455234228614
26 0.298540346423877
27 0.487245563193296
28 0.603424467791033
29 0.356885009163709
30 0.069825690280223
31 0.154077443386182
32 0.0763726458331348
33 0.102949683606279
34 0.160947370932029
35 0.110704182221555
36 0.110704182221555
37 0.110704182221555
38 0.110704182221555
39 0.110704182221555
40 0.110704182221555
41 0.110704182221555
42 0.110704182221555
43 0.110704182221555
44 0.110704182221555
45 0.110704182221555
46 0.110704182221555
47 0.110704182221555
48 0.110704182221555
49 0.110704182221555
50 0.110704182221555
51 0.110704182221555
52 0.110704182221555
53 0.110704182221555
54 0.110704182221555
55 0.110704182221555
56 0.110704182221555
57 0.110704182221555
58 0.110704182221555
59 0.110704182221555
60 0.193661287426511
61 0.0803753808702726
62 0.0257047272872711
63 0.118819359556358
64 0.255987723568507
65 0.0955916742771348
66 0.182784163039924
67 0.0655266653203569
68 0.206381201989831
69 0.284512392515153
70 0.218322327184057
71 0.375144959696964
72 0.42583356095422
73 0.243673761433346
74 0.0903863218027377
75 0.189806921627192
76 0.287293515789283
77 0.44573950826256
78 0.358621371350008
79 0.494057774762813
80 0.62592654012827
81 0.638080318265771
82 0.860766977102702
83 0.733276116307116
84 0.689815196333366
85 0.844547463002903
86 0.844547463002903
87 0.844547463002903
88 0.844547463002903
89 0.844547463002903
90 0.844547463002903
91 0.844547463002903
92 0.844547463002903
93 0.844547463002903
94 0.844547463002903
95 0.844547463002903
96 0.844547463002903
97 0.844547463002903
98 0.844547463002903
99 0.844547463002903
};
\plotNetwork
table {%
0 0.257945483991187
1 0.24608705635515
2 0.23588472652703
3 0.230562227110413
4 0.228766139251353
5 0.220835935458193
6 0.21936799480507
7 0.223070656974481
8 0.218266840289634
9 0.220114110866727
10 0.21524036224036
11 0.210775829148594
12 0.281785009382861
13 0.229384735848463
14 0.203416198476246
15 0.255592632819104
16 0.207026092801937
17 0.246262786496357
18 0.214448052992344
19 0.20776099049095
20 0.208600760402903
21 0.28652865578402
22 0.239748531310314
23 0.205471457656717
24 0.208320712691165
25 0.245300190532203
26 0.235385024979685
27 0.483899846488648
28 0.601754638241767
29 0.349700115270201
30 0.0683485591237702
31 0.149914071827525
32 0.0769744745127422
33 0.10229253602999
34 0.155373614011904
35 0.108070956035012
36 0.108086806919118
37 0.108798004494907
38 0.108460814183097
39 0.104542275317033
40 0.114319042029842
41 0.108801125561445
42 0.109554442016004
43 0.111597135006452
44 0.111719497079811
45 0.106974194643751
46 0.104082300873252
47 0.106813814987101
48 0.106141842062682
49 0.105082961044352
50 0.107655704519757
51 0.106987387873371
52 0.112099665389489
53 0.105733060979819
54 0.108653969095671
55 0.108221091178659
56 0.110445081467686
57 0.107311007545421
58 0.110520073970958
59 0.107431206402945
60 0.190509667541613
61 0.0736648823322855
62 0.0222263473666977
63 0.11003186498779
64 0.253212377202433
65 0.0922907892004
66 0.18036490832037
67 0.0641376949054551
68 0.200695294407503
69 0.280696689773622
70 0.216386730741523
71 0.375230201951646
72 0.424907309256999
73 0.237541965169586
74 0.0884178885370846
75 0.193667472577915
76 0.286242307136572
77 0.440291991270286
78 0.362709209881198
79 0.495914470522185
80 0.625656701554437
81 0.636397668631127
82 0.860645422705288
83 0.73232702543739
84 0.68877908003226
85 0.843292198116125
86 0.843878145083434
87 0.845055341302422
88 0.844950751045094
89 0.844709428606303
90 0.842357683692036
91 0.844775096596347
92 0.843733403187634
93 0.844790844624001
94 0.847749044818676
95 0.846113376120151
96 0.843753687797669
97 0.845659244646935
98 0.845154060576915
99 0.845317413997551
};
\plotInvscat
table {%
0 0.263804703950882
1 0.276769697666168
2 0.257909625768661
3 0.228806510567665
4 0.259206980466843
5 0.237914368510246
6 0.266375303268433
7 0.273920714855194
8 0.257651507854462
9 0.264161378145218
10 0.301670789718628
11 0.2932348549366
12 0.272649556398392
13 0.264174580574036
14 0.303663522005081
15 0.274351984262466
16 0.38533017039299
17 0.265907973051071
18 0.284508615732193
19 0.324039876461029
20 0.320102959871292
21 0.248298346996307
22 0.278807431459427
23 0.229680016636848
24 0.293307900428772
25 0.13981431722641
26 0.321974486112595
27 0.504577875137329
28 0.532053411006927
29 0.464271783828735
30 0.22796830534935
31 0.256818056106567
32 0.26346144080162
33 0.265323311090469
34 0.335535049438477
35 0.265698224306107
36 0.274710536003113
37 0.269968718290329
38 0.271023869514465
39 0.268409132957458
40 0.28764995932579
41 0.297730833292007
42 0.263902187347412
43 0.274656563997269
44 0.2599276304245
45 0.270490229129791
46 0.245884016156197
47 0.266092270612717
48 0.260706722736359
49 0.270478665828705
50 0.299232095479965
51 0.275221824645996
52 0.253532707691193
53 0.264811098575592
54 0.273413896560669
55 0.279544144868851
56 0.324920386075974
57 0.271491318941116
58 0.287515670061111
59 0.281277924776077
60 0.33710128068924
61 0.284177988767624
62 0.260694444179535
63 0.265727281570435
64 0.336457401514053
65 0.227838292717934
66 0.322998076677322
67 0.278729468584061
68 0.411367475986481
69 0.369873344898224
70 0.259613484144211
71 0.476468026638031
72 0.523672878742218
73 0.294351786375046
74 0.252061814069748
75 0.279117196798325
76 0.334571272134781
77 0.366232335567474
78 0.398353517055511
79 0.690429508686066
80 0.528174459934235
81 0.644400775432587
82 0.432781994342804
83 0.586021244525909
84 0.483237862586975
85 0.512553095817566
86 0.50925475358963
87 0.545404195785522
88 0.483592689037323
89 0.5296710729599
90 0.392950266599655
91 0.486143261194229
92 0.481059700250626
93 0.466647952795029
94 0.50713312625885
95 0.493383020162582
96 0.483377814292908
97 0.466277420520782
98 0.436066657304764
99 0.558471858501434
};
%================= Fig3 ===============
\nextgplot
\plotTrue
table {%
0 0.963992089322708
1 0.963992089322708
2 0.963992089322708
3 0.963992089322708
4 0.963992089322708
5 0.963992089322708
6 0.963992089322708
7 0.963992089322708
8 0.963992089322708
9 0.963992089322708
10 0.963992089322708
11 0.963992089322708
12 0.963992089322708
13 0.963992089322708
14 0.963992089322708
15 0.963992089322708
16 0.963992089322708
17 0.963992089322708
18 0.963992089322708
19 0.963992089322708
20 0.963992089322708
21 0.963992089322708
22 0.963992089322708
23 0.963992089322708
24 0.963992089322708
25 0.963992089322708
26 0.963992089322708
27 0.963992089322708
28 0.963992089322708
29 0.963992089322708
30 0.963992089322708
31 0.963992089322708
32 0.963992089322708
33 0.963992089322708
34 0.963992089322708
35 0.963992089322708
36 0.963992089322708
37 0.963992089322708
38 0.963992089322708
39 0.963992089322708
40 0.963992089322708
41 0.963992089322708
42 0.963992089322708
43 0.963992089322708
44 0.963992089322708
45 0.963992089322708
46 0.963992089322708
47 0.963992089322708
48 0.963992089322708
49 0.963992089322708
50 0.963992089322708
51 0.963992089322708
52 0.963992089322708
53 0.963992089322708
54 0.963992089322708
55 0.963992089322708
56 0.963992089322708
57 0.963992089322708
58 0.963992089322708
59 0.963992089322708
60 0.963992089322708
61 0.963992089322708
62 0.963992089322708
63 0.963992089322708
64 0.963992089322708
65 0.963992089322708
66 0.963992089322708
67 0.963992089322708
68 0.963992089322708
69 0.963992089322708
70 0.963992089322708
71 0.963992089322708
72 0.963992089322708
73 0.963992089322708
74 0.963992089322708
75 0.963992089322708
76 0.963992089322708
77 0.963992089322708
78 0.963992089322708
79 0.963992089322708
80 0.963992089322708
81 0.963992089322708
82 0.963992089322708
83 0.963992089322708
84 0.963992089322708
85 0.963992089322708
86 0.963992089322708
87 0.963992089322708
88 0.963992089322708
89 0.963992089322708
90 0.963992089322708
91 0.963992089322708
92 0.963992089322708
93 0.963992089322708
94 0.963992089322708
95 0.963992089322708
96 0.963992089322708
97 0.963992089322708
98 0.963992089322708
99 0.963992089322708
};
\plotNetwork
table {%
0 0.6761837411735
1 0.720091239931864
2 0.743425742575201
3 0.769317698742847
4 0.788788397904203
5 0.805633601043022
6 0.8257483205579
7 0.840968353737627
8 0.83729944311677
9 0.837704646580398
10 0.871819205424068
11 0.955763814126645
12 0.725796202298764
13 0.810989094524957
14 0.960468340960738
15 0.747056147731065
16 0.956460628803193
17 0.691712130523213
18 0.986162364562819
19 0.971200182305468
20 0.9893004628705
21 0.707374248265803
22 0.813849224483072
23 0.962073364603083
24 0.954560310923881
25 0.623592574437667
26 0.991246469194614
27 0.967813471494019
28 0.962436531485868
29 0.973854668017629
30 0.96961353308943
31 0.986056580556829
32 0.987358510568494
33 0.963597135388234
34 0.963420809095722
35 0.968718947530883
36 0.965546076238579
37 0.966724732258919
38 0.967240439618621
39 0.96761885642124
40 0.966400017945669
41 0.969807038444258
42 0.964025103962062
43 0.956399466900395
44 0.965984428255144
45 0.965156201005135
46 0.955576451091169
47 0.962426646915018
48 0.963228586040279
49 0.958094744869886
50 0.955343622465046
51 0.9623315025297
52 0.963699583635504
53 0.967919686082827
54 0.963052654306211
55 0.962601973200073
56 0.965006599236274
57 0.965438234285793
58 0.967240139556482
59 0.968065694690495
60 0.982174974790607
61 0.987222318336108
62 0.947494564326556
63 0.964714470799831
64 0.961789745100481
65 0.97147085392911
66 0.992559102948218
67 0.983156917512598
68 0.992144736241131
69 0.968333343301744
70 0.973502846460365
71 0.962976742958277
72 0.965977382568075
73 0.972198090344432
74 0.98276807989809
75 0.944116874313882
76 0.9706989139793
77 0.970026499782992
78 0.951734020150807
79 0.957915630062141
80 0.964147129860777
81 0.958322914565908
82 0.961802769018187
83 0.962816029078073
84 0.967038661654897
85 0.959379717925624
86 0.964385149140831
87 0.960058052231478
88 0.963250503184939
89 0.964185458699535
90 0.965001402219217
91 0.963076915933817
92 0.965819221729039
93 0.962099864966485
94 0.957816363367899
95 0.962504003110192
96 0.964973724951439
97 0.962264192216133
98 0.965793072193949
99 0.963378447372591
};
\plotInvscat
table {%
0 0.95821624994278
1 0.736408710479736
2 0.919333457946777
3 0.467130303382874
4 0.504831433296204
5 0.407972365617752
6 0.940692245960236
7 0.712833344936371
8 0.816754639148712
9 0.830506265163422
10 0.467214196920395
11 0.436853766441345
12 0.782279789447784
13 0.880033254623413
14 0.805629909038544
15 0.206221953034401
16 0.141293972730637
17 0.564785182476044
18 0.930589973926544
19 0.891399264335632
20 0.540598034858704
21 0.412613660097122
22 0.633056342601776
23 0.521649301052094
24 0.981374800205231
25 0.0930530354380608
26 0.263046234846115
27 0.510432064533234
28 0.41733255982399
29 0.46825122833252
30 0.251878499984741
31 0.770939528942108
32 0.725094556808472
33 0.550104558467865
34 0.179101228713989
35 0.807236969470978
36 0.609011650085449
37 0.232626467943192
38 0.99925822019577
39 0.519873261451721
40 0.533807337284088
41 0.570052087306976
42 0.654709994792938
43 0.701563000679016
44 0.908403396606445
45 0.746540248394012
46 0.609906852245331
47 0.97189873456955
48 0.642430484294891
49 0.864175200462341
50 0.543405711650848
51 0.969177603721619
52 0.648393929004669
53 0.838748097419739
54 0.834661841392517
55 0.857539296150208
56 0.220683231949806
57 0.884952664375305
58 0.752937197685242
59 0.78791344165802
60 0.423405557870865
61 0.659443438053131
62 0.820914149284363
63 0.611216187477112
64 0.934934854507446
65 0.250591576099396
66 0.577692568302155
67 0.671850442886353
68 0.212632119655609
69 0.937262058258057
70 0.648382127285004
71 0.54257345199585
72 0.86626261472702
73 0.604395985603333
74 0.871331989765167
75 0.304278820753098
76 0.991322040557861
77 0.659083425998688
78 0.377029895782471
79 0.323786526918411
80 0.813436567783356
81 0.498794764280319
82 0.50571346282959
83 0.556605756282806
84 0.711707293987274
85 0.472226142883301
86 0.475496768951416
87 0.481912344694138
88 0.481186866760254
89 0.4618821144104
90 0.515771329402924
91 0.457651227712631
92 0.487068772315979
93 0.529647588729858
94 0.490212291479111
95 0.463726550340652
96 0.527878940105438
97 0.561855554580688
98 0.482744842767715
99 0.615122497081757
};

%================= Fig4 ===============
\nextgplot
\plotTrue
table {%
0 0.260667597303856
1 0.260667597303856
2 0.260667597303856
3 0.260667597303856
4 0.260667597303856
5 0.260667597303856
6 0.260667597303856
7 0.260667597303856
8 0.260667597303856
9 0.260667597303856
10 0.260667597303856
11 0.260667597303856
12 0.260667597303856
13 0.260667597303856
14 0.260667597303856
15 0.260667597303856
16 0.260667597303856
17 0.260667597303856
18 0.260667597303856
19 0.260667597303856
20 0.260667597303856
21 0.260667597303856
22 0.260667597303856
23 0.260667597303856
24 0.260667597303856
25 0.260667597303856
26 0.260667597303856
27 0.260667597303856
28 0.260667597303856
29 0.260667597303856
30 0.260667597303856
31 0.260667597303856
32 0.260667597303856
33 0.260667597303856
34 0.260667597303856
35 0.260667597303856
36 0.260667597303856
37 0.260667597303856
38 0.260667597303856
39 0.260667597303856
40 0.260667597303856
41 0.260667597303856
42 0.260667597303856
43 0.260667597303856
44 0.260667597303856
45 0.260667597303856
46 0.260667597303856
47 0.260667597303856
48 0.260667597303856
49 0.260667597303856
50 0.260667597303856
51 0.260667597303856
52 0.260667597303856
53 0.260667597303856
54 0.260667597303856
55 0.260667597303856
56 0.260667597303856
57 0.260667597303856
58 0.260667597303856
59 0.260667597303856
60 0.260667597303856
61 0.260667597303856
62 0.260667597303856
63 0.260667597303856
64 0.260667597303856
65 0.260667597303856
66 0.260667597303856
67 0.260667597303856
68 0.260667597303856
69 0.260667597303856
70 0.260667597303856
71 0.260667597303856
72 0.260667597303856
73 0.260667597303856
74 0.260667597303856
75 0.260667597303856
76 0.260667597303856
77 0.260667597303856
78 0.260667597303856
79 0.260667597303856
80 0.260667597303856
81 0.260667597303856
82 0.260667597303856
83 0.260667597303856
84 0.260667597303856
85 0.260667597303856
86 0.260667597303856
87 0.260667597303856
88 0.260667597303856
89 0.260667597303856
90 0.260667597303856
91 0.260667597303856
92 0.260667597303856
93 0.260667597303856
94 0.260667597303856
95 0.260667597303856
96 0.260667597303856
97 0.260667597303856
98 0.260667597303856
99 0.260667597303856
};
\plotNetwork
table {%
0 0.154320601243664
1 0.136369312377108
2 0.134848200511106
3 0.131556932119175
4 0.12037097448813
5 0.127482966462895
6 0.120891948791605
7 0.112814608374666
8 0.117800423519341
9 0.115677698210571
10 0.130744351334353
11 0.189661330812228
12 0.101805833049912
13 0.0754235017368128
14 0.193821036611285
15 0.115124454390183
16 0.183974321649934
17 0.0258005675670521
18 0.229413449796778
19 0.206288881286175
20 0.228271731176941
21 0.100929604385163
22 0.05667731150673
23 0.188537255690372
24 0.182800471608134
25 0.0378383829175005
26 0.282453956115146
27 0.258021559618386
28 0.259119985045886
29 0.255963073992688
30 0.262258177445772
31 0.255465531248516
32 0.255829617764322
33 0.272478770643131
34 0.269976913836945
35 0.268300048289151
36 0.272191643192585
37 0.259915593982474
38 0.26263023705972
39 0.268264696522098
40 0.262993551823365
41 0.264162228414133
42 0.25797901745466
43 0.259682301730121
44 0.262463587626768
45 0.273183381657754
46 0.277904446205794
47 0.269902019812102
48 0.277042175246349
49 0.275844049215702
50 0.271615931641971
51 0.272514326495965
52 0.269166129005442
53 0.265268253869881
54 0.269156652374411
55 0.272607889854103
56 0.270023907029548
57 0.268469106806165
58 0.26893873943306
59 0.26670799009989
60 0.257969072954165
61 0.256771843487892
62 0.256536828156207
63 0.27432941474193
64 0.26734960506936
65 0.267428225414161
66 0.252613863697755
67 0.258562019701212
68 0.251080341291037
69 0.263167280725584
70 0.263443634628379
71 0.262221702177494
72 0.259798319057261
73 0.257097170535305
74 0.252467887200966
75 0.267205448570434
76 0.258189891242548
77 0.258317452825638
78 0.264139038248035
79 0.268037055339671
80 0.257560146400762
81 0.263752976374354
82 0.262150568497982
83 0.262424795237174
84 0.260492887263483
85 0.260822555578505
86 0.261154317320704
87 0.262122496280406
88 0.26431359912606
89 0.262355037669727
90 0.258829854417569
91 0.258064652452597
92 0.256821274941783
93 0.262516960226365
94 0.265024863592201
95 0.259193133955929
96 0.259541349188038
97 0.263001756678464
98 0.261437791055494
99 0.261640807698319
};
\plotInvscat
table {%
0 0.0180447287857533
1 0.0409614108502865
2 0.0303216427564621
3 0.0451742857694626
4 0.0246679037809372
5 0.0462200865149498
6 0.0167431589215994
7 0.041748471558094
8 0.0198766458779573
9 0.0198462530970573
10 0.0493126548826694
11 0.082231231033802
12 0.0346246138215065
13 0.0241866800934076
14 0.0499453507363796
15 0.0539971552789211
16 0.160215392708778
17 0.0228943321853876
18 0.0614748001098633
19 0.0545553043484688
20 0.0634443387389183
21 0.055873055011034
22 0.0293090529739857
23 0.0633535608649254
24 0.0527754537761211
25 0.395081639289856
26 0.283606886863708
27 0.258885949850082
28 0.492926567792892
29 0.18927338719368
30 0.116972900927067
31 0.0585777647793293
32 0.0281218606978655
33 0.0470310188829899
34 0.140136763453484
35 0.025875823572278
36 0.0445579960942268
37 0.0629940330982208
38 0.0208416823297739
39 0.0252350438386202
40 0.0386053174734116
41 0.0497029423713684
42 0.0367074236273766
43 0.02809171192348
44 0.0356036685407162
45 0.034818209707737
46 0.0310605112463236
47 0.0421408005058765
48 0.0353397876024246
49 0.0345092862844467
50 0.0488747321069241
51 0.0249429550021887
52 0.0263547617942095
53 0.0274151023477316
54 0.0158402696251869
55 0.031040970236063
56 0.06196179240942
57 0.0415473021566868
58 0.0303908716887236
59 0.0406664945185184
60 0.0556754767894745
61 0.0338261388242245
62 0.0165420807898045
63 0.0376735404133797
64 0.0789454653859138
65 0.0538027696311474
66 0.063243992626667
67 0.0240422412753105
68 0.134882584214211
69 0.0956785380840302
70 0.0612832345068455
71 0.145844593644142
72 0.232368499040604
73 0.0877287536859512
74 0.0266542304307222
75 0.120588131248951
76 0.0924768894910812
77 0.274107098579407
78 0.228822723031044
79 0.438722103834152
80 0.412020355463028
81 0.435457289218903
82 0.47108393907547
83 0.485562354326248
84 0.452389627695084
85 0.505009829998016
86 0.432421058416367
87 0.41338786482811
88 0.404444754123688
89 0.308612257242203
90 0.461412400007248
91 0.22475691139698
92 0.493244558572769
93 0.486399590969086
94 0.505401611328125
95 0.493745535612106
96 0.452590763568878
97 0.47648099064827
98 0.450847387313843
99 0.446504771709442
};
%================= Fig5 ===============
\lastgplot
\plotTrue
table {%
0 0.737354162123236
1 0.737354162123236
2 0.737354162123236
3 0.737354162123236
4 0.737354162123236
5 0.737354162123236
6 0.737354162123236
7 0.737354162123236
8 0.737354162123236
9 0.737354162123236
10 0.737354162123236
11 0.737354162123236
12 0.737354162123236
13 0.737354162123236
14 0.737354162123236
15 0.737354162123236
16 0.737354162123236
17 0.737354162123236
18 0.737354162123236
19 0.737354162123236
20 0.737354162123236
21 0.737354162123236
22 0.737354162123236
23 0.737354162123236
24 0.737354162123236
25 0.737354162123236
26 0.737354162123236
27 0.737354162123236
28 0.737354162123236
29 0.737354162123236
30 0.737354162123236
31 0.737354162123236
32 0.737354162123236
33 0.737354162123236
34 0.737354162123236
35 0.737354162123236
36 0.737354162123236
37 0.737354162123236
38 0.737354162123236
39 0.737354162123236
40 0.737354162123236
41 0.737354162123236
42 0.737354162123236
43 0.737354162123236
44 0.737354162123236
45 0.737354162123236
46 0.737354162123236
47 0.737354162123236
48 0.737354162123236
49 0.737354162123236
50 0.737354162123236
51 0.737354162123236
52 0.737354162123236
53 0.737354162123236
54 0.737354162123236
55 0.737354162123236
56 0.737354162123236
57 0.737354162123236
58 0.737354162123236
59 0.737354162123236
60 0.737354162123236
61 0.737354162123236
62 0.737354162123236
63 0.737354162123236
64 0.737354162123236
65 0.737354162123236
66 0.737354162123236
67 0.737354162123236
68 0.737354162123236
69 0.737354162123236
70 0.737354162123236
71 0.737354162123236
72 0.737354162123236
73 0.737354162123236
74 0.737354162123236
75 0.737354162123236
76 0.737354162123236
77 0.737354162123236
78 0.737354162123236
79 0.737354162123236
80 0.737354162123236
81 0.737354162123236
82 0.737354162123236
83 0.737354162123236
84 0.737354162123236
85 0.737354162123236
86 0.737354162123236
87 0.737354162123236
88 0.737354162123236
89 0.737354162123236
90 0.737354162123236
91 0.737354162123236
92 0.737354162123236
93 0.737354162123236
94 0.737354162123236
95 0.737354162123236
96 0.737354162123236
97 0.737354162123236
98 0.737354162123236
99 0.737354162123236
};
\plotNetwork
table {%
0 0.742478787261134
1 0.709861658941487
2 0.682963039625374
3 0.653114098686505
4 0.639250038555783
5 0.605989210263315
6 0.581210349023337
7 0.564412814542122
8 0.559554788622561
9 0.543950179949743
10 0.520945428897702
11 0.47280510172621
12 0.178277919075078
13 0.35142826424158
14 0.392076834369822
15 0.0253530989678811
16 0.383655693452258
17 0.47486475818124
18 0.457011094880224
19 0.45605013653967
20 0.442972104202858
21 0.183958941518744
22 0.339112806160182
23 0.407159936023783
24 0.429409276891679
25 0.586327233358207
26 0.380528492775121
27 0.743246337646154
28 0.733183959737457
29 0.757703273177739
30 0.720397490859259
31 0.772837020703683
32 0.770726554161786
33 0.692801410931225
34 0.697967825213624
35 0.719690921178351
36 0.692369988575462
37 0.718238915815486
38 0.72814212165375
39 0.696483158043621
40 0.735545923510031
41 0.725835352637937
42 0.742039577565949
43 0.751213152590621
44 0.717468442612497
45 0.692606849765448
46 0.658917644855301
47 0.675709060325561
48 0.674710854122239
49 0.671185282681503
50 0.662903720021989
51 0.680654141242616
52 0.690857328355318
53 0.695205381858397
54 0.680243807137102
55 0.673063820625834
56 0.698466460515718
57 0.702173486167672
58 0.702844794978858
59 0.705662106875723
60 0.768956928666655
61 0.770120881620133
62 0.761995977118265
63 0.659147024267325
64 0.716776503782624
65 0.713824390149453
66 0.799905018366263
67 0.769733274347379
68 0.798745193801343
69 0.743846406319778
70 0.756815772843163
71 0.73578728196424
72 0.739346153367216
73 0.749079934186152
74 0.761076156158828
75 0.711129655391568
76 0.751017708023783
77 0.750548711057696
78 0.713288135602864
79 0.723260310356199
80 0.738505859480298
81 0.724979686975786
82 0.732669551878711
83 0.738020066493313
84 0.743840212628267
85 0.725251702122603
86 0.739616852921389
87 0.731429108036995
88 0.735828307755891
89 0.739506600933413
90 0.73489440013389
91 0.732594362452531
92 0.741075723379381
93 0.731264793257664
94 0.721511551912043
95 0.726665144543622
96 0.742103314017784
97 0.734340056385995
98 0.741571631524701
99 0.737744349767787
};
\plotInvscat
table {%
0 0.728237569332123
1 0.630641937255859
2 0.629461109638214
3 0.577544867992401
4 0.375148922204971
5 0.78435868024826
6 0.70535147190094
7 0.877840340137482
8 0.530405938625336
9 0.537621557712555
10 0.688578963279724
11 0.763240158557892
12 0.579296231269836
13 0.612863481044769
14 0.600334167480469
15 0.771778762340546
16 0.68986451625824
17 0.426485538482666
18 0.782626450061798
19 0.712275147438049
20 0.645944893360138
21 0.717006266117096
22 0.314870923757553
23 0.709199905395508
24 0.795690715312958
25 0.705492436885834
26 0.824418246746063
27 0.642326176166534
28 0.756206154823303
29 0.650830030441284
30 0.784879148006439
31 0.643692910671234
32 0.601231157779694
33 0.588945746421814
34 0.714015007019043
35 0.514716148376465
36 0.820708096027374
37 0.647423207759857
38 0.667258203029633
39 0.670579969882965
40 0.7122722864151
41 0.862009584903717
42 0.635596513748169
43 0.741009473800659
44 0.803696513175964
45 0.695409774780273
46 0.637110888957977
47 0.840144455432892
48 0.524664640426636
49 0.540545105934143
50 0.835602521896362
51 0.604630172252655
52 0.4866603910923
53 0.919659078121185
54 0.333785086870193
55 0.65137904882431
56 0.573119938373566
57 0.651283204555511
58 0.729602038860321
59 0.576328337192535
60 0.632863223552704
61 0.741091132164001
62 0.716103374958038
63 0.633393466472626
64 0.818655431270599
65 0.744399011135101
66 0.661736488342285
67 0.575340628623962
68 0.761913299560547
69 0.345318108797073
70 0.567408561706543
71 0.401173412799835
72 0.675870358943939
73 0.564943552017212
74 0.800659954547882
75 0.778183102607727
76 0.650036692619324
77 0.812907874584198
78 0.641543388366699
79 0.817378580570221
80 0.595073163509369
81 0.706800758838654
82 0.623124361038208
83 0.673567950725555
84 0.538588345050812
85 0.797978281974792
86 0.757101237773895
87 0.828388333320618
88 0.644318342208862
89 0.855063140392303
90 0.65866231918335
91 0.843858957290649
92 0.760265231132507
93 0.610323190689087
94 0.678544044494629
95 0.742800116539001
96 0.61644572019577
97 0.641060411930084
98 0.835386455059052
99 0.745161414146423
};
\end{groupplot}

==> Figs/random_phi_change/n_free.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm, x descriptions at=edge bottom, group name=column1 plots,}]

\nextgroupplot[
width=\w cm,
height=\h cm,
legend cell align={left},
legend style={at={(1.1,1.85)}, anchor=north west, legend cell align=left, align=left, font=\footnotesize, draw=white!15!black},
legend columns=3,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=\xmin, xmax=\xmax,
xtick style={color=black,font=\footnotesize},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_0(t)|\)},
title = {(a) Noise free},
title style ={color=black,font=\footnotesize, yshift=-0.2cm},
ymin=0, ymax=1.2,
ytick style={color=black,font=\footnotesize},
%-------- Horizantal ----
%xtick style={color=black,font=\footnotesize},
%xlabel = {time \(t\)},
%title={\(\displaystyle |\cos\phi_1(t)|\)},
%-------- Vertical ----
xtick style={color=white,font=\footnotesize},
xticklabels ={},
%xlabel = {time \(t\)},
ylabel={\(\displaystyle |\cos\phi_1(k)|\)},
% xtick style={color=white},
% xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}


\plotTrue
table {%
0 0.733099880094478
1 0.733099880094478
2 0.733099880094478
3 0.733099880094478
4 0.733099880094478
5 0.733099880094478
6 0.733099880094478
7 0.733099880094478
8 0.733099880094478
9 0.733099880094478
10 0.733099880094478
11 0.733099880094478
12 0.733099880094478
13 0.733099880094478
14 0.733099880094478
15 0.733099880094478
16 0.733099880094478
17 0.733099880094478
18 0.733099880094478
19 0.733099880094478
20 0.733099880094478
21 0.733099880094478
22 0.733099880094478
23 0.733099880094478
24 0.733099880094478
25 0.733099880094478
26 0.733099880094478
27 0.733099880094478
28 0.733099880094478
29 0.733099880094478
30 0.733099880094478
31 0.733099880094478
32 0.733099880094478
33 0.733099880094478
34 0.733099880094478
35 0.733099880094478
36 0.733099880094478
37 0.733099880094478
38 0.733099880094478
39 0.733099880094478
40 0.733099880094478
41 0.733099880094478
42 0.733099880094478
43 0.733099880094478
44 0.733099880094478
45 0.733099880094478
46 0.733099880094478
47 0.733099880094478
48 0.733099880094478
49 0.733099880094478
50 0.733099880094478
51 0.733099880094478
52 0.733099880094478
53 0.733099880094478
54 0.733099880094478
55 0.733099880094478
56 0.733099880094478
57 0.733099880094478
58 0.733099880094478
59 0.733099880094478
60 0.733099880094478
61 0.733099880094478
62 0.733099880094478
63 0.733099880094478
64 0.733099880094478
65 0.733099880094478
66 0.733099880094478
67 0.733099880094478
68 0.733099880094478
69 0.733099880094478
70 0.733099880094478
71 0.733099880094478
72 0.733099880094478
73 0.733099880094478
74 0.733099880094478
75 0.733099880094478
76 0.733099880094478
77 0.733099880094478
78 0.733099880094478
79 0.733099880094478
80 0.733099880094478
81 0.733099880094478
82 0.733099880094478
83 0.733099880094478
84 0.733099880094478
85 0.733099880094478
86 0.733099880094478
87 0.733099880094478
88 0.733099880094478
89 0.733099880094478
90 0.733099880094478
91 0.733099880094478
92 0.733099880094478
93 0.733099880094478
94 0.733099880094478
95 0.733099880094478
96 0.733099880094478
97 0.733099880094478
98 0.733099880094478
99 0.733099880094478
};
\addlegendentry{True}
\plotNetwork
table {%
0 0.733099880094478
1 0.733099880094478
2 0.733099880094478
3 0.733099880094478
4 0.733099880094478
5 0.733099880094478
6 0.733099880094478
7 0.733099880094478
8 0.733099880094478
9 0.733099880094478
10 0.733099887874164
11 0.733099903011418
12 0.733099877986555
13 0.733099854653115
14 0.733255053367201
15 0.733099873832386
16 0.733099879787111
17 0.733221332545144
18 0.733099883041524
19 0.73309988174266
20 0.733099889043406
21 0.73309988027978
22 0.733099877928222
23 0.733099880928617
24 0.73309987237803
25 0.733100065109505
26 0.733099884270701
27 0.732623303617308
28 0.733100893851716
29 0.733906398272881
30 0.733096356525524
31 0.747710440348865
32 0.738039355869284
33 0.73309988420012
34 0.797371578169404
35 0.733099881203111
36 0.733099880094477
37 0.733247307549857
38 0.733099880917666
39 0.731848743983897
40 0.734067209378112
41 0.733038095687793
42 0.732452919957756
43 0.732819676222663
44 0.733057625978366
45 0.732505652072121
46 0.732672168247469
47 0.732357926155153
48 0.733055804646309
49 0.732937298796913
50 0.733115176677968
51 0.733087293997446
52 0.736317722645978
53 0.734210495640812
54 0.73312119913974
55 0.733058168205595
56 0.732930888375493
57 0.7329726923469
58 0.73292853679967
59 0.73366550534271
60 0.733105381737365
61 0.738930354558689
62 0.733350124353663
63 0.733115915250902
64 0.733101056243493
65 0.733105076573467
66 0.733099894007253
67 0.733100813396532
68 0.733045073248857
69 0.733099332860435
70 0.733428467546461
71 0.733099883867077
72 0.733099882230186
73 0.733099872849181
74 0.732963092742244
75 0.733183485004489
76 0.732875168696037
77 0.733099884479005
78 0.730769799191353
79 0.733099882222748
80 0.73309987173654
81 0.733333718547531
82 0.732712861460676
83 0.733100114515526
84 0.73312393509353
85 0.733099882806942
86 0.733049776814265
87 0.733099878880881
88 0.733099870681467
89 0.733068033026684
90 0.733100615774517
91 0.733099886596868
92 0.73310204696755
93 0.734271323848056
94 0.733099879295168
95 0.733099931614564
96 0.733088057922973
97 0.732853351510426
98 0.733102536113178
99 0.730057214792456
};
\addlegendentry{Learning Approach}
\plotInvscat
table {%
0 0.73309987783432
1 0.73309987783432
2 0.73309987783432
3 0.73309987783432
4 0.73309987783432
5 0.73309987783432
6 0.73309987783432
7 0.73309987783432
8 0.73309987783432
9 0.73309987783432
10 0.73309987783432
11 0.733099937438965
12 0.73309987783432
13 0.733099937438965
14 0.733099937438965
15 0.733099937438965
16 0.733099937438965
17 0.733099937438965
18 0.733099937438965
19 0.733099937438965
20 0.733099937438965
21 0.733099937438965
22 0.73309987783432
23 0.733099937438965
24 0.733100056648254
25 0.733102202415466
26 0.733100473880768
27 0.73309999704361
28 0.733100116252899
29 0.733102202415466
30 0.733100473880768
31 0.733159244060516
32 0.733032286167145
33 0.733099699020386
34 0.732950866222382
35 0.733099818229675
36 0.733099818229675
37 0.733099818229675
38 0.733099818229675
39 0.733099818229675
40 0.733099818229675
41 0.733099818229675
42 0.733099818229675
43 0.733099818229675
44 0.733099818229675
45 0.733099818229675
46 0.733099818229675
47 0.733099818229675
48 0.733099818229675
49 0.733099818229675
50 0.733099818229675
51 0.733099818229675
52 0.733099818229675
53 0.733099818229675
54 0.733099818229675
55 0.733099818229675
56 0.733099818229675
57 0.733099818229675
58 0.733099818229675
59 0.733099818229675
60 0.733099818229675
61 0.733108937740326
62 0.733092844486237
63 0.733086705207825
64 0.733097076416016
65 0.733099639415741
66 0.733099818229675
67 0.733099818229675
68 0.733099758625031
69 0.733099758625031
70 0.733099818229675
71 0.733099818229675
72 0.733099818229675
73 0.733099818229675
74 0.733099818229675
75 0.733099639415741
76 0.733099699020386
77 0.733099818229675
78 0.733099818229675
79 0.733099818229675
80 0.733099818229675
81 0.733099818229675
82 0.73309713602066
83 0.73310399055481
84 0.733103394508362
85 0.73309999704361
86 0.73309999704361
87 0.73309999704361
88 0.73309999704361
89 0.73309999704361
90 0.73309999704361
91 0.73309999704361
92 0.73309999704361
93 0.73309999704361
94 0.73309999704361
95 0.73309999704361
96 0.73309999704361
97 0.73309999704361
98 0.73309999704361
99 0.73309999704361
};
\addlegendentry{Inverse Scattering\cite{noe_polarization-dependent_2015}}
%==================================== Fig 2 ==============================
\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=\xmin, xmax=\xmax,
y grid style={darkgray176},
ylabel={\(\displaystyle |\cos\phi_2(k)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
xtick style={color=white},
xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\perturbation

\plotTrue
table {%
0 0.935516519885526
1 0.935516519885526
2 0.935516519885526
3 0.935516519885526
4 0.935516519885526
5 0.935516519885526
6 0.935516519885526
7 0.935516519885526
8 0.935516519885526
9 0.935516519885526
10 0.869667569548439
11 0.727246223885405
12 0.840885440553651
13 0.669861263673315
14 0.695062251008769
15 0.653367486580926
16 0.656677578070439
17 0.60377798372569
18 0.40326589007199
19 0.544277543208332
20 0.634658637120049
21 0.771370029605121
22 0.807328666767555
23 0.705765479890902
24 0.294400085499
25 0.122840677718215
26 0.197476673071808
27 0.344663137249381
28 0.280526511787189
29 0.122459958543774
30 0.199148910512332
31 0.0403795856982413
32 0.0377646706314038
33 0.285823945820197
34 0.0291006444692511
35 0.408406259801238
36 0.408406259801238
37 0.408406259801238
38 0.408406259801238
39 0.408406259801238
40 0.408406259801238
41 0.408406259801238
42 0.408406259801238
43 0.408406259801238
44 0.408406259801238
45 0.408406259801238
46 0.408406259801238
47 0.408406259801238
48 0.408406259801238
49 0.408406259801238
50 0.408406259801238
51 0.408406259801238
52 0.408406259801238
53 0.408406259801238
54 0.408406259801238
55 0.408406259801238
56 0.408406259801238
57 0.408406259801238
58 0.408406259801238
59 0.408406259801238
60 0.402191409831325
61 0.0764337403055456
62 0.0795973866253387
63 0.0646871585761395
64 0.108009977372683
65 0.254616719700893
66 0.472565933463051
67 0.434779798744271
68 0.310130512503765
69 0.335406009918958
70 0.385910215050476
71 0.723644828986625
72 0.677641239833845
73 0.546856821471035
74 0.415658991542201
75 0.241671090622782
76 0.281803188796102
77 0.451510825833016
78 0.503227302170066
79 0.623984732537678
80 0.390940740100067
81 0.383177631440228
82 0.108923776814901
83 0.10020607423564
84 0.106528490954389
85 0.356305650239709
86 0.356305650239709
87 0.356305650239709
88 0.356305650239709
89 0.356305650239709
90 0.356305650239709
91 0.356305650239709
92 0.356305650239709
93 0.356305650239709
94 0.356305650239709
95 0.356305650239709
96 0.356305650239709
97 0.356305650239709
98 0.356305650239709
99 0.356305650239709
};
\plotNetwork
table {%
0 0.935516519885526
1 0.935516519885526
2 0.935516519885526
3 0.935516519885526
4 0.935516519885526
5 0.935516519885526
6 0.935516519885526
7 0.935516519885526
8 0.935516519885526
9 0.935516519885526
10 0.869667569743951
11 0.727246222931323
12 0.840885451349219
13 0.66986126209636
14 0.695062158251806
15 0.653367489476736
16 0.656677578294034
17 0.603777569287096
18 0.403265910381466
19 0.544277546780428
20 0.634658638585368
21 0.771370029813809
22 0.807328664354449
23 0.7057654700065
24 0.294400112347341
25 0.122840674412357
26 0.19747666575041
27 0.344658258878467
28 0.280526578307019
29 0.122495245704127
30 0.199149312565074
31 0.0405376465450581
32 0.0378082281365803
33 0.285823926471467
34 0.0308980842254162
35 0.408406286042731
36 0.408406259801236
37 0.408406450698526
38 0.408406259779693
39 0.40840389520259
40 0.408421972827373
41 0.40841596210541
42 0.408430428657216
43 0.408399359499322
44 0.408405327893248
45 0.408393407109671
46 0.408400339184258
47 0.408387152158403
48 0.408507631880166
49 0.40835611328181
50 0.408408124144589
51 0.408409616089787
52 0.408925570645913
53 0.410069670571618
54 0.409031002528899
55 0.408179646111878
56 0.408340868488624
57 0.409077188844806
58 0.408172664866313
59 0.413077493302732
60 0.402178904824364
61 0.0763571116871755
62 0.0796083422578106
63 0.0646876867054762
64 0.108009976194427
65 0.254616697860051
66 0.472565914372968
67 0.434779804800786
68 0.310130250945379
69 0.335405991826088
70 0.385912602921306
71 0.72364480902873
72 0.677641235835052
73 0.546856820843074
74 0.415661199392922
75 0.241675188242445
76 0.281809804418004
77 0.451510810932369
78 0.503314743834044
79 0.623984741636025
80 0.390940713911644
81 0.383179311360421
82 0.108923627189942
83 0.10020604411885
84 0.106524210973446
85 0.356305649540552
86 0.356304936554577
87 0.35630565023536
88 0.356305650544652
89 0.356305809507217
90 0.356305660580052
91 0.356305650685598
92 0.356305638512368
93 0.356524013405796
94 0.356305650169959
95 0.356305656373799
96 0.356304257998649
97 0.356162520501466
98 0.356306552838501
99 0.355159976512981
};
\plotInvscat
table {%
0 0.935516536235809
1 0.935516536235809
2 0.935516536235809
3 0.935516536235809
4 0.935516536235809
5 0.935516536235809
6 0.935516536235809
7 0.935516536235809
8 0.935516536235809
9 0.935516536235809
10 0.869667589664459
11 0.727246224880219
12 0.84088546037674
13 0.669861257076263
14 0.695062279701233
15 0.653367459774017
16 0.656677603721619
17 0.603778004646301
18 0.40326589345932
19 0.544277548789978
20 0.634658634662628
21 0.771370053291321
22 0.807328641414642
23 0.70576548576355
24 0.294400095939636
25 0.12284079939127
26 0.197476789355278
27 0.344663143157959
28 0.280526518821716
29 0.122460074722767
30 0.199149027466774
31 0.0403810143470764
32 0.0377626456320286
33 0.285823941230774
34 0.0290973074734211
35 0.408406257629395
36 0.408406257629395
37 0.408406257629395
38 0.408406257629395
39 0.408406257629395
40 0.408406257629395
41 0.408406257629395
42 0.408406257629395
43 0.408406257629395
44 0.408406257629395
45 0.408406257629395
46 0.408406257629395
47 0.408406257629395
48 0.408406257629395
49 0.408406257629395
50 0.408406257629395
51 0.408406257629395
52 0.408406257629395
53 0.408406257629395
54 0.408406257629395
55 0.408406257629395
56 0.408406257629395
57 0.408406257629395
58 0.408406257629395
59 0.408406257629395
60 0.402191400527954
61 0.0764340981841087
62 0.0795969143509865
63 0.0646864473819733
64 0.108009740710258
65 0.254616618156433
66 0.472565919160843
67 0.434779793024063
68 0.310130506753922
69 0.335406005382538
70 0.385910212993622
71 0.723644852638245
72 0.677641212940216
73 0.546856820583344
74 0.415658980607986
75 0.241670981049538
76 0.28180319070816
77 0.451510816812515
78 0.503227293491364
79 0.623984754085541
80 0.390940725803375
81 0.383177638053894
82 0.10892353951931
83 0.100206308066845
84 0.106528729200363
85 0.356305658817291
86 0.356305658817291
87 0.356305658817291
88 0.356305658817291
89 0.356305658817291
90 0.356305658817291
91 0.356305658817291
92 0.356305658817291
93 0.356305658817291
94 0.356305658817291
95 0.356305658817291
96 0.356305658817291
97 0.356305658817291
98 0.356305658817291
99 0.356305658817291
};


%=========================== Fig 3 ====================
\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=\xmin, xmax=\xmax,
y grid style={darkgray176},
ylabel={\(\displaystyle |\cos\phi_3(k)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
xtick style={color=white},
xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\trueLineWidth pt, dotted]
table {%
0 0.824356457355511
1 0.824356457355511
2 0.824356457355511
3 0.824356457355511
4 0.824356457355511
5 0.824356457355511
6 0.824356457355511
7 0.824356457355511
8 0.824356457355511
9 0.824356457355511
10 0.824356457355511
11 0.824356457355511
12 0.824356457355511
13 0.824356457355511
14 0.824356457355511
15 0.824356457355511
16 0.824356457355511
17 0.824356457355511
18 0.824356457355511
19 0.824356457355511
20 0.824356457355511
21 0.824356457355511
22 0.824356457355511
23 0.824356457355511
24 0.824356457355511
25 0.824356457355511
26 0.824356457355511
27 0.824356457355511
28 0.824356457355511
29 0.824356457355511
30 0.824356457355511
31 0.824356457355511
32 0.824356457355511
33 0.824356457355511
34 0.824356457355511
35 0.824356457355511
36 0.824356457355511
37 0.824356457355511
38 0.824356457355511
39 0.824356457355511
40 0.824356457355511
41 0.824356457355511
42 0.824356457355511
43 0.824356457355511
44 0.824356457355511
45 0.824356457355511
46 0.824356457355511
47 0.824356457355511
48 0.824356457355511
49 0.824356457355511
50 0.824356457355511
51 0.824356457355511
52 0.824356457355511
53 0.824356457355511
54 0.824356457355511
55 0.824356457355511
56 0.824356457355511
57 0.824356457355511
58 0.824356457355511
59 0.824356457355511
60 0.824356457355511
61 0.824356457355511
62 0.824356457355511
63 0.824356457355511
64 0.824356457355511
65 0.824356457355511
66 0.824356457355511
67 0.824356457355511
68 0.824356457355511
69 0.824356457355511
70 0.824356457355511
71 0.824356457355511
72 0.824356457355511
73 0.824356457355511
74 0.824356457355511
75 0.824356457355511
76 0.824356457355511
77 0.824356457355511
78 0.824356457355511
79 0.824356457355511
80 0.824356457355511
81 0.824356457355511
82 0.824356457355511
83 0.824356457355511
84 0.824356457355511
85 0.824356457355511
86 0.824356457355511
87 0.824356457355511
88 0.824356457355511
89 0.824356457355511
90 0.824356457355511
91 0.824356457355511
92 0.824356457355511
93 0.824356457355511
94 0.824356457355511
95 0.824356457355511
96 0.824356457355511
97 0.824356457355511
98 0.824356457355511
99 0.824356457355511
};
\plotNetwork
table {%
0 0.82435645735551
1 0.82435645735551
2 0.82435645735551
3 0.82435645735551
4 0.824356457355511
5 0.82435645735551
6 0.824356457355511
7 0.82435645735551
8 0.82435645735551
9 0.824356457355511
10 0.824356456316568
11 0.824356450315932
12 0.824356458134348
13 0.824356472772402
14 0.825166419091379
15 0.824356457865681
16 0.824356457482692
17 0.824581350105875
18 0.824356462805712
19 0.824356456888125
20 0.824356453176303
21 0.824356456654755
22 0.824356458921715
23 0.824356458492815
24 0.824356451667786
25 0.824356510228724
26 0.824356454709064
27 0.823650835373947
28 0.824357438989837
29 0.824517751363044
30 0.824349945329756
31 0.827426265537046
32 0.824555714581153
33 0.824356451167658
34 0.779639663599777
35 0.824356470747711
36 0.824356457355512
37 0.824476748595607
38 0.824356458060747
39 0.823341709466652
40 0.82522508347073
41 0.82422649897325
42 0.823618942941109
43 0.824110501288509
44 0.824342703977302
45 0.823910439014495
46 0.824039494771982
47 0.823797429758144
48 0.824204734465653
49 0.824311077784181
50 0.824368557958459
51 0.824344878950139
52 0.827015702292893
53 0.82495234709517
54 0.824383642893771
55 0.824317408367161
56 0.824228545569564
57 0.824318977287165
58 0.824211262118761
59 0.825023119738052
60 0.824347532131019
61 0.82460847411528
62 0.824265810574101
63 0.824351178745061
64 0.824357544931123
65 0.824361344065449
66 0.824356445235553
67 0.824357103254403
68 0.824317135668364
69 0.824356153862579
70 0.824614633616612
71 0.824356450607129
72 0.824356454996435
73 0.824356466414979
74 0.824278660012739
75 0.824390207918486
76 0.824213663368678
77 0.824356451817205
78 0.822811748017169
79 0.82435645542237
80 0.824356460894534
81 0.824508904207536
82 0.824085413386913
83 0.824356507736347
84 0.82439055590999
85 0.82435645847458
86 0.82432068706062
87 0.824356456418615
88 0.824356451702873
89 0.824328495087668
90 0.824357042226458
91 0.824356461425662
92 0.824358175642438
93 0.825093322026763
94 0.8243564567116
95 0.824356497104326
96 0.824344099401678
97 0.824242896701355
98 0.824358630125391
99 0.820650582268632
};
\plotInvscat
table {%
0 0.824356436729431
1 0.824356436729431
2 0.824356436729431
3 0.824356436729431
4 0.824356436729431
5 0.824356436729431
6 0.824356436729431
7 0.824356436729431
8 0.824356436729431
9 0.824356436729431
10 0.824356436729431
11 0.824356436729431
12 0.824356436729431
13 0.824356436729431
14 0.824356436729431
15 0.824356436729431
16 0.824356436729431
17 0.824356436729431
18 0.824356317520142
19 0.824356436729431
20 0.824356436729431
21 0.824356436729431
22 0.824356436729431
23 0.824356436729431
24 0.824356198310852
25 0.824353098869324
26 0.824355661869049
27 0.824356317520142
28 0.824356198310852
29 0.824353098869324
30 0.824355661869049
31 0.824261844158173
32 0.824478030204773
33 0.824356853961945
34 0.82462078332901
35 0.824356615543365
36 0.824356615543365
37 0.824356615543365
38 0.824356615543365
39 0.824356615543365
40 0.824356615543365
41 0.824356615543365
42 0.824356615543365
43 0.824356615543365
44 0.824356615543365
45 0.824356615543365
46 0.824356615543365
47 0.824356615543365
48 0.824356615543365
49 0.824356615543365
50 0.824356615543365
51 0.824356615543365
52 0.824356615543365
53 0.824356615543365
54 0.824356615543365
55 0.824356615543365
56 0.824356615543365
57 0.824356615543365
58 0.824356615543365
59 0.824356615543365
60 0.824356615543365
61 0.824342668056488
62 0.824369966983795
63 0.824381172657013
64 0.824361979961395
65 0.824356973171234
66 0.824356615543365
67 0.824356615543365
68 0.824356734752655
69 0.824356734752655
70 0.824356615543365
71 0.824356436729431
72 0.824356436729431
73 0.824356615543365
74 0.824356615543365
75 0.824356973171234
76 0.824356853961945
77 0.824356615543365
78 0.824356615543365
79 0.824356436729431
80 0.824356615543365
81 0.824356615543365
82 0.824361860752106
83 0.824350357055664
84 0.82435131072998
85 0.824356317520142
86 0.824356317520142
87 0.824356317520142
88 0.824356317520142
89 0.824356317520142
90 0.824356317520142
91 0.824356317520142
92 0.824356317520142
93 0.824356317520142
94 0.824356317520142
95 0.824356317520142
96 0.824356317520142
97 0.824356317520142
98 0.824356317520142
99 0.824356317520142
};
%=============================== Fig 4 =========================
\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=\xmin, xmax=\xmax,
y grid style={darkgray176},
ylabel={\(\displaystyle |\cos\phi_4(k)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
xtick style={color=white},
xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\trueLineWidth pt, dotted]
table {%
0 0.753602486017811
1 0.753602486017811
2 0.753602486017811
3 0.753602486017811
4 0.753602486017811
5 0.753602486017811
6 0.753602486017811
7 0.753602486017811
8 0.753602486017811
9 0.753602486017811
10 0.753602486017811
11 0.753602486017811
12 0.753602486017811
13 0.753602486017811
14 0.753602486017811
15 0.753602486017811
16 0.753602486017811
17 0.753602486017811
18 0.753602486017811
19 0.753602486017811
20 0.753602486017811
21 0.753602486017811
22 0.753602486017811
23 0.753602486017811
24 0.753602486017811
25 0.753602486017811
26 0.753602486017811
27 0.753602486017811
28 0.753602486017811
29 0.753602486017811
30 0.753602486017811
31 0.753602486017811
32 0.753602486017811
33 0.753602486017811
34 0.753602486017811
35 0.753602486017811
36 0.753602486017811
37 0.753602486017811
38 0.753602486017811
39 0.753602486017811
40 0.753602486017811
41 0.753602486017811
42 0.753602486017811
43 0.753602486017811
44 0.753602486017811
45 0.753602486017811
46 0.753602486017811
47 0.753602486017811
48 0.753602486017811
49 0.753602486017811
50 0.753602486017811
51 0.753602486017811
52 0.753602486017811
53 0.753602486017811
54 0.753602486017811
55 0.753602486017811
56 0.753602486017811
57 0.753602486017811
58 0.753602486017811
59 0.753602486017811
60 0.753602486017811
61 0.753602486017811
62 0.753602486017811
63 0.753602486017811
64 0.753602486017811
65 0.753602486017811
66 0.753602486017811
67 0.753602486017811
68 0.753602486017811
69 0.753602486017811
70 0.753602486017811
71 0.753602486017811
72 0.753602486017811
73 0.753602486017811
74 0.753602486017811
75 0.753602486017811
76 0.753602486017811
77 0.753602486017811
78 0.753602486017811
79 0.753602486017811
80 0.753602486017811
81 0.753602486017811
82 0.753602486017811
83 0.753602486017811
84 0.753602486017811
85 0.753602486017811
86 0.753602486017811
87 0.753602486017811
88 0.753602486017811
89 0.753602486017811
90 0.753602486017811
91 0.753602486017811
92 0.753602486017811
93 0.753602486017811
94 0.753602486017811
95 0.753602486017811
96 0.753602486017811
97 0.753602486017811
98 0.753602486017811
99 0.753602486017811
};
\plotNetwork
table {%
0 0.75360248601781
1 0.75360248601781
2 0.75360248601781
3 0.75360248601781
4 0.75360248601781
5 0.75360248601781
6 0.75360248601781
7 0.75360248601781
8 0.75360248601781
9 0.75360248601781
10 0.753602477759896
11 0.753602470405212
12 0.753602484396138
13 0.753602504333984
14 0.753698055177375
15 0.753602487131109
16 0.75360248617446
17 0.753689427417967
18 0.753602483690719
19 0.753602484757353
20 0.75360248242839
21 0.753602487213994
22 0.75360248814433
23 0.753602486107288
24 0.753602483136805
25 0.753602455566452
26 0.753602487446987
27 0.753509130254324
28 0.753602576894554
29 0.753557625821095
30 0.753601463108276
31 0.753333961224418
32 0.753698533490304
33 0.753602486893142
34 0.755949225427938
35 0.753602496884583
36 0.753602486017811
37 0.753589793756203
38 0.753602485883828
39 0.753753071216912
40 0.753488087285513
41 0.753570321529686
42 0.753763651867209
43 0.753705772282774
44 0.753649618760208
45 0.753909843112207
46 0.753848862475685
47 0.754133068751718
48 0.753220134798612
49 0.753848048276355
50 0.753583849399218
51 0.753601794295022
52 0.750506817377645
53 0.751401349723562
54 0.753307877261761
55 0.753622340848893
56 0.753765958285141
57 0.753530574465466
58 0.753816299948809
59 0.751608792532419
60 0.753572636879033
61 0.753072559774666
62 0.753625047020657
63 0.753603650529517
64 0.753602428957478
65 0.753601821801192
66 0.753602485853435
67 0.753602238849411
68 0.753610138842027
69 0.753602492499384
70 0.7535419540971
71 0.753602485749365
72 0.753602486509449
73 0.753602483971722
74 0.753600199688417
75 0.753599072353679
76 0.753643377418768
77 0.753602485043802
78 0.753933668782228
79 0.75360249154843
80 0.753602474572072
81 0.753566045327424
82 0.753615505461857
83 0.753602458441317
84 0.753601405420851
85 0.753602485998162
86 0.753594494780796
87 0.753602485782056
88 0.753602485015306
89 0.753588052109714
90 0.753602771164676
91 0.753602489003957
92 0.753603997053032
93 0.754449567776235
94 0.75360248534275
95 0.753602530044295
96 0.753590155162333
97 0.753347990539917
98 0.753604906183109
99 0.749593895606362
};
\plotInvscat
table {%
0 0.753602504730225
1 0.753602504730225
2 0.753602504730225
3 0.753602504730225
4 0.753602504730225
5 0.753602504730225
6 0.753602504730225
7 0.753602504730225
8 0.753602504730225
9 0.753602504730225
10 0.753602504730225
11 0.753602504730225
12 0.753602504730225
13 0.753602504730225
14 0.753602504730225
15 0.753602504730225
16 0.753602504730225
17 0.753602504730225
18 0.75360244512558
19 0.753602504730225
20 0.753602504730225
21 0.753602504730225
22 0.753602504730225
23 0.753602504730225
24 0.75360244512558
25 0.753602266311646
26 0.753602385520935
27 0.75360244512558
28 0.75360244512558
29 0.753602266311646
30 0.753602385520935
31 0.753600299358368
32 0.753599882125854
33 0.753602385520935
34 0.753598034381866
35 0.75360244512558
36 0.75360244512558
37 0.75360244512558
38 0.75360244512558
39 0.75360244512558
40 0.75360244512558
41 0.75360244512558
42 0.75360244512558
43 0.75360244512558
44 0.75360244512558
45 0.75360244512558
46 0.75360244512558
47 0.75360244512558
48 0.75360244512558
49 0.75360244512558
50 0.75360244512558
51 0.75360244512558
52 0.75360244512558
53 0.75360244512558
54 0.75360244512558
55 0.75360244512558
56 0.75360244512558
57 0.75360244512558
58 0.75360244512558
59 0.75360244512558
60 0.75360244512558
61 0.753601908683777
62 0.753601849079132
63 0.753601610660553
64 0.753602147102356
65 0.753602385520935
66 0.75360244512558
67 0.75360244512558
68 0.75360244512558
69 0.75360244512558
70 0.75360244512558
71 0.753602504730225
72 0.753602504730225
73 0.75360244512558
74 0.75360244512558
75 0.753602385520935
76 0.753602385520935
77 0.75360244512558
78 0.75360244512558
79 0.75360244512558
80 0.75360244512558
81 0.75360244512558
82 0.753602147102356
83 0.753602147102356
84 0.753602147102356
85 0.75360244512558
86 0.75360244512558
87 0.75360244512558
88 0.75360244512558
89 0.75360244512558
90 0.75360244512558
91 0.75360244512558
92 0.75360244512558
93 0.75360244512558
94 0.75360244512558
95 0.75360244512558
96 0.75360244512558
97 0.75360244512558
98 0.75360244512558
99 0.75360244512558
};

%====================== Fig 5 ==================
\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=\xmin, xmax=\xmax,
y grid style={darkgray176},
ylabel={\(\displaystyle |\cos\phi_5(k)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
xlabel = {time step \(k\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%xtick style={color=white},
%xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\trueLineWidth pt, dotted]
table {%
0 0.935826238137458
1 0.935826238137458
2 0.935826238137458
3 0.935826238137458
4 0.935826238137458
5 0.935826238137458
6 0.935826238137458
7 0.935826238137458
8 0.935826238137458
9 0.935826238137458
10 0.935826238137458
11 0.935826238137458
12 0.935826238137458
13 0.935826238137458
14 0.935826238137458
15 0.935826238137458
16 0.935826238137458
17 0.935826238137458
18 0.935826238137458
19 0.935826238137458
20 0.935826238137458
21 0.935826238137458
22 0.935826238137458
23 0.935826238137458
24 0.935826238137458
25 0.935826238137458
26 0.935826238137458
27 0.935826238137458
28 0.935826238137458
29 0.935826238137458
30 0.935826238137458
31 0.935826238137458
32 0.935826238137458
33 0.935826238137458
34 0.935826238137458
35 0.935826238137458
36 0.935826238137458
37 0.935826238137458
38 0.935826238137458
39 0.935826238137458
40 0.935826238137458
41 0.935826238137458
42 0.935826238137458
43 0.935826238137458
44 0.935826238137458
45 0.935826238137458
46 0.935826238137458
47 0.935826238137458
48 0.935826238137458
49 0.935826238137458
50 0.935826238137458
51 0.935826238137458
52 0.935826238137458
53 0.935826238137458
54 0.935826238137458
55 0.935826238137458
56 0.935826238137458
57 0.935826238137458
58 0.935826238137458
59 0.935826238137458
60 0.935826238137458
61 0.935826238137458
62 0.935826238137458
63 0.935826238137458
64 0.935826238137458
65 0.935826238137458
66 0.935826238137458
67 0.935826238137458
68 0.935826238137458
69 0.935826238137458
70 0.935826238137458
71 0.935826238137458
72 0.935826238137458
73 0.935826238137458
74 0.935826238137458
75 0.935826238137458
76 0.935826238137458
77 0.935826238137458
78 0.935826238137458
79 0.935826238137458
80 0.935826238137458
81 0.935826238137458
82 0.935826238137458
83 0.935826238137458
84 0.935826238137458
85 0.935826238137458
86 0.935826238137458
87 0.935826238137458
88 0.935826238137458
89 0.935826238137458
90 0.935826238137458
91 0.935826238137458
92 0.935826238137458
93 0.935826238137458
94 0.935826238137458
95 0.935826238137458
96 0.935826238137458
97 0.935826238137458
98 0.935826238137458
99 0.935826238137458
};
\plotNetwork
table {%
0 0.935826238137458
1 0.935826238137458
2 0.935826238137458
3 0.935826238137458
4 0.935826238137458
5 0.935826238137458
6 0.935826238137458
7 0.935826238137458
8 0.935826238137458
9 0.935826238137458
10 0.935826236892214
11 0.935826236770857
12 0.935826237542283
13 0.935826236761034
14 0.936065313651657
15 0.935826237509643
16 0.935826238132452
17 0.935935162209105
18 0.935826235589941
19 0.935826237635033
20 0.935826237770446
21 0.935826236123657
22 0.935826238180394
23 0.935826235819045
24 0.935826238502945
25 0.935826226256869
26 0.935826238215398
27 0.935650443860692
28 0.935826470097923
29 0.935910144896606
30 0.93582404077304
31 0.937542686953441
32 0.935076067391066
33 0.935826235873228
34 0.936317981238362
35 0.935826232537896
36 0.935826238137457
37 0.935839000500626
38 0.935826238096434
39 0.935605621454625
40 0.936371947474817
41 0.935492789038664
42 0.935251545558468
43 0.935792354030996
44 0.93593235132459
45 0.935759670738093
46 0.935714201452772
47 0.935732680996642
48 0.935031294609463
49 0.93599836503546
50 0.935818974954332
51 0.935804776383994
52 0.936008833516691
53 0.934274548789463
54 0.935640084111777
55 0.935694858973299
56 0.935835447012421
57 0.935874623536835
58 0.935847701065514
59 0.935474960512244
60 0.935759353516004
61 0.935662110193505
62 0.935831994643882
63 0.935826547721148
64 0.935826302202612
65 0.935826246681285
66 0.93582624018364
67 0.93582568167637
68 0.935838406511868
69 0.935826088858469
70 0.935889996012834
71 0.935826244974846
72 0.935826238815873
73 0.93582623593353
74 0.935689717664618
75 0.935835253229753
76 0.935865001228979
77 0.935826241456211
78 0.934407017190267
79 0.935826239292471
80 0.935826242004874
81 0.935849979149344
82 0.935780983798652
83 0.935826228312997
84 0.935827946718199
85 0.935826235229716
86 0.935812116760807
87 0.935826237769288
88 0.935826235981485
89 0.935811180062937
90 0.935826556807307
91 0.935826240867535
92 0.935827229169318
93 0.93636268819389
94 0.935826237745668
95 0.935826261348857
96 0.935819450381247
97 0.935682515408594
98 0.935827364171803
99 0.933604964016431
};
\plotInvscat
table {%
0 0.935826241970062
1 0.935826241970062
2 0.935826241970062
3 0.935826241970062
4 0.935826241970062
5 0.935826241970062
6 0.935826241970062
7 0.935826241970062
8 0.935826241970062
9 0.935826241970062
10 0.935826241970062
11 0.935826241970062
12 0.935826241970062
13 0.935826241970062
14 0.935826241970062
15 0.935826241970062
16 0.935826241970062
17 0.935826241970062
18 0.935826241970062
19 0.935826241970062
20 0.935826241970062
21 0.935826241970062
22 0.935826241970062
23 0.935826241970062
24 0.935826241970062
25 0.935826301574707
26 0.935826241970062
27 0.935826241970062
28 0.935826241970062
29 0.935826301574707
30 0.935826241970062
31 0.935826420783997
32 0.935826063156128
33 0.935826241970062
34 0.935826003551483
35 0.935826241970062
36 0.935826241970062
37 0.935826241970062
38 0.935826241970062
39 0.935826241970062
40 0.935826241970062
41 0.935826241970062
42 0.935826241970062
43 0.935826241970062
44 0.935826241970062
45 0.935826241970062
46 0.935826241970062
47 0.935826241970062
48 0.935826241970062
49 0.935826241970062
50 0.935826241970062
51 0.935826241970062
52 0.935826241970062
53 0.935826241970062
54 0.935826241970062
55 0.935826241970062
56 0.935826241970062
57 0.935826241970062
58 0.935826241970062
59 0.935826241970062
60 0.935826241970062
61 0.935826301574707
62 0.935826182365417
63 0.935826182365417
64 0.935826182365417
65 0.935826241970062
66 0.935826241970062
67 0.935826241970062
68 0.935826241970062
69 0.935826241970062
70 0.935826241970062
71 0.935826241970062
72 0.935826241970062
73 0.935826241970062
74 0.935826241970062
75 0.935826241970062
76 0.935826241970062
77 0.935826241970062
78 0.935826241970062
79 0.935826241970062
80 0.935826241970062
81 0.935826241970062
82 0.935826182365417
83 0.935826301574707
84 0.935826301574707
85 0.935826241970062
86 0.935826241970062
87 0.935826241970062
88 0.935826241970062
89 0.935826241970062
90 0.935826241970062
91 0.935826241970062
92 0.935826241970062
93 0.935826241970062
94 0.935826241970062
95 0.935826241970062
96 0.935826241970062
97 0.935826241970062
98 0.935826241970062
99 0.935826241970062
};

\end{groupplot}

==> Figs/random_phi_change/noise_0.001.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm, group name=column2 plots,}]

\firstgplot{column1}{(b) $\sigma^2_{z}=0.001$}
\plotTrue
table {%
0 0.733099880094478
1 0.733099880094478
2 0.733099880094478
3 0.733099880094478
4 0.733099880094478
5 0.733099880094478
6 0.733099880094478
7 0.733099880094478
8 0.733099880094478
9 0.733099880094478
10 0.733099880094478
11 0.733099880094478
12 0.733099880094478
13 0.733099880094478
14 0.733099880094478
15 0.733099880094478
16 0.733099880094478
17 0.733099880094478
18 0.733099880094478
19 0.733099880094478
20 0.733099880094478
21 0.733099880094478
22 0.733099880094478
23 0.733099880094478
24 0.733099880094478
25 0.733099880094478
26 0.733099880094478
27 0.733099880094478
28 0.733099880094478
29 0.733099880094478
30 0.733099880094478
31 0.733099880094478
32 0.733099880094478
33 0.733099880094478
34 0.733099880094478
35 0.733099880094478
36 0.733099880094478
37 0.733099880094478
38 0.733099880094478
39 0.733099880094478
40 0.733099880094478
41 0.733099880094478
42 0.733099880094478
43 0.733099880094478
44 0.733099880094478
45 0.733099880094478
46 0.733099880094478
47 0.733099880094478
48 0.733099880094478
49 0.733099880094478
50 0.733099880094478
51 0.733099880094478
52 0.733099880094478
53 0.733099880094478
54 0.733099880094478
55 0.733099880094478
56 0.733099880094478
57 0.733099880094478
58 0.733099880094478
59 0.733099880094478
60 0.733099880094478
61 0.733099880094478
62 0.733099880094478
63 0.733099880094478
64 0.733099880094478
65 0.733099880094478
66 0.733099880094478
67 0.733099880094478
68 0.733099880094478
69 0.733099880094478
70 0.733099880094478
71 0.733099880094478
72 0.733099880094478
73 0.733099880094478
74 0.733099880094478
75 0.733099880094478
76 0.733099880094478
77 0.733099880094478
78 0.733099880094478
79 0.733099880094478
80 0.733099880094478
81 0.733099880094478
82 0.733099880094478
83 0.733099880094478
84 0.733099880094478
85 0.733099880094478
86 0.733099880094478
87 0.733099880094478
88 0.733099880094478
89 0.733099880094478
90 0.733099880094478
91 0.733099880094478
92 0.733099880094478
93 0.733099880094478
94 0.733099880094478
95 0.733099880094478
96 0.733099880094478
97 0.733099880094478
98 0.733099880094478
99 0.733099880094478
};

\plotNetwork
table {%
0 0.729319201582755
1 0.73276137679316
2 0.735752313890213
3 0.739535333891654
4 0.728211111080606
5 0.737451719389608
6 0.727818057231807
7 0.729747476663003
8 0.737531565232823
9 0.737176276796054
10 0.737127409191296
11 0.748520951710596
12 0.729276298683192
13 0.740471234729042
14 0.734072341964223
15 0.742135059191372
16 0.734020533606089
17 0.731044913376071
18 0.720538949640792
19 0.726800451748516
20 0.748577421658583
21 0.746331181604226
22 0.731972298994098
23 0.752128848495869
24 0.715841355205616
25 0.765721232820956
26 0.712046447452547
27 0.726006963374474
28 0.749545264347452
29 0.683590235377624
30 0.761333867816165
31 0.869733965868464
32 0.858639649867254
33 0.729810712472467
34 0.933784321726523
35 0.723435476761136
36 0.691002921106156
37 0.73891178786859
38 0.742936069676508
39 0.725122867246019
40 0.72945900373754
41 0.740044032513077
42 0.73428028839251
43 0.727750035523283
44 0.720554125202716
45 0.738635167798756
46 0.737209442987541
47 0.737837224537761
48 0.72558383894492
49 0.717340695878102
50 0.747749479380025
51 0.717167842992725
52 0.720317042277946
53 0.737940455376637
54 0.750236261436726
55 0.705526567164959
56 0.722920742518832
57 0.732408415051592
58 0.756285455976621
59 0.737153808715406
60 0.745999795694006
61 0.770039963397839
62 0.705923331133002
63 0.775533655185505
64 0.778624779839659
65 0.737167405609356
66 0.749264201503399
67 0.747124857249642
68 0.7346742923451
69 0.74681569248726
70 0.746991206012558
71 0.739332587559497
72 0.74246279358821
73 0.728211110333338
74 0.725411897292875
75 0.695630258021596
76 0.773466654176007
77 0.726034976348635
78 0.728362318893114
79 0.73503057850249
80 0.731784671248506
81 0.738518587692284
82 0.748621369223878
83 0.782074517881985
84 0.664406907065427
85 0.781116570251836
86 0.747522437602458
87 0.750669198212523
88 0.738615803210335
89 0.719944310835215
90 0.757823800801854
91 0.761737953426716
92 0.742391550328588
93 0.745200177135922
94 0.756735755256699
95 0.753000671161738
96 0.719503198577407
97 0.722313401771234
98 0.726198841080199
99 0.724739985380226
};

\plotInvscat
table {%
0 0.72292947769165
1 0.743376910686493
2 0.730382680892944
3 0.746846497058868
4 0.7271968126297
5 0.731141805648804
6 0.737849771976471
7 0.74114590883255
8 0.735116243362427
9 0.735976099967957
10 0.74371999502182
11 0.759178876876831
12 0.7479567527771
13 0.767851054668427
14 0.747498750686646
15 0.744250774383545
16 0.746647298336029
17 0.755470752716064
18 0.673729419708252
19 0.824181914329529
20 0.795238256454468
21 0.737778306007385
22 0.749621093273163
23 0.776601850986481
24 0.84341961145401
25 0.942687094211578
26 0.976913273334503
27 0.867782652378082
28 0.942969381809235
29 0.951567888259888
30 0.725902259349823
31 0.935538470745087
32 0.892531454563141
33 0.589043140411377
34 0.91327840089798
35 0.725986957550049
36 0.605531096458435
37 0.753952622413635
38 0.738088130950928
39 0.621393203735352
40 0.788572788238525
41 0.733471274375916
42 0.846415638923645
43 0.736884474754333
44 0.687947869300842
45 0.751635372638702
46 0.730733931064606
47 0.636429607868195
48 0.631785869598389
49 0.692318558692932
50 0.738306820392609
51 0.651324331760406
52 0.731996774673462
53 0.893468976020813
54 0.671535611152649
55 0.697271049022675
56 0.687977373600006
57 0.629411399364471
58 0.688868343830109
59 0.633933067321777
60 0.78998726606369
61 0.947069406509399
62 0.904732763767242
63 0.897200286388397
64 0.826858937740326
65 0.885390877723694
66 0.82463937997818
67 0.814436614513397
68 0.955629646778107
69 0.743950247764587
70 0.857869505882263
71 0.73840993642807
72 0.728017449378967
73 0.713949739933014
74 0.863398909568787
75 0.644471287727356
76 0.637135803699493
77 0.838240265846252
78 0.640199184417725
79 0.699765741825104
80 0.850940763950348
81 0.766830384731293
82 0.860307991504669
83 0.956340432167053
84 0.953193306922913
85 0.785702288150787
86 0.692179381847382
87 0.564204454421997
88 0.911361575126648
89 0.755868494510651
90 0.91887891292572
91 0.665454864501953
92 0.702394485473633
93 0.770425915718079
94 0.770683825016022
95 0.738673031330109
96 0.85953277349472
97 0.894066691398621
98 0.760958254337311
99 0.584981977939606
};

\nextgplot
\perturbation
\plotTrue
table {%
0 0.935516519885526
1 0.935516519885526
2 0.935516519885526
3 0.935516519885526
4 0.935516519885526
5 0.935516519885526
6 0.935516519885526
7 0.935516519885526
8 0.935516519885526
9 0.935516519885526
10 0.869667569548439
11 0.727246223885405
12 0.840885440553651
13 0.669861263673315
14 0.695062251008769
15 0.653367486580926
16 0.656677578070439
17 0.60377798372569
18 0.40326589007199
19 0.544277543208332
20 0.634658637120049
21 0.771370029605121
22 0.807328666767555
23 0.705765479890902
24 0.294400085499
25 0.122840677718215
26 0.197476673071808
27 0.344663137249381
28 0.280526511787189
29 0.122459958543774
30 0.199148910512332
31 0.0403795856982413
32 0.0377646706314038
33 0.285823945820197
34 0.0291006444692511
35 0.408406259801238
36 0.408406259801238
37 0.408406259801238
38 0.408406259801238
39 0.408406259801238
40 0.408406259801238
41 0.408406259801238
42 0.408406259801238
43 0.408406259801238
44 0.408406259801238
45 0.408406259801238
46 0.408406259801238
47 0.408406259801238
48 0.408406259801238
49 0.408406259801238
50 0.408406259801238
51 0.408406259801238
52 0.408406259801238
53 0.408406259801238
54 0.408406259801238
55 0.408406259801238
56 0.408406259801238
57 0.408406259801238
58 0.408406259801238
59 0.408406259801238
60 0.402191409831325
61 0.0764337403055456
62 0.0795973866253387
63 0.0646871585761395
64 0.108009977372683
65 0.254616719700893
66 0.472565933463051
67 0.434779798744271
68 0.310130512503765
69 0.335406009918958
70 0.385910215050476
71 0.723644828986625
72 0.677641239833845
73 0.546856821471035
74 0.415658991542201
75 0.241671090622782
76 0.281803188796102
77 0.451510825833016
78 0.503227302170066
79 0.623984732537678
80 0.390940740100067
81 0.383177631440228
82 0.108923776814901
83 0.10020607423564
84 0.106528490954389
85 0.356305650239709
86 0.356305650239709
87 0.356305650239709
88 0.356305650239709
89 0.356305650239709
90 0.356305650239709
91 0.356305650239709
92 0.356305650239709
93 0.356305650239709
94 0.356305650239709
95 0.356305650239709
96 0.356305650239709
97 0.356305650239709
98 0.356305650239709
99 0.356305650239709
};
\plotNetwork
table {%
0 0.937008249790274
1 0.93228152528236
2 0.934681655544366
3 0.940306189008545
4 0.933587990036835
5 0.940835046438332
6 0.936570775494951
7 0.93420340881695
8 0.939329787507813
9 0.933083358981372
10 0.870900408576047
11 0.73789562667266
12 0.842915217569265
13 0.67296813883154
14 0.694941399432263
15 0.658339330302628
16 0.661468613949725
17 0.600541188770209
18 0.411646233028087
19 0.536818481180003
20 0.647409037413542
21 0.783681983949582
22 0.809213732429459
23 0.712058967714881
24 0.296737806650993
25 0.12508469802547
26 0.194739660372333
27 0.329615399349956
28 0.291212811132583
29 0.127808177662935
30 0.215582935088567
31 0.0513131410111266
32 0.0414684928033494
33 0.279570788737977
34 0.027784234503272
35 0.405721087489021
36 0.392467136861572
37 0.419342209835422
38 0.41161564705478
39 0.406178232173927
40 0.41808025398518
41 0.406358463543525
42 0.407240106610816
43 0.410378793993597
44 0.41118259664431
45 0.398090056002662
46 0.39993210278203
47 0.414638853337219
48 0.403845494494099
49 0.402461982735044
50 0.403102214769602
51 0.398202634563599
52 0.41950151572242
53 0.405263284334874
54 0.402412480302431
55 0.407174976311729
56 0.405206022053639
57 0.408675333644624
58 0.419600328102971
59 0.416312846566759
60 0.39777281735889
61 0.0684054711202413
62 0.0918094694095458
63 0.0699603038455095
64 0.116808864440323
65 0.247993003630732
66 0.486107368965571
67 0.455436536881048
68 0.315341573888802
69 0.346674568572516
70 0.372457844113645
71 0.73345859269306
72 0.687912034487404
73 0.55039230410943
74 0.41349676762856
75 0.235013344890034
76 0.281862976429687
77 0.456140730447581
78 0.491381067502036
79 0.613074817378563
80 0.378283170425656
81 0.384452903350201
82 0.10948649440257
83 0.113037646698464
84 0.0911324696846427
85 0.387321286129061
86 0.358615512443052
87 0.358293724308265
88 0.358533709904222
89 0.361884930324889
90 0.364679155986524
91 0.358302750842933
92 0.376904175881704
93 0.358604266798576
94 0.371056245177571
95 0.374403637172375
96 0.357238866692169
97 0.359596646424151
98 0.351273811989109
99 0.357673259151875
};
\plotInvscat
table {%
0 0.937590062618256
1 0.93377810716629
2 0.933303713798523
3 0.938013255596161
4 0.934341609477997
5 0.936702489852905
6 0.928189337253571
7 0.932527542114258
8 0.939745366573334
9 0.933881640434265
10 0.877060115337372
11 0.750461339950562
12 0.842519700527191
13 0.687214493751526
14 0.693723559379578
15 0.650655627250671
16 0.643907845020294
17 0.604818880558014
18 0.438315212726593
19 0.565626204013824
20 0.643522977828979
21 0.775923132896423
22 0.807161748409271
23 0.717244803905487
24 0.286499828100204
25 0.268650770187378
26 0.357445180416107
27 0.294281601905823
28 0.299461662769318
29 0.758662283420563
30 0.247898355126381
31 0.743307411670685
32 0.705825388431549
33 0.757457137107849
34 0.74998539686203
35 0.397328495979309
36 0.494360983371735
37 0.425228327512741
38 0.440925389528275
39 0.484663784503937
40 0.412968069314957
41 0.454484224319458
42 0.372689664363861
43 0.401392549276352
44 0.429087311029434
45 0.444736003875732
46 0.460228085517883
47 0.506758987903595
48 0.466681241989136
49 0.423700362443924
50 0.485979974269867
51 0.44602108001709
52 0.427301615476608
53 0.383714467287064
54 0.446976155042648
55 0.482931077480316
56 0.433276057243347
57 0.480424255132675
58 0.51862233877182
59 0.526852905750275
60 0.415063977241516
61 0.694038689136505
62 0.932928502559662
63 0.868824064731598
64 0.546482503414154
65 0.327510952949524
66 0.477876633405685
67 0.443749159574509
68 0.370432794094086
69 0.336748838424683
70 0.356239914894104
71 0.728031158447266
72 0.715067327022552
73 0.567563652992249
74 0.391675859689713
75 0.553022801876068
76 0.450450032949448
77 0.418966174125671
78 0.603665769100189
79 0.632021844387054
80 0.35116371512413
81 0.402660012245178
82 0.656267106533051
83 0.790334165096283
84 0.725721895694733
85 0.39368087053299
86 0.364321947097778
87 0.477303862571716
88 0.365632027387619
89 0.384704262018204
90 0.375413030385971
91 0.383618623018265
92 0.376277565956116
93 0.386429816484451
94 0.384587168693542
95 0.361544370651245
96 0.340595871210098
97 0.354805052280426
98 0.39489021897316
99 0.652908980846405
};

\nextgplot
\plotTrue
table {%
0 0.824356457355511
1 0.824356457355511
2 0.824356457355511
3 0.824356457355511
4 0.824356457355511
5 0.824356457355511
6 0.824356457355511
7 0.824356457355511
8 0.824356457355511
9 0.824356457355511
10 0.824356457355511
11 0.824356457355511
12 0.824356457355511
13 0.824356457355511
14 0.824356457355511
15 0.824356457355511
16 0.824356457355511
17 0.824356457355511
18 0.824356457355511
19 0.824356457355511
20 0.824356457355511
21 0.824356457355511
22 0.824356457355511
23 0.824356457355511
24 0.824356457355511
25 0.824356457355511
26 0.824356457355511
27 0.824356457355511
28 0.824356457355511
29 0.824356457355511
30 0.824356457355511
31 0.824356457355511
32 0.824356457355511
33 0.824356457355511
34 0.824356457355511
35 0.824356457355511
36 0.824356457355511
37 0.824356457355511
38 0.824356457355511
39 0.824356457355511
40 0.824356457355511
41 0.824356457355511
42 0.824356457355511
43 0.824356457355511
44 0.824356457355511
45 0.824356457355511
46 0.824356457355511
47 0.824356457355511
48 0.824356457355511
49 0.824356457355511
50 0.824356457355511
51 0.824356457355511
52 0.824356457355511
53 0.824356457355511
54 0.824356457355511
55 0.824356457355511
56 0.824356457355511
57 0.824356457355511
58 0.824356457355511
59 0.824356457355511
60 0.824356457355511
61 0.824356457355511
62 0.824356457355511
63 0.824356457355511
64 0.824356457355511
65 0.824356457355511
66 0.824356457355511
67 0.824356457355511
68 0.824356457355511
69 0.824356457355511
70 0.824356457355511
71 0.824356457355511
72 0.824356457355511
73 0.824356457355511
74 0.824356457355511
75 0.824356457355511
76 0.824356457355511
77 0.824356457355511
78 0.824356457355511
79 0.824356457355511
80 0.824356457355511
81 0.824356457355511
82 0.824356457355511
83 0.824356457355511
84 0.824356457355511
85 0.824356457355511
86 0.824356457355511
87 0.824356457355511
88 0.824356457355511
89 0.824356457355511
90 0.824356457355511
91 0.824356457355511
92 0.824356457355511
93 0.824356457355511
94 0.824356457355511
95 0.824356457355511
96 0.824356457355511
97 0.824356457355511
98 0.824356457355511
99 0.824356457355511
};
\plotNetwork
table {%
0 0.824918097106847
1 0.820805473213107
2 0.828472308367963
3 0.812617850050961
4 0.823493238962109
5 0.818162713317453
6 0.824445123610635
7 0.818480028608659
8 0.825962798694261
9 0.827469587123433
10 0.827328391690207
11 0.823091456118911
12 0.825769547908097
13 0.820411373049875
14 0.820711516059964
15 0.825168869506147
16 0.822629948625476
17 0.822090221162817
18 0.826285081879092
19 0.822253898109393
20 0.820269623036023
21 0.816654208792078
22 0.830749773815934
23 0.817302395178878
24 0.830648468839112
25 0.812755934104617
26 0.82557523171586
27 0.822299789006603
28 0.819324859061303
29 0.803509795636962
30 0.793862515973959
31 0.667955377763708
32 0.680906938466793
33 0.831884189355057
34 0.606659483134413
35 0.825965659679777
36 0.848423209204983
37 0.813450033612018
38 0.821313611677879
39 0.831698523084578
40 0.825545262995
41 0.82689264249719
42 0.817997720017116
43 0.819672784526886
44 0.824747163102983
45 0.823794936676618
46 0.824063603311838
47 0.815051412004305
48 0.831250522455995
49 0.836938058687949
50 0.823264830164416
51 0.839897594896012
52 0.829317551809204
53 0.821175031126535
54 0.813978577535757
55 0.845653536337044
56 0.833381079791454
57 0.827657483270769
58 0.816215385023334
59 0.816088971866439
60 0.809500890885212
61 0.781905224377604
62 0.833692747322618
63 0.790312757102203
64 0.780431720632574
65 0.817420922622318
66 0.816838333461772
67 0.808332537054545
68 0.822790050761497
69 0.822653986803072
70 0.821489856298283
71 0.818897054124881
72 0.813780383291536
73 0.829653950770275
74 0.831059152302501
75 0.841849219533456
76 0.808767737428718
77 0.827249101722096
78 0.825126932065271
79 0.826401564246548
80 0.82907266691811
81 0.818450441451776
82 0.824370549844991
83 0.805459805612383
84 0.865001744256248
85 0.796857125971991
86 0.824346553628545
87 0.819643777789211
88 0.828704627256444
89 0.819778939845764
90 0.811016099417677
91 0.818453127832454
92 0.808077070677335
93 0.82530629881134
94 0.81563742636852
95 0.811970482966281
96 0.822371102252437
97 0.835626194232124
98 0.838590272808172
99 0.820161630074723
};
\plotInvscat
table {%
0 0.826118171215057
1 0.819175541400909
2 0.825987696647644
3 0.810961246490479
4 0.823848783969879
5 0.828949093818665
6 0.820728421211243
7 0.807135164737701
8 0.830820560455322
9 0.829845488071442
10 0.808938145637512
11 0.808563709259033
12 0.825683414936066
13 0.811578214168549
14 0.818180620670319
15 0.813442945480347
16 0.834097802639008
17 0.812789559364319
18 0.959390580654144
19 0.764434278011322
20 0.80391263961792
21 0.836773157119751
22 0.811366558074951
23 0.807386755943298
24 0.825904607772827
25 0.38533091545105
26 0.448476999998093
27 0.796378314495087
28 0.653123736381531
29 0.170539319515228
30 0.775648832321167
31 0.719486951828003
32 0.25947704911232
33 0.870226263999939
34 0.786252021789551
35 0.876884758472443
36 0.857750535011292
37 0.780718684196472
38 0.780907213687897
39 0.922427535057068
40 0.76628041267395
41 0.764958322048187
42 0.768586218357086
43 0.832319855690002
44 0.872885346412659
45 0.738358020782471
46 0.759409189224243
47 0.917904257774353
48 0.945412337779999
49 0.841683030128479
50 0.737103819847107
51 0.890260457992554
52 0.797455668449402
53 0.676310062408447
54 0.914264380931854
55 0.772879183292389
56 0.847297489643097
57 0.908163905143738
58 0.796705663204193
59 0.955634713172913
60 0.731623947620392
61 0.35390967130661
62 0.157999396324158
63 0.276242017745972
64 0.247377440333366
65 0.484331965446472
66 0.734599053859711
67 0.729989647865295
68 0.507282376289368
69 0.887809693813324
70 0.719929933547974
71 0.830412447452545
72 0.824100911617279
73 0.837259411811829
74 0.714009702205658
75 0.804185271263123
76 0.761443853378296
77 0.777647078037262
78 0.865281403064728
79 0.865645825862885
80 0.745762288570404
81 0.734923601150513
82 0.461039215326309
83 0.20957887172699
84 0.216678768396378
85 0.776257932186127
86 0.838222563266754
87 0.851630210876465
88 0.739989936351776
89 0.755538523197174
90 0.717871427536011
91 0.847862899303436
92 0.846059322357178
93 0.855170667171478
94 0.791229486465454
95 0.830167412757874
96 0.773104250431061
97 0.768534243106842
98 0.714451372623444
99 0.968196153640747
};

\nextgplot
\plotTrue
table {%
0 0.753602486017811
1 0.753602486017811
2 0.753602486017811
3 0.753602486017811
4 0.753602486017811
5 0.753602486017811
6 0.753602486017811
7 0.753602486017811
8 0.753602486017811
9 0.753602486017811
10 0.753602486017811
11 0.753602486017811
12 0.753602486017811
13 0.753602486017811
14 0.753602486017811
15 0.753602486017811
16 0.753602486017811
17 0.753602486017811
18 0.753602486017811
19 0.753602486017811
20 0.753602486017811
21 0.753602486017811
22 0.753602486017811
23 0.753602486017811
24 0.753602486017811
25 0.753602486017811
26 0.753602486017811
27 0.753602486017811
28 0.753602486017811
29 0.753602486017811
30 0.753602486017811
31 0.753602486017811
32 0.753602486017811
33 0.753602486017811
34 0.753602486017811
35 0.753602486017811
36 0.753602486017811
37 0.753602486017811
38 0.753602486017811
39 0.753602486017811
40 0.753602486017811
41 0.753602486017811
42 0.753602486017811
43 0.753602486017811
44 0.753602486017811
45 0.753602486017811
46 0.753602486017811
47 0.753602486017811
48 0.753602486017811
49 0.753602486017811
50 0.753602486017811
51 0.753602486017811
52 0.753602486017811
53 0.753602486017811
54 0.753602486017811
55 0.753602486017811
56 0.753602486017811
57 0.753602486017811
58 0.753602486017811
59 0.753602486017811
60 0.753602486017811
61 0.753602486017811
62 0.753602486017811
63 0.753602486017811
64 0.753602486017811
65 0.753602486017811
66 0.753602486017811
67 0.753602486017811
68 0.753602486017811
69 0.753602486017811
70 0.753602486017811
71 0.753602486017811
72 0.753602486017811
73 0.753602486017811
74 0.753602486017811
75 0.753602486017811
76 0.753602486017811
77 0.753602486017811
78 0.753602486017811
79 0.753602486017811
80 0.753602486017811
81 0.753602486017811
82 0.753602486017811
83 0.753602486017811
84 0.753602486017811
85 0.753602486017811
86 0.753602486017811
87 0.753602486017811
88 0.753602486017811
89 0.753602486017811
90 0.753602486017811
91 0.753602486017811
92 0.753602486017811
93 0.753602486017811
94 0.753602486017811
95 0.753602486017811
96 0.753602486017811
97 0.753602486017811
98 0.753602486017811
99 0.753602486017811
};
\plotNetwork
table {%
0 0.756658633313087
1 0.758112336457293
2 0.753866318719009
3 0.758046274285873
4 0.756437303675497
5 0.753436369395479
6 0.756894130003363
7 0.743901105085812
8 0.74986748077773
9 0.751521810630191
10 0.739972705619684
11 0.744547637309059
12 0.756513723533636
13 0.753226309045404
14 0.761907698876359
15 0.755428172860475
16 0.750498965648106
17 0.751453127204149
18 0.755973695029891
19 0.755763903000447
20 0.743445255298062
21 0.745995715206324
22 0.75056479036052
23 0.736297707272107
24 0.755351965968844
25 0.747211218368944
26 0.757773814262203
27 0.758010981246058
28 0.752881596817825
29 0.768170925456723
30 0.746988172555567
31 0.741800979573317
32 0.762582440683985
33 0.74747941885651
34 0.748701382670807
35 0.748589682343185
36 0.732691576389301
37 0.756129959957879
38 0.766926380448189
39 0.751692412153566
40 0.756831821683899
41 0.760762146138877
42 0.759197429559509
43 0.751956074985802
44 0.751181858972488
45 0.758239127253753
46 0.761861785594236
47 0.759676353624678
48 0.759744849549725
49 0.748152838698405
50 0.760714736910984
51 0.740646270113544
52 0.749527844669729
53 0.751519430424586
54 0.754294614553682
55 0.743816770911572
56 0.752804277815104
57 0.751838733875491
58 0.761390389206923
59 0.760400044971924
60 0.761974040730453
61 0.754212568859263
62 0.748751145455918
63 0.762518424254598
64 0.764300663447258
65 0.757962830165492
66 0.761827957426383
67 0.759066612072308
68 0.765737877658296
69 0.758140587648946
70 0.76573355703881
71 0.763761574802872
72 0.755347793191554
73 0.750245068150617
74 0.753403553046212
75 0.749863949309668
76 0.767280888893683
77 0.755553078269048
78 0.744354569328434
79 0.751548776802022
80 0.755175610172128
81 0.75325665868013
82 0.755406825942717
83 0.755787646877689
84 0.765532326059897
85 0.733395875730224
86 0.747692074774075
87 0.755107477600537
88 0.765318293498251
89 0.763574959629035
90 0.74413032974455
91 0.743297722438877
92 0.750130425186743
93 0.755057587915789
94 0.736210049214179
95 0.741267656415925
96 0.765285052885183
97 0.753585698919908
98 0.757529896814226
99 0.753190783672525
};
\plotInvscat
table {%
0 0.765485644340515
1 0.743608474731445
2 0.759783565998077
3 0.748197138309479
4 0.757139325141907
5 0.757455408573151
6 0.736839175224304
7 0.730532228946686
8 0.753419041633606
9 0.756273448467255
10 0.735128343105316
11 0.741503536701202
12 0.734744906425476
13 0.728635251522064
14 0.752566158771515
15 0.762928605079651
16 0.741893231868744
17 0.732393801212311
18 0.80504322052002
19 0.681286454200745
20 0.705391943454742
21 0.752124965190887
22 0.735611438751221
23 0.715493559837341
24 0.710643708705902
25 0.63262540102005
26 0.529463171958923
27 0.709796369075775
28 0.747408866882324
29 0.368635326623917
30 0.751903057098389
31 0.0468631498515606
32 0.170688301324844
33 0.550658464431763
34 0.0339839123189449
35 0.735814332962036
36 0.690836131572723
37 0.76999843120575
38 0.764298498630524
39 0.708936929702759
40 0.783700585365295
41 0.750074982643127
42 0.800572752952576
43 0.751893043518066
44 0.732159852981567
45 0.760867059230804
46 0.754486978054047
47 0.703615188598633
48 0.715050339698792
49 0.738860666751862
50 0.753443956375122
51 0.710836350917816
52 0.753164887428284
53 0.822261273860931
54 0.71344381570816
55 0.732096135616302
56 0.741585433483124
57 0.706904113292694
58 0.730911016464233
59 0.694978833198547
60 0.790401697158813
61 0.144316956400871
62 0.317562103271484
63 0.175176069140434
64 0.553827166557312
65 0.830596208572388
66 0.805016458034515
67 0.794123530387878
68 0.882252275943756
69 0.747471451759338
70 0.813896775245667
71 0.764928996562958
72 0.745576798915863
73 0.740409374237061
74 0.818698346614838
75 0.577649235725403
76 0.715736329555511
77 0.800718784332275
78 0.690972864627838
79 0.728834986686707
80 0.797002136707306
81 0.76758486032486
82 0.21536086499691
83 0.374850004911423
84 0.262014716863632
85 0.730629086494446
86 0.770918786525726
87 0.823908269405365
88 0.678847074508667
89 0.751074492931366
90 0.66613894701004
91 0.777786374092102
92 0.764000952243805
93 0.824736297130585
94 0.726815342903137
95 0.751832067966461
96 0.712317109107971
97 0.708563387393951
98 0.757635831832886
99 0.845717549324036
};
\lastgplot{5}
\plotTrue
table {%
0 0.935826238137458
1 0.935826238137458
2 0.935826238137458
3 0.935826238137458
4 0.935826238137458
5 0.935826238137458
6 0.935826238137458
7 0.935826238137458
8 0.935826238137458
9 0.935826238137458
10 0.935826238137458
11 0.935826238137458
12 0.935826238137458
13 0.935826238137458
14 0.935826238137458
15 0.935826238137458
16 0.935826238137458
17 0.935826238137458
18 0.935826238137458
19 0.935826238137458
20 0.935826238137458
21 0.935826238137458
22 0.935826238137458
23 0.935826238137458
24 0.935826238137458
25 0.935826238137458
26 0.935826238137458
27 0.935826238137458
28 0.935826238137458
29 0.935826238137458
30 0.935826238137458
31 0.935826238137458
32 0.935826238137458
33 0.935826238137458
34 0.935826238137458
35 0.935826238137458
36 0.935826238137458
37 0.935826238137458
38 0.935826238137458
39 0.935826238137458
40 0.935826238137458
41 0.935826238137458
42 0.935826238137458
43 0.935826238137458
44 0.935826238137458
45 0.935826238137458
46 0.935826238137458
47 0.935826238137458
48 0.935826238137458
49 0.935826238137458
50 0.935826238137458
51 0.935826238137458
52 0.935826238137458
53 0.935826238137458
54 0.935826238137458
55 0.935826238137458
56 0.935826238137458
57 0.935826238137458
58 0.935826238137458
59 0.935826238137458
60 0.935826238137458
61 0.935826238137458
62 0.935826238137458
63 0.935826238137458
64 0.935826238137458
65 0.935826238137458
66 0.935826238137458
67 0.935826238137458
68 0.935826238137458
69 0.935826238137458
70 0.935826238137458
71 0.935826238137458
72 0.935826238137458
73 0.935826238137458
74 0.935826238137458
75 0.935826238137458
76 0.935826238137458
77 0.935826238137458
78 0.935826238137458
79 0.935826238137458
80 0.935826238137458
81 0.935826238137458
82 0.935826238137458
83 0.935826238137458
84 0.935826238137458
85 0.935826238137458
86 0.935826238137458
87 0.935826238137458
88 0.935826238137458
89 0.935826238137458
90 0.935826238137458
91 0.935826238137458
92 0.935826238137458
93 0.935826238137458
94 0.935826238137458
95 0.935826238137458
96 0.935826238137458
97 0.935826238137458
98 0.935826238137458
99 0.935826238137458
};
\plotNetwork
table {%
0 0.932496165935702
1 0.939059021339415
2 0.938267655613657
3 0.940753784941949
4 0.932927189302818
5 0.93831761853484
6 0.938550892781673
7 0.935714384728785
8 0.934285131400605
9 0.93367046011082
10 0.933889671785219
11 0.932253118994358
12 0.935904111938848
13 0.936348266570327
14 0.936657636220485
15 0.93321355549188
16 0.938642472606434
17 0.933663851425937
18 0.934440585223916
19 0.936301391894993
20 0.936674698979961
21 0.936759660875247
22 0.935063652897508
23 0.934081236234154
24 0.934060039849845
25 0.935590457983809
26 0.938949674274355
27 0.934181322147956
28 0.92945154189157
29 0.932077215958626
30 0.93385836091723
31 0.928265605089783
32 0.939383500545753
33 0.93544976830031
34 0.934358385965256
35 0.933778700332574
36 0.933664066857236
37 0.936083589292542
38 0.937731058614872
39 0.934027004717849
40 0.941243139428584
41 0.935870653479343
42 0.935227193520271
43 0.938328000236214
44 0.936640332793648
45 0.936108974875476
46 0.936861703576487
47 0.934073140107091
48 0.935975009751585
49 0.934674979038702
50 0.934762000275245
51 0.929243421255006
52 0.931913270214935
53 0.933149899522974
54 0.933395269883336
55 0.933183555880362
56 0.932336311150301
57 0.937085122220454
58 0.940977901210475
59 0.933801000921232
60 0.939959774807744
61 0.933874181488063
62 0.93175804378107
63 0.936536667843127
64 0.93478120455052
65 0.932062546450337
66 0.939446660351899
67 0.943004129342372
68 0.936486296889439
69 0.93559419454582
70 0.93863618857543
71 0.941427659098514
72 0.938404895191101
73 0.935858053761902
74 0.931756571430617
75 0.936825909011827
76 0.937737790459246
77 0.937234280963579
78 0.935169256216919
79 0.936754460680673
80 0.933607188017634
81 0.944966325818166
82 0.939035449765745
83 0.935387942305792
84 0.937288914277197
85 0.933872539351418
86 0.936021214423398
87 0.929064646912235
88 0.935062203012433
89 0.939060517767322
90 0.933213176525754
91 0.934448733720871
92 0.936803750107657
93 0.935970719428859
94 0.934701988506175
95 0.938234016008683
96 0.935622002578045
97 0.937633515641471
98 0.931842623682334
99 0.935327146007421
};
\plotInvscat
table {%
0 0.935478329658508
1 0.935988903045654
2 0.941328942775726
3 0.939885139465332
4 0.935139238834381
5 0.932519018650055
6 0.934479713439941
7 0.934692978858948
8 0.93408215045929
9 0.933540344238281
10 0.943984746932983
11 0.937299311161041
12 0.927669703960419
13 0.936007857322693
14 0.936262428760529
15 0.938920438289642
16 0.932485103607178
17 0.92876797914505
18 0.921623051166534
19 0.927580654621124
20 0.926243305206299
21 0.929543793201447
22 0.939578950405121
23 0.931917190551758
24 0.919988691806793
25 0.940652251243591
26 0.92027884721756
27 0.91811203956604
28 0.900859475135803
29 0.930002450942993
30 0.931769013404846
31 0.782492101192474
32 0.834356129169464
33 0.94639778137207
34 0.803377330303192
35 0.921040952205658
36 0.944006562232971
37 0.940845131874084
38 0.942033231258392
39 0.929262638092041
40 0.93747466802597
41 0.950068295001984
42 0.926220118999481
43 0.93650758266449
44 0.927292883396149
45 0.945561528205872
46 0.945005774497986
47 0.922697484493256
48 0.939450025558472
49 0.93846732378006
50 0.951403796672821
51 0.923181891441345
52 0.933490514755249
53 0.928642690181732
54 0.92754065990448
55 0.951437652111053
56 0.935454785823822
57 0.938190340995789
58 0.955077350139618
59 0.92485386133194
60 0.948755979537964
61 0.825660586357117
62 0.873731851577759
63 0.833996534347534
64 0.967193007469177
65 0.936348378658295
66 0.944916367530823
67 0.946979403495789
68 0.931073009967804
69 0.928756773471832
70 0.938057243824005
71 0.934084832668304
72 0.94188529253006
73 0.935397922992706
74 0.925875842571259
75 0.925759792327881
76 0.956682145595551
77 0.924597859382629
78 0.94838809967041
79 0.931387722492218
80 0.927379190921783
81 0.948466062545776
82 0.83814948797226
83 0.855083525180817
84 0.823061943054199
85 0.934764564037323
86 0.944090962409973
87 0.936683356761932
88 0.906428515911102
89 0.940659284591675
90 0.914661288261414
91 0.936943650245667
92 0.938408493995667
93 0.919454276561737
94 0.935905635356903
95 0.940755367279053
96 0.925517976284027
97 0.907075881958008
98 0.942062973976135
99 0.930044889450073
};
\end{groupplot}

==> Figs/random_phi_change/noise_0.05.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm, group name=column4 plots,}]

%================= Fig1 ===============
\firstgplot{column3}{$\sigma^2_{z}=0.05$}
\plotTrue
table {%
0 0.733099880094478
1 0.733099880094478
2 0.733099880094478
3 0.733099880094478
4 0.733099880094478
5 0.733099880094478
6 0.733099880094478
7 0.733099880094478
8 0.733099880094478
9 0.733099880094478
10 0.733099880094478
11 0.733099880094478
12 0.733099880094478
13 0.733099880094478
14 0.733099880094478
15 0.733099880094478
16 0.733099880094478
17 0.733099880094478
18 0.733099880094478
19 0.733099880094478
20 0.733099880094478
21 0.733099880094478
22 0.733099880094478
23 0.733099880094478
24 0.733099880094478
25 0.733099880094478
26 0.733099880094478
27 0.733099880094478
28 0.733099880094478
29 0.733099880094478
30 0.733099880094478
31 0.733099880094478
32 0.733099880094478
33 0.733099880094478
34 0.733099880094478
35 0.733099880094478
36 0.733099880094478
37 0.733099880094478
38 0.733099880094478
39 0.733099880094478
40 0.733099880094478
41 0.733099880094478
42 0.733099880094478
43 0.733099880094478
44 0.733099880094478
45 0.733099880094478
46 0.733099880094478
47 0.733099880094478
48 0.733099880094478
49 0.733099880094478
50 0.733099880094478
51 0.733099880094478
52 0.733099880094478
53 0.733099880094478
54 0.733099880094478
55 0.733099880094478
56 0.733099880094478
57 0.733099880094478
58 0.733099880094478
59 0.733099880094478
60 0.733099880094478
61 0.733099880094478
62 0.733099880094478
63 0.733099880094478
64 0.733099880094478
65 0.733099880094478
66 0.733099880094478
67 0.733099880094478
68 0.733099880094478
69 0.733099880094478
70 0.733099880094478
71 0.733099880094478
72 0.733099880094478
73 0.733099880094478
74 0.733099880094478
75 0.733099880094478
76 0.733099880094478
77 0.733099880094478
78 0.733099880094478
79 0.733099880094478
80 0.733099880094478
81 0.733099880094478
82 0.733099880094478
83 0.733099880094478
84 0.733099880094478
85 0.733099880094478
86 0.733099880094478
87 0.733099880094478
88 0.733099880094478
89 0.733099880094478
90 0.733099880094478
91 0.733099880094478
92 0.733099880094478
93 0.733099880094478
94 0.733099880094478
95 0.733099880094478
96 0.733099880094478
97 0.733099880094478
98 0.733099880094478
99 0.733099880094478
};
\plotNetwork
table {%
0 0.701037757660696
1 0.718209130871583
2 0.74758864961937
3 0.824353916215254
4 0.681511377916777
5 0.79009312052309
6 0.630297281255304
7 0.620845079020654
8 0.797605293274455
9 0.820536001860519
10 0.788452510728887
11 0.814486791636274
12 0.693252624431775
13 0.778843276400072
14 0.769159430660787
15 0.92337083151805
16 0.746385548119403
17 0.751275377990453
18 0.603164392861955
19 0.211821121226158
20 0.981062243874762
21 0.994275648126738
22 0.968524435437576
23 0.707140675109942
24 0.90928688892463
25 0.653320358211108
26 0.80103587148403
27 0.975006887655294
28 0.725799905558197
29 0.508522621519687
30 0.319524186323321
31 0.347283402335658
32 0.854839571225869
33 0.701784617342509
34 0.820190918908312
35 0.596307867966686
36 0.328961953221582
37 0.737857865022689
38 0.763119450429465
39 0.704831120760853
40 0.708763362013017
41 0.81807463124234
42 0.750386831413146
43 0.696186242202723
44 0.677923959843279
45 0.739086861653739
46 0.792665170159163
47 0.824415078133492
48 0.829121093966165
49 0.913588215224891
50 0.017418138789787
51 0.851854788207698
52 0.720380547512732
53 0.694534077298912
54 0.672032239335589
55 0.791229063207301
56 0.64993200890174
57 0.730867519177868
58 0.610860949891164
59 0.789728429964152
60 0.72210698491416
61 0.742777011297312
62 0.789395231450567
63 0.715396615833244
64 0.721889694598315
65 0.739055957058581
66 0.771390793435708
67 0.745636245654569
68 0.918739423584038
69 0.60270045622613
70 0.68539213272199
71 0.575928700416139
72 0.403226238236469
73 0.759110097714513
74 0.729412306387297
75 0.807345108100836
76 0.69510555560801
77 0.688812987859503
78 0.744043978348694
79 0.734034965648194
80 0.785547530538224
81 0.724363735080346
82 0.713631912813801
83 0.76667340750435
84 0.686644314530265
85 0.783865957931501
86 0.824306725477438
87 0.796475247482322
88 0.758058374982748
89 0.621292990865178
90 0.778390162457789
91 0.789969098341779
92 0.731234711660586
93 0.748136293336782
94 0.783672871315179
95 0.763075849406034
96 0.667495294039547
97 0.713056673520131
98 0.734356027566899
99 0.682261379655806
};
\plotInvscat
table {%
0 0.650964200496674
1 0.868047595024109
2 0.645489513874054
3 0.92617791891098
4 0.675906717777252
5 0.718429207801819
6 0.956974506378174
7 0.978378653526306
8 0.897055506706238
9 0.868464350700378
10 0.901603400707245
11 0.846219301223755
12 0.807828843593597
13 0.883489608764648
14 0.967899739742279
15 0.968582212924957
16 0.977492809295654
17 0.963654518127441
18 0.978018999099731
19 0.897722363471985
20 0.944060266017914
21 0.999095022678375
22 0.836026847362518
23 0.713215231895447
24 0.788799524307251
25 0.869330108165741
26 0.911834239959717
27 0.856816112995148
28 0.896671891212463
29 0.953168034553528
30 0.914775013923645
31 0.858295381069183
32 0.906507074832916
33 0.689737677574158
34 0.842579066753387
35 0.83554208278656
36 0.821429550647736
37 0.755707025527954
38 0.746000349521637
39 0.614566147327423
40 0.822428405284882
41 0.864647150039673
42 0.849678218364716
43 0.944554805755615
44 0.642213106155396
45 0.776568830013275
46 0.625036001205444
47 0.692387640476227
48 0.912317276000977
49 0.964655697345734
50 0.893039166927338
51 0.935515165328979
52 0.882047533988953
53 0.624517440795898
54 0.692585825920105
55 0.78101646900177
56 0.597664177417755
57 0.866927087306976
58 0.939165949821472
59 0.863916516304016
60 0.757529497146606
61 0.800810098648071
62 0.750938057899475
63 0.633297979831696
64 0.787122189998627
65 0.718626081943512
66 0.88569974899292
67 0.860125720500946
68 0.990552365779877
69 0.544388294219971
70 0.811367273330688
71 0.984160661697388
72 0.936759650707245
73 0.939813315868378
74 0.627211570739746
75 0.8066685795784
76 0.86497437953949
77 0.839003026485443
78 0.907007932662964
79 0.664039373397827
80 0.76863557100296
81 0.865499556064606
82 0.908938944339752
83 0.96473902463913
84 0.929736852645874
85 0.757835745811462
86 0.749137938022614
87 0.713777244091034
88 0.961768090724945
89 0.783295929431915
90 0.93220454454422
91 0.782213807106018
92 0.746971607208252
93 0.731738865375519
94 0.73894077539444
95 0.696846187114716
96 0.82795912027359
97 0.873764514923096
98 0.772973656654358
99 0.609536170959473
};

%================= Fig2 ===============
\nextgplot
\plotTrue
table {%
0 0.869667569548439
1 0.727246223885405
2 0.840885440553651
3 0.669861263673315
4 0.695062251008769
5 0.653367486580926
6 0.656677578070439
7 0.60377798372569
8 0.40326589007199
9 0.544277543208332
10 0.634658637120049
11 0.771370029605121
12 0.807328666767555
13 0.705765479890902
14 0.294400085499
15 0.122840677718215
16 0.197476673071808
17 0.344663137249381
18 0.280526511787189
19 0.122459958543774
20 0.199148910512332
21 0.0403795856982413
22 0.0377646706314038
23 0.285823945820197
24 0.0291006444692511
25 0.408406259801238
26 0.402191409831325
27 0.0764337403055456
28 0.0795973866253387
29 0.0646871585761395
30 0.108009977372683
31 0.254616719700893
32 0.472565933463051
33 0.434779798744271
34 0.310130512503765
35 0.335406009918958
36 0.385910215050476
37 0.723644828986625
38 0.677641239833845
39 0.546856821471035
40 0.415658991542201
41 0.241671090622782
42 0.281803188796102
43 0.451510825833016
44 0.503227302170066
45 0.623984732537678
46 0.390940740100067
47 0.383177631440228
48 0.108923776814901
49 0.10020607423564
50 0.106528490954389
51 0.356305650239709
52 0.509202138693795
53 0.74413390158102
54 0.81101706693246
55 0.810240320487004
56 0.786082444625873
57 0.624447951542734
58 0.628205739649137
59 0.778406648557381
60 0.912853453932987
61 0.927722589024184
62 0.90177220250271
63 0.803403009410264
64 0.906760898229527
65 0.73492833905465
66 0.76219373229
67 0.573644458638233
68 0.289492391785003
69 0.646380087598337
70 0.588199277469668
71 0.553075559497109
72 0.275274238102345
73 0.406329057913021
74 0.593899997693344
75 0.700896359886824
76 0.803060462023582
77 0.546610904651393
78 0.437422359479522
79 0.51582077325451
80 0.632650269024677
81 0.608144950244214
82 0.586839840006901
83 0.506294720218665
84 0.707796078209189
85 0.806236508567857
86 0.560211747194239
87 0.613261338539432
88 0.472899698708128
89 0.353479066535235
90 0.637576222061667
91 0.767451809236169
92 0.889307839253587
93 0.925314520932734
94 0.827617243600845
95 0.763608670049797
96 0.738720375838479
97 0.629119639711527
98 0.903428257766421
99 0.742557403873145
};
\plotNetwork
table {%
0 0.886905960206787
1 0.699371826688955
2 0.829010856258512
3 0.768017762041934
4 0.658321395395425
5 0.732133660592768
6 0.620408613855504
7 0.478400130793998
8 0.488328269918267
9 0.587266150055454
10 0.654440032823355
11 0.833140855384313
12 0.812961232336846
13 0.727118535950975
14 0.244001138571272
15 0.667390013319938
16 0.245433839546645
17 0.364852049172897
18 0.362962443046667
19 0.0535332188786805
20 0.394292265905469
21 0.474692600139641
22 0.47032249897376
23 0.422465880981253
24 0.01088068971245
25 0.379563841327514
26 0.416306012405317
27 0.0940696832434959
28 0.0174282970744097
29 0.146186062814773
30 0.0740540924667967
31 0.207924375816397
32 0.477849044662456
33 0.378844199476362
34 0.256384398871546
35 0.306095496463405
36 0.319796592009623
37 0.765164837073851
38 0.692017852953222
39 0.552436491086325
40 0.465735591429308
41 0.253940407043263
42 0.247994806964485
43 0.490110934490416
44 0.525177830605152
45 0.558183737603856
46 0.343920770906482
47 0.435702916405835
48 0.102218336874091
49 0.184900966974971
50 0.207745484938555
51 0.528365936437719
52 0.43364363491595
53 0.669507077689759
54 0.845418623259523
55 0.79302706575338
56 0.68643693686782
57 0.654229216642238
58 0.544194731727899
59 0.811036469679697
60 0.89197469538672
61 0.906494797141938
62 0.903737934591535
63 0.714119820279714
64 0.889279602092147
65 0.75072925900402
66 0.713276062607847
67 0.518049319843304
68 0.315288759625203
69 0.554587406272117
70 0.5635446184228
71 0.415319234633577
72 0.231089599011751
73 0.376085755939881
74 0.600470377988535
75 0.733135963222739
76 0.784970232011953
77 0.422415812736415
78 0.587053833814135
79 0.638415707243718
80 0.640475911512147
81 0.591289581777452
82 0.614222613676906
83 0.497206578383012
84 0.635538419528637
85 0.866185818078147
86 0.581644353238371
87 0.627427466857216
88 0.478370907894213
89 0.384372411897403
90 0.642375599922114
91 0.757657728434689
92 0.921252708762492
93 0.913136493058283
94 0.896547384716672
95 0.816578997036175
96 0.718707682424538
97 0.649371482375051
98 0.897428043758278
99 0.74114445467213
};
\plotInvscat
table {%
0 0.907985627651215
1 0.799874007701874
2 0.855573952198029
3 0.814481675624847
4 0.654519021511078
5 0.685006380081177
6 0.724644303321838
7 0.834904193878174
8 0.537715435028076
9 0.568016946315765
10 0.786475539207458
11 0.870562851428986
12 0.86906111240387
13 0.803560078144073
14 0.606497406959534
15 0.614240407943726
16 0.764671683311462
17 0.732868492603302
18 0.925377309322357
19 0.826867282390594
20 0.725832343101501
21 0.544109523296356
22 0.803411424160004
23 0.586462378501892
24 0.754185080528259
25 0.642565488815308
26 0.474680662155151
27 0.875406622886658
28 0.873602390289307
29 0.901014745235443
30 0.44187718629837
31 0.833190500736237
32 0.511555314064026
33 0.750616669654846
34 0.767375469207764
35 0.888940572738647
36 0.741707623004913
37 0.751530885696411
38 0.751019179821014
39 0.862871825695038
40 0.546595692634583
41 0.994423151016235
42 0.945204496383667
43 0.818181037902832
44 0.682206153869629
45 0.660971283912659
46 0.660616755485535
47 0.786165118217468
48 0.817305505275726
49 0.81824254989624
50 0.860466778278351
51 0.878096699714661
52 0.631619930267334
53 0.850128531455994
54 0.844970345497131
55 0.817430257797241
56 0.774996817111969
57 0.685357630252838
58 0.668820321559906
59 0.850277423858643
60 0.886224269866943
61 0.897939443588257
62 0.886452376842499
63 0.61254209280014
64 0.861404240131378
65 0.80286431312561
66 0.73410040140152
67 0.622812807559967
68 0.614718973636627
69 0.624194383621216
70 0.565080583095551
71 0.759974002838135
72 0.818785309791565
73 0.591146469116211
74 0.652330458164215
75 0.744364023208618
76 0.752013444900513
77 0.464223116636276
78 0.632040977478027
79 0.654129862785339
80 0.620521128177643
81 0.602456331253052
82 0.791552364826202
83 0.642370045185089
84 0.657659828662872
85 0.854652523994446
86 0.508301138877869
87 0.755664885044098
88 0.627735376358032
89 0.501227200031281
90 0.674298524856567
91 0.78253960609436
92 0.914167284965515
93 0.88948929309845
94 0.897024571895599
95 0.799589097499847
96 0.647133588790894
97 0.672952234745026
98 0.912498354911804
99 0.838185787200928
};
%================= Fig3 ===============
\nextgplot
\plotTrue
table {%
0 0.824356457355511
1 0.824356457355511
2 0.824356457355511
3 0.824356457355511
4 0.824356457355511
5 0.824356457355511
6 0.824356457355511
7 0.824356457355511
8 0.824356457355511
9 0.824356457355511
10 0.824356457355511
11 0.824356457355511
12 0.824356457355511
13 0.824356457355511
14 0.824356457355511
15 0.824356457355511
16 0.824356457355511
17 0.824356457355511
18 0.824356457355511
19 0.824356457355511
20 0.824356457355511
21 0.824356457355511
22 0.824356457355511
23 0.824356457355511
24 0.824356457355511
25 0.824356457355511
26 0.824356457355511
27 0.824356457355511
28 0.824356457355511
29 0.824356457355511
30 0.824356457355511
31 0.824356457355511
32 0.824356457355511
33 0.824356457355511
34 0.824356457355511
35 0.824356457355511
36 0.824356457355511
37 0.824356457355511
38 0.824356457355511
39 0.824356457355511
40 0.824356457355511
41 0.824356457355511
42 0.824356457355511
43 0.824356457355511
44 0.824356457355511
45 0.824356457355511
46 0.824356457355511
47 0.824356457355511
48 0.824356457355511
49 0.824356457355511
50 0.824356457355511
51 0.824356457355511
52 0.824356457355511
53 0.824356457355511
54 0.824356457355511
55 0.824356457355511
56 0.824356457355511
57 0.824356457355511
58 0.824356457355511
59 0.824356457355511
60 0.824356457355511
61 0.824356457355511
62 0.824356457355511
63 0.824356457355511
64 0.824356457355511
65 0.824356457355511
66 0.824356457355511
67 0.824356457355511
68 0.824356457355511
69 0.824356457355511
70 0.824356457355511
71 0.824356457355511
72 0.824356457355511
73 0.824356457355511
74 0.824356457355511
75 0.824356457355511
76 0.824356457355511
77 0.824356457355511
78 0.824356457355511
79 0.824356457355511
80 0.824356457355511
81 0.824356457355511
82 0.824356457355511
83 0.824356457355511
84 0.824356457355511
85 0.824356457355511
86 0.824356457355511
87 0.824356457355511
88 0.824356457355511
89 0.824356457355511
90 0.824356457355511
91 0.824356457355511
92 0.824356457355511
93 0.824356457355511
94 0.824356457355511
95 0.824356457355511
96 0.824356457355511
97 0.824356457355511
98 0.824356457355511
99 0.824356457355511
};
\plotNetwork
table {%
0 0.836408529062361
1 0.804847572440662
2 0.847076068892805
3 0.74016854353318
4 0.83377197372406
5 0.753548179237932
6 0.863661941653838
7 0.842933180690537
8 0.795640004917149
9 0.779808768976218
10 0.80405788673944
11 0.833247209499628
12 0.842052644364343
13 0.809825181237947
14 0.753449993756716
15 0.356866096211665
16 0.786965624427925
17 0.785720265790184
18 0.834859866526942
19 0.957403176303488
20 0.549273491531582
21 0.405364007158992
22 0.210463690861854
23 0.730803705439865
24 0.634051866755926
25 0.909696514696426
26 0.815248575343516
27 0.575370970988136
28 0.861179276313498
29 0.98277959427011
30 0.991510737340818
31 0.979838035010123
32 0.743451475410438
33 0.869904500068442
34 0.744162789378032
35 0.869845628634165
36 0.963040297580355
37 0.796349303807827
38 0.820586508876064
39 0.852454961382258
40 0.842421970367545
41 0.820335202249234
42 0.760215678869312
43 0.777366290859892
44 0.795394843279131
45 0.826531661474763
46 0.779520457269277
47 0.760122593673562
48 0.711999817074159
49 0.77087027900556
50 0.931928423917561
51 0.66213473560391
52 0.805632288480388
53 0.867824041914648
54 0.871540172565247
55 0.803135691803677
56 0.819946793584816
57 0.814872266818696
58 0.878146028141605
59 0.811633995300571
60 0.801701826076277
61 0.827168600132534
62 0.816936678942657
63 0.816314844865508
64 0.785126770887507
65 0.848900880868086
66 0.858156500153355
67 0.888841026949382
68 0.608582705586342
69 0.862683875712743
70 0.811830776170995
71 0.903012397443594
72 0.92060363876487
73 0.755074132483819
74 0.831415365187737
75 0.840655337006011
76 0.852923945250288
77 0.804465597371715
78 0.795568626161527
79 0.861801934417032
80 0.809279437083183
81 0.834722564592268
82 0.833344260323618
83 0.861086448693649
84 0.763300373664089
85 0.849387114204449
86 0.821211734891348
87 0.79015484966185
88 0.846752654644436
89 0.819497592251682
90 0.825444148540031
91 0.835397561358112
92 0.80429183317642
93 0.853621217078402
94 0.853173027204308
95 0.8047863010089
96 0.822572085573714
97 0.8525288452235
98 0.837730467955472
99 0.790439359718922
};
\plotInvscat
table {%
0 0.880014538764954
1 0.812232792377472
2 0.901679515838623
3 0.752340793609619
4 0.908093750476837
5 0.914713144302368
6 0.799895823001862
7 0.778248250484467
8 0.80712366104126
9 0.861599266529083
10 0.831508994102478
11 0.801329076290131
12 0.847221851348877
13 0.841871619224548
14 0.604539752006531
15 0.570365607738495
16 0.51931244134903
17 0.82666027545929
18 0.398106247186661
19 0.89031445980072
20 0.866486489772797
21 0.571031272411346
22 0.755204975605011
23 0.701155185699463
24 0.935644686222076
25 0.556257843971252
26 0.574646413326263
27 0.730488419532776
28 0.588345766067505
29 0.375430107116699
30 0.735858082771301
31 0.699928283691406
32 0.720593154430389
33 0.990707576274872
34 0.780469179153442
35 0.513551712036133
36 0.866305291652679
37 0.784652173519135
38 0.785453617572784
39 0.949939489364624
40 0.632406234741211
41 0.334262162446976
42 0.396005153656006
43 0.323351919651031
44 0.86873584985733
45 0.732204556465149
46 0.792486786842346
47 0.925231754779816
48 0.76928585767746
49 0.619527637958527
50 0.686772525310516
51 0.387437909841537
52 0.807628512382507
53 0.939401566982269
54 0.862625539302826
55 0.904392659664154
56 0.892930388450623
57 0.759675920009613
58 0.815868318080902
59 0.783169031143188
60 0.845412135124207
61 0.859984159469604
62 0.849198639392853
63 0.804903149604797
64 0.790969431400299
65 0.832181870937347
66 0.853431522846222
67 0.845357239246368
68 0.42827782034874
69 0.936964809894562
70 0.818524777889252
71 0.615495383739471
72 0.935046136379242
73 0.765745341777802
74 0.839905798435211
75 0.808702170848846
76 0.845953047275543
77 0.717409491539001
78 0.883315801620483
79 0.846966087818146
80 0.797835409641266
81 0.88881254196167
82 0.781249046325684
83 0.643576860427856
84 0.76388281583786
85 0.896024346351624
86 0.881010115146637
87 0.757034242153168
88 0.733060836791992
89 0.651979088783264
90 0.773230195045471
91 0.815888583660126
92 0.850429058074951
93 0.920069873332977
94 0.882202565670013
95 0.891376554965973
96 0.780353486537933
97 0.822462141513824
98 0.756027162075043
99 0.96109265089035
};

%================= Fig4 ===============
\nextgplot
\plotTrue
table {%
0 0.753602486017811
1 0.753602486017811
2 0.753602486017811
3 0.753602486017811
4 0.753602486017811
5 0.753602486017811
6 0.753602486017811
7 0.753602486017811
8 0.753602486017811
9 0.753602486017811
10 0.753602486017811
11 0.753602486017811
12 0.753602486017811
13 0.753602486017811
14 0.753602486017811
15 0.753602486017811
16 0.753602486017811
17 0.753602486017811
18 0.753602486017811
19 0.753602486017811
20 0.753602486017811
21 0.753602486017811
22 0.753602486017811
23 0.753602486017811
24 0.753602486017811
25 0.753602486017811
26 0.753602486017811
27 0.753602486017811
28 0.753602486017811
29 0.753602486017811
30 0.753602486017811
31 0.753602486017811
32 0.753602486017811
33 0.753602486017811
34 0.753602486017811
35 0.753602486017811
36 0.753602486017811
37 0.753602486017811
38 0.753602486017811
39 0.753602486017811
40 0.753602486017811
41 0.753602486017811
42 0.753602486017811
43 0.753602486017811
44 0.753602486017811
45 0.753602486017811
46 0.753602486017811
47 0.753602486017811
48 0.753602486017811
49 0.753602486017811
50 0.753602486017811
51 0.753602486017811
52 0.753602486017811
53 0.753602486017811
54 0.753602486017811
55 0.753602486017811
56 0.753602486017811
57 0.753602486017811
58 0.753602486017811
59 0.753602486017811
60 0.753602486017811
61 0.753602486017811
62 0.753602486017811
63 0.753602486017811
64 0.753602486017811
65 0.753602486017811
66 0.753602486017811
67 0.753602486017811
68 0.753602486017811
69 0.753602486017811
70 0.753602486017811
71 0.753602486017811
72 0.753602486017811
73 0.753602486017811
74 0.753602486017811
75 0.753602486017811
76 0.753602486017811
77 0.753602486017811
78 0.753602486017811
79 0.753602486017811
80 0.753602486017811
81 0.753602486017811
82 0.753602486017811
83 0.753602486017811
84 0.753602486017811
85 0.753602486017811
86 0.753602486017811
87 0.753602486017811
88 0.753602486017811
89 0.753602486017811
90 0.753602486017811
91 0.753602486017811
92 0.753602486017811
93 0.753602486017811
94 0.753602486017811
95 0.753602486017811
96 0.753602486017811
97 0.753602486017811
98 0.753602486017811
99 0.753602486017811
};
\plotNetwork
table {%
0 0.777916661901542
1 0.786390499240394
2 0.754535274761165
3 0.75099872127762
4 0.797006698677243
5 0.731167918580989
6 0.809633184879754
7 0.808118134728712
8 0.718259875764508
9 0.706364027411238
10 0.633677846225779
11 0.708957193843187
12 0.783639844630368
13 0.754310702352844
14 0.777451577573546
15 0.526255462313553
16 0.729558663085904
17 0.725416850142035
18 0.777849746742385
19 0.777065925659022
20 0.555030822335311
21 0.530201300349404
22 0.952043194906432
23 0.768551203275467
24 0.709440448960885
25 0.708313497919528
26 0.787262111721242
27 0.807145320197923
28 0.770853299390217
29 0.789959745039797
30 0.737264035092754
31 0.708459623347824
32 0.850102297170005
33 0.6993917791936
34 0.683991412974597
35 0.70190731192719
36 0.650560834936232
37 0.743085036750199
38 0.824580436650526
39 0.731924184140081
40 0.774272730311415
41 0.810760134074193
42 0.788341682801851
43 0.761305758539948
44 0.743207753444452
45 0.770223794802131
46 0.822113441989416
47 0.800114282389451
48 0.827998695337737
49 0.733249145750303
50 0.797951833418452
51 0.69203138584458
52 0.734518313594338
53 0.760671967136588
54 0.787077835010558
55 0.742903721579663
56 0.765680335210035
57 0.724750169665591
58 0.81164242386057
59 0.696092440132747
60 0.731784728133434
61 0.746209289126306
62 0.697605341092551
63 0.804436829588474
64 0.751675608266988
65 0.743806466744062
66 0.681470051102196
67 0.706913771719109
68 0.694097954020038
69 0.800042130808636
70 0.789249380521016
71 0.811219166545988
72 0.777721198866946
73 0.724097541935828
74 0.787519604445371
75 0.777559568447816
76 0.741249960975897
77 0.772942773140311
78 0.754049497896356
79 0.78764230016265
80 0.733836408678426
81 0.751750463581162
82 0.761447627715147
83 0.797758295313751
84 0.807983858127337
85 0.733068356951137
86 0.700256144449599
87 0.758465230989086
88 0.837211935956843
89 0.831505710075215
90 0.722710524139849
91 0.735100783704315
92 0.750518256952038
93 0.815345637783119
94 0.694218782518063
95 0.727079322962818
96 0.822480678039812
97 0.732935748228008
98 0.761208675578487
99 0.753285774133314
};
\plotInvscat
table {%
0 0.840107321739197
1 0.617724299430847
2 0.840583860874176
3 0.628798007965088
4 0.818173408508301
5 0.794602513313293
6 0.44951269030571
7 0.334816724061966
8 0.697193503379822
9 0.69399082660675
10 0.440897613763809
11 0.720856845378876
12 0.642000019550323
13 0.630383431911469
14 0.525490701198578
15 0.380834698677063
16 0.397244393825531
17 0.31803759932518
18 0.606771290302277
19 0.217681631445885
20 0.270091682672501
21 0.455860525369644
22 0.323043197393417
23 0.439340561628342
24 0.332553774118423
25 0.712967813014984
26 0.884447872638702
27 0.230058923363686
28 0.26972171664238
29 0.515294313430786
30 0.548721790313721
31 0.336211353540421
32 0.852119743824005
33 0.436866223812103
34 0.348005443811417
35 0.459016531705856
36 0.270230442285538
37 0.795987367630005
38 0.806317985057831
39 0.615498960018158
40 0.823933303356171
41 0.652975797653198
42 0.566506862640381
43 0.773777544498444
44 0.65381395816803
45 0.795298218727112
46 0.512803316116333
47 0.621366083621979
48 0.185879707336426
49 0.374117612838745
50 0.256181001663208
51 0.747567534446716
52 0.589263081550598
53 0.882900714874268
54 0.790626049041748
55 0.7822425365448
56 0.848117291927338
57 0.596568167209625
58 0.495755255222321
59 0.606716454029083
60 0.658324956893921
61 0.701968669891357
62 0.778467416763306
63 0.88466215133667
64 0.66240394115448
65 0.779867827892303
66 0.541299104690552
67 0.579246819019318
68 0.400949448347092
69 0.820603430271149
70 0.712700188159943
71 0.481361389160156
72 0.293351680040359
73 0.533822476863861
74 0.949512183666229
75 0.783948659896851
76 0.622005581855774
77 0.896245241165161
78 0.651342213153839
79 0.843992590904236
80 0.759559690952301
81 0.566663861274719
82 0.563105702400208
83 0.817833423614502
84 0.606302380561829
85 0.780771017074585
86 0.762451410293579
87 0.855049014091492
88 0.597233712673187
89 0.687516272068024
90 0.61869078874588
91 0.785722196102142
92 0.756453037261963
93 0.839291274547577
94 0.738397002220154
95 0.772279620170593
96 0.753352344036102
97 0.647059261798859
98 0.757953703403473
99 0.852342963218689
};
%================= Fig5 ===============
\lastgplot{5}
\plotTrue
table {%
0 0.935826238137458
1 0.935826238137458
2 0.935826238137458
3 0.935826238137458
4 0.935826238137458
5 0.935826238137458
6 0.935826238137458
7 0.935826238137458
8 0.935826238137458
9 0.935826238137458
10 0.935826238137458
11 0.935826238137458
12 0.935826238137458
13 0.935826238137458
14 0.935826238137458
15 0.935826238137458
16 0.935826238137458
17 0.935826238137458
18 0.935826238137458
19 0.935826238137458
20 0.935826238137458
21 0.935826238137458
22 0.935826238137458
23 0.935826238137458
24 0.935826238137458
25 0.935826238137458
26 0.935826238137458
27 0.935826238137458
28 0.935826238137458
29 0.935826238137458
30 0.935826238137458
31 0.935826238137458
32 0.935826238137458
33 0.935826238137458
34 0.935826238137458
35 0.935826238137458
36 0.935826238137458
37 0.935826238137458
38 0.935826238137458
39 0.935826238137458
40 0.935826238137458
41 0.935826238137458
42 0.935826238137458
43 0.935826238137458
44 0.935826238137458
45 0.935826238137458
46 0.935826238137458
47 0.935826238137458
48 0.935826238137458
49 0.935826238137458
50 0.935826238137458
51 0.935826238137458
52 0.935826238137458
53 0.935826238137458
54 0.935826238137458
55 0.935826238137458
56 0.935826238137458
57 0.935826238137458
58 0.935826238137458
59 0.935826238137458
60 0.935826238137458
61 0.935826238137458
62 0.935826238137458
63 0.935826238137458
64 0.935826238137458
65 0.935826238137458
66 0.935826238137458
67 0.935826238137458
68 0.935826238137458
69 0.935826238137458
70 0.935826238137458
71 0.935826238137458
72 0.935826238137458
73 0.935826238137458
74 0.935826238137458
75 0.935826238137458
76 0.935826238137458
77 0.935826238137458
78 0.935826238137458
79 0.935826238137458
80 0.935826238137458
81 0.935826238137458
82 0.935826238137458
83 0.935826238137458
84 0.935826238137458
85 0.935826238137458
86 0.935826238137458
87 0.935826238137458
88 0.935826238137458
89 0.935826238137458
90 0.935826238137458
91 0.935826238137458
92 0.935826238137458
93 0.935826238137458
94 0.935826238137458
95 0.935826238137458
96 0.935826238137458
97 0.935826238137458
98 0.935826238137458
99 0.935826238137458
};
\plotNetwork
table {%
0 0.913642468313039
1 0.95947630955953
2 0.951467690931742
3 0.960581440984317
4 0.931182277640952
5 0.950874616718856
6 0.96367333867358
7 0.934437060573251
8 0.94473924024181
9 0.929174555682834
10 0.924357538098063
11 0.912947521746947
12 0.939635728881744
13 0.940818170376363
14 0.919693771195571
15 0.965339230983949
16 0.951229840602511
17 0.92289307807595
18 0.927224865131608
19 0.956806148033622
20 0.907388745853962
21 0.866268117948212
22 0.953346662938107
23 0.928889357305832
24 0.91306605410592
25 0.937205651815123
26 0.953145528209371
27 0.927397280948839
28 0.888491746947177
29 0.891120265041165
30 0.910491396426725
31 0.86570355868614
32 0.960011958481311
33 0.934664969146616
34 0.927735393416176
35 0.916409736951424
36 0.91248309143266
37 0.929544330029427
38 0.944715748993326
39 0.931121844981066
40 0.966750755790444
41 0.937519106416526
42 0.9357825748783
43 0.948451990000993
44 0.950079833354295
45 0.940431061503375
46 0.951444747921079
47 0.931428043809156
48 0.945178925085238
49 0.910704100800959
50 0.952898982688634
51 0.939034282266911
52 0.90990590621771
53 0.946704726410529
54 0.944634604153635
55 0.93753573571117
56 0.93124176710552
57 0.935193376691741
58 0.920868673433567
59 0.94501518978847
60 0.936307538458668
61 0.939174134545311
62 0.939324773682868
63 0.944433150571827
64 0.919339320325211
65 0.914659120549287
66 0.911008757761646
67 0.919864352565376
68 0.930264911520037
69 0.941537555859151
70 0.926351147492542
71 0.943235879528742
72 0.938945262101522
73 0.944982263340962
74 0.945213114657855
75 0.916331698105502
76 0.934957483016481
77 0.957971937305519
78 0.953018735011244
79 0.91555483694534
80 0.946671408142483
81 0.950314695538111
82 0.94253879823247
83 0.927286967222027
84 0.93625056101264
85 0.931082413936176
86 0.940899734626798
87 0.896471325772966
88 0.934699931641878
89 0.952128633212177
90 0.912847150466765
91 0.927835012170623
92 0.9493581111967
93 0.883482828035511
94 0.927488672093158
95 0.949746204882514
96 0.911549021063309
97 0.936939645872388
98 0.916132623699881
99 0.918823231676658
};
\plotInvscat
table {%
0 0.929152607917786
1 0.894014120101929
2 0.936992645263672
3 0.917267680168152
4 0.908027291297913
5 0.906108558177948
6 0.850872039794922
7 0.812853276729584
8 0.877308130264282
9 0.883434474468231
10 0.859920024871826
11 0.932036995887756
12 0.852651417255402
13 0.916942536830902
14 0.6829674243927
15 0.836867928504944
16 0.752559542655945
17 0.654637932777405
18 0.811535716056824
19 0.672111451625824
20 0.667330324649811
21 0.749713003635406
22 0.389211148023605
23 0.782819926738739
24 0.804817795753479
25 0.83044821023941
26 0.910885155200958
27 0.679050028324127
28 0.762343645095825
29 0.685558676719666
30 0.710414588451385
31 0.705686390399933
32 0.89040732383728
33 0.806968629360199
34 0.869274139404297
35 0.537609457969666
36 0.790310502052307
37 0.945113480091095
38 0.951322495937347
39 0.873131513595581
40 0.928147077560425
41 0.94591748714447
42 0.819657564163208
43 0.91902494430542
44 0.877830624580383
45 0.955155968666077
46 0.831530213356018
47 0.854521811008453
48 0.547566831111908
49 0.633842408657074
50 0.807346403598785
51 0.981715857982635
52 0.894333600997925
53 0.940654575824738
54 0.937610030174255
55 0.883658468723297
56 0.931756973266602
57 0.862109303474426
58 0.740227401256561
59 0.934650599956512
60 0.892926096916199
61 0.874094367027283
62 0.971014261245728
63 0.959890127182007
64 0.883605122566223
65 0.933649957180023
66 0.802139759063721
67 0.809250712394714
68 0.76009202003479
69 0.923591375350952
70 0.925692975521088
71 0.767570018768311
72 0.663100719451904
73 0.888300538063049
74 0.938220202922821
75 0.93820321559906
76 0.839179217815399
77 0.949320793151855
78 0.816005885601044
79 0.932930767536163
80 0.944747030735016
81 0.851934492588043
82 0.896669149398804
83 0.821612238883972
84 0.798622846603394
85 0.926944553852081
86 0.938099443912506
87 0.922920644283295
88 0.755478203296661
89 0.920884311199188
90 0.827600240707397
91 0.939436674118042
92 0.925458014011383
93 0.878693222999573
94 0.926047801971436
95 0.941441893577576
96 0.898711681365967
97 0.802883267402649
98 0.947013735771179
99 0.890082240104675
};
\end{groupplot}

==> Figs/random_phi_change/noise_01.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm,group name=column3 plots,}]
%====================== Fig1 =============
\firstgplot{column2}{(c) $\sigma^2_{z}=0.01$}
\plotTrue
table {%
0 0.733099880094478
1 0.733099880094478
2 0.733099880094478
3 0.733099880094478
4 0.733099880094478
5 0.733099880094478
6 0.733099880094478
7 0.733099880094478
8 0.733099880094478
9 0.733099880094478
10 0.733099880094478
11 0.733099880094478
12 0.733099880094478
13 0.733099880094478
14 0.733099880094478
15 0.733099880094478
16 0.733099880094478
17 0.733099880094478
18 0.733099880094478
19 0.733099880094478
20 0.733099880094478
21 0.733099880094478
22 0.733099880094478
23 0.733099880094478
24 0.733099880094478
25 0.733099880094478
26 0.733099880094478
27 0.733099880094478
28 0.733099880094478
29 0.733099880094478
30 0.733099880094478
31 0.733099880094478
32 0.733099880094478
33 0.733099880094478
34 0.733099880094478
35 0.733099880094478
36 0.733099880094478
37 0.733099880094478
38 0.733099880094478
39 0.733099880094478
40 0.733099880094478
41 0.733099880094478
42 0.733099880094478
43 0.733099880094478
44 0.733099880094478
45 0.733099880094478
46 0.733099880094478
47 0.733099880094478
48 0.733099880094478
49 0.733099880094478
50 0.733099880094478
51 0.733099880094478
52 0.733099880094478
53 0.733099880094478
54 0.733099880094478
55 0.733099880094478
56 0.733099880094478
57 0.733099880094478
58 0.733099880094478
59 0.733099880094478
60 0.733099880094478
61 0.733099880094478
62 0.733099880094478
63 0.733099880094478
64 0.733099880094478
65 0.733099880094478
66 0.733099880094478
67 0.733099880094478
68 0.733099880094478
69 0.733099880094478
70 0.733099880094478
71 0.733099880094478
72 0.733099880094478
73 0.733099880094478
74 0.733099880094478
75 0.733099880094478
76 0.733099880094478
77 0.733099880094478
78 0.733099880094478
79 0.733099880094478
80 0.733099880094478
81 0.733099880094478
82 0.733099880094478
83 0.733099880094478
84 0.733099880094478
85 0.733099880094478
86 0.733099880094478
87 0.733099880094478
88 0.733099880094478
89 0.733099880094478
90 0.733099880094478
91 0.733099880094478
92 0.733099880094478
93 0.733099880094478
94 0.733099880094478
95 0.733099880094478
96 0.733099880094478
97 0.733099880094478
98 0.733099880094478
99 0.733099880094478
};
\plotNetwork
table {%
0 0.720894667031761
1 0.731683096918732
2 0.741504813006962
3 0.75453939345891
4 0.717975115883141
5 0.744598965286079
6 0.714373538657841
7 0.721251798009728
8 0.747746371556262
9 0.74679106510306
10 0.747640996820416
11 0.777035369348875
12 0.720009327432949
13 0.754726484955846
14 0.736150425096391
15 0.759789911457464
16 0.735504464294772
17 0.727156032249483
18 0.69051860157211
19 0.708067698174675
20 0.78461801614548
21 0.767636936502544
22 0.728802050370446
23 0.790289338584344
24 0.680900589093207
25 0.846639266392005
26 0.658396307696767
27 0.691277681760614
28 0.764655102116752
29 0.46846914662831
30 0.783525028365816
31 0.975781392802323
32 0.921718440018113
33 0.708187653495184
34 0.855241180143323
35 0.694548608166972
36 0.581200939501025
37 0.74732926612499
38 0.765205285198042
39 0.71004584328457
40 0.721430643153088
41 0.753755871722766
42 0.737659380732761
43 0.715761715831066
44 0.6972435388827
45 0.753879932683088
46 0.752954630205653
47 0.763793047151032
48 0.713700913339329
49 0.675091183796277
50 0.770967438529145
51 0.67030099518218
52 0.691121101347545
53 0.752129897102177
54 0.793186670665886
55 0.644439820992177
56 0.698815582692096
57 0.723756208461237
58 0.798703863338716
59 0.7446114954346
60 0.77081487328437
61 0.643847335169483
62 0.62898856153729
63 0.752853871197687
64 0.82848520061159
65 0.748582372093547
66 0.779420745246515
67 0.767804988303011
68 0.731329388509325
69 0.771629640473203
70 0.783470142294027
71 0.751332125974995
72 0.760261957030532
73 0.714093928898645
74 0.711714085005139
75 0.596018319288987
76 0.834821231019886
77 0.714957235333678
78 0.715403965266632
79 0.739975897194078
80 0.725701602162723
81 0.750858768838007
82 0.764731629183885
83 0.843008084501898
84 0.558427263191252
85 0.844707164928575
86 0.781133691183505
87 0.783343775200543
88 0.745321179272476
89 0.690281811906756
90 0.802441751640903
91 0.807954951014881
92 0.747683768002129
93 0.760965631546312
94 0.803948653246387
95 0.791281511814327
96 0.678769297405524
97 0.701440878341354
98 0.701772144147795
99 0.707114715390024
};
\plotInvscat
table {%
0 0.702981472015381
1 0.764521837234497
2 0.724980354309082
3 0.777909755706787
4 0.71561735868454
5 0.7294682264328
6 0.761931419372559
7 0.764041483402252
8 0.740812182426453
9 0.742223799228668
10 0.769624054431915
11 0.804468631744385
12 0.77280855178833
13 0.823347091674805
14 0.772177934646606
15 0.773143291473389
16 0.785820007324219
17 0.815793454647064
18 0.949031591415405
19 0.912662446498871
20 0.876377522945404
21 0.748447299003601
22 0.781134903430939
23 0.838895559310913
24 0.949700176715851
25 0.96916538476944
26 0.978057265281677
27 0.97955584526062
28 0.989666163921356
29 0.955018877983093
30 0.697254419326782
31 0.951959073543549
32 0.865838050842285
33 0.74625825881958
34 0.930836915969849
35 0.849331438541412
36 0.643686532974243
37 0.774189710617065
38 0.761746406555176
39 0.564529120922089
40 0.823583781719208
41 0.774189293384552
42 0.953266978263855
43 0.752869963645935
44 0.593736529350281
45 0.79198944568634
46 0.730537235736847
47 0.623894453048706
48 0.733407914638519
49 0.717408061027527
50 0.827533900737762
51 0.562398493289948
52 0.777486979961395
53 0.996479034423828
54 0.680861532688141
55 0.759599626064301
56 0.632523834705353
57 0.557279884815216
58 0.69867867231369
59 0.665892541408539
60 0.861498057842255
61 0.940096020698547
62 0.905557751655579
63 0.888652861118317
64 0.715551793575287
65 0.870348334312439
66 0.919053494930267
67 0.893519103527069
68 0.982548594474792
69 0.764198422431946
70 0.99266117811203
71 0.747033059597015
72 0.733522891998291
73 0.70645946264267
74 0.978309333324432
75 0.8014315366745
76 0.628927946090698
77 0.972150862216949
78 0.634145259857178
79 0.675048112869263
80 0.965366542339325
81 0.881908595561981
82 0.862962603569031
83 0.962885916233063
84 0.928870260715485
85 0.84233558177948
86 0.712200343608856
87 0.692189276218414
88 0.980189263820648
89 0.792641699314117
90 0.989314258098602
91 0.600862801074982
92 0.772303402423859
93 0.975035905838013
94 0.814825356006622
95 0.76122123003006
96 0.976405203342438
97 0.9846311211586
98 0.906419157981873
99 0.987767934799194
};
%====================== Fig2 =============
\nextgplot
\perturbation
\plotTrue
table {%
0 0.935516519885526
1 0.935516519885526
2 0.935516519885526
3 0.935516519885526
4 0.935516519885526
5 0.935516519885526
6 0.935516519885526
7 0.935516519885526
8 0.935516519885526
9 0.935516519885526
10 0.869667569548439
11 0.727246223885405
12 0.840885440553651
13 0.669861263673315
14 0.695062251008769
15 0.653367486580926
16 0.656677578070439
17 0.60377798372569
18 0.40326589007199
19 0.544277543208332
20 0.634658637120049
21 0.771370029605121
22 0.807328666767555
23 0.705765479890902
24 0.294400085499
25 0.122840677718215
26 0.197476673071808
27 0.344663137249381
28 0.280526511787189
29 0.122459958543774
30 0.199148910512332
31 0.0403795856982413
32 0.0377646706314038
33 0.285823945820197
34 0.0291006444692511
35 0.408406259801238
36 0.408406259801238
37 0.408406259801238
38 0.408406259801238
39 0.408406259801238
40 0.408406259801238
41 0.408406259801238
42 0.408406259801238
43 0.408406259801238
44 0.408406259801238
45 0.408406259801238
46 0.408406259801238
47 0.408406259801238
48 0.408406259801238
49 0.408406259801238
50 0.408406259801238
51 0.408406259801238
52 0.408406259801238
53 0.408406259801238
54 0.408406259801238
55 0.408406259801238
56 0.408406259801238
57 0.408406259801238
58 0.408406259801238
59 0.408406259801238
60 0.402191409831325
61 0.0764337403055456
62 0.0795973866253387
63 0.0646871585761395
64 0.108009977372683
65 0.254616719700893
66 0.472565933463051
67 0.434779798744271
68 0.310130512503765
69 0.335406009918958
70 0.385910215050476
71 0.723644828986625
72 0.677641239833845
73 0.546856821471035
74 0.415658991542201
75 0.241671090622782
76 0.281803188796102
77 0.451510825833016
78 0.503227302170066
79 0.623984732537678
80 0.390940740100067
81 0.383177631440228
82 0.108923776814901
83 0.10020607423564
84 0.106528490954389
85 0.356305650239709
86 0.356305650239709
87 0.356305650239709
88 0.356305650239709
89 0.356305650239709
90 0.356305650239709
91 0.356305650239709
92 0.356305650239709
93 0.356305650239709
94 0.356305650239709
95 0.356305650239709
96 0.356305650239709
97 0.356305650239709
98 0.356305650239709
99 0.356305650239709
};
\plotNetwork
table {%
0 0.940643377865759
1 0.925073028675357
2 0.932285556382814
3 0.950766686165244
4 0.929440065124434
5 0.950640060476552
6 0.93785784805479
7 0.931006447674971
8 0.948059160056364
9 0.928201137095969
10 0.875388758499012
11 0.760006038094444
12 0.846191234180571
13 0.679678912522654
14 0.693846394663838
15 0.667847445728298
16 0.671477650871567
17 0.594192257500259
18 0.430107593437495
19 0.516665630908261
20 0.680260484877427
21 0.804995153035804
22 0.813610460234666
23 0.726686245749734
24 0.304438786091049
25 0.130165931178375
26 0.189563382959768
27 0.291919957077673
28 0.306553645993702
29 0.135250400460532
30 0.246430856175465
31 0.167341179172095
32 0.228660776253465
33 0.261481976534838
34 0.00144234297516561
35 0.396838759776789
36 0.363342012367828
37 0.4432527330604
38 0.419662610420929
39 0.404250068317599
40 0.435899007935268
41 0.402027541578003
42 0.402443136184188
43 0.418257444846405
44 0.41902975363198
45 0.378026834177654
46 0.383325751953905
47 0.428892940336186
48 0.394008971742216
49 0.38811124878123
50 0.394213446981658
51 0.372862725241616
52 0.437914415096018
53 0.400693268888784
54 0.391893868348843
55 0.409625429750953
56 0.400631351163837
57 0.405347766887166
58 0.439797923035339
59 0.434258496193872
60 0.389567733833023
61 0.022215121692917
62 0.115908651169597
63 0.0718229604963294
64 0.124063893941353
65 0.233414862863156
66 0.51317487316271
67 0.498201438654563
68 0.325996341872723
69 0.37041574897089
70 0.348206990634563
71 0.752993424091934
72 0.711006194140251
73 0.557573806891459
74 0.410568541496677
75 0.222295963964549
76 0.28294726506917
77 0.467258782367499
78 0.46106306529644
79 0.590003998094488
80 0.351980752412718
81 0.388670493065611
82 0.109310661529546
83 0.136408658301495
84 0.0678898764513387
85 0.456093964203585
86 0.364121986728014
87 0.361735961905972
88 0.360431020438799
89 0.373212421008402
90 0.380574042165095
91 0.354768064080116
92 0.421449264878088
93 0.3567302510325
94 0.41409725366484
95 0.418967460805429
96 0.354278806034906
97 0.368449466510773
98 0.341287169975319
99 0.359894071678057
};
\plotInvscat
table {%
0 0.943255245685577
1 0.932965278625488
2 0.927819967269897
3 0.945767045021057
4 0.931944727897644
5 0.939231753349304
6 0.908872842788696
7 0.93108057975769
8 0.950878381729126
9 0.931147754192352
10 0.894274711608887
11 0.794629693031311
12 0.85673999786377
13 0.725114226341248
14 0.687627077102661
15 0.650427162647247
16 0.631834864616394
17 0.626436054706573
18 0.549088954925537
19 0.666075766086578
20 0.692587375640869
21 0.793945372104645
22 0.807949304580688
23 0.750449299812317
24 0.344289124011993
25 0.444269597530365
26 0.599481642246246
27 0.556365072727203
28 0.517102062702179
29 0.891895711421967
30 0.350506693124771
31 0.74357533454895
32 0.694799244403839
33 0.73846298456192
34 0.701931953430176
35 0.457634270191193
36 0.682677030563354
37 0.46656334400177
38 0.491091698408127
39 0.847025096416473
40 0.451950281858444
41 0.530436456203461
42 0.360378384590149
43 0.380993962287903
44 0.563598573207855
45 0.53223729133606
46 0.552356958389282
47 0.721429049968719
48 0.54718291759491
49 0.422921478748322
50 0.664858162403107
51 0.700006127357483
52 0.44534769654274
53 0.559446394443512
54 0.673736393451691
55 0.574393928050995
56 0.486957967281342
57 0.789361774921417
58 0.661676049232483
59 0.702514708042145
60 0.505860686302185
61 0.81310772895813
62 0.885160982608795
63 0.852906703948975
64 0.467929512262344
65 0.811551749706268
66 0.555900573730469
67 0.504602134227753
68 0.546053111553192
69 0.463073909282684
70 0.451653778553009
71 0.744536519050598
72 0.783750474452972
73 0.594324290752411
74 0.510915815830231
75 0.679291307926178
76 0.663291454315186
77 0.49322110414505
78 0.823081135749817
79 0.667259275913239
80 0.373301893472672
81 0.549925923347473
82 0.719710469245911
83 0.809338629245758
84 0.808847486972809
85 0.464763849973679
86 0.324885338544846
87 0.586094260215759
88 0.51030308008194
89 0.445718705654144
90 0.537679672241211
91 0.540072679519653
92 0.378785341978073
93 0.605904102325439
94 0.437128186225891
95 0.377788215875626
96 0.395046174526215
97 0.547336876392365
98 0.524343132972717
99 0.729164481163025
};
%====================== Fig3 =============
\nextgplot
\plotTrue
table {%
0 0.824356457355511
1 0.824356457355511
2 0.824356457355511
3 0.824356457355511
4 0.824356457355511
5 0.824356457355511
6 0.824356457355511
7 0.824356457355511
8 0.824356457355511
9 0.824356457355511
10 0.824356457355511
11 0.824356457355511
12 0.824356457355511
13 0.824356457355511
14 0.824356457355511
15 0.824356457355511
16 0.824356457355511
17 0.824356457355511
18 0.824356457355511
19 0.824356457355511
20 0.824356457355511
21 0.824356457355511
22 0.824356457355511
23 0.824356457355511
24 0.824356457355511
25 0.824356457355511
26 0.824356457355511
27 0.824356457355511
28 0.824356457355511
29 0.824356457355511
30 0.824356457355511
31 0.824356457355511
32 0.824356457355511
33 0.824356457355511
34 0.824356457355511
35 0.824356457355511
36 0.824356457355511
37 0.824356457355511
38 0.824356457355511
39 0.824356457355511
40 0.824356457355511
41 0.824356457355511
42 0.824356457355511
43 0.824356457355511
44 0.824356457355511
45 0.824356457355511
46 0.824356457355511
47 0.824356457355511
48 0.824356457355511
49 0.824356457355511
50 0.824356457355511
51 0.824356457355511
52 0.824356457355511
53 0.824356457355511
54 0.824356457355511
55 0.824356457355511
56 0.824356457355511
57 0.824356457355511
58 0.824356457355511
59 0.824356457355511
60 0.824356457355511
61 0.824356457355511
62 0.824356457355511
63 0.824356457355511
64 0.824356457355511
65 0.824356457355511
66 0.824356457355511
67 0.824356457355511
68 0.824356457355511
69 0.824356457355511
70 0.824356457355511
71 0.824356457355511
72 0.824356457355511
73 0.824356457355511
74 0.824356457355511
75 0.824356457355511
76 0.824356457355511
77 0.824356457355511
78 0.824356457355511
79 0.824356457355511
80 0.824356457355511
81 0.824356457355511
82 0.824356457355511
83 0.824356457355511
84 0.824356457355511
85 0.824356457355511
86 0.824356457355511
87 0.824356457355511
88 0.824356457355511
89 0.824356457355511
90 0.824356457355511
91 0.824356457355511
92 0.824356457355511
93 0.824356457355511
94 0.824356457355511
95 0.824356457355511
96 0.824356457355511
97 0.824356457355511
98 0.824356457355511
99 0.824356457355511
};
\plotNetwork
table {%
0 0.826669904107929
1 0.813694391931989
2 0.837118754364526
3 0.787077805869022
4 0.821594945210731
5 0.806075847771987
6 0.825446712899649
7 0.803520096465319
8 0.830902004659285
9 0.834487542598454
10 0.834011638897791
11 0.823282610015686
12 0.829553497733448
13 0.813093502329562
14 0.813058596968017
15 0.826823407580353
16 0.819166521366642
17 0.817434238368186
18 0.83295691416483
19 0.819590188262822
20 0.813360870834438
21 0.802749767599896
22 0.844646296914519
23 0.807909498946639
24 0.843258402480352
25 0.776846686598141
26 0.834946298449448
27 0.825801036651235
28 0.82244329885261
29 0.82765868043868
30 0.74693540915587
31 0.763651619307933
32 0.7320995088591312
33 0.858530069793176
34 0.771497859784407
35 0.835715262953947
36 0.900888802281919
37 0.79218337369499
38 0.814410942297986
39 0.84343612516148
40 0.830255898856758
41 0.833687143312501
42 0.803899915681613
43 0.807316435115324
44 0.820882697779449
45 0.820522531875202
46 0.817657381950103
47 0.804255776948927
48 0.842118549366609
49 0.868373633870287
50 0.828415535022808
51 0.880320224421792
52 0.842297240510506
53 0.813045397395406
54 0.78728995290319
55 0.887153733841176
56 0.852466768773322
57 0.842556081054462
58 0.798778003357745
59 0.799632897722139
60 0.779748373430559
61 0.924650490870635
62 0.864988718371718
63 0.811798169041715
64 0.748796428998905
65 0.804234641823572
66 0.804616452844685
67 0.781125239693133
68 0.823702622609293
69 0.821490569951964
70 0.812284401546401
71 0.809093626106938
72 0.792238387972636
73 0.842748846645778
74 0.841487469036401
75 0.87695701360913
76 0.788812933909035
77 0.830669549612366
78 0.830940533855954
79 0.830664776868834
80 0.84223861069652
81 0.803932500536976
82 0.831728819051453
83 0.788445791681195
84 0.921323955246385
85 0.761143268052875
86 0.823424252096287
87 0.807660989507888
88 0.840017909070028
89 0.813394397715252
90 0.791154731614632
91 0.816753019905269
92 0.77774499705951
93 0.83507904867692
94 0.798693239250807
95 0.785711598278816
96 0.821371934626693
97 0.855199386532921
98 0.870459562092109
99 0.812097076585977
};
\plotInvscat
table {%
0 0.831840634346008
1 0.813367486000061
2 0.829346656799316
3 0.789120495319366
4 0.824005544185638
5 0.839792251586914
6 0.816884756088257
7 0.773460268974304
8 0.843863129615784
9 0.84421569108963
10 0.777271926403046
11 0.793381333351135
12 0.831093966960907
13 0.806450843811035
14 0.83129096031189
15 0.79272735118866
16 0.849421679973602
17 0.791352689266205
18 0.581517696380615
19 0.737343668937683
20 0.797933876514435
21 0.858872532844543
22 0.797608971595764
23 0.802692770957947
24 0.695560872554779
25 0.45274955034256
26 0.520435631275177
27 0.541757106781006
28 0.399573504924774
29 0.347720742225647
30 0.778712153434753
31 0.899160802364349
32 0.537846446037292
33 0.869792699813843
34 0.671945452690125
35 0.802738130092621
36 0.76739090681076
37 0.728341937065125
38 0.709145784378052
39 0.94275838136673
40 0.700941622257233
41 0.643975675106049
42 0.718124628067017
43 0.844571232795715
44 0.925493955612183
45 0.610249578952789
46 0.694888412952423
47 0.948850989341736
48 0.923922836780548
49 0.92499440908432
50 0.52029025554657
51 0.966896533966064
52 0.743801712989807
53 0.40258264541626
54 0.973969578742981
55 0.639381647109985
56 0.855942845344543
57 0.96708869934082
58 0.779137253761292
59 0.977148652076721
60 0.553597927093506
61 0.288131594657898
62 0.330980688333511
63 0.61490386724472
64 0.541847467422485
65 0.207934826612473
66 0.595820784568787
67 0.604928851127625
68 0.340831309556961
69 0.910944879055023
70 0.48176047205925
71 0.846011996269226
72 0.824463844299316
73 0.84320741891861
74 0.509334325790405
75 0.624739527702332
76 0.793400645256042
77 0.623850226402283
78 0.895079433917999
79 0.939399838447571
80 0.61487489938736
81 0.436487197875977
82 0.783423542976379
83 0.444074749946594
84 0.781905710697174
85 0.765996158123016
86 0.886789083480835
87 0.637961864471436
88 0.649415194988251
89 0.646677017211914
90 0.618815839290619
91 0.813862800598145
92 0.900735318660736
93 0.483566880226135
94 0.803319811820984
95 0.877413153648376
96 0.633532524108887
97 0.589201986789703
98 0.536863207817078
99 0.313245445489883
};
%====================== Fig4 =============
\nextgplot
\plotTrue
table {%
0 0.753602486017811
1 0.753602486017811
2 0.753602486017811
3 0.753602486017811
4 0.753602486017811
5 0.753602486017811
6 0.753602486017811
7 0.753602486017811
8 0.753602486017811
9 0.753602486017811
10 0.753602486017811
11 0.753602486017811
12 0.753602486017811
13 0.753602486017811
14 0.753602486017811
15 0.753602486017811
16 0.753602486017811
17 0.753602486017811
18 0.753602486017811
19 0.753602486017811
20 0.753602486017811
21 0.753602486017811
22 0.753602486017811
23 0.753602486017811
24 0.753602486017811
25 0.753602486017811
26 0.753602486017811
27 0.753602486017811
28 0.753602486017811
29 0.753602486017811
30 0.753602486017811
31 0.753602486017811
32 0.753602486017811
33 0.753602486017811
34 0.753602486017811
35 0.753602486017811
36 0.753602486017811
37 0.753602486017811
38 0.753602486017811
39 0.753602486017811
40 0.753602486017811
41 0.753602486017811
42 0.753602486017811
43 0.753602486017811
44 0.753602486017811
45 0.753602486017811
46 0.753602486017811
47 0.753602486017811
48 0.753602486017811
49 0.753602486017811
50 0.753602486017811
51 0.753602486017811
52 0.753602486017811
53 0.753602486017811
54 0.753602486017811
55 0.753602486017811
56 0.753602486017811
57 0.753602486017811
58 0.753602486017811
59 0.753602486017811
60 0.753602486017811
61 0.753602486017811
62 0.753602486017811
63 0.753602486017811
64 0.753602486017811
65 0.753602486017811
66 0.753602486017811
67 0.753602486017811
68 0.753602486017811
69 0.753602486017811
70 0.753602486017811
71 0.753602486017811
72 0.753602486017811
73 0.753602486017811
74 0.753602486017811
75 0.753602486017811
76 0.753602486017811
77 0.753602486017811
78 0.753602486017811
79 0.753602486017811
80 0.753602486017811
81 0.753602486017811
82 0.753602486017811
83 0.753602486017811
84 0.753602486017811
85 0.753602486017811
86 0.753602486017811
87 0.753602486017811
88 0.753602486017811
89 0.753602486017811
90 0.753602486017811
91 0.753602486017811
92 0.753602486017811
93 0.753602486017811
94 0.753602486017811
95 0.753602486017811
96 0.753602486017811
97 0.753602486017811
98 0.753602486017811
99 0.753602486017811
};
\plotNetwork
table {%
0 0.763817754356689
1 0.767813863526996
2 0.755083193919541
3 0.7675204229698
4 0.763932477683603
5 0.754616294960066
6 0.763740940993297
7 0.72429231616489
8 0.74062730895128
9 0.747348793939148
10 0.708634237289955
11 0.727699223491308
12 0.764086009277244
13 0.753136496615158
14 0.781357441776979
15 0.760435502997108
16 0.744482747896431
17 0.746837583368816
18 0.76287115832569
19 0.763189455810223
20 0.715374944735929
21 0.735326589232893
22 0.74437888667957
23 0.695376057885171
24 0.758461292477162
25 0.730941504325577
26 0.766693817585852
27 0.77314410230772
28 0.7566482853148
29 0.802611039545654
30 0.741714860398765
31 0.65305539219112
32 0.850233939454678
33 0.72939384035909
34 0.709380667721191
35 0.734755335748212
36 0.691274494956283
37 0.759775022739206
38 0.795607130441758
39 0.748653707676603
40 0.763275222553493
41 0.776267164982905
42 0.771324144624954
43 0.750421980904217
44 0.747557268740655
45 0.767945101751139
46 0.782546139003894
47 0.767167944083269
48 0.774921110380421
49 0.735731393702211
50 0.774790468592869
51 0.711570502827996
52 0.740120314865189
53 0.749824726756581
54 0.759674322654962
55 0.72671937372882
56 0.749693922043794
57 0.744198243426337
58 0.783041552735018
59 0.775208296501277
60 0.779551923677947
61 0.767081383188499
62 0.736132523956063
63 0.772542708948931
64 0.78183818128476
65 0.768072829782952
66 0.779458457425075
67 0.771229956417821
68 0.7891683411893
69 0.766535043502524
70 0.792050841123137
71 0.785077301393092
72 0.760016196767235
73 0.740939177151851
74 0.755030984212246
75 0.744296296168149
76 0.7893339144584
77 0.761685749705684
78 0.722355543164849
79 0.748908060272707
80 0.758163810851462
81 0.754433699543938
82 0.756810775777692
83 0.761734155694929
84 0.781320385096321
85 0.690266001745364
86 0.733313216340052
87 0.761240415387415
88 0.791579601109386
89 0.786526890257506
90 0.723680653538952
91 0.724867985146291
92 0.749009932639986
93 0.761318175933138
94 0.692515870703185
95 0.713928204031185
96 0.793507300201173
97 0.752644387874284
98 0.768110112599215
99 0.752524411322167
};
\plotInvscat
table {%
0 0.790649056434631
1 0.724162340164185
2 0.773563921451569
3 0.736302077770233
4 0.766147792339325
5 0.766899943351746
6 0.696793735027313
7 0.676671028137207
8 0.753718435764313
9 0.762704312801361
10 0.696945786476135
11 0.72228342294693
12 0.697942078113556
13 0.680013358592987
14 0.751666903495789
15 0.777340650558472
16 0.719508349895477
17 0.664889097213745
18 0.829236626625061
19 0.535378396511078
20 0.616420149803162
21 0.751253485679626
22 0.697245359420776
23 0.643709540367126
24 0.676847338676453
25 0.424632370471954
26 0.268672823905945
27 0.410886943340302
28 0.68960440158844
29 0.250024944543839
30 0.761069536209106
31 0.106766737997532
32 0.192477121949196
33 0.344788014888763
34 0.132264837622643
35 0.71397864818573
36 0.493191778659821
37 0.796401977539062
38 0.789092063903809
39 0.63457864522934
40 0.815949678421021
41 0.738032817840576
42 0.815623998641968
43 0.75216943025589
44 0.675560474395752
45 0.773917317390442
46 0.698001205921173
47 0.646223485469818
48 0.639081656932831
49 0.715889751911163
50 0.777906179428101
51 0.61594694852829
52 0.769072949886322
53 0.95326966047287
54 0.599267661571503
55 0.727651238441467
56 0.724411308765411
57 0.610542893409729
58 0.6967693567276
59 0.614508509635925
60 0.873587131500244
61 0.227354273200035
62 0.275359511375427
63 0.112770207226276
64 0.521288931369781
65 0.754719793796539
66 0.926771461963654
67 0.872485399246216
68 0.967008233070374
69 0.706765711307526
70 0.925610601902008
71 0.784695744514465
72 0.738477885723114
73 0.731957137584686
74 0.940783500671387
75 0.354654371738434
76 0.670021116733551
77 0.876640260219574
78 0.555382192134857
79 0.686550676822662
80 0.814939558506012
81 0.834502696990967
82 0.163567006587982
83 0.283008188009262
84 0.0985917896032333
85 0.684545040130615
86 0.770482420921326
87 0.901380896568298
88 0.561249136924744
89 0.742724120616913
90 0.507250547409058
91 0.830923080444336
92 0.757576942443848
93 0.761638939380646
94 0.671530187129974
95 0.74225378036499
96 0.619856476783752
97 0.592328548431396
98 0.644567966461182
99 0.847435772418976
};
%====================== Fig5 =============
\lastgplot{5}
\plotTrue
table {%
0 0.935826238137458
1 0.935826238137458
2 0.935826238137458
3 0.935826238137458
4 0.935826238137458
5 0.935826238137458
6 0.935826238137458
7 0.935826238137458
8 0.935826238137458
9 0.935826238137458
10 0.935826238137458
11 0.935826238137458
12 0.935826238137458
13 0.935826238137458
14 0.935826238137458
15 0.935826238137458
16 0.935826238137458
17 0.935826238137458
18 0.935826238137458
19 0.935826238137458
20 0.935826238137458
21 0.935826238137458
22 0.935826238137458
23 0.935826238137458
24 0.935826238137458
25 0.935826238137458
26 0.935826238137458
27 0.935826238137458
28 0.935826238137458
29 0.935826238137458
30 0.935826238137458
31 0.935826238137458
32 0.935826238137458
33 0.935826238137458
34 0.935826238137458
35 0.935826238137458
36 0.935826238137458
37 0.935826238137458
38 0.935826238137458
39 0.935826238137458
40 0.935826238137458
41 0.935826238137458
42 0.935826238137458
43 0.935826238137458
44 0.935826238137458
45 0.935826238137458
46 0.935826238137458
47 0.935826238137458
48 0.935826238137458
49 0.935826238137458
50 0.935826238137458
51 0.935826238137458
52 0.935826238137458
53 0.935826238137458
54 0.935826238137458
55 0.935826238137458
56 0.935826238137458
57 0.935826238137458
58 0.935826238137458
59 0.935826238137458
60 0.935826238137458
61 0.935826238137458
62 0.935826238137458
63 0.935826238137458
64 0.935826238137458
65 0.935826238137458
66 0.935826238137458
67 0.935826238137458
68 0.935826238137458
69 0.935826238137458
70 0.935826238137458
71 0.935826238137458
72 0.935826238137458
73 0.935826238137458
74 0.935826238137458
75 0.935826238137458
76 0.935826238137458
77 0.935826238137458
78 0.935826238137458
79 0.935826238137458
80 0.935826238137458
81 0.935826238137458
82 0.935826238137458
83 0.935826238137458
84 0.935826238137458
85 0.935826238137458
86 0.935826238137458
87 0.935826238137458
88 0.935826238137458
89 0.935826238137458
90 0.935826238137458
91 0.935826238137458
92 0.935826238137458
93 0.935826238137458
94 0.935826238137458
95 0.935826238137458
96 0.935826238137458
97 0.935826238137458
98 0.935826238137458
99 0.935826238137458
};
\plotNetwork
table {%
0 0.925342395404915
1 0.946613658342603
2 0.943767340027575
3 0.950916770036074
4 0.927190046215747
5 0.943519252979025
6 0.944261612930901
7 0.935380811897003
8 0.931346543739142
9 0.929912832278008
10 0.930097017437124
11 0.924506001142616
12 0.936670589492478
13 0.937848760275475
14 0.938043506226347
15 0.929671947721502
16 0.945005767994657
17 0.929005401147838
18 0.931492311111676
19 0.938232132158042
20 0.938373650884779
21 0.93932316970455
22 0.934249779372029
23 0.929345484973708
24 0.930008545101399
25 0.933641712809219
26 0.945127377482902
27 0.931260317067362
28 0.914170139614798
29 0.922303146405296
30 0.932644150145323
31 0.910141371638922
32 0.94905699256094
33 0.933252335746985
34 0.927143218711446
35 0.928770215873721
36 0.927233221620148
37 0.935413007186486
38 0.941772601090728
39 0.931234434777431
40 0.951957204677938
41 0.935694926150979
42 0.934460932583308
43 0.943174119323626
44 0.940160941988125
45 0.937343369435144
46 0.940880544343057
47 0.931898588770917
48 0.937077128473885
49 0.930163906179848
50 0.932689265887257
51 0.912840752039713
52 0.923234545516944
53 0.927959124587075
54 0.92831864088616
55 0.927281179122052
56 0.924626045133092
57 0.938311552688114
58 0.950867700265573
59 0.929602455779661
60 0.947654362449566
61 0.931063216856264
62 0.920511021400346
63 0.936848027456005
64 0.931860991548743
65 0.924670485331045
66 0.947907115240517
67 0.957020375609073
68 0.937018045012012
69 0.935443331335997
70 0.944363257316626
71 0.952740042292269
72 0.943043173982532
73 0.935924941686237
74 0.924239704271026
75 0.937410645618587
76 0.93997945248412
77 0.940866784660769
78 0.933844524106418
79 0.939687799416963
80 0.928700388280599
81 0.962811648980533
82 0.945140381564776
83 0.934420237894384
84 0.938466295251693
85 0.931903565968513
86 0.935844907906824
87 0.914271213477877
88 0.934666817408059
89 0.944987884916642
90 0.926203610324039
91 0.930787262545608
92 0.940883363224484
93 0.935569710768899
94 0.931487357607488
95 0.944265165129978
96 0.933540279661653
97 0.941469829953323
98 0.924479269453255
99 0.933682271405785
};
\plotInvscat
table {%
0 0.934522867202759
1 0.937845587730408
2 0.951844394207001
3 0.945066869258881
4 0.932937979698181
5 0.925799369812012
6 0.931330680847168
7 0.929796993732452
8 0.930428504943848
9 0.927751481533051
10 0.95908910036087
11 0.937124609947205
12 0.90973424911499
13 0.936225831508636
14 0.925829529762268
15 0.944839060306549
16 0.922749161720276
17 0.902243614196777
18 0.888154625892639
19 0.888080239295959
20 0.898278176784515
21 0.917163193225861
22 0.942171096801758
23 0.917492091655731
24 0.875304758548737
25 0.891384482383728
26 0.85667085647583
27 0.83540141582489
28 0.824497222900391
29 0.718172073364258
30 0.921007394790649
31 0.668225288391113
32 0.705218315124512
33 0.891601264476776
34 0.725548028945923
35 0.868392646312714
36 0.953947067260742
37 0.945599973201752
38 0.950485646724701
39 0.907019555568695
40 0.939283132553101
41 0.975694298744202
42 0.908632040023804
43 0.942864298820496
44 0.906556308269501
45 0.958798050880432
46 0.953290462493896
47 0.893958210945129
48 0.93825888633728
49 0.902533352375031
50 0.973571836948395
51 0.892023980617523
52 0.918857097625732
53 0.905313491821289
54 0.884380102157593
55 0.965944647789001
56 0.934836864471436
57 0.942229509353638
58 0.975091576576233
59 0.888432145118713
60 0.967403948307037
61 0.751057267189026
62 0.684019088745117
63 0.655041933059692
64 0.959853053092957
65 0.927315413951874
66 0.960387587547302
67 0.961587131023407
68 0.909804940223694
69 0.909225583076477
70 0.922748863697052
71 0.929825663566589
72 0.949474990367889
73 0.929997146129608
74 0.8944993019104
75 0.840701580047607
76 0.974945724010468
77 0.900979161262512
78 0.95941162109375
79 0.92266571521759
80 0.902121663093567
81 0.956745564937592
82 0.644664704799652
83 0.702662825584412
84 0.410124152898788
85 0.926738381385803
86 0.949648499488831
87 0.930053651332855
88 0.82854425907135
89 0.945528745651245
90 0.852297842502594
91 0.939345717430115
92 0.9212526679039
93 0.865758717060089
94 0.92478084564209
95 0.941921353340149
96 0.901877343654633
97 0.832408905029297
98 0.946486830711365
99 0.895308673381805
};
\coordinate (split) at (rel axis cs:1.035,-1);
\end{groupplot}

==> Figs/random_phi_change/noise_01_new.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm,group name=column3 plots,}]
%====================== Fig1 =============
\firstgplot{column2}{(c) $\sigma^2_{z}=0.01$}
\plotTrue
table {%
0 0.733099880094478
1 0.733099880094478
2 0.733099880094478
3 0.733099880094478
4 0.733099880094478
5 0.733099880094478
6 0.733099880094478
7 0.733099880094478
8 0.733099880094478
9 0.733099880094478
10 0.733099880094478
11 0.733099880094478
12 0.733099880094478
13 0.733099880094478
14 0.733099880094478
15 0.733099880094478
16 0.733099880094478
17 0.733099880094478
18 0.733099880094478
19 0.733099880094478
20 0.733099880094478
21 0.733099880094478
22 0.733099880094478
23 0.733099880094478
24 0.733099880094478
25 0.733099880094478
26 0.733099880094478
27 0.733099880094478
28 0.733099880094478
29 0.733099880094478
30 0.733099880094478
31 0.733099880094478
32 0.733099880094478
33 0.733099880094478
34 0.733099880094478
35 0.733099880094478
36 0.733099880094478
37 0.733099880094478
38 0.733099880094478
39 0.733099880094478
40 0.733099880094478
41 0.733099880094478
42 0.733099880094478
43 0.733099880094478
44 0.733099880094478
45 0.733099880094478
46 0.733099880094478
47 0.733099880094478
48 0.733099880094478
49 0.733099880094478
50 0.733099880094478
51 0.733099880094478
52 0.733099880094478
53 0.733099880094478
54 0.733099880094478
55 0.733099880094478
56 0.733099880094478
57 0.733099880094478
58 0.733099880094478
59 0.733099880094478
60 0.733099880094478
61 0.733099880094478
62 0.733099880094478
63 0.733099880094478
64 0.733099880094478
65 0.733099880094478
66 0.733099880094478
67 0.733099880094478
68 0.733099880094478
69 0.733099880094478
70 0.733099880094478
71 0.733099880094478
72 0.733099880094478
73 0.733099880094478
74 0.733099880094478
75 0.733099880094478
76 0.733099880094478
77 0.733099880094478
78 0.733099880094478
79 0.733099880094478
80 0.733099880094478
81 0.733099880094478
82 0.733099880094478
83 0.733099880094478
84 0.733099880094478
85 0.733099880094478
86 0.733099880094478
87 0.733099880094478
88 0.733099880094478
89 0.733099880094478
90 0.733099880094478
91 0.733099880094478
92 0.733099880094478
93 0.733099880094478
94 0.733099880094478
95 0.733099880094478
96 0.733099880094478
97 0.733099880094478
98 0.733099880094478
99 0.733099880094478
};
\plotNetwork
table {%
0 0.724245355818533
1 0.743429297526683
2 0.755327839078728
3 0.739428433327197
4 0.714224746366622
5 0.763483971792913
6 0.733886927837546
7 0.748000086982436
8 0.723242872421789
9 0.732411980859654
10 0.726353333242746
11 0.746736109182416
12 0.727253356913611
13 0.772855761093104
14 0.678206903339655
15 0.714801547446887
16 0.729520262055449
17 0.708116921957845
18 0.702944427894496
19 0.70300018954386
20 0.689076498887292
21 0.737030170459399
22 0.724664126851586
23 0.709686074223245
24 0.717379599598518
25 0.637248902253692
26 0.654514375899505
27 0.594422979273164
28 0.879148059140869
29 0.536901265469631
30 0.754941168675547
31 0.384777070343129
32 0.653719437207528
33 0.75744471576769
34 0.412827740462919
35 0.695607957213356
36 0.679657475596554
37 0.653972936022923
38 0.7043310343684
39 0.713161936421974
40 0.732404248589363
41 0.669143393818182
42 0.731485433667779
43 0.663978471076773
44 0.71340249211864
45 0.731877959852792
46 0.706574078717935
47 0.720800401517162
48 0.684044056258544
49 0.739140103743409
50 0.718776570183092
51 0.62617818573835
52 0.648914566777358
53 0.76524035673258
54 0.762255576493313
55 0.729689324421253
56 0.715099245863462
57 0.731681652443605
58 0.767642832995865
59 0.719832417805036
60 0.764799056306729
61 0.681129385920228
62 0.567844181853094
63 0.612922451950823
64 0.716272885688105
65 0.724141744822842
66 0.692533878983695
67 0.670469095209251
68 0.737958740369425
69 0.669096511990883
70 0.724112770193744
71 0.747528992735477
72 0.72209620220593
73 0.732130681574352
74 0.683898954311952
75 0.688893694392606
76 0.774856546703404
77 0.682773821584689
78 0.744079957508215
79 0.739724948221762
80 0.806873087924498
81 0.684719387037341
82 0.407603672646232
83 0.483057046425132
84 0.364126225214309
85 0.768703349584119
86 0.818475320919496
87 0.717444863339324
88 0.681001298408431
89 0.770868052985891
90 0.737694790984364
91 0.714782819081964
92 0.709897061983765
93 0.761785364661798
94 0.723012657018055
95 0.834767337118545
96 0.809401297755791
97 0.699660124360512
98 0.7148147270712
99 0.643145708465586
};
\plotInvscat
table {%
0 0.713381469249725
1 0.75138521194458
2 0.763847470283508
3 0.745952546596527
4 0.710946917533875
5 0.774254977703094
6 0.757054090499878
7 0.748341023921967
8 0.736632227897644
9 0.756694555282593
10 0.750130891799927
11 0.776463985443115
12 0.710509181022644
13 0.744416475296021
14 0.678224742412567
15 0.65998363494873
16 0.635172665119171
17 0.68774139881134
18 0.723239958286285
19 0.941826105117798
20 0.815487504005432
21 0.756416738033295
22 0.708232641220093
23 0.693236351013184
24 0.981993436813354
25 0.957210719585419
26 0.96570760011673
27 0.985235631465912
28 0.927610516548157
29 0.91963404417038
30 0.974661350250244
31 0.949191033840179
32 0.90591949224472
33 0.97519063949585
34 0.830650627613068
35 0.933889269828796
36 0.619555056095123
37 0.670183122158051
38 0.698196709156036
39 0.757230937480927
40 0.657638311386108
41 0.543069899082184
42 0.695365488529205
43 0.988965213298798
44 0.79091477394104
45 0.998701632022858
46 0.955300152301788
47 0.595638275146484
48 0.856569111347198
49 0.828307807445526
50 0.795806884765625
51 0.754857540130615
52 0.720036506652832
53 0.848629534244537
54 0.757501900196075
55 0.666159749031067
56 0.535293996334076
57 0.937406003475189
58 0.779024064540863
59 0.726056635379791
60 0.694822907447815
61 0.944755256175995
62 0.850436508655548
63 0.867998957633972
64 0.82702112197876
65 0.84344756603241
66 0.705239355564117
67 0.744477808475494
68 0.672934889793396
69 0.667664527893066
70 0.769090592861176
71 0.749149084091187
72 0.786912202835083
73 0.791811645030975
74 0.841645538806915
75 0.89041393995285
76 0.597248017787933
77 0.835092425346375
78 0.73237019777298
79 0.746217012405396
80 0.661512315273285
81 0.810803532600403
82 0.841420888900757
83 0.919595777988434
84 0.961828231811523
85 0.948700964450836
86 0.828872203826904
87 0.908987045288086
88 0.71951425075531
89 0.984222948551178
90 0.858778297901154
91 0.99139279127121
92 0.890430867671967
93 0.946821212768555
94 0.800593376159668
95 0.963743805885315
96 0.949863851070404
97 0.986726939678192
98 0.911070764064789
99 0.989980697631836
};

%====================== Fig2 =============
\nextgplot
\perturbation
\plotTrue
table {%
0 0.935516519885526
1 0.935516519885526
2 0.935516519885526
3 0.935516519885526
4 0.935516519885526
5 0.935516519885526
6 0.935516519885526
7 0.935516519885526
8 0.935516519885526
9 0.935516519885526
10 0.869667569548439
11 0.727246223885405
12 0.840885440553651
13 0.669861263673315
14 0.695062251008769
15 0.653367486580926
16 0.656677578070439
17 0.60377798372569
18 0.40326589007199
19 0.544277543208332
20 0.634658637120049
21 0.771370029605121
22 0.807328666767555
23 0.705765479890902
24 0.294400085499
25 0.122840677718215
26 0.197476673071808
27 0.344663137249381
28 0.280526511787189
29 0.122459958543774
30 0.199148910512332
31 0.0403795856982413
32 0.0377646706314038
33 0.285823945820197
34 0.0291006444692511
35 0.408406259801238
36 0.408406259801238
37 0.408406259801238
38 0.408406259801238
39 0.408406259801238
40 0.408406259801238
41 0.408406259801238
42 0.408406259801238
43 0.408406259801238
44 0.408406259801238
45 0.408406259801238
46 0.408406259801238
47 0.408406259801238
48 0.408406259801238
49 0.408406259801238
50 0.408406259801238
51 0.408406259801238
52 0.408406259801238
53 0.408406259801238
54 0.408406259801238
55 0.408406259801238
56 0.408406259801238
57 0.408406259801238
58 0.408406259801238
59 0.408406259801238
60 0.402191409831325
61 0.0764337403055456
62 0.0795973866253387
63 0.0646871585761395
64 0.108009977372683
65 0.254616719700893
66 0.472565933463051
67 0.434779798744271
68 0.310130512503765
69 0.335406009918958
70 0.385910215050476
71 0.723644828986625
72 0.677641239833845
73 0.546856821471035
74 0.415658991542201
75 0.241671090622782
76 0.281803188796102
77 0.451510825833016
78 0.503227302170066
79 0.623984732537678
80 0.390940740100067
81 0.383177631440228
82 0.108923776814901
83 0.10020607423564
84 0.106528490954389
85 0.356305650239709
86 0.356305650239709
87 0.356305650239709
88 0.356305650239709
89 0.356305650239709
90 0.356305650239709
91 0.356305650239709
92 0.356305650239709
93 0.356305650239709
94 0.356305650239709
95 0.356305650239709
96 0.356305650239709
97 0.356305650239709
98 0.356305650239709
99 0.356305650239709
};
\plotNetwork
table {%
0 0.925470704185338
1 0.937849271095156
2 0.941378334349784
3 0.945428757368676
4 0.901177574964006
5 0.934391974945282
6 0.929094646371155
7 0.956098757999094
8 0.926287654854069
9 0.947984294323883
10 0.894992923494869
11 0.703632893742834
12 0.856748436200301
13 0.690556663033831
14 0.650530527539549
15 0.635118331743641
16 0.623494235198216
17 0.616291689336054
18 0.418840864122275
19 0.530096661629573
20 0.62991066035287
21 0.78603997159867
22 0.785810528114527
23 0.729752758301226
24 0.285874898304797
25 0.190087789924572
26 0.146193135925655
27 0.325053378587814
28 0.34006421543817
29 0.0924612401791791
30 0.259216354459022
31 0.0140548263446162
32 0.0278661442032604
33 0.276498730935026
34 0.0330746869436107
35 0.430147999355689
36 0.372487763099419
37 0.399822123693457
38 0.406479668139195
39 0.388145664977288
40 0.435254299736833
41 0.334620234871208
42 0.407671617567366
43 0.381766837767045
44 0.43817988077355
45 0.425914012198983
46 0.448605109408654
47 0.423159771712946
48 0.402438620345478
49 0.396715223124999
50 0.453156043122631
51 0.357102483511275
52 0.361876130101073
53 0.435209261041176
54 0.377756233526626
55 0.408143063592138
56 0.37892145029925
57 0.409128595013036
58 0.441722332657733
59 0.444593411448509
60 0.39194335683278
61 0.0943696011253332
62 0.093377682048297
63 0.0529176199025446
64 0.123294442752525
65 0.255378420099093
66 0.442305276674533
67 0.383904634867513
68 0.273743633719496
69 0.301003583796096
70 0.408544415071804
71 0.719486695927678
72 0.656391673429332
73 0.566758142471601
74 0.385022919480291
75 0.203621756762655
76 0.312176808269377
77 0.470607959412935
78 0.510523298052668
79 0.611985908231942
80 0.39821072054195
81 0.362633232983558
82 0.0853462133683748
83 0.0932718928146064
84 0.0331040403624877
85 0.360981535794264
86 0.411950766405002
87 0.380886275372253
88 0.338161750823527
89 0.351619242789125
90 0.377217515630412
91 0.360188928665314
92 0.377119106495697
93 0.317998509936369
94 0.387155042807435
95 0.3939537172217
96 0.389940989681246
97 0.306017931892426
98 0.300363965367804
99 0.329644151097596
};
\plotInvscat
table {%
0 0.927297592163086
1 0.93019837141037
2 0.936083972454071
3 0.940785109996796
4 0.902097821235657
5 0.925904333591461
6 0.931163966655731
7 0.955995380878448
8 0.939309060573578
9 0.937866568565369
10 0.87427681684494
11 0.722346782684326
12 0.833488285541534
13 0.684057414531708
14 0.630531847476959
15 0.643037617206573
16 0.677031517028809
17 0.625371932983398
18 0.622599005699158
19 0.562061071395874
20 0.647355020046234
21 0.799311101436615
22 0.79296201467514
23 0.725236356258392
24 0.710734069347382
25 0.849868834018707
26 0.948137640953064
27 0.590519785881042
28 0.282998710870743
29 0.790227949619293
30 0.837875723838806
31 0.786051511764526
32 0.741554379463196
33 0.499833822250366
34 0.709585726261139
35 0.443364322185516
36 0.774067878723145
37 0.758820652961731
38 0.558655261993408
39 0.433723151683807
40 0.726191580295563
41 0.633774518966675
42 0.487252414226532
43 0.542591094970703
44 0.617435693740845
45 0.600641489028931
46 0.54633355140686
47 0.676377356052399
48 0.588101506233215
49 0.347468256950378
50 0.447983175516129
51 0.317163556814194
52 0.628123342990875
53 0.451358288526535
54 0.495913296937943
55 0.682324707508087
56 0.825079441070557
57 0.46729388833046
58 0.437845170497894
59 0.492038875818253
60 0.510143756866455
61 0.773432672023773
62 0.698264420032501
63 0.780746936798096
64 0.593974709510803
65 0.618495523929596
66 0.502025663852692
67 0.447780460119247
68 0.64318585395813
69 0.497297316789627
70 0.461903482675552
71 0.703122198581696
72 0.622361361980438
73 0.526640713214874
74 0.513815224170685
75 0.687982439994812
76 0.770656287670135
77 0.548686563968658
78 0.559612154960632
79 0.62200915813446
80 0.63018262386322
81 0.328030049800873
82 0.716111063957214
83 0.811421573162079
84 0.599974453449249
85 0.611395120620728
86 0.474578708410263
87 0.489026874303818
88 0.555655300617218
89 0.627765536308289
90 0.361916691064835
91 0.636415660381317
92 0.705834090709686
93 0.59990930557251
94 0.398183912038803
95 0.440962225198746
96 0.46239823102951
97 0.410817176103592
98 0.686237215995789
99 0.493979096412659
};
%====================== Fig3 =============
\nextgplot
\plotTrue
table {%
0 0.824356457355511
1 0.824356457355511
2 0.824356457355511
3 0.824356457355511
4 0.824356457355511
5 0.824356457355511
6 0.824356457355511
7 0.824356457355511
8 0.824356457355511
9 0.824356457355511
10 0.824356457355511
11 0.824356457355511
12 0.824356457355511
13 0.824356457355511
14 0.824356457355511
15 0.824356457355511
16 0.824356457355511
17 0.824356457355511
18 0.824356457355511
19 0.824356457355511
20 0.824356457355511
21 0.824356457355511
22 0.824356457355511
23 0.824356457355511
24 0.824356457355511
25 0.824356457355511
26 0.824356457355511
27 0.824356457355511
28 0.824356457355511
29 0.824356457355511
30 0.824356457355511
31 0.824356457355511
32 0.824356457355511
33 0.824356457355511
34 0.824356457355511
35 0.824356457355511
36 0.824356457355511
37 0.824356457355511
38 0.824356457355511
39 0.824356457355511
40 0.824356457355511
41 0.824356457355511
42 0.824356457355511
43 0.824356457355511
44 0.824356457355511
45 0.824356457355511
46 0.824356457355511
47 0.824356457355511
48 0.824356457355511
49 0.824356457355511
50 0.824356457355511
51 0.824356457355511
52 0.824356457355511
53 0.824356457355511
54 0.824356457355511
55 0.824356457355511
56 0.824356457355511
57 0.824356457355511
58 0.824356457355511
59 0.824356457355511
60 0.824356457355511
61 0.824356457355511
62 0.824356457355511
63 0.824356457355511
64 0.824356457355511
65 0.824356457355511
66 0.824356457355511
67 0.824356457355511
68 0.824356457355511
69 0.824356457355511
70 0.824356457355511
71 0.824356457355511
72 0.824356457355511
73 0.824356457355511
74 0.824356457355511
75 0.824356457355511
76 0.824356457355511
77 0.824356457355511
78 0.824356457355511
79 0.824356457355511
80 0.824356457355511
81 0.824356457355511
82 0.824356457355511
83 0.824356457355511
84 0.824356457355511
85 0.824356457355511
86 0.824356457355511
87 0.824356457355511
88 0.824356457355511
89 0.824356457355511
90 0.824356457355511
91 0.824356457355511
92 0.824356457355511
93 0.824356457355511
94 0.824356457355511
95 0.824356457355511
96 0.824356457355511
97 0.824356457355511
98 0.824356457355511
99 0.824356457355511
};
\plotNetwork
table {%
0 0.855330058232372
1 0.829761148241245
2 0.814397366533726
3 0.846072061274547
4 0.818867879839262
5 0.805031697398218
6 0.827055546379916
7 0.83756888992465
8 0.849931087987594
9 0.839819221826912
10 0.810591142840236
11 0.828805223725519
12 0.824407437512548
13 0.814667930868378
14 0.833271596137368
15 0.828822763486118
16 0.830807240785563
17 0.837754758754873
18 0.852172220180925
19 0.818487718586808
20 0.8336764489448
21 0.812454917975347
22 0.837027684439542
23 0.822586231934992
24 0.848512208254053
25 0.783331756905821
26 0.879252040971062
27 0.874676427098194
28 0.725805546387625
29 0.955646477066552
30 0.808721738678512
31 0.999492142613322
32 0.916377664071351
33 0.78825909522943
34 0.983480309358815
35 0.837670629183792
36 0.885386143241918
37 0.843688515491949
38 0.859051482276828
39 0.841721105951929
40 0.83252728938492
41 0.872355151760987
42 0.822366408190339
43 0.870787839642513
44 0.827943757651871
45 0.82573458269436
46 0.843128981819936
47 0.829459472254056
48 0.861395778782633
49 0.807804122705086
50 0.844955614984649
51 0.860375811958528
52 0.888087822304669
53 0.805414445443082
54 0.821642456376422
55 0.782172691260675
56 0.842891363267301
57 0.820453485045913
58 0.808525832423304
59 0.802777046473784
60 0.840763205517079
61 0.88346910496206
62 0.929064444190566
63 0.945060274440064
64 0.924837618755385
65 0.836760272769468
66 0.853746437727846
67 0.883948731719238
68 0.836608413276319
69 0.874645379183391
70 0.845368380859481
71 0.82437494626838
72 0.82787610370648
73 0.823198880004132
74 0.873283468617601
75 0.887783220338839
76 0.770119584736761
77 0.850882753147918
78 0.801478217190155
79 0.828140118918535
80 0.795059376381759
81 0.861257946298578
82 0.954363249090131
83 0.864812018613858
84 0.930866319017618
85 0.785522051676438
86 0.743440735782507
87 0.824820346991942
88 0.873948353961505
89 0.800964541231003
90 0.78404760701156
91 0.795810764312295
92 0.815395760847931
93 0.795604689773195
94 0.834541842301117
95 0.782483511542912
96 0.790077820936528
97 0.862305956486684
98 0.88630470709167
99 0.861676986635022
};
\plotInvscat
table {%
0 0.82437926530838
1 0.842081904411316
2 0.832702934741974
3 0.849853992462158
4 0.815138220787048
5 0.806384325027466
6 0.819285213947296
7 0.830004155635834
8 0.823944747447968
9 0.860693037509918
10 0.861645758152008
11 0.809569537639618
12 0.826862633228302
13 0.840484976768494
14 0.915342330932617
15 0.91758120059967
16 0.886952579021454
17 0.887867093086243
18 0.607633113861084
19 0.652767837047577
20 0.799284696578979
21 0.798762142658234
22 0.884693622589111
23 0.875838041305542
24 0.33412230014801
25 0.637163817882538
26 0.244569301605225
27 0.322858244180679
28 0.540039539337158
29 0.90748393535614
30 0.22426737844944
31 0.470648139715195
32 0.807712614536285
33 0.333133012056351
34 0.586485385894775
35 0.733056008815765
36 0.925433456897736
37 0.771586775779724
38 0.718525409698486
39 0.788022100925446
40 0.801961719989777
41 0.913175642490387
42 0.784210324287415
43 0.520162224769592
44 0.602208971977234
45 0.464386940002441
46 0.629339039325714
47 0.958249270915985
48 0.688918471336365
49 0.671893894672394
50 0.834752798080444
51 0.87633615732193
52 0.847238063812256
53 0.669071853160858
54 0.70211124420166
55 0.679166734218597
56 0.943507730960846
57 0.634631335735321
58 0.80561900138855
59 0.739399015903473
60 0.832571685314178
61 0.899694979190826
62 0.636404395103455
63 0.824848055839539
64 0.295235484838486
65 0.432781964540482
66 0.765971481800079
67 0.925306379795074
68 0.683270335197449
69 0.931552827358246
70 0.903645396232605
71 0.844733953475952
72 0.838662803173065
73 0.790195822715759
74 0.566422402858734
75 0.289188265800476
76 0.926349818706512
77 0.836290240287781
78 0.785325646400452
79 0.828288674354553
80 0.814848005771637
81 0.809660196304321
82 0.653323233127594
83 0.732822597026825
84 0.339553385972977
85 0.645953834056854
86 0.676450908184052
87 0.694863379001617
88 0.602737784385681
89 0.307680279016495
90 0.728331804275513
91 0.682312846183777
92 0.330573469400406
93 0.542978346347809
94 0.917461574077606
95 0.553330481052399
96 0.76913720369339
97 0.435186177492142
98 0.479274183511734
99 0.561076045036316
};
%====================== Fig4 =============
\nextgplot
\plotTrue
table {%
0 0.753602486017811
1 0.753602486017811
2 0.753602486017811
3 0.753602486017811
4 0.753602486017811
5 0.753602486017811
6 0.753602486017811
7 0.753602486017811
8 0.753602486017811
9 0.753602486017811
10 0.753602486017811
11 0.753602486017811
12 0.753602486017811
13 0.753602486017811
14 0.753602486017811
15 0.753602486017811
16 0.753602486017811
17 0.753602486017811
18 0.753602486017811
19 0.753602486017811
20 0.753602486017811
21 0.753602486017811
22 0.753602486017811
23 0.753602486017811
24 0.753602486017811
25 0.753602486017811
26 0.753602486017811
27 0.753602486017811
28 0.753602486017811
29 0.753602486017811
30 0.753602486017811
31 0.753602486017811
32 0.753602486017811
33 0.753602486017811
34 0.753602486017811
35 0.753602486017811
36 0.753602486017811
37 0.753602486017811
38 0.753602486017811
39 0.753602486017811
40 0.753602486017811
41 0.753602486017811
42 0.753602486017811
43 0.753602486017811
44 0.753602486017811
45 0.753602486017811
46 0.753602486017811
47 0.753602486017811
48 0.753602486017811
49 0.753602486017811
50 0.753602486017811
51 0.753602486017811
52 0.753602486017811
53 0.753602486017811
54 0.753602486017811
55 0.753602486017811
56 0.753602486017811
57 0.753602486017811
58 0.753602486017811
59 0.753602486017811
60 0.753602486017811
61 0.753602486017811
62 0.753602486017811
63 0.753602486017811
64 0.753602486017811
65 0.753602486017811
66 0.753602486017811
67 0.753602486017811
68 0.753602486017811
69 0.753602486017811
70 0.753602486017811
71 0.753602486017811
72 0.753602486017811
73 0.753602486017811
74 0.753602486017811
75 0.753602486017811
76 0.753602486017811
77 0.753602486017811
78 0.753602486017811
79 0.753602486017811
80 0.753602486017811
81 0.753602486017811
82 0.753602486017811
83 0.753602486017811
84 0.753602486017811
85 0.753602486017811
86 0.753602486017811
87 0.753602486017811
88 0.753602486017811
89 0.753602486017811
90 0.753602486017811
91 0.753602486017811
92 0.753602486017811
93 0.753602486017811
94 0.753602486017811
95 0.753602486017811
96 0.753602486017811
97 0.753602486017811
98 0.753602486017811
99 0.753602486017811
};
\plotNetwork
table {%
0 0.759990783166443
1 0.7640856571115
2 0.755296625471858
3 0.745755213361773
4 0.77569802588456
5 0.757185349666332
6 0.732209063999254
7 0.761258353785487
8 0.780980368901775
9 0.754686521924657
10 0.763540275029612
11 0.743168839462873
12 0.755375342963351
13 0.71673870006924
14 0.769641150597418
15 0.744446186483949
16 0.756673343130281
17 0.757097573913349
18 0.771433914639102
19 0.766319496846418
20 0.772015511593491
21 0.765404466819452
22 0.757067917354524
23 0.754271330854988
24 0.762142289587362
25 0.782792533284621
26 0.773345952489174
27 0.788150752239495
28 0.68178263144933
29 0.790980667561427
30 0.732862146591935
31 0.776164184377789
32 0.749905583770774
33 0.770874255684915
34 0.771439971492539
35 0.757718241809169
36 0.740124586928071
37 0.707195788607872
38 0.748552595035003
39 0.731397801276328
40 0.752757931930564
41 0.733439930723117
42 0.749362431445107
43 0.732278694926489
44 0.754532252117953
45 0.774318755403436
46 0.739871605619205
47 0.739936957241592
48 0.736440378293064
49 0.758288646067335
50 0.754972269182306
51 0.684979079364622
52 0.713515795953247
53 0.795761624943773
54 0.774683160371579
55 0.755308934498527
56 0.741657406607615
57 0.763901715136917
58 0.755532933189494
59 0.731297384360599
60 0.757888961416507
61 0.753864520454346
62 0.749523634475031
63 0.762780849133081
64 0.742862558802925
65 0.756086122264486
66 0.725250740173751
67 0.74006995992937
68 0.749121751098179
69 0.738650379104197
70 0.779952747054614
71 0.757443033447613
72 0.727262108127781
73 0.758297274538763
74 0.735918815616118
75 0.768786366998013
76 0.736140141974805
77 0.748562495413592
78 0.73851106866062
79 0.736246826646334
80 0.768931576895947
81 0.751817704508277
82 0.752630230457641
83 0.769728564658045
84 0.762475265641424
85 0.758354495316565
86 0.717172799833171
87 0.731555965581238
88 0.761272409102282
89 0.751027968482283
90 0.757552442626043
91 0.767864055829543
92 0.750521188551249
93 0.751965909984637
94 0.769043385479314
95 0.731160856941937
96 0.735088624211009
97 0.770370896210139
98 0.77600061533861
99 0.782539635052374
};
\plotInvscat
table {%
0 0.778927803039551
1 0.739945650100708
2 0.746434092521667
3 0.738224923610687
4 0.766630947589874
5 0.728367924690247
6 0.710052490234375
7 0.737324714660645
8 0.79345291852951
9 0.711042881011963
10 0.720336258411407
11 0.718893945217133
12 0.76026862859726
13 0.735741138458252
14 0.779932379722595
15 0.773992836475372
16 0.815507888793945
17 0.76263964176178
18 0.924981117248535
19 0.743101298809052
20 0.669940292835236
21 0.741710305213928
22 0.76714015007019
23 0.738741993904114
24 0.726512372493744
25 0.177717745304108
26 0.339148730039597
27 0.786962568759918
28 0.656317174434662
29 0.0519649051129818
30 0.760638356208801
31 0.142427787184715
32 0.0415341109037399
33 0.892127335071564
34 0.229273572564125
35 0.828855216503143
36 0.527586817741394
37 0.531122148036957
38 0.701032519340515
39 0.76777970790863
40 0.644629418849945
41 0.657652735710144
42 0.752447545528412
43 0.922679841518402
44 0.797695577144623
45 0.978446841239929
46 0.815701067447662
47 0.581789374351501
48 0.667745172977448
49 0.793625950813293
50 0.784821093082428
51 0.700482785701752
52 0.619156002998352
53 0.836855173110962
54 0.769140839576721
55 0.663491487503052
56 0.516362011432648
57 0.764693439006805
58 0.765627920627594
59 0.731353282928467
60 0.738692343235016
61 0.0667261406779289
62 0.149739339947701
63 0.122732661664486
64 0.467835128307343
65 0.528282999992371
66 0.737736284732819
67 0.721633076667786
68 0.609878659248352
69 0.659056782722473
70 0.752039134502411
71 0.754067122936249
72 0.761600971221924
73 0.806951701641083
74 0.792551219463348
75 0.699787139892578
76 0.529045939445496
77 0.729224979877472
78 0.743136644363403
79 0.749205410480499
80 0.66278350353241
81 0.78742116689682
82 0.169048443436623
83 0.127088874578476
84 0.260458052158356
85 0.503267526626587
86 0.691369235515594
87 0.58594411611557
88 0.935175597667694
89 0.708998620510101
90 0.839251935482025
91 0.393533259630203
92 0.935764908790588
93 0.510634422302246
94 0.781226694583893
95 0.77806681394577
96 0.581986844539642
97 0.740639388561249
98 0.64421272277832
99 0.612559258937836
};
%====================== Fig5 =============
\lastgplot{5}
\plotTrue
table {%
0 0.935826238137458
1 0.935826238137458
2 0.935826238137458
3 0.935826238137458
4 0.935826238137458
5 0.935826238137458
6 0.935826238137458
7 0.935826238137458
8 0.935826238137458
9 0.935826238137458
10 0.935826238137458
11 0.935826238137458
12 0.935826238137458
13 0.935826238137458
14 0.935826238137458
15 0.935826238137458
16 0.935826238137458
17 0.935826238137458
18 0.935826238137458
19 0.935826238137458
20 0.935826238137458
21 0.935826238137458
22 0.935826238137458
23 0.935826238137458
24 0.935826238137458
25 0.935826238137458
26 0.935826238137458
27 0.935826238137458
28 0.935826238137458
29 0.935826238137458
30 0.935826238137458
31 0.935826238137458
32 0.935826238137458
33 0.935826238137458
34 0.935826238137458
35 0.935826238137458
36 0.935826238137458
37 0.935826238137458
38 0.935826238137458
39 0.935826238137458
40 0.935826238137458
41 0.935826238137458
42 0.935826238137458
43 0.935826238137458
44 0.935826238137458
45 0.935826238137458
46 0.935826238137458
47 0.935826238137458
48 0.935826238137458
49 0.935826238137458
50 0.935826238137458
51 0.935826238137458
52 0.935826238137458
53 0.935826238137458
54 0.935826238137458
55 0.935826238137458
56 0.935826238137458
57 0.935826238137458
58 0.935826238137458
59 0.935826238137458
60 0.935826238137458
61 0.935826238137458
62 0.935826238137458
63 0.935826238137458
64 0.935826238137458
65 0.935826238137458
66 0.935826238137458
67 0.935826238137458
68 0.935826238137458
69 0.935826238137458
70 0.935826238137458
71 0.935826238137458
72 0.935826238137458
73 0.935826238137458
74 0.935826238137458
75 0.935826238137458
76 0.935826238137458
77 0.935826238137458
78 0.935826238137458
79 0.935826238137458
80 0.935826238137458
81 0.935826238137458
82 0.935826238137458
83 0.935826238137458
84 0.935826238137458
85 0.935826238137458
86 0.935826238137458
87 0.935826238137458
88 0.935826238137458
89 0.935826238137458
90 0.935826238137458
91 0.935826238137458
92 0.935826238137458
93 0.935826238137458
94 0.935826238137458
95 0.935826238137458
96 0.935826238137458
97 0.935826238137458
98 0.935826238137458
99 0.935826238137458
};
\plotNetwork
table {%
0 0.917054398468542
1 0.935300723150759
2 0.938980268846757
3 0.924890289536618
4 0.94712291149231
5 0.950899084738631
6 0.943233286756485
7 0.935582548056877
8 0.931573920814944
9 0.933924635268045
10 0.95519029009141
11 0.932864227947932
12 0.949843730874542
13 0.93966750456766
14 0.935160687489897
15 0.931319553356643
16 0.92493770048929
17 0.931432879058668
18 0.94068784973985
19 0.916577656245815
20 0.945545546902177
21 0.934800821115323
22 0.936471951515545
23 0.936646351860724
24 0.926209160764817
25 0.947912138218869
26 0.934368386100015
27 0.951818384586236
28 0.930650359838214
29 0.940823386048394
30 0.930565237819513
31 0.940619708855195
32 0.944229279507551
33 0.939739114888715
34 0.92085108147359
35 0.931365430761337
36 0.911730816889181
37 0.928908190004544
38 0.904282373011423
39 0.930260434558436
40 0.917697436641962
41 0.929689539512353
42 0.932436532299725
43 0.929835689506884
44 0.943171567856882
45 0.933442834408833
46 0.931544607242735
47 0.921651795345924
48 0.933935223904717
49 0.939031745695149
50 0.93065988685626
51 0.921613664419903
52 0.919557889482569
53 0.941101391953695
54 0.925014099033313
55 0.939728222617116
56 0.934474849726639
57 0.94331390066429
58 0.931557141077846
59 0.927293277880206
60 0.932079298099005
61 0.936913801501741
62 0.928104275385367
63 0.924503634874119
64 0.929581936948999
65 0.934097218503631
66 0.938486046783579
67 0.915918285861148
68 0.94736967995141
69 0.937581614753756
70 0.938105562169913
71 0.924483251073452
72 0.943973088533501
73 0.951116205074354
74 0.92534120254082
75 0.929522156446841
76 0.941463409805301
77 0.939674512539735
78 0.949205919709675
79 0.926578175254997
80 0.950953105307243
81 0.942774496401476
82 0.92467579851855
83 0.94853618625461
84 0.926928123171589
85 0.92163654915191
86 0.935232365808566
87 0.944007693815456
88 0.949782129444723
89 0.933818218923904
90 0.949095927449703
91 0.944666455997204
92 0.935433414982421
93 0.935901018486468
94 0.953899333796737
95 0.925844219744325
96 0.92215229161071
97 0.940792871137359
98 0.934739195129525
99 0.944337244879448
};
\plotInvscat
table {%
0 0.937572300434113
1 0.91571718454361
2 0.911813795566559
3 0.919854462146759
4 0.940189898014069
5 0.933124005794525
6 0.945930063724518
7 0.94175112247467
8 0.951275944709778
9 0.910393953323364
10 0.917783856391907
11 0.927592575550079
12 0.948601186275482
13 0.938393652439117
14 0.901778876781464
15 0.908226370811462
16 0.925330460071564
17 0.922205626964569
18 0.953356921672821
19 0.832679569721222
20 0.920197486877441
21 0.932594835758209
22 0.91603946685791
23 0.902854144573212
24 0.856390416622162
25 0.778736233711243
26 0.920231759548187
27 0.917486131191254
28 0.942998826503754
29 0.478738635778427
30 0.915707170963287
31 0.821128785610199
32 0.485855370759964
33 0.905673086643219
34 0.65497237443924
35 0.903449535369873
36 0.947480440139771
37 0.977069079875946
38 0.953209817409515
39 0.92719030380249
40 0.957165837287903
41 0.93740701675415
42 0.960544228553772
43 0.878163397312164
44 0.966400682926178
45 0.885862946510315
46 0.849739253520966
47 0.942148566246033
48 0.866149306297302
49 0.947156071662903
50 0.899646162986755
51 0.891709744930267
52 0.859679877758026
53 0.935984551906586
54 0.967523574829102
55 0.981795907020569
56 0.961738586425781
57 0.905758738517761
58 0.936054050922394
59 0.951460838317871
60 0.949373245239258
61 0.671451091766357
62 0.643483936786652
63 0.838417649269104
64 0.810358285903931
65 0.81404572725296
66 0.96434211730957
67 0.883014380931854
68 0.963560342788696
69 0.932668328285217
70 0.912017464637756
71 0.925499677658081
72 0.912513971328735
73 0.952278554439545
74 0.938883662223816
75 0.854123175144196
76 0.959877908229828
77 0.862549304962158
78 0.963953733444214
79 0.907254159450531
80 0.972041249275208
81 0.944351136684418
82 0.714078962802887
83 0.849609613418579
84 0.849709153175354
85 0.897207975387573
86 0.921350061893463
87 0.961975753307343
88 0.958113074302673
89 0.899667143821716
90 0.923284232616425
91 0.822717547416687
92 0.966521143913269
93 0.931774795055389
94 0.935510993003845
95 0.872281491756439
96 0.819779098033905
97 0.9441819190979
98 0.9857377409935
99 0.853428184986115
};
\coordinate (split) at (rel axis cs:1.035,-1);
\end{groupplot}

==> Figs/random_phi_psi_change/failed_ase_noise_0.0001.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm, group name=column4 plots }]


%================= Fig1 ===============
\firstgplot{column3}{(d) Overparam.~($\sigma^2_z=0.0001$)}

\plotTrue
table {%
0 0.0245707776166385
1 0.0245707776166385
2 0.0245707776166385
3 0.0245707776166385
4 0.0245707776166385
5 0.0245707776166385
6 0.0245707776166385
7 0.0245707776166385
8 0.0245707776166385
9 0.0245707776166385
10 0.0245707776166385
11 0.0245707776166385
12 0.0245707776166385
13 0.0245707776166385
14 0.0245707776166385
15 0.0245707776166385
16 0.0245707776166385
17 0.0245707776166385
18 0.0245707776166385
19 0.0245707776166385
20 0.0245707776166385
21 0.0245707776166385
22 0.0245707776166385
23 0.0245707776166385
24 0.0245707776166385
25 0.0245707776166385
26 0.0245707776166385
27 0.0245707776166385
28 0.0245707776166385
29 0.0245707776166385
30 0.0245707776166385
31 0.0245707776166385
32 0.0245707776166385
33 0.0245707776166385
34 0.0245707776166385
35 0.0245707776166385
36 0.0245707776166385
37 0.0245707776166385
38 0.0245707776166385
39 0.0245707776166385
40 0.0245707776166385
41 0.0245707776166385
42 0.0245707776166385
43 0.0245707776166385
44 0.0245707776166385
45 0.0245707776166385
46 0.0245707776166385
47 0.0245707776166385
48 0.0245707776166385
49 0.0245707776166385
50 0.0245707776166385
51 0.0245707776166385
52 0.0245707776166385
53 0.0245707776166385
54 0.0245707776166385
55 0.0245707776166385
56 0.0245707776166385
57 0.0245707776166385
58 0.0245707776166385
59 0.0245707776166385
60 0.0245707776166385
61 0.0245707776166385
62 0.0245707776166385
63 0.0245707776166385
64 0.0245707776166385
65 0.0245707776166385
66 0.0245707776166385
67 0.0245707776166385
68 0.0245707776166385
69 0.0245707776166385
70 0.0245707776166385
71 0.0245707776166385
72 0.0245707776166385
73 0.0245707776166385
74 0.0245707776166385
75 0.0245707776166385
76 0.0245707776166385
77 0.0245707776166385
78 0.0245707776166385
79 0.0245707776166385
80 0.0245707776166385
81 0.0245707776166385
82 0.0245707776166385
83 0.0245707776166385
84 0.0245707776166385
85 0.0245707776166385
86 0.0245707776166385
87 0.0245707776166385
88 0.0245707776166385
89 0.0245707776166385
90 0.0245707776166385
91 0.0245707776166385
92 0.0245707776166385
93 0.0245707776166385
94 0.0245707776166385
95 0.0245707776166385
96 0.0245707776166385
97 0.0245707776166385
98 0.0245707776166385
99 0.0245707776166385
};
\plotNetwork
table {%
0 0.994391001904268
1 0.993590825410883
2 0.992023489465153
3 0.990713486320866
4 0.991419552162517
5 0.989441351270044
6 0.985967987035861
7 0.986591439748254
8 0.984670286347738
9 0.986597615414255
10 0.979080746438938
11 0.936462525974394
12 0.958460205980893
13 0.977461709767043
14 0.926143567044687
15 0.969877221779873
16 0.925972885044056
17 0.97643929816115
18 0.88611663820043
19 0.917625243931487
20 0.877145740184788
21 0.953381472009079
22 0.974847852348981
23 0.927111812334532
24 0.934531518335522
25 0.980827984776332
26 0.739449302714185
27 0.0165268251851707
28 0.0242172410413297
29 0.00721320476851423
30 0.0570705396937386
31 0.0713426995687485
32 0.117299555830363
33 0.135229538847016
34 0.063600727763936
35 0.0706248524204548
36 0.119392320335038
37 0.0381834501022485
38 0.0255290641058863
39 0.117753979288055
40 0.0117760812682947
41 0.0436763182753637
42 0.0363630434644735
43 0.0823891634208204
44 0.0360113232634925
45 0.155558850091638
46 0.269960569866067
47 0.19046165186407
48 0.20123595690344
49 0.215823860533451
50 0.214196769809024
51 0.164617758683008
52 0.136165602457356
53 0.130171659975048
54 0.170701750460507
55 0.190553967781076
56 0.0990810814671496
57 0.0853072985246207
58 0.0969155607001727
59 0.09353936753321
60 0.0349658762122373
61 0.130589459020042
62 0.398867311071014
63 0.244857360686911
64 0.00909265722371248
65 0.113311248326232
66 0.109276162333659
67 0.167700735509685
68 0.0823485802881675
69 0.0144209031988826
70 0.00617759899796809
71 0.0230910450464928
72 0.0171292712908548
73 0.000829106975726176
74 0.0708381570410189
75 0.0779399967969744
76 0.010724288558744
77 0.0133747985210881
78 0.046208956696191
79 0.0379587511395605
80 0.0289124910834945
81 0.0319568722933578
82 0.0236896821174848
83 0.0271253953733398
84 0.0228206963786261
85 0.0298576086148561
86 0.0265755521574235
87 0.0318396664205288
88 0.0255345841104967
89 0.0245550493549986
90 0.0230087042339706
91 0.0238996101735972
92 0.0257473363806445
93 0.0235924636438903
94 0.0306389142081135
95 0.0275012346579162
96 0.0202740045058776
97 0.0279627903401782
98 0.0242651126117082
99 0.0237469148287655
};
\plotInvscat
table {%
0 0.969182074069977
1 0.976240277290344
2 0.959551930427551
3 0.976244568824768
4 0.966413378715515
5 0.915303528308868
6 0.961997985839844
7 0.952916920185089
8 0.976226449012756
9 0.97721666097641
10 0.965310633182526
11 0.989404678344727
12 0.967788100242615
13 0.977948665618896
14 0.966520845890045
15 0.938928544521332
16 0.980758488178253
17 0.969111382961273
18 0.983753502368927
19 0.875054657459259
20 0.980845510959625
21 0.911844849586487
22 0.964713215827942
23 0.953747570514679
24 0.954650819301605
25 0.927320778369904
26 0.83820778131485
27 0.864595830440521
28 0.802489519119263
29 0.978740811347961
30 0.976535499095917
31 0.992749154567719
32 0.961867928504944
33 0.976606249809265
34 0.987753331661224
35 0.97024929523468
36 0.956831395626068
37 0.954851031303406
38 0.960090398788452
39 0.9508096575737
40 0.947561144828796
41 0.951627671718597
42 0.957270741462708
43 0.977704346179962
44 0.948898375034332
45 0.951896965503693
46 0.964131832122803
47 0.95647794008255
48 0.969967603683472
49 0.974561095237732
50 0.938155770301819
51 0.960932791233063
52 0.977557003498077
53 0.965994536876678
54 0.963357090950012
55 0.960285186767578
56 0.952984511852264
57 0.970089495182037
58 0.946129381656647
59 0.962903797626495
60 0.96126663684845
61 0.96542090177536
62 0.983666598796844
63 0.96205997467041
64 0.920154333114624
65 0.980610430240631
66 0.953224003314972
67 0.954712092876434
68 0.976130962371826
69 0.979389607906342
70 0.944278955459595
71 0.954823315143585
72 0.912834644317627
73 0.995994448661804
74 0.981224000453949
75 0.911551058292389
76 0.953721821308136
77 0.564257860183716
78 0.985868275165558
79 0.990012347698212
80 0.454087495803833
81 0.933582186698914
82 0.540674388408661
83 0.795141100883484
84 0.879168927669525
85 0.597076117992401
86 0.713367462158203
87 0.926122903823853
88 0.719994246959686
89 0.485396146774292
90 0.446164488792419
91 0.402833968400955
92 0.540696799755096
93 0.470048189163208
94 0.66285765171051
95 0.916391730308533
96 0.724520206451416
97 0.466566860675812
98 0.575414419174194
99 0.742052435874939
};
%================= Fig2 ===============
\nextgplot
\perturbation
\plotTrue
table {%
0 0.0796525557961304
1 0.0796525557961304
2 0.0796525557961304
3 0.0796525557961304
4 0.0796525557961304
5 0.0796525557961304
6 0.0796525557961304
7 0.0796525557961304
8 0.0796525557961304
9 0.0796525557961304
10 0.0953390684937343
11 0.15832830576006
12 0.074209401453014
13 0.0562947809910471
14 0.162434262577782
15 0.0786592992134329
16 0.153351841476454
17 0.0136003632408747
18 0.208244430342285
19 0.18081998010704
20 0.211445263738759
21 0.0754756573444908
22 0.0432501349440016
23 0.156436015696073
24 0.151514144877208
25 0.0153455234228614
26 0.298540346423877
27 0.487245563193296
28 0.603424467791033
29 0.356885009163709
30 0.069825690280223
31 0.154077443386182
32 0.0763726458331348
33 0.102949683606279
34 0.160947370932029
35 0.110704182221555
36 0.110704182221555
37 0.110704182221555
38 0.110704182221555
39 0.110704182221555
40 0.110704182221555
41 0.110704182221555
42 0.110704182221555
43 0.110704182221555
44 0.110704182221555
45 0.110704182221555
46 0.110704182221555
47 0.110704182221555
48 0.110704182221555
49 0.110704182221555
50 0.110704182221555
51 0.110704182221555
52 0.110704182221555
53 0.110704182221555
54 0.110704182221555
55 0.110704182221555
56 0.110704182221555
57 0.110704182221555
58 0.110704182221555
59 0.110704182221555
60 0.193661287426511
61 0.0803753808702726
62 0.0257047272872711
63 0.118819359556358
64 0.255987723568507
65 0.0955916742771348
66 0.182784163039924
67 0.0655266653203569
68 0.206381201989831
69 0.284512392515153
70 0.218322327184057
71 0.375144959696964
72 0.42583356095422
73 0.243673761433346
74 0.0903863218027377
75 0.189806921627192
76 0.287293515789283
77 0.44573950826256
78 0.358621371350008
79 0.494057774762813
80 0.62592654012827
81 0.638080318265771
82 0.860766977102702
83 0.733276116307116
84 0.689815196333366
85 0.844547463002903
86 0.844547463002903
87 0.844547463002903
88 0.844547463002903
89 0.844547463002903
90 0.844547463002903
91 0.844547463002903
92 0.844547463002903
93 0.844547463002903
94 0.844547463002903
95 0.844547463002903
96 0.844547463002903
97 0.844547463002903
98 0.844547463002903
99 0.844547463002903
};
\plotNetwork
table {%
0 0.257945483991187
1 0.24608705635515
2 0.23588472652703
3 0.230562227110413
4 0.228766139251353
5 0.220835935458193
6 0.21936799480507
7 0.223070656974481
8 0.218266840289634
9 0.220114110866727
10 0.21524036224036
11 0.210775829148594
12 0.281785009382861
13 0.229384735848463
14 0.203416198476246
15 0.255592632819104
16 0.207026092801937
17 0.246262786496357
18 0.214448052992344
19 0.20776099049095
20 0.208600760402903
21 0.28652865578402
22 0.239748531310314
23 0.205471457656717
24 0.208320712691165
25 0.245300190532203
26 0.235385024979685
27 0.483899846488648
28 0.601754638241767
29 0.349700115270201
30 0.0683485591237702
31 0.149914071827525
32 0.0769744745127422
33 0.10229253602999
34 0.155373614011904
35 0.108070956035012
36 0.108086806919118
37 0.108798004494907
38 0.108460814183097
39 0.104542275317033
40 0.114319042029842
41 0.108801125561445
42 0.109554442016004
43 0.111597135006452
44 0.111719497079811
45 0.106974194643751
46 0.104082300873252
47 0.106813814987101
48 0.106141842062682
49 0.105082961044352
50 0.107655704519757
51 0.106987387873371
52 0.112099665389489
53 0.105733060979819
54 0.108653969095671
55 0.108221091178659
56 0.110445081467686
57 0.107311007545421
58 0.110520073970958
59 0.107431206402945
60 0.190509667541613
61 0.0736648823322855
62 0.0222263473666977
63 0.11003186498779
64 0.253212377202433
65 0.0922907892004
66 0.18036490832037
67 0.0641376949054551
68 0.200695294407503
69 0.280696689773622
70 0.216386730741523
71 0.375230201951646
72 0.424907309256999
73 0.237541965169586
74 0.0884178885370846
75 0.193667472577915
76 0.286242307136572
77 0.440291991270286
78 0.362709209881198
79 0.495914470522185
80 0.625656701554437
81 0.636397668631127
82 0.860645422705288
83 0.73232702543739
84 0.68877908003226
85 0.843292198116125
86 0.843878145083434
87 0.845055341302422
88 0.844950751045094
89 0.844709428606303
90 0.842357683692036
91 0.844775096596347
92 0.843733403187634
93 0.844790844624001
94 0.847749044818676
95 0.846113376120151
96 0.843753687797669
97 0.845659244646935
98 0.845154060576915
99 0.845317413997551
};
\plotInvscat
table {%
0 0.263804703950882
1 0.276769697666168
2 0.257909625768661
3 0.228806510567665
4 0.259206980466843
5 0.237914368510246
6 0.266375303268433
7 0.273920714855194
8 0.257651507854462
9 0.264161378145218
10 0.301670789718628
11 0.2932348549366
12 0.272649556398392
13 0.264174580574036
14 0.303663522005081
15 0.274351984262466
16 0.38533017039299
17 0.265907973051071
18 0.284508615732193
19 0.324039876461029
20 0.320102959871292
21 0.248298346996307
22 0.278807431459427
23 0.229680016636848
24 0.293307900428772
25 0.13981431722641
26 0.321974486112595
27 0.504577875137329
28 0.532053411006927
29 0.464271783828735
30 0.22796830534935
31 0.256818056106567
32 0.26346144080162
33 0.265323311090469
34 0.335535049438477
35 0.265698224306107
36 0.274710536003113
37 0.269968718290329
38 0.271023869514465
39 0.268409132957458
40 0.28764995932579
41 0.297730833292007
42 0.263902187347412
43 0.274656563997269
44 0.2599276304245
45 0.270490229129791
46 0.245884016156197
47 0.266092270612717
48 0.260706722736359
49 0.270478665828705
50 0.299232095479965
51 0.275221824645996
52 0.253532707691193
53 0.264811098575592
54 0.273413896560669
55 0.279544144868851
56 0.324920386075974
57 0.271491318941116
58 0.287515670061111
59 0.281277924776077
60 0.33710128068924
61 0.284177988767624
62 0.260694444179535
63 0.265727281570435
64 0.336457401514053
65 0.227838292717934
66 0.322998076677322
67 0.278729468584061
68 0.411367475986481
69 0.369873344898224
70 0.259613484144211
71 0.476468026638031
72 0.523672878742218
73 0.294351786375046
74 0.252061814069748
75 0.279117196798325
76 0.334571272134781
77 0.366232335567474
78 0.398353517055511
79 0.690429508686066
80 0.528174459934235
81 0.644400775432587
82 0.432781994342804
83 0.586021244525909
84 0.483237862586975
85 0.512553095817566
86 0.50925475358963
87 0.545404195785522
88 0.483592689037323
89 0.5296710729599
90 0.392950266599655
91 0.486143261194229
92 0.481059700250626
93 0.466647952795029
94 0.50713312625885
95 0.493383020162582
96 0.483377814292908
97 0.466277420520782
98 0.436066657304764
99 0.558471858501434
};
%================= Fig3 ===============
\nextgplot
\plotTrue
table {%
0 0.963992089322708
1 0.963992089322708
2 0.963992089322708
3 0.963992089322708
4 0.963992089322708
5 0.963992089322708
6 0.963992089322708
7 0.963992089322708
8 0.963992089322708
9 0.963992089322708
10 0.963992089322708
11 0.963992089322708
12 0.963992089322708
13 0.963992089322708
14 0.963992089322708
15 0.963992089322708
16 0.963992089322708
17 0.963992089322708
18 0.963992089322708
19 0.963992089322708
20 0.963992089322708
21 0.963992089322708
22 0.963992089322708
23 0.963992089322708
24 0.963992089322708
25 0.963992089322708
26 0.963992089322708
27 0.963992089322708
28 0.963992089322708
29 0.963992089322708
30 0.963992089322708
31 0.963992089322708
32 0.963992089322708
33 0.963992089322708
34 0.963992089322708
35 0.963992089322708
36 0.963992089322708
37 0.963992089322708
38 0.963992089322708
39 0.963992089322708
40 0.963992089322708
41 0.963992089322708
42 0.963992089322708
43 0.963992089322708
44 0.963992089322708
45 0.963992089322708
46 0.963992089322708
47 0.963992089322708
48 0.963992089322708
49 0.963992089322708
50 0.963992089322708
51 0.963992089322708
52 0.963992089322708
53 0.963992089322708
54 0.963992089322708
55 0.963992089322708
56 0.963992089322708
57 0.963992089322708
58 0.963992089322708
59 0.963992089322708
60 0.963992089322708
61 0.963992089322708
62 0.963992089322708
63 0.963992089322708
64 0.963992089322708
65 0.963992089322708
66 0.963992089322708
67 0.963992089322708
68 0.963992089322708
69 0.963992089322708
70 0.963992089322708
71 0.963992089322708
72 0.963992089322708
73 0.963992089322708
74 0.963992089322708
75 0.963992089322708
76 0.963992089322708
77 0.963992089322708
78 0.963992089322708
79 0.963992089322708
80 0.963992089322708
81 0.963992089322708
82 0.963992089322708
83 0.963992089322708
84 0.963992089322708
85 0.963992089322708
86 0.963992089322708
87 0.963992089322708
88 0.963992089322708
89 0.963992089322708
90 0.963992089322708
91 0.963992089322708
92 0.963992089322708
93 0.963992089322708
94 0.963992089322708
95 0.963992089322708
96 0.963992089322708
97 0.963992089322708
98 0.963992089322708
99 0.963992089322708
};
\plotNetwork
table {%
0 0.6761837411735
1 0.720091239931864
2 0.743425742575201
3 0.769317698742847
4 0.788788397904203
5 0.805633601043022
6 0.8257483205579
7 0.840968353737627
8 0.83729944311677
9 0.837704646580398
10 0.871819205424068
11 0.955763814126645
12 0.725796202298764
13 0.810989094524957
14 0.960468340960738
15 0.747056147731065
16 0.956460628803193
17 0.691712130523213
18 0.986162364562819
19 0.971200182305468
20 0.9893004628705
21 0.707374248265803
22 0.813849224483072
23 0.962073364603083
24 0.954560310923881
25 0.623592574437667
26 0.991246469194614
27 0.967813471494019
28 0.962436531485868
29 0.973854668017629
30 0.96961353308943
31 0.986056580556829
32 0.987358510568494
33 0.963597135388234
34 0.963420809095722
35 0.968718947530883
36 0.965546076238579
37 0.966724732258919
38 0.967240439618621
39 0.96761885642124
40 0.966400017945669
41 0.969807038444258
42 0.964025103962062
43 0.956399466900395
44 0.965984428255144
45 0.965156201005135
46 0.955576451091169
47 0.962426646915018
48 0.963228586040279
49 0.958094744869886
50 0.955343622465046
51 0.9623315025297
52 0.963699583635504
53 0.967919686082827
54 0.963052654306211
55 0.962601973200073
56 0.965006599236274
57 0.965438234285793
58 0.967240139556482
59 0.968065694690495
60 0.982174974790607
61 0.987222318336108
62 0.947494564326556
63 0.964714470799831
64 0.961789745100481
65 0.97147085392911
66 0.992559102948218
67 0.983156917512598
68 0.992144736241131
69 0.968333343301744
70 0.973502846460365
71 0.962976742958277
72 0.965977382568075
73 0.972198090344432
74 0.98276807989809
75 0.944116874313882
76 0.9706989139793
77 0.970026499782992
78 0.951734020150807
79 0.957915630062141
80 0.964147129860777
81 0.958322914565908
82 0.961802769018187
83 0.962816029078073
84 0.967038661654897
85 0.959379717925624
86 0.964385149140831
87 0.960058052231478
88 0.963250503184939
89 0.964185458699535
90 0.965001402219217
91 0.963076915933817
92 0.965819221729039
93 0.962099864966485
94 0.957816363367899
95 0.962504003110192
96 0.964973724951439
97 0.962264192216133
98 0.965793072193949
99 0.963378447372591
};
\plotInvscat
table {%
0 0.95821624994278
1 0.736408710479736
2 0.919333457946777
3 0.467130303382874
4 0.504831433296204
5 0.407972365617752
6 0.940692245960236
7 0.712833344936371
8 0.816754639148712
9 0.830506265163422
10 0.467214196920395
11 0.436853766441345
12 0.782279789447784
13 0.880033254623413
14 0.805629909038544
15 0.206221953034401
16 0.141293972730637
17 0.564785182476044
18 0.930589973926544
19 0.891399264335632
20 0.540598034858704
21 0.412613660097122
22 0.633056342601776
23 0.521649301052094
24 0.981374800205231
25 0.0930530354380608
26 0.263046234846115
27 0.510432064533234
28 0.41733255982399
29 0.46825122833252
30 0.251878499984741
31 0.770939528942108
32 0.725094556808472
33 0.550104558467865
34 0.179101228713989
35 0.807236969470978
36 0.609011650085449
37 0.232626467943192
38 0.99925822019577
39 0.519873261451721
40 0.533807337284088
41 0.570052087306976
42 0.654709994792938
43 0.701563000679016
44 0.908403396606445
45 0.746540248394012
46 0.609906852245331
47 0.97189873456955
48 0.642430484294891
49 0.864175200462341
50 0.543405711650848
51 0.969177603721619
52 0.648393929004669
53 0.838748097419739
54 0.834661841392517
55 0.857539296150208
56 0.220683231949806
57 0.884952664375305
58 0.752937197685242
59 0.78791344165802
60 0.423405557870865
61 0.659443438053131
62 0.820914149284363
63 0.611216187477112
64 0.934934854507446
65 0.250591576099396
66 0.577692568302155
67 0.671850442886353
68 0.212632119655609
69 0.937262058258057
70 0.648382127285004
71 0.54257345199585
72 0.86626261472702
73 0.604395985603333
74 0.871331989765167
75 0.304278820753098
76 0.991322040557861
77 0.659083425998688
78 0.377029895782471
79 0.323786526918411
80 0.813436567783356
81 0.498794764280319
82 0.50571346282959
83 0.556605756282806
84 0.711707293987274
85 0.472226142883301
86 0.475496768951416
87 0.481912344694138
88 0.481186866760254
89 0.4618821144104
90 0.515771329402924
91 0.457651227712631
92 0.487068772315979
93 0.529647588729858
94 0.490212291479111
95 0.463726550340652
96 0.527878940105438
97 0.561855554580688
98 0.482744842767715
99 0.615122497081757
};

%================= Fig4 ===============
\nextgplot
\plotTrue
table {%
0 0.260667597303856
1 0.260667597303856
2 0.260667597303856
3 0.260667597303856
4 0.260667597303856
5 0.260667597303856
6 0.260667597303856
7 0.260667597303856
8 0.260667597303856
9 0.260667597303856
10 0.260667597303856
11 0.260667597303856
12 0.260667597303856
13 0.260667597303856
14 0.260667597303856
15 0.260667597303856
16 0.260667597303856
17 0.260667597303856
18 0.260667597303856
19 0.260667597303856
20 0.260667597303856
21 0.260667597303856
22 0.260667597303856
23 0.260667597303856
24 0.260667597303856
25 0.260667597303856
26 0.260667597303856
27 0.260667597303856
28 0.260667597303856
29 0.260667597303856
30 0.260667597303856
31 0.260667597303856
32 0.260667597303856
33 0.260667597303856
34 0.260667597303856
35 0.260667597303856
36 0.260667597303856
37 0.260667597303856
38 0.260667597303856
39 0.260667597303856
40 0.260667597303856
41 0.260667597303856
42 0.260667597303856
43 0.260667597303856
44 0.260667597303856
45 0.260667597303856
46 0.260667597303856
47 0.260667597303856
48 0.260667597303856
49 0.260667597303856
50 0.260667597303856
51 0.260667597303856
52 0.260667597303856
53 0.260667597303856
54 0.260667597303856
55 0.260667597303856
56 0.260667597303856
57 0.260667597303856
58 0.260667597303856
59 0.260667597303856
60 0.260667597303856
61 0.260667597303856
62 0.260667597303856
63 0.260667597303856
64 0.260667597303856
65 0.260667597303856
66 0.260667597303856
67 0.260667597303856
68 0.260667597303856
69 0.260667597303856
70 0.260667597303856
71 0.260667597303856
72 0.260667597303856
73 0.260667597303856
74 0.260667597303856
75 0.260667597303856
76 0.260667597303856
77 0.260667597303856
78 0.260667597303856
79 0.260667597303856
80 0.260667597303856
81 0.260667597303856
82 0.260667597303856
83 0.260667597303856
84 0.260667597303856
85 0.260667597303856
86 0.260667597303856
87 0.260667597303856
88 0.260667597303856
89 0.260667597303856
90 0.260667597303856
91 0.260667597303856
92 0.260667597303856
93 0.260667597303856
94 0.260667597303856
95 0.260667597303856
96 0.260667597303856
97 0.260667597303856
98 0.260667597303856
99 0.260667597303856
};
\plotNetwork
table {%
0 0.154320601243664
1 0.136369312377108
2 0.134848200511106
3 0.131556932119175
4 0.12037097448813
5 0.127482966462895
6 0.120891948791605
7 0.112814608374666
8 0.117800423519341
9 0.115677698210571
10 0.130744351334353
11 0.189661330812228
12 0.101805833049912
13 0.0754235017368128
14 0.193821036611285
15 0.115124454390183
16 0.183974321649934
17 0.0258005675670521
18 0.229413449796778
19 0.206288881286175
20 0.228271731176941
21 0.100929604385163
22 0.05667731150673
23 0.188537255690372
24 0.182800471608134
25 0.0378383829175005
26 0.282453956115146
27 0.258021559618386
28 0.259119985045886
29 0.255963073992688
30 0.262258177445772
31 0.255465531248516
32 0.255829617764322
33 0.272478770643131
34 0.269976913836945
35 0.268300048289151
36 0.272191643192585
37 0.259915593982474
38 0.26263023705972
39 0.268264696522098
40 0.262993551823365
41 0.264162228414133
42 0.25797901745466
43 0.259682301730121
44 0.262463587626768
45 0.273183381657754
46 0.277904446205794
47 0.269902019812102
48 0.277042175246349
49 0.275844049215702
50 0.271615931641971
51 0.272514326495965
52 0.269166129005442
53 0.265268253869881
54 0.269156652374411
55 0.272607889854103
56 0.270023907029548
57 0.268469106806165
58 0.26893873943306
59 0.26670799009989
60 0.257969072954165
61 0.256771843487892
62 0.256536828156207
63 0.27432941474193
64 0.26734960506936
65 0.267428225414161
66 0.252613863697755
67 0.258562019701212
68 0.251080341291037
69 0.263167280725584
70 0.263443634628379
71 0.262221702177494
72 0.259798319057261
73 0.257097170535305
74 0.252467887200966
75 0.267205448570434
76 0.258189891242548
77 0.258317452825638
78 0.264139038248035
79 0.268037055339671
80 0.257560146400762
81 0.263752976374354
82 0.262150568497982
83 0.262424795237174
84 0.260492887263483
85 0.260822555578505
86 0.261154317320704
87 0.262122496280406
88 0.26431359912606
89 0.262355037669727
90 0.258829854417569
91 0.258064652452597
92 0.256821274941783
93 0.262516960226365
94 0.265024863592201
95 0.259193133955929
96 0.259541349188038
97 0.263001756678464
98 0.261437791055494
99 0.261640807698319
};
\plotInvscat
table {%
0 0.0180447287857533
1 0.0409614108502865
2 0.0303216427564621
3 0.0451742857694626
4 0.0246679037809372
5 0.0462200865149498
6 0.0167431589215994
7 0.041748471558094
8 0.0198766458779573
9 0.0198462530970573
10 0.0493126548826694
11 0.082231231033802
12 0.0346246138215065
13 0.0241866800934076
14 0.0499453507363796
15 0.0539971552789211
16 0.160215392708778
17 0.0228943321853876
18 0.0614748001098633
19 0.0545553043484688
20 0.0634443387389183
21 0.055873055011034
22 0.0293090529739857
23 0.0633535608649254
24 0.0527754537761211
25 0.395081639289856
26 0.283606886863708
27 0.258885949850082
28 0.492926567792892
29 0.18927338719368
30 0.116972900927067
31 0.0585777647793293
32 0.0281218606978655
33 0.0470310188829899
34 0.140136763453484
35 0.025875823572278
36 0.0445579960942268
37 0.0629940330982208
38 0.0208416823297739
39 0.0252350438386202
40 0.0386053174734116
41 0.0497029423713684
42 0.0367074236273766
43 0.02809171192348
44 0.0356036685407162
45 0.034818209707737
46 0.0310605112463236
47 0.0421408005058765
48 0.0353397876024246
49 0.0345092862844467
50 0.0488747321069241
51 0.0249429550021887
52 0.0263547617942095
53 0.0274151023477316
54 0.0158402696251869
55 0.031040970236063
56 0.06196179240942
57 0.0415473021566868
58 0.0303908716887236
59 0.0406664945185184
60 0.0556754767894745
61 0.0338261388242245
62 0.0165420807898045
63 0.0376735404133797
64 0.0789454653859138
65 0.0538027696311474
66 0.063243992626667
67 0.0240422412753105
68 0.134882584214211
69 0.0956785380840302
70 0.0612832345068455
71 0.145844593644142
72 0.232368499040604
73 0.0877287536859512
74 0.0266542304307222
75 0.120588131248951
76 0.0924768894910812
77 0.274107098579407
78 0.228822723031044
79 0.438722103834152
80 0.412020355463028
81 0.435457289218903
82 0.47108393907547
83 0.485562354326248
84 0.452389627695084
85 0.505009829998016
86 0.432421058416367
87 0.41338786482811
88 0.404444754123688
89 0.308612257242203
90 0.461412400007248
91 0.22475691139698
92 0.493244558572769
93 0.486399590969086
94 0.505401611328125
95 0.493745535612106
96 0.452590763568878
97 0.47648099064827
98 0.450847387313843
99 0.446504771709442
};
%================= Fig5 ===============
\lastgplot
\plotTrue
table {%
0 0.737354162123236
1 0.737354162123236
2 0.737354162123236
3 0.737354162123236
4 0.737354162123236
5 0.737354162123236
6 0.737354162123236
7 0.737354162123236
8 0.737354162123236
9 0.737354162123236
10 0.737354162123236
11 0.737354162123236
12 0.737354162123236
13 0.737354162123236
14 0.737354162123236
15 0.737354162123236
16 0.737354162123236
17 0.737354162123236
18 0.737354162123236
19 0.737354162123236
20 0.737354162123236
21 0.737354162123236
22 0.737354162123236
23 0.737354162123236
24 0.737354162123236
25 0.737354162123236
26 0.737354162123236
27 0.737354162123236
28 0.737354162123236
29 0.737354162123236
30 0.737354162123236
31 0.737354162123236
32 0.737354162123236
33 0.737354162123236
34 0.737354162123236
35 0.737354162123236
36 0.737354162123236
37 0.737354162123236
38 0.737354162123236
39 0.737354162123236
40 0.737354162123236
41 0.737354162123236
42 0.737354162123236
43 0.737354162123236
44 0.737354162123236
45 0.737354162123236
46 0.737354162123236
47 0.737354162123236
48 0.737354162123236
49 0.737354162123236
50 0.737354162123236
51 0.737354162123236
52 0.737354162123236
53 0.737354162123236
54 0.737354162123236
55 0.737354162123236
56 0.737354162123236
57 0.737354162123236
58 0.737354162123236
59 0.737354162123236
60 0.737354162123236
61 0.737354162123236
62 0.737354162123236
63 0.737354162123236
64 0.737354162123236
65 0.737354162123236
66 0.737354162123236
67 0.737354162123236
68 0.737354162123236
69 0.737354162123236
70 0.737354162123236
71 0.737354162123236
72 0.737354162123236
73 0.737354162123236
74 0.737354162123236
75 0.737354162123236
76 0.737354162123236
77 0.737354162123236
78 0.737354162123236
79 0.737354162123236
80 0.737354162123236
81 0.737354162123236
82 0.737354162123236
83 0.737354162123236
84 0.737354162123236
85 0.737354162123236
86 0.737354162123236
87 0.737354162123236
88 0.737354162123236
89 0.737354162123236
90 0.737354162123236
91 0.737354162123236
92 0.737354162123236
93 0.737354162123236
94 0.737354162123236
95 0.737354162123236
96 0.737354162123236
97 0.737354162123236
98 0.737354162123236
99 0.737354162123236
};
\plotNetwork
table {%
0 0.742478787261134
1 0.709861658941487
2 0.682963039625374
3 0.653114098686505
4 0.639250038555783
5 0.605989210263315
6 0.581210349023337
7 0.564412814542122
8 0.559554788622561
9 0.543950179949743
10 0.520945428897702
11 0.47280510172621
12 0.178277919075078
13 0.35142826424158
14 0.392076834369822
15 0.0253530989678811
16 0.383655693452258
17 0.47486475818124
18 0.457011094880224
19 0.45605013653967
20 0.442972104202858
21 0.183958941518744
22 0.339112806160182
23 0.407159936023783
24 0.429409276891679
25 0.586327233358207
26 0.380528492775121
27 0.743246337646154
28 0.733183959737457
29 0.757703273177739
30 0.720397490859259
31 0.772837020703683
32 0.770726554161786
33 0.692801410931225
34 0.697967825213624
35 0.719690921178351
36 0.692369988575462
37 0.718238915815486
38 0.72814212165375
39 0.696483158043621
40 0.735545923510031
41 0.725835352637937
42 0.742039577565949
43 0.751213152590621
44 0.717468442612497
45 0.692606849765448
46 0.658917644855301
47 0.675709060325561
48 0.674710854122239
49 0.671185282681503
50 0.662903720021989
51 0.680654141242616
52 0.690857328355318
53 0.695205381858397
54 0.680243807137102
55 0.673063820625834
56 0.698466460515718
57 0.702173486167672
58 0.702844794978858
59 0.705662106875723
60 0.768956928666655
61 0.770120881620133
62 0.761995977118265
63 0.659147024267325
64 0.716776503782624
65 0.713824390149453
66 0.799905018366263
67 0.769733274347379
68 0.798745193801343
69 0.743846406319778
70 0.756815772843163
71 0.73578728196424
72 0.739346153367216
73 0.749079934186152
74 0.761076156158828
75 0.711129655391568
76 0.751017708023783
77 0.750548711057696
78 0.713288135602864
79 0.723260310356199
80 0.738505859480298
81 0.724979686975786
82 0.732669551878711
83 0.738020066493313
84 0.743840212628267
85 0.725251702122603
86 0.739616852921389
87 0.731429108036995
88 0.735828307755891
89 0.739506600933413
90 0.73489440013389
91 0.732594362452531
92 0.741075723379381
93 0.731264793257664
94 0.721511551912043
95 0.726665144543622
96 0.742103314017784
97 0.734340056385995
98 0.741571631524701
99 0.737744349767787
};
\plotInvscat
table {%
0 0.728237569332123
1 0.630641937255859
2 0.629461109638214
3 0.577544867992401
4 0.375148922204971
5 0.78435868024826
6 0.70535147190094
7 0.877840340137482
8 0.530405938625336
9 0.537621557712555
10 0.688578963279724
11 0.763240158557892
12 0.579296231269836
13 0.612863481044769
14 0.600334167480469
15 0.771778762340546
16 0.68986451625824
17 0.426485538482666
18 0.782626450061798
19 0.712275147438049
20 0.645944893360138
21 0.717006266117096
22 0.314870923757553
23 0.709199905395508
24 0.795690715312958
25 0.705492436885834
26 0.824418246746063
27 0.642326176166534
28 0.756206154823303
29 0.650830030441284
30 0.784879148006439
31 0.643692910671234
32 0.601231157779694
33 0.588945746421814
34 0.714015007019043
35 0.514716148376465
36 0.820708096027374
37 0.647423207759857
38 0.667258203029633
39 0.670579969882965
40 0.7122722864151
41 0.862009584903717
42 0.635596513748169
43 0.741009473800659
44 0.803696513175964
45 0.695409774780273
46 0.637110888957977
47 0.840144455432892
48 0.524664640426636
49 0.540545105934143
50 0.835602521896362
51 0.604630172252655
52 0.4866603910923
53 0.919659078121185
54 0.333785086870193
55 0.65137904882431
56 0.573119938373566
57 0.651283204555511
58 0.729602038860321
59 0.576328337192535
60 0.632863223552704
61 0.741091132164001
62 0.716103374958038
63 0.633393466472626
64 0.818655431270599
65 0.744399011135101
66 0.661736488342285
67 0.575340628623962
68 0.761913299560547
69 0.345318108797073
70 0.567408561706543
71 0.401173412799835
72 0.675870358943939
73 0.564943552017212
74 0.800659954547882
75 0.778183102607727
76 0.650036692619324
77 0.812907874584198
78 0.641543388366699
79 0.817378580570221
80 0.595073163509369
81 0.706800758838654
82 0.623124361038208
83 0.673567950725555
84 0.538588345050812
85 0.797978281974792
86 0.757101237773895
87 0.828388333320618
88 0.644318342208862
89 0.855063140392303
90 0.65866231918335
91 0.843858957290649
92 0.760265231132507
93 0.610323190689087
94 0.678544044494629
95 0.742800116539001
96 0.61644572019577
97 0.641060411930084
98 0.835386455059052
99 0.745161414146423
};
\end{groupplot}

==> Figs/random_phi_psi_change/noise_0.001.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm, group name=column2 plots,}]

\firstgplot{column1}{(b) $\sigma^2_{z}=0.001$}
\plotTrue
table {%
0 0.891181610926154
1 0.891181610926154
2 0.891181610926154
3 0.891181610926154
4 0.891181610926154
5 0.891181610926154
6 0.891181610926154
7 0.891181610926154
8 0.891181610926154
9 0.891181610926154
10 0.891181610926154
11 0.891181610926154
12 0.891181610926154
13 0.891181610926154
14 0.891181610926154
15 0.891181610926154
16 0.891181610926154
17 0.891181610926154
18 0.891181610926154
19 0.891181610926154
20 0.891181610926154
21 0.891181610926154
22 0.891181610926154
23 0.891181610926154
24 0.891181610926154
25 0.891181610926154
26 0.891181610926154
27 0.891181610926154
28 0.891181610926154
29 0.891181610926154
30 0.891181610926154
31 0.891181610926154
32 0.891181610926154
33 0.891181610926154
34 0.891181610926154
35 0.891181610926154
36 0.891181610926154
37 0.891181610926154
38 0.891181610926154
39 0.891181610926154
40 0.891181610926154
41 0.891181610926154
42 0.891181610926154
43 0.891181610926154
44 0.891181610926154
45 0.891181610926154
46 0.891181610926154
47 0.891181610926154
48 0.891181610926154
49 0.891181610926154
};

\plotNetwork
table {%
0 0.886020987282656
1 0.861775673797525
2 0.851010300811483
3 0.891248453110091
4 0.872866185519094
5 0.905419407475053
6 0.881457569726928
7 0.903580565803012
8 0.870222447900953
9 0.878829413493935
10 0.889312762247703
11 0.957471161868853
12 0.919336053957072
13 0.901930031615468
14 0.891107241531651
15 0.891247749207879
16 0.891169304715073
17 0.890453688136526
18 0.903376931876952
19 0.892682533471418
20 0.886580474057514
21 0.886027977876551
22 0.898611897756561
23 0.89105290651008
24 0.90157436417185
25 0.893224610453625
26 0.883696991329078
27 0.884155482711525
28 0.874380433584897
29 0.892388701134724
30 0.892749809077375
31 0.893014789154698
32 0.899916532810716
33 0.903956823749298
34 0.88955816045473
35 0.889714404843164
36 0.887903657172712
37 0.890629981527934
38 0.881802453538519
39 0.883012788664005
40 0.895324109202068
41 0.901378859148553
42 0.89498687121245
43 0.893663472231837
44 0.884181406515072
45 0.892233626797848
46 0.887451112471239
47 0.886550915628255
48 0.891871307455923
49 0.89235349590642
};

\plotInvscat
table {%
0 0.892493367195129
1 0.890091896057129
2 0.894009172916412
3 0.888365268707275
4 0.899050772190094
5 0.910716652870178
6 0.839045286178589
7 0.907890439033508
8 0.87809282541275
9 0.874687969684601
10 0.887063682079315
11 0.598102271556854
12 0.891690969467163
13 0.807609260082245
14 0.547406911849976
15 0.86795175075531
16 0.770195960998535
17 0.689260840415955
18 0.575443625450134
19 0.905777037143707
20 0.89705753326416
21 0.90256255865097
22 0.875231087207794
23 0.888391673564911
24 0.911759078502655
25 0.914415776729584
26 0.911666393280029
27 0.952084720134735
28 0.724086463451385
29 0.982415616512299
30 0.901866614818573
31 0.856114327907562
32 0.889350056648254
33 0.902489244937897
34 0.887379765510559
35 0.886911034584045
36 0.888893783092499
37 0.889907419681549
38 0.888859808444977
39 0.891112327575684
40 0.893143951892853
41 0.886816740036011
42 0.895675480365753
43 0.896046221256256
44 0.892433881759644
45 0.88530021905899
46 0.888595819473267
47 0.890091300010681
48 0.888519644737244
49 0.887397527694702
};

\nextgplot
\perturbation
\plotTrue
table {%
0 0.266381141862022
1 0.266381141862022
2 0.266381141862022
3 0.266381141862022
4 0.266381141862022
5 0.266381141862022
6 0.266381141862022
7 0.266381141862022
8 0.266381141862022
9 0.266381141862022
10 0.70133566926749
11 0.0689057085608183
12 0.305741099815992
13 0.139771199029424
14 0.130001698173358
15 0.39881817527929
16 0.375217448502849
17 0.109685257419572
18 0.288105114261699
19 0.481366388188413
20 0.436122721795109
21 0.535927573608293
22 0.714645038266339
23 0.725904646292618
24 0.438476767544669
25 0.348461233937566
26 0.671943876645627
27 0.330788110973136
28 0.246607899843114
29 0.202600091430629
30 0.506342110892236
31 0.286540499557685
32 0.369426861178431
33 0.267697585478029
34 0.684944979864667
35 0.793632875923133
36 0.793632875923133
37 0.793632875923133
38 0.793632875923133
39 0.793632875923133
40 0.793632875923133
41 0.793632875923133
42 0.793632875923133
43 0.793632875923133
44 0.793632875923133
45 0.793632875923133
46 0.793632875923133
47 0.793632875923133
48 0.793632875923133
49 0.793632875923133
};
\plotNetwork
table {%
0 0.282947853774518
1 0.270149981370353
2 0.290946817046207
3 0.264962555335108
4 0.278351408402075
5 0.249006753960698
6 0.262011765266523
7 0.266766346645716
8 0.263312594068529
9 0.297817149974201
10 0.707644523842629
11 0.0600989334611055
12 0.278600784562125
13 0.121655332342138
14 0.146435924896331
15 0.403503484560268
16 0.363447548768942
17 0.121625428458829
18 0.290783001410326
19 0.487848449697443
20 0.439523011075161
21 0.527240145079583
22 0.711017871359599
23 0.711784768472781
24 0.454121973814162
25 0.351548786403513
26 0.662054655025376
27 0.322136295017679
28 0.248185188123824
29 0.20473041905001
30 0.515034654961919
31 0.284350117152034
32 0.346143562580814
33 0.260714340883693
34 0.678252890220605
35 0.799790424354644
36 0.786150750528028
37 0.78668608350979
38 0.817621649226093
39 0.80113044275878
40 0.78987278841618
41 0.789379087471611
42 0.791978156317515
43 0.792070990555471
44 0.788734945291778
45 0.792593765726565
46 0.808993425965373
47 0.789639002300244
48 0.795218871131919
49 0.787057911695487
};
\plotInvscat
table {%
0 0.294901847839355
1 0.279331356287003
2 0.249064683914185
3 0.251769572496414
4 0.277735680341721
5 0.254016160964966
6 0.337256014347076
7 0.27000567317009
8 0.379356175661087
9 0.310123831033707
10 0.685520112514496
11 0.752162039279938
12 0.298313707113266
13 0.272096008062363
14 0.560544848442078
15 0.501676142215729
16 0.430548906326294
17 0.421915739774704
18 0.371600687503815
19 0.498160660266876
20 0.448290944099426
21 0.538275361061096
22 0.709836661815643
23 0.726547122001648
24 0.464447140693665
25 0.343156307935715
26 0.683208405971527
27 0.318596631288528
28 0.35353884100914
29 0.246528998017311
30 0.51977664232254
31 0.332266628742218
32 0.382052272558212
33 0.285106033086777
34 0.67469334602356
35 0.807987630367279
36 0.808454096317291
37 0.791381776332855
38 0.801604330539703
39 0.792512834072113
40 0.79212087392807
41 0.79774796962738
42 0.781333982944489
43 0.786200821399689
44 0.793665647506714
45 0.798293232917786
46 0.781517684459686
47 0.794269561767578
48 0.798485994338989
49 0.802693068981171
};

\nextgplot
\plotTrue
table {%
0 0.68575365760968
1 0.68575365760968
2 0.68575365760968
3 0.68575365760968
4 0.68575365760968
5 0.68575365760968
6 0.68575365760968
7 0.68575365760968
8 0.68575365760968
9 0.68575365760968
10 0.68575365760968
11 0.68575365760968
12 0.68575365760968
13 0.68575365760968
14 0.68575365760968
15 0.68575365760968
16 0.68575365760968
17 0.68575365760968
18 0.68575365760968
19 0.68575365760968
20 0.68575365760968
21 0.68575365760968
22 0.68575365760968
23 0.68575365760968
24 0.68575365760968
25 0.68575365760968
26 0.68575365760968
27 0.68575365760968
28 0.68575365760968
29 0.68575365760968
30 0.68575365760968
31 0.68575365760968
32 0.68575365760968
33 0.68575365760968
34 0.68575365760968
35 0.68575365760968
36 0.68575365760968
37 0.68575365760968
38 0.68575365760968
39 0.68575365760968
40 0.68575365760968
41 0.68575365760968
42 0.68575365760968
43 0.68575365760968
44 0.68575365760968
45 0.68575365760968
46 0.68575365760968
47 0.68575365760968
48 0.68575365760968
49 0.68575365760968
};
\plotNetwork
table {%
0 0.670783264926815
1 0.654922149533206
2 0.613756217156729
3 0.683025535371635
4 0.651409009265914
5 0.712987365879136
6 0.67083038441245
7 0.711291176535677
8 0.642842446739436
9 0.647814739125534
10 0.690999945582951
11 0.81495993577051
12 0.715714413881772
13 0.723042103052848
14 0.693923881621379
15 0.687127166315953
16 0.70981971446625
17 0.688579397474192
18 0.659728438759877
19 0.681255722263391
20 0.691659094972013
21 0.690398754859243
22 0.672199703665887
23 0.682499850787067
24 0.670479088253408
25 0.675016996468988
26 0.69780047426355
27 0.686830337252335
28 0.706217926620567
29 0.687839162706131
30 0.678543274939733
31 0.674382421956274
32 0.692184942550123
33 0.694557850074815
34 0.681674936472776
35 0.67821765846823
36 0.687023776081232
37 0.677053877712967
38 0.669917621561392
39 0.679375974624091
40 0.687668857157421
41 0.677713059584428
42 0.689264763287369
43 0.685816604168014
44 0.686593928222146
45 0.684519288598385
46 0.683485793600953
47 0.683777383919299
48 0.698688623796935
49 0.678055900014981
};
\plotInvscat
table {%
0 0.697387993335724
1 0.69445389509201
2 0.699541687965393
3 0.676884412765503
4 0.706483542919159
5 0.729066252708435
6 0.599660634994507
7 0.739850282669067
8 0.597362637519836
9 0.615197002887726
10 0.679181218147278
11 0.264425337314606
12 0.673892736434937
13 0.516703605651855
14 0.239287823438644
15 0.551353514194489
16 0.801426231861115
17 0.339632570743561
18 0.814925789833069
19 0.704588294029236
20 0.659119725227356
21 0.685078024864197
22 0.706478178501129
23 0.693314433097839
24 0.666705131530762
25 0.654932141304016
26 0.667496502399445
27 0.639511585235596
28 0.931450545787811
29 0.63539844751358
30 0.649385333061218
31 0.747471690177917
32 0.759641289710999
33 0.654036521911621
34 0.70077520608902
35 0.680185437202454
36 0.69149786233902
37 0.680803418159485
38 0.669059753417969
39 0.698154151439667
40 0.680322647094727
41 0.676187515258789
42 0.692692756652832
43 0.690469086170197
44 0.673956155776978
45 0.676445841789246
46 0.707278668880463
47 0.681823253631592
48 0.690565586090088
49 0.694410800933838
};

\nextgplot
\plotTrue
table {%
0 0.662800577692675
1 0.662800577692675
2 0.662800577692675
3 0.662800577692675
4 0.662800577692675
5 0.662800577692675
6 0.662800577692675
7 0.662800577692675
8 0.662800577692675
9 0.662800577692675
10 0.662800577692675
11 0.662800577692675
12 0.662800577692675
13 0.662800577692675
14 0.662800577692675
15 0.662800577692675
16 0.662800577692675
17 0.662800577692675
18 0.662800577692675
19 0.662800577692675
20 0.662800577692675
21 0.662800577692675
22 0.662800577692675
23 0.662800577692675
24 0.662800577692675
25 0.662800577692675
26 0.662800577692675
27 0.662800577692675
28 0.662800577692675
29 0.662800577692675
30 0.662800577692675
31 0.662800577692675
32 0.662800577692675
33 0.662800577692675
34 0.662800577692675
35 0.662800577692675
36 0.662800577692675
37 0.662800577692675
38 0.662800577692675
39 0.662800577692675
40 0.662800577692675
41 0.662800577692675
42 0.662800577692675
43 0.662800577692675
44 0.662800577692675
45 0.662800577692675
46 0.662800577692675
47 0.662800577692675
48 0.662800577692675
49 0.662800577692675
};
\plotNetwork
table {%
0 0.672946640414587
1 0.655046907675366
2 0.669746756284168
3 0.657017930171059
4 0.676299688754941
5 0.660355558827781
6 0.653968261894625
7 0.648443592130067
8 0.670956884533116
9 0.674629798058913
10 0.657467952638435
11 0.656952906992237
12 0.698818716268466
13 0.667450346654466
14 0.662858097080395
15 0.661485858253239
16 0.663361336381013
17 0.668398237777444
18 0.656465969511357
19 0.655585055154603
20 0.660355566739275
21 0.672541906812175
22 0.655650582137434
23 0.676428605098735
24 0.658207527893052
25 0.658289436584752
26 0.670910174695618
27 0.665796700480001
28 0.653024731030371
29 0.666601051039924
30 0.667721741052038
31 0.662554266628754
32 0.654188684153102
33 0.667331760779578
34 0.657995942923014
35 0.664120139179728
36 0.659432734218396
37 0.664156187974937
38 0.683210787188074
39 0.675295763468266
40 0.665769188499799
41 0.665931947195439
42 0.662428200910983
43 0.664391880335252
44 0.639344850232264
45 0.65777106909369
46 0.658545635528963
47 0.667954977377956
48 0.667032821167869
49 0.673977384042133
};
\plotInvscat
table {%
0 0.56430721282959
1 0.628885447978973
2 0.696508169174194
3 0.714684724807739
4 0.662046909332275
5 0.696447610855103
6 0.60845160484314
7 0.765723049640656
8 0.617867767810822
9 0.6985182762146
10 0.678350210189819
11 0.345506876707077
12 0.699675738811493
13 0.537183940410614
14 0.568214774131775
15 0.716832280158997
16 0.5872563123703
17 0.501925766468048
18 0.811918675899506
19 0.631904244422913
20 0.647124111652374
21 0.660429120063782
22 0.699114084243774
23 0.651063323020935
24 0.663261473178864
25 0.680958092212677
26 0.627551257610321
27 0.654915690422058
28 0.518973290920258
29 0.660851657390594
30 0.671842694282532
31 0.588495910167694
32 0.600041687488556
33 0.67605859041214
34 0.658212721347809
35 0.663216352462769
36 0.659514188766479
37 0.657218456268311
38 0.67029744386673
39 0.651236295700073
40 0.674983143806458
41 0.660926342010498
42 0.642088234424591
43 0.66244512796402
44 0.659516274929047
45 0.65320760011673
46 0.639342784881592
47 0.659736037254333
48 0.648861169815063
49 0.676078021526337
};
\lastgplot{5}
\plotTrue
table {%
0 0.594214027218682
1 0.594214027218682
2 0.594214027218682
3 0.594214027218682
4 0.594214027218682
5 0.594214027218682
6 0.594214027218682
7 0.594214027218682
8 0.594214027218682
9 0.594214027218682
10 0.594214027218682
11 0.594214027218682
12 0.594214027218682
13 0.594214027218682
14 0.594214027218682
15 0.594214027218682
16 0.594214027218682
17 0.594214027218682
18 0.594214027218682
19 0.594214027218682
20 0.594214027218682
21 0.594214027218682
22 0.594214027218682
23 0.594214027218682
24 0.594214027218682
25 0.594214027218682
26 0.594214027218682
27 0.594214027218682
28 0.594214027218682
29 0.594214027218682
30 0.594214027218682
31 0.594214027218682
32 0.594214027218682
33 0.594214027218682
34 0.594214027218682
35 0.594214027218682
36 0.594214027218682
37 0.594214027218682
38 0.594214027218682
39 0.594214027218682
40 0.594214027218682
41 0.594214027218682
42 0.594214027218682
43 0.594214027218682
44 0.594214027218682
45 0.594214027218682
46 0.594214027218682
47 0.594214027218682
48 0.594214027218682
49 0.594214027218682
};
\plotNetwork
table {%
0 0.597026415687789
1 0.58871102652807
2 0.611049250376141
3 0.597751806015077
4 0.608491674035851
5 0.583361061982725
6 0.596447097030303
7 0.57955442877245
8 0.593972067285072
9 0.614229465096985
10 0.594190843510988
11 0.590767800643875
12 0.612238008166226
13 0.572864847276702
14 0.602585297875824
15 0.591800793832704
16 0.58282865346818
17 0.601740665688057
18 0.587357169554761
19 0.58992569319407
20 0.595197457546151
21 0.595070302953176
22 0.591042559309313
23 0.596206625044418
24 0.618878075251926
25 0.58165388696753
26 0.594847087041584
27 0.596121966735369
28 0.586615766393662
29 0.591943908013467
30 0.595048388660519
31 0.615478261799554
32 0.578691233083803
33 0.59199324181872
34 0.593743729033229
35 0.610778151594013
36 0.588277027138798
37 0.590459823244031
38 0.609608971067725
39 0.596658926014527
40 0.579393863289936
41 0.594991095755528
42 0.589846874282563
43 0.586271695604265
44 0.583757065485232
45 0.599286859750893
46 0.622983203346119
47 0.588508569234205
48 0.592416844992675
49 0.588406603620226
};
\plotInvscat
table {%
0 0.653292417526245
1 0.631315767765045
2 0.559006035327911
3 0.546970427036285
4 0.619555294513702
5 0.573070645332336
6 0.685614824295044
7 0.463078588247299
8 0.71481317281723
9 0.637822151184082
10 0.568373501300812
11 0.596472680568695
12 0.618663787841797
13 0.63408499956131
14 0.607426702976227
15 0.661893129348755
16 0.575934886932373
17 0.662200927734375
18 0.610860705375671
19 0.570995450019836
20 0.610506653785706
21 0.624828398227692
22 0.621895432472229
23 0.577954888343811
24 0.632371366024017
25 0.660498142242432
26 0.605509161949158
27 0.651188910007477
28 0.64949107170105
29 0.658095300197601
30 0.641163766384125
31 0.65000718832016
32 0.653146326541901
33 0.61248791217804
34 0.565612614154816
35 0.62007611989975
36 0.600852906703949
37 0.585867524147034
38 0.603669285774231
39 0.616047441959381
40 0.583523571491241
41 0.597952425479889
42 0.583921134471893
43 0.599211573600769
44 0.619252979755402
45 0.608448803424835
46 0.582660436630249
47 0.602611899375916
48 0.600997030735016
49 0.59448915719986
};
\end{groupplot}

==> Figs/random_phi_psi_change/noise_0.01.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm,group name=column3 plots,}]
%====================== Fig1 =============
\firstgplot{column2}{(c) $\sigma^2_{z}=0.01$}
\plotTrue
table {%
0 0.891181610926154
1 0.891181610926154
2 0.891181610926154
3 0.891181610926154
4 0.891181610926154
5 0.891181610926154
6 0.891181610926154
7 0.891181610926154
8 0.891181610926154
9 0.891181610926154
10 0.891181610926154
11 0.891181610926154
12 0.891181610926154
13 0.891181610926154
14 0.891181610926154
15 0.891181610926154
16 0.891181610926154
17 0.891181610926154
18 0.891181610926154
19 0.891181610926154
20 0.891181610926154
21 0.891181610926154
22 0.891181610926154
23 0.891181610926154
24 0.891181610926154
25 0.891181610926154
26 0.891181610926154
27 0.891181610926154
28 0.891181610926154
29 0.891181610926154
30 0.891181610926154
31 0.891181610926154
32 0.891181610926154
33 0.891181610926154
34 0.891181610926154
35 0.891181610926154
36 0.891181610926154
37 0.891181610926154
38 0.891181610926154
39 0.891181610926154
40 0.891181610926154
41 0.891181610926154
42 0.891181610926154
43 0.891181610926154
44 0.891181610926154
45 0.891181610926154
46 0.891181610926154
47 0.891181610926154
48 0.891181610926154
49 0.891181610926154
};
\plotNetwork
table {%
0 0.941077968771569
1 0.875560074309461
2 0.89888259569822
3 0.83451712522635
4 0.919588362736822
5 0.747366403136604
6 0.954687884203056
7 0.906597757124432
8 0.805954861857325
9 0.809862096944607
10 0.878506111436396
11 0.984779750241058
12 0.841445159390787
13 0.94439906587733
14 0.92216825208135
15 0.866493135158677
16 0.842989581045593
17 0.5643502369411
18 0.749249712885715
19 0.896497837816866
20 0.868366320863564
21 0.906812956528323
22 0.896503938062792
23 0.889319656137754
24 0.907226207923335
25 0.867408830213606
26 0.903332131314612
27 0.867234178004127
28 0.892421945713955
29 0.876023616363128
30 0.863689513217297
31 0.948728662181502
32 0.890311362229522
33 0.938796966758338
34 0.89309477217774
35 0.872374697160291
36 0.870499991821255
37 0.891365568358305
38 0.902608173870712
39 0.881565739571861
40 0.887437394392182
41 0.886958411521009
42 0.897547571985495
43 0.868265706436046
44 0.892088892322904
45 0.911025061174113
46 0.902161960432077
47 0.867295406092326
48 0.878446405217021
49 0.904594618398521
};
\plotInvscat
table {%
0 0.827941238880157
1 0.956060767173767
2 0.955585122108459
3 0.891963481903076
4 0.922139406204224
5 0.85566908121109
6 0.797620892524719
7 0.856465101242065
8 0.924876630306244
9 0.851613938808441
10 0.910266995429993
11 0.653395354747772
12 0.798631012439728
13 0.713279783725739
14 0.679064571857452
15 0.780042707920074
16 0.822789311408997
17 0.768271327018738
18 0.996477842330933
19 0.969443798065186
20 0.959566712379456
21 0.962914347648621
22 0.893936991691589
23 0.882345199584961
24 0.970766842365265
25 0.912065744400024
26 0.931068062782288
27 0.935599029064178
28 0.813581585884094
29 0.701436102390289
30 0.94890034198761
31 0.978301823139191
32 0.986170172691345
33 0.881484568119049
34 0.911233186721802
35 0.877394378185272
36 0.879082322120667
37 0.911412417888641
38 0.881499886512756
39 0.917023062705994
40 0.884266436100006
41 0.881755948066711
42 0.885261237621307
43 0.878667533397675
44 0.902997732162476
45 0.908862054347992
46 0.883259892463684
47 0.897240340709686
48 0.907577097415924
49 0.865623295307159
};
%====================== Fig2 =============
\nextgplot
\perturbation
\plotTrue
table {%
0 0.266381141862022
1 0.266381141862022
2 0.266381141862022
3 0.266381141862022
4 0.266381141862022
5 0.266381141862022
6 0.266381141862022
7 0.266381141862022
8 0.266381141862022
9 0.266381141862022
10 0.70133566926749
11 0.0689057085608183
12 0.305741099815992
13 0.139771199029424
14 0.130001698173358
15 0.39881817527929
16 0.375217448502849
17 0.109685257419572
18 0.288105114261699
19 0.481366388188413
20 0.436122721795109
21 0.535927573608293
22 0.714645038266339
23 0.725904646292618
24 0.438476767544669
25 0.348461233937566
26 0.671943876645627
27 0.330788110973136
28 0.246607899843114
29 0.202600091430629
30 0.506342110892236
31 0.286540499557685
32 0.369426861178431
33 0.267697585478029
34 0.684944979864667
35 0.793632875923133
36 0.793632875923133
37 0.793632875923133
38 0.793632875923133
39 0.793632875923133
40 0.793632875923133
41 0.793632875923133
42 0.793632875923133
43 0.793632875923133
44 0.793632875923133
45 0.793632875923133
46 0.793632875923133
47 0.793632875923133
48 0.793632875923133
49 0.793632875923133
};
\plotNetwork
table {%
0 0.246902844441091
1 0.276856598324686
2 0.227258195870009
3 0.331328204865255
4 0.280305924540894
5 0.403831091555198
6 0.225425061302704
7 0.258359298717549
8 0.339861910509069
9 0.308311347620562
10 0.707959961407958
11 0.0370016075209062
12 0.301765011924486
13 0.0699211936836874
14 0.115442673554483
15 0.39803021476778
16 0.326105352472327
17 0.0496182219172312
18 0.277050111045823
19 0.473498163006148
20 0.436378286250236
21 0.560871523535427
22 0.698624531141423
23 0.735495204908273
24 0.449277935674814
25 0.351893581922997
26 0.690043398403546
27 0.329021618610874
28 0.268852985877183
29 0.214709837239942
30 0.508491616242175
31 0.290198474660266
32 0.364078565463326
33 0.31669088013847
34 0.682787520249055
35 0.776965354654525
36 0.804011558567752
37 0.791026994477518
38 0.819235023066048
39 0.794053149813251
40 0.780156796026748
41 0.794370943507209
42 0.787591834492147
43 0.816407434662428
44 0.794663001631125
45 0.769934583177368
46 0.786677170748772
47 0.793567887444938
48 0.796024421670321
49 0.743082993478422
};
\plotInvscat
table {%
0 0.416965931653976
1 0.256150543689728
2 0.329775780439377
3 0.457944571971893
4 0.23215040564537
5 0.315767467021942
6 0.481976270675659
7 0.43449592590332
8 0.500313460826874
9 0.348755538463593
10 0.694142580032349
11 0.469220638275146
12 0.300277382135391
13 0.849798917770386
14 0.420890033245087
15 0.652893483638763
16 0.425112366676331
17 0.91121107339859
18 0.667425334453583
19 0.682990193367004
20 0.606118679046631
21 0.581138432025909
22 0.722803950309753
23 0.688243329524994
24 0.559862077236176
25 0.629832684993744
26 0.7491055727005
27 0.58952271938324
28 0.531517028808594
29 0.41904890537262
30 0.503422319889069
31 0.440147191286087
32 0.438002228736877
33 0.367599785327911
34 0.718729615211487
35 0.852544188499451
36 0.819138944149017
37 0.782124161720276
38 0.81081622838974
39 0.771888673305511
40 0.838570654392242
41 0.839976906776428
42 0.835652947425842
43 0.791299521923065
44 0.742790877819061
45 0.818522930145264
46 0.801367461681366
47 0.73605489730835
48 0.793045520782471
49 0.810285091400146
};
%====================== Fig3 =============
\nextgplot
\plotTrue
table {%
0 0.68575365760968
1 0.68575365760968
2 0.68575365760968
3 0.68575365760968
4 0.68575365760968
5 0.68575365760968
6 0.68575365760968
7 0.68575365760968
8 0.68575365760968
9 0.68575365760968
10 0.68575365760968
11 0.68575365760968
12 0.68575365760968
13 0.68575365760968
14 0.68575365760968
15 0.68575365760968
16 0.68575365760968
17 0.68575365760968
18 0.68575365760968
19 0.68575365760968
20 0.68575365760968
21 0.68575365760968
22 0.68575365760968
23 0.68575365760968
24 0.68575365760968
25 0.68575365760968
26 0.68575365760968
27 0.68575365760968
28 0.68575365760968
29 0.68575365760968
30 0.68575365760968
31 0.68575365760968
32 0.68575365760968
33 0.68575365760968
34 0.68575365760968
35 0.68575365760968
36 0.68575365760968
37 0.68575365760968
38 0.68575365760968
39 0.68575365760968
40 0.68575365760968
41 0.68575365760968
42 0.68575365760968
43 0.68575365760968
44 0.68575365760968
45 0.68575365760968
46 0.68575365760968
47 0.68575365760968
48 0.68575365760968
49 0.68575365760968
};
\plotNetwork
table {%
0 0.750707393504917
1 0.658599355289296
2 0.682139553231811
3 0.605474921766775
4 0.732945773455658
5 0.477671854407918
6 0.800297156497596
7 0.718317831353677
8 0.547956993197496
9 0.745024480266963
10 0.690804925294206
11 0.852788542193966
12 0.60747271215223
13 0.802517688982874
14 0.846436753253094
15 0.710348637848145
16 0.785472251398091
17 0.884956467746676
18 0.835233036047495
19 0.672973525227345
20 0.740182640879376
21 0.709137999941077
22 0.673275795918317
23 0.683528990077684
24 0.688509510352433
25 0.728741452116404
26 0.695742185708024
27 0.679798484787428
28 0.690952291517044
29 0.656096113506051
30 0.700270143486404
31 0.586364551175584
32 0.674766885837765
33 0.663930714242296
34 0.708890066219991
35 0.714556379266249
36 0.704150222899934
37 0.691049421836425
38 0.664695954654317
39 0.723289210679354
40 0.714755651886556
41 0.698439630851123
42 0.656820818538657
43 0.662336419273569
44 0.694585510599644
45 0.735437408456349
46 0.68288935817508
47 0.683721420225849
48 0.661762201339511
49 0.696169587813558
};
\plotInvscat
table {%
0 0.576645076274872
1 0.80124044418335
2 0.7432821393013
3 0.641641497612
4 0.793412387371063
5 0.692600131034851
6 0.508836209774017
7 0.582373321056366
8 0.497324645519257
9 0.729221761226654
10 0.641190648078918
11 0.640490531921387
12 0.47873717546463
13 0.432170957326889
14 0.790039896965027
15 0.539990484714508
16 0.838492333889008
17 0.18120664358139
18 0.778275907039642
19 0.648932635784149
20 0.610377848148346
21 0.635406017303467
22 0.694257915019989
23 0.633856654167175
24 0.593020915985107
25 0.336172074079514
26 0.747780561447144
27 0.61312609910965
28 0.781650602817535
29 0.88609766960144
30 0.660453677177429
31 0.425324380397797
32 0.55608081817627
33 0.889818787574768
34 0.720265567302704
35 0.648126542568207
36 0.681443870067596
37 0.700594425201416
38 0.674192786216736
39 0.730465590953827
40 0.694205403327942
41 0.664627432823181
42 0.691100895404816
43 0.656435191631317
44 0.718786895275116
45 0.651172339916229
46 0.716186761856079
47 0.735807716846466
48 0.720179855823517
49 0.706526160240173
};
%====================== Fig4 =============
\nextgplot
\plotTrue
table {%
0 0.662800577692675
1 0.662800577692675
2 0.662800577692675
3 0.662800577692675
4 0.662800577692675
5 0.662800577692675
6 0.662800577692675
7 0.662800577692675
8 0.662800577692675
9 0.662800577692675
10 0.662800577692675
11 0.662800577692675
12 0.662800577692675
13 0.662800577692675
14 0.662800577692675
15 0.662800577692675
16 0.662800577692675
17 0.662800577692675
18 0.662800577692675
19 0.662800577692675
20 0.662800577692675
21 0.662800577692675
22 0.662800577692675
23 0.662800577692675
24 0.662800577692675
25 0.662800577692675
26 0.662800577692675
27 0.662800577692675
28 0.662800577692675
29 0.662800577692675
30 0.662800577692675
31 0.662800577692675
32 0.662800577692675
33 0.662800577692675
34 0.662800577692675
35 0.662800577692675
36 0.662800577692675
37 0.662800577692675
38 0.662800577692675
39 0.662800577692675
40 0.662800577692675
41 0.662800577692675
42 0.662800577692675
43 0.662800577692675
44 0.662800577692675
45 0.662800577692675
46 0.662800577692675
47 0.662800577692675
48 0.662800577692675
49 0.662800577692675
};
\plotNetwork
table {%
0 0.666572618263069
1 0.691124398739898
2 0.66556420017323
3 0.667857390138319
4 0.648924165747489
5 0.668513320290088
6 0.651177269059381
7 0.711539176994916
8 0.698361126272436
9 0.556283415158162
10 0.63020869081892
11 0.653776638349269
12 0.665687765457653
13 0.668956104097962
14 0.65875561252156
15 0.627894411921656
16 0.631904356573543
17 0.621244125359135
18 0.718935126899376
19 0.656928528633917
20 0.719783927246659
21 0.648158160449362
22 0.659383126078906
23 0.652001705446968
24 0.650753881810054
25 0.650608103227846
26 0.631562542443217
27 0.665273881479869
28 0.650997477888222
29 0.683029795232581
30 0.674838981001198
31 0.686555804246442
32 0.660888612286486
33 0.712669508733316
34 0.69683112386136
35 0.660859485146568
36 0.610036121725657
37 0.658113279837461
38 0.673500760254293
39 0.633232631373365
40 0.62971126206177
41 0.672368428685671
42 0.658274005658812
43 0.651987279983334
44 0.662125110363318
45 0.643598494458695
46 0.672501549772014
47 0.669004307510896
48 0.676294588227671
49 0.654424061317362
};
\plotInvscat
table {%
0 0.6119664311409
1 0.725099325180054
2 0.619466662406921
3 0.556200861930847
4 0.690243601799011
5 0.616193175315857
6 0.772627532482147
7 0.596912920475006
8 0.639801681041718
9 0.589319288730621
10 0.679517149925232
11 0.553129434585571
12 0.797553420066833
13 0.419829577207565
14 0.446621268987656
15 0.710798740386963
16 0.591809153556824
17 0.576015532016754
18 0.242812439799309
19 0.46281760931015
20 0.449656754732132
21 0.703380823135376
22 0.634966909885406
23 0.712936758995056
24 0.490382939577103
25 0.817283093929291
26 0.605734288692474
27 0.421762824058533
28 0.376110434532166
29 0.456565320491791
30 0.715524733066559
31 0.82475346326828
32 0.760055780410767
33 0.502809524536133
34 0.652250051498413
35 0.656056880950928
36 0.681213021278381
37 0.72844922542572
38 0.650696992874146
39 0.636909067630768
40 0.661530315876007
41 0.662410259246826
42 0.653362631797791
43 0.663370966911316
44 0.651733636856079
45 0.703756988048553
46 0.663052022457123
47 0.62336939573288
48 0.689302921295166
49 0.683644473552704
};
%====================== Fig5 =============
\lastgplot{5}
\plotTrue
table {%
0 0.594214027218682
1 0.594214027218682
2 0.594214027218682
3 0.594214027218682
4 0.594214027218682
5 0.594214027218682
6 0.594214027218682
7 0.594214027218682
8 0.594214027218682
9 0.594214027218682
10 0.594214027218682
11 0.594214027218682
12 0.594214027218682
13 0.594214027218682
14 0.594214027218682
15 0.594214027218682
16 0.594214027218682
17 0.594214027218682
18 0.594214027218682
19 0.594214027218682
20 0.594214027218682
21 0.594214027218682
22 0.594214027218682
23 0.594214027218682
24 0.594214027218682
25 0.594214027218682
26 0.594214027218682
27 0.594214027218682
28 0.594214027218682
29 0.594214027218682
30 0.594214027218682
31 0.594214027218682
32 0.594214027218682
33 0.594214027218682
34 0.594214027218682
35 0.594214027218682
36 0.594214027218682
37 0.594214027218682
38 0.594214027218682
39 0.594214027218682
40 0.594214027218682
41 0.594214027218682
42 0.594214027218682
43 0.594214027218682
44 0.594214027218682
45 0.594214027218682
46 0.594214027218682
47 0.594214027218682
48 0.594214027218682
49 0.594214027218682
};
\plotNetwork
table {%
0 0.573531640348036
1 0.587365463381265
2 0.597620955239772
3 0.659772699903691
4 0.618925402715506
5 0.618693628909929
6 0.584312332609036
7 0.598665262825689
8 0.619594946682871
9 0.612436319748698
10 0.620916736380449
11 0.579855902862186
12 0.623136537236316
13 0.574522652277895
14 0.560337204616422
15 0.611519589707181
16 0.584302467790777
17 0.586191635859389
18 0.610236612943211
19 0.594559436894654
20 0.574000941898774
21 0.592425984875284
22 0.598576163639249
23 0.637060620768172
24 0.619480790307925
25 0.534757392723639
26 0.624508026448691
27 0.583575599728638
28 0.569648910698404
29 0.608905318125337
30 0.587960661893468
31 0.568084449636003
32 0.609862961257828
33 0.64210765461339
34 0.556005026342646
35 0.587489502239884
36 0.640833317887239
37 0.620465589644336
38 0.629597860639385
39 0.639586036944517
40 0.622616706794918
41 0.608939613959425
42 0.603537514810594
43 0.631325792472514
44 0.597965405956917
45 0.560279924260759
46 0.547363927924878
47 0.579142152270684
48 0.600020303929727
49 0.580635289307991
};
\plotInvscat
table {%
0 0.700943648815155
1 0.600218117237091
2 0.739484846591949
3 0.780907332897186
4 0.466233432292938
5 0.66165953874588
6 0.690365254878998
7 0.769462645053864
8 0.89657074213028
9 0.715201079845428
10 0.626250505447388
11 0.718567430973053
12 0.67469584941864
13 0.889686286449432
14 0.550570607185364
15 0.775653421878815
16 0.59381902217865
17 0.611866354942322
18 0.554842233657837
19 0.627653896808624
20 0.693334102630615
21 0.70300418138504
22 0.555213212966919
23 0.693438827991486
24 0.598812162876129
25 0.610471963882446
26 0.634159207344055
27 0.499233245849609
28 0.849794149398804
29 0.604126274585724
30 0.588565766811371
31 0.625892162322998
32 0.626250445842743
33 0.721584916114807
34 0.652768075466156
35 0.689828813076019
36 0.596268773078918
37 0.543310284614563
38 0.656167924404144
39 0.630765974521637
40 0.637391269207001
41 0.660245060920715
42 0.66905277967453
43 0.61977881193161
44 0.53205007314682
45 0.659293234348297
46 0.623067438602448
47 0.521486878395081
48 0.56537938117981
49 0.53992748260498
};
\coordinate (split) at (rel axis cs:1.035,-1);
\end{groupplot}

==> Figs/random_phi_psi_change/noise_free.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm, x descriptions at=edge bottom, group name=column1 plots,}]

\nextgroupplot[
width=\w cm,
height=\h cm,
legend cell align={left},
legend style={at={(0.8,1.85)}, anchor=north west, legend cell align=left, align=left, font=\footnotesize, draw=white!15!black},
legend columns=3,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=\xmin, xmax=\xmax,
xtick style={color=black,font=\footnotesize},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_0(t)|\)},
title = {(a) Noise-free $(\sigma^2_{z}=0)$},
title style ={color=black,font=\footnotesize, yshift=-0.2cm},
ymin=0, ymax=1.2,
ytick style={color=black,font=\footnotesize},
%-------- Horizantal ----
%xtick style={color=black,font=\footnotesize},
%xlabel = {time \(t\)},
%title={\(\displaystyle |\cos\phi_1(t)|\)},
%-------- Vertical ----
xtick style={color=white,font=\footnotesize},
xticklabels ={},
%xlabel = {time \(t\)},
ylabel={\(\displaystyle |\cos\phi_1(k)|\)},
% xtick style={color=white},
% xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}


\plotTrue
table {%
0 0.891181610926154
1 0.891181610926154
2 0.891181610926154
3 0.891181610926154
4 0.891181610926154
5 0.891181610926154
6 0.891181610926154
7 0.891181610926154
8 0.891181610926154
9 0.891181610926154
10 0.891181610926154
11 0.891181610926154
12 0.891181610926154
13 0.891181610926154
14 0.891181610926154
15 0.891181610926154
16 0.891181610926154
17 0.891181610926154
18 0.891181610926154
19 0.891181610926154
20 0.891181610926154
21 0.891181610926154
22 0.891181610926154
23 0.891181610926154
24 0.891181610926154
25 0.891181610926154
26 0.891181610926154
27 0.891181610926154
28 0.891181610926154
29 0.891181610926154
30 0.891181610926154
31 0.891181610926154
32 0.891181610926154
33 0.891181610926154
34 0.891181610926154
35 0.891181610926154
36 0.891181610926154
37 0.891181610926154
38 0.891181610926154
39 0.891181610926154
40 0.891181610926154
41 0.891181610926154
42 0.891181610926154
43 0.891181610926154
44 0.891181610926154
45 0.891181610926154
46 0.891181610926154
47 0.891181610926154
48 0.891181610926154
49 0.891181610926154
};
\addlegendentry{True}
\plotNetwork
table {%
0 0.891181610924818
1 0.891181610926154
2 0.891181610926154
3 0.891181610926154
4 0.891181610926154
5 0.891170391416761
6 0.891181610928637
7 0.891181622403209
8 0.893390654201436
9 0.891287200483602
10 0.891181610856789
11 0.892748035484884
12 0.891189370071483
13 0.891999327367509
14 0.893573733403073
15 0.891181610968623
16 0.891181610926709
17 0.895366858080287
18 0.889887191165648
19 0.891135281563751
20 0.89065112034655
21 0.891155499155449
22 0.89118161137536
23 0.891181610924494
24 0.891189174784466
25 0.891116017513972
26 0.891181610954018
27 0.890959293068161
28 0.891181610972867
29 0.891210746708234
30 0.891181610962604
31 0.891181265896779
32 0.891181610987876
33 0.89118161089059
34 0.891181610891376
35 0.891181610929399
36 0.891181610926153
37 0.891181610926154
38 0.891181610926154
39 0.891181610926153
40 0.891181610926154
41 0.891181610926171
42 0.891181610866125
43 0.89118375467729
44 0.891181174230223
45 0.891179467361321
46 0.89118138137371
47 0.891185980291658
48 0.891238556463789
49 0.891094024325531
};
\addlegendentry{Learning Approach}
\plotInvscat
table {%
0 0.891181647777557
1 0.891181647777557
2 0.891181647777557
3 0.891181647777557
4 0.891181647777557
5 0.891181647777557
6 0.891181647777557
7 0.891181647777557
8 0.891181647777557
9 0.891181647777557
10 0.891181647777557
11 0.891178488731384
12 0.891181528568268
13 0.891181290149689
14 0.891181111335754
15 0.891181588172913
16 0.891181588172913
17 0.891180157661438
18 0.891181766986847
19 0.891181647777557
20 0.891181647777557
21 0.891181647777557
22 0.891181647777557
23 0.891181647777557
24 0.891181647777557
25 0.891181707382202
26 0.891181647777557
27 0.891181766986847
28 0.891181409358978
29 0.891181588172913
30 0.891181588172913
31 0.891181468963623
32 0.891181588172913
33 0.891181588172913
34 0.891181647777557
35 0.891181647777557
36 0.891181647777557
37 0.891181647777557
38 0.891181647777557
39 0.891181647777557
40 0.891181647777557
41 0.891181647777557
42 0.891181647777557
43 0.891181647777557
44 0.891181647777557
45 0.891181647777557
46 0.891181647777557
47 0.891181647777557
48 0.891181647777557
49 0.891181647777557
};
\addlegendentry{Inverse Scattering Algorithm (ISA)\cite{noe_polarization-dependent_2015}}
%==================================== Fig 2 ==============================
\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=\xmin, xmax=\xmax,
y grid style={darkgray176},
ylabel={\(\displaystyle |\cos\phi_2(k)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
xtick style={color=white},
xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\perturbation

\plotTrue
table {%
0 0.266381141862022
1 0.266381141862022
2 0.266381141862022
3 0.266381141862022
4 0.266381141862022
5 0.266381141862022
6 0.266381141862022
7 0.266381141862022
8 0.266381141862022
9 0.266381141862022
10 0.70133566926749
11 0.0689057085608183
12 0.305741099815992
13 0.139771199029424
14 0.130001698173358
15 0.39881817527929
16 0.375217448502849
17 0.109685257419572
18 0.288105114261699
19 0.481366388188413
20 0.436122721795109
21 0.535927573608293
22 0.714645038266339
23 0.725904646292618
24 0.438476767544669
25 0.348461233937566
26 0.671943876645627
27 0.330788110973136
28 0.246607899843114
29 0.202600091430629
30 0.506342110892236
31 0.286540499557685
32 0.369426861178431
33 0.267697585478029
34 0.684944979864667
35 0.793632875923133
36 0.793632875923133
37 0.793632875923133
38 0.793632875923133
39 0.793632875923133
40 0.793632875923133
41 0.793632875923133
42 0.793632875923133
43 0.793632875923133
44 0.793632875923133
45 0.793632875923133
46 0.793632875923133
47 0.793632875923133
48 0.793632875923133
49 0.793632875923133
};
\plotNetwork
table {%
0 0.266381141863534
1 0.266381141862022
2 0.266381141862022
3 0.266381141862022
4 0.266381141862022
5 0.266360869156278
6 0.266381141856452
7 0.266381155507616
8 0.265424139331283
9 0.263764323104163
10 0.701335669140419
11 0.0556793065082198
12 0.30573020905325
13 0.140060868982923
14 0.130384048980283
15 0.398818175407074
16 0.375217448492954
17 0.110661999282286
18 0.284420085365285
19 0.481238588951618
20 0.435868418595937
21 0.535930726512882
22 0.714645038636747
23 0.725904646290997
24 0.438485700039119
25 0.3484207776814
26 0.671943876579488
27 0.330756598410486
28 0.246607900124175
29 0.202642112208608
30 0.506342110906961
31 0.286539577558223
32 0.369426861181135
33 0.267697585349728
34 0.684944979895284
35 0.793632875922802
36 0.793632875923133
37 0.793632875923133
38 0.793632875923133
39 0.793632875923133
40 0.793632875923133
41 0.793632875923131
42 0.793632875932269
43 0.793632644251377
44 0.793633789743973
45 0.793632832748695
46 0.793632476579119
47 0.793622077592515
48 0.793562411190865
49 0.79344497654406
};
\plotInvscat
table {%
0 0.266381144523621
1 0.266381144523621
2 0.266381144523621
3 0.266381144523621
4 0.266381144523621
5 0.266381144523621
6 0.266381144523621
7 0.266381144523621
8 0.266381144523621
9 0.266381144523621
10 0.701335668563843
11 0.0689060688018799
12 0.305741220712662
13 0.139771074056625
14 0.130002170801163
15 0.398818284273148
16 0.37521755695343
17 0.109685964882374
18 0.288105100393295
19 0.481366395950317
20 0.436122715473175
21 0.535927593708038
22 0.714645028114319
23 0.725904643535614
24 0.438476771116257
25 0.348461359739304
26 0.67194390296936
27 0.330788344144821
28 0.246607780456543
29 0.202599972486496
30 0.506342113018036
31 0.286540508270264
32 0.369426846504211
33 0.267697483301163
34 0.684944987297058
35 0.793632864952087
36 0.793632864952087
37 0.793632864952087
38 0.793632864952087
39 0.793632864952087
40 0.793632864952087
41 0.793632864952087
42 0.793632864952087
43 0.793632864952087
44 0.793632864952087
45 0.793632864952087
46 0.793632864952087
47 0.793632864952087
48 0.793632864952087
49 0.793632864952087
};


%=========================== Fig 3 ====================
\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=\xmin, xmax=\xmax,
y grid style={darkgray176},
ylabel={\(\displaystyle |\cos\phi_3(k)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
xtick style={color=white},
xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\trueLineWidth pt, dotted]
table {%
0 0.68575365760968
1 0.68575365760968
2 0.68575365760968
3 0.68575365760968
4 0.68575365760968
5 0.68575365760968
6 0.68575365760968
7 0.68575365760968
8 0.68575365760968
9 0.68575365760968
10 0.68575365760968
11 0.68575365760968
12 0.68575365760968
13 0.68575365760968
14 0.68575365760968
15 0.68575365760968
16 0.68575365760968
17 0.68575365760968
18 0.68575365760968
19 0.68575365760968
20 0.68575365760968
21 0.68575365760968
22 0.68575365760968
23 0.68575365760968
24 0.68575365760968
25 0.68575365760968
26 0.68575365760968
27 0.68575365760968
28 0.68575365760968
29 0.68575365760968
30 0.68575365760968
31 0.68575365760968
32 0.68575365760968
33 0.68575365760968
34 0.68575365760968
35 0.68575365760968
36 0.68575365760968
37 0.68575365760968
38 0.68575365760968
39 0.68575365760968
40 0.68575365760968
41 0.68575365760968
42 0.68575365760968
43 0.68575365760968
44 0.68575365760968
45 0.68575365760968
46 0.68575365760968
47 0.68575365760968
48 0.68575365760968
49 0.68575365760968
};
\plotNetwork
table {%
0 0.685753657605287
1 0.68575365760968
2 0.68575365760968
3 0.68575365760968
4 0.68575365760968
5 0.685760379353679
6 0.685753657617271
7 0.685753670692705
8 0.684597591549971
9 0.686320918650368
10 0.685753657517112
11 0.688845194663562
12 0.685784173874392
13 0.684896749545888
14 0.683909193897632
15 0.685753657373037
16 0.685753657612702
17 0.681190249669241
18 0.690348174661875
19 0.685849473513525
20 0.685845908885882
21 0.685745757814845
22 0.685753657367205
23 0.685753657607228
24 0.685747410024799
25 0.68578239653311
26 0.685753657485446
27 0.685727847693147
28 0.685753656914469
29 0.68562080502278
30 0.68575365761352
31 0.685755189879114
32 0.685753657585737
33 0.68575365783072
34 0.685753657529638
35 0.685753657579821
36 0.68575365760968
37 0.68575365760968
38 0.68575365760968
39 0.68575365760968
40 0.68575365760968
41 0.68575365760967
42 0.685753657755232
43 0.685746505257586
44 0.685755680986646
45 0.685762428785528
46 0.685753503583965
47 0.685756497135085
48 0.685810430563854
49 0.684440173033644
};
\plotInvscat
table {%
0 0.685753583908081
1 0.685753583908081
2 0.685753583908081
3 0.685753583908081
4 0.685753583908081
5 0.685753583908081
6 0.685753583908081
7 0.685753583908081
8 0.685753583908081
9 0.685753583908081
10 0.685753643512726
11 0.685752272605896
12 0.685753643512726
13 0.685754060745239
14 0.685751557350159
15 0.685753583908081
16 0.685753583908081
17 0.685750544071198
18 0.685753643512726
19 0.685753643512726
20 0.685753583908081
21 0.685753643512726
22 0.685753643512726
23 0.685753643512726
24 0.685753643512726
25 0.685753464698792
26 0.685753643512726
27 0.685753345489502
28 0.685754299163818
29 0.685754239559174
30 0.685753703117371
31 0.68575394153595
32 0.685753762722015
33 0.685754060745239
34 0.685753643512726
35 0.685753643512726
36 0.685753643512726
37 0.685753643512726
38 0.685753643512726
39 0.685753643512726
40 0.685753643512726
41 0.685753643512726
42 0.685753643512726
43 0.685753643512726
44 0.685753643512726
45 0.685753643512726
46 0.685753643512726
47 0.685753643512726
48 0.685753643512726
49 0.685753643512726
};
%=============================== Fig 4 =========================
\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=\xmin, xmax=\xmax,
y grid style={darkgray176},
ylabel={\(\displaystyle |\cos\phi_4(k)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
xtick style={color=white},
xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\trueLineWidth pt, dotted]
table {%
0 0.662800577692675
1 0.662800577692675
2 0.662800577692675
3 0.662800577692675
4 0.662800577692675
5 0.662800577692675
6 0.662800577692675
7 0.662800577692675
8 0.662800577692675
9 0.662800577692675
10 0.662800577692675
11 0.662800577692675
12 0.662800577692675
13 0.662800577692675
14 0.662800577692675
15 0.662800577692675
16 0.662800577692675
17 0.662800577692675
18 0.662800577692675
19 0.662800577692675
20 0.662800577692675
21 0.662800577692675
22 0.662800577692675
23 0.662800577692675
24 0.662800577692675
25 0.662800577692675
26 0.662800577692675
27 0.662800577692675
28 0.662800577692675
29 0.662800577692675
30 0.662800577692675
31 0.662800577692675
32 0.662800577692675
33 0.662800577692675
34 0.662800577692675
35 0.662800577692675
36 0.662800577692675
37 0.662800577692675
38 0.662800577692675
39 0.662800577692675
40 0.662800577692675
41 0.662800577692675
42 0.662800577692675
43 0.662800577692675
44 0.662800577692675
45 0.662800577692675
46 0.662800577692675
47 0.662800577692675
48 0.662800577692675
49 0.662800577692675
};
\plotNetwork
table {%
0 0.662800577695823
1 0.662800577692675
2 0.662800577692675
3 0.662800577692674
4 0.662800577692675
5 0.662787872667053
6 0.662800577688412
7 0.662800542609303
8 0.666072903979201
9 0.66346263527378
10 0.662800577668066
11 0.660786952068487
12 0.662774177862563
13 0.66202462698295
14 0.664026019932092
15 0.662800577684533
16 0.662800577688738
17 0.664131253615585
18 0.663808555214181
19 0.662824870007985
20 0.662959152617369
21 0.662802590923258
22 0.662800577896791
23 0.6628005776991
24 0.662797597374798
25 0.662824720105514
26 0.662800577795307
27 0.662866393478008
28 0.662800577942884
29 0.66285586371668
30 0.662800577629224
31 0.662799783383198
32 0.662800577689873
33 0.662800577610432
34 0.662800577561667
35 0.662800577714321
36 0.662800577692675
37 0.662800577692675
38 0.662800577692675
39 0.662800577692675
40 0.662800577692675
41 0.662800577692674
42 0.662800577706134
43 0.662800908628081
44 0.662799901329935
45 0.662797325429817
46 0.66280213346422
47 0.662814922853316
48 0.662839986674855
49 0.664615249087021
};
\plotInvscat
table {%
0 0.662800490856171
1 0.662800490856171
2 0.662800490856171
3 0.662800490856171
4 0.662800490856171
5 0.662800490856171
6 0.662800490856171
7 0.662800490856171
8 0.662800490856171
9 0.662800490856171
10 0.662800550460815
11 0.66280072927475
12 0.662800550460815
13 0.66280072927475
14 0.662800908088684
15 0.662800550460815
16 0.662800550460815
17 0.66280072927475
18 0.662800490856171
19 0.662800550460815
20 0.662800490856171
21 0.662800490856171
22 0.662800550460815
23 0.662800550460815
24 0.662800490856171
25 0.662800431251526
26 0.662800550460815
27 0.662800371646881
28 0.662800371646881
29 0.662800192832947
30 0.662800550460815
31 0.662800431251526
32 0.662800490856171
33 0.662800371646881
34 0.662800550460815
35 0.662800550460815
36 0.662800550460815
37 0.662800550460815
38 0.662800550460815
39 0.662800550460815
40 0.662800550460815
41 0.662800550460815
42 0.662800550460815
43 0.662800550460815
44 0.662800550460815
45 0.662800550460815
46 0.662800550460815
47 0.662800550460815
48 0.662800550460815
49 0.662800550460815
};

%====================== Fig 5 ==================
\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=\xmin, xmax=\xmax,
y grid style={darkgray176},
ylabel={\(\displaystyle |\cos\phi_5(k)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
xlabel = {time step \(k\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%xtick style={color=white},
%xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\trueLineWidth pt, dotted]
table {%
0 0.594214027218682
1 0.594214027218682
2 0.594214027218682
3 0.594214027218682
4 0.594214027218682
5 0.594214027218682
6 0.594214027218682
7 0.594214027218682
8 0.594214027218682
9 0.594214027218682
10 0.594214027218682
11 0.594214027218682
12 0.594214027218682
13 0.594214027218682
14 0.594214027218682
15 0.594214027218682
16 0.594214027218682
17 0.594214027218682
18 0.594214027218682
19 0.594214027218682
20 0.594214027218682
21 0.594214027218682
22 0.594214027218682
23 0.594214027218682
24 0.594214027218682
25 0.594214027218682
26 0.594214027218682
27 0.594214027218682
28 0.594214027218682
29 0.594214027218682
30 0.594214027218682
31 0.594214027218682
32 0.594214027218682
33 0.594214027218682
34 0.594214027218682
35 0.594214027218682
36 0.594214027218682
37 0.594214027218682
38 0.594214027218682
39 0.594214027218682
40 0.594214027218682
41 0.594214027218682
42 0.594214027218682
43 0.594214027218682
44 0.594214027218682
45 0.594214027218682
46 0.594214027218682
47 0.594214027218682
48 0.594214027218682
49 0.594214027218682
};
\plotNetwork
table {%
0 0.594214027219341
1 0.594214027218682
2 0.594214027218682
3 0.594214027218682
4 0.594214027218682
5 0.594334353145828
6 0.594214027226692
7 0.594214004736788
8 0.593087909277778
9 0.596501036200318
10 0.594214027124104
11 0.585682916779743
12 0.594213840425748
13 0.594182187415192
14 0.594610191140828
15 0.594214027232305
16 0.594214027215452
17 0.59459886707511
18 0.591787247326722
19 0.594048320998135
20 0.593497012028619
21 0.594164239026874
22 0.594214029843438
23 0.594214027232719
24 0.594227712992769
25 0.59415818827004
26 0.594214027316609
27 0.594078969435945
28 0.59421402721439
29 0.594222440386049
30 0.594214027366906
31 0.594213673998198
32 0.594214027195033
33 0.594214027204073
34 0.594214027261747
35 0.594214027229716
36 0.594214027218682
37 0.594214027218682
38 0.594214027218682
39 0.594214027218682
40 0.594214027218682
41 0.594214027218681
42 0.594214027258629
43 0.594212029259184
44 0.594215061079481
45 0.594217408282241
46 0.594214299173036
47 0.594222713751328
48 0.594309967992752
49 0.593431330954225
};
\plotInvscat
table {%
0 0.594214141368866
1 0.594214141368866
2 0.594214141368866
3 0.594214141368866
4 0.594214141368866
5 0.594214141368866
6 0.594214141368866
7 0.594214141368866
8 0.594214141368866
9 0.594214141368866
10 0.594214081764221
11 0.594214379787445
12 0.594213902950287
13 0.594214141368866
14 0.594213902950287
15 0.594214022159576
16 0.594214022159576
17 0.594214081764221
18 0.594213962554932
19 0.594213962554932
20 0.594213962554932
21 0.594213962554932
22 0.594214022159576
23 0.594214022159576
24 0.594213962554932
25 0.594213902950287
26 0.594213962554932
27 0.594213902950287
28 0.594214141368866
29 0.594214200973511
30 0.594214081764221
31 0.594214081764221
32 0.594214081764221
33 0.594214141368866
34 0.594214081764221
35 0.594214081764221
36 0.594214081764221
37 0.594214081764221
38 0.594214081764221
39 0.594214081764221
40 0.594214081764221
41 0.594214081764221
42 0.594214081764221
43 0.594214081764221
44 0.594214081764221
45 0.594214081764221
46 0.594214081764221
47 0.594214081764221
48 0.594214081764221
49 0.594214081764221
};
\end{groupplot}

==> Figs/structured_phi_change/n_free.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm, x descriptions at=edge bottom, group name=left0 plots}]
\nextgroupplot[
width=\w cm,
height=\h cm,
legend cell align={left},
legend style={at={(1,2)}, anchor=north west, legend cell align=left, align=left, font=\footnotesize, draw=white!15!black},
legend columns=3,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black,font=\footnotesize},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_0(t)|\)},
title = {Noise free},
title style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
ytick style={color=black,font=\footnotesize},
%-------- Horizantal ----
%xtick style={color=black,font=\footnotesize},
%xlabel = {time \(t\)},
%title={\(\displaystyle |\cos\phi_1(t)|\)},
%-------- Vertical ----
xtick style={color=white,font=\footnotesize},
xticklabels ={},
%xlabel = {time \(t\)},
ylabel={\(\displaystyle |\cos\phi_1(t)|\)},
% xtick style={color=white},
% xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
%\addplot [semithick, blue,line width=\LineWidth pt]
%\addplot [semithick, green,line width=\LineWidth pt, dotted]
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.733099880094478
1 0.733099880094478
2 0.733099880094478
3 0.733099880094478
4 0.733099880094478
5 0.733099880094478
6 0.733099880094478
7 0.733099880094478
8 0.733099880094478
9 0.733099880094478
10 0.733099880094478
11 0.733099880094478
12 0.733099880094478
13 0.733099880094478
14 0.733099880094478
15 0.733099880094478
16 0.733099880094478
17 0.733099880094478
18 0.733099880094478
19 0.733099880094478
20 0.733099880094478
21 0.733099880094478
22 0.733099880094478
23 0.733099880094478
24 0.733099880094478
25 0.733099880094478
26 0.733099880094478
27 0.733099880094478
28 0.733099880094478
29 0.733099880094478
30 0.733099880094478
31 0.733099880094478
32 0.733099880094478
33 0.733099880094478
34 0.733099880094478
35 0.733099880094478
36 0.733099880094478
37 0.733099880094478
38 0.733099880094478
39 0.733099880094478
40 0.733099880094478
41 0.733099880094478
42 0.733099880094478
43 0.733099880094478
44 0.733099880094478
45 0.733099880094478
46 0.733099880094478
47 0.733099880094478
48 0.733099880094478
49 0.733099880094478
50 0.733099880094478
51 0.733099880094478
52 0.733099880094478
53 0.733099880094478
54 0.733099880094478
55 0.733099880094478
56 0.733099880094478
57 0.733099880094478
58 0.733099880094478
59 0.733099880094478
60 0.733099880094478
61 0.733099880094478
62 0.733099880094478
63 0.733099880094478
64 0.733099880094478
65 0.733099880094478
66 0.733099880094478
67 0.733099880094478
68 0.733099880094478
69 0.733099880094478
70 0.733099880094478
71 0.733099880094478
72 0.733099880094478
73 0.733099880094478
74 0.733099880094478
75 0.733099880094478
76 0.733099880094478
77 0.733099880094478
78 0.733099880094478
79 0.733099880094478
80 0.733099880094478
81 0.733099880094478
82 0.733099880094478
83 0.733099880094478
84 0.733099880094478
85 0.733099880094478
86 0.733099880094478
87 0.733099880094478
88 0.733099880094478
89 0.733099880094478
90 0.733099880094478
91 0.733099880094478
92 0.733099880094478
93 0.733099880094478
94 0.733099880094478
95 0.733099880094478
96 0.733099880094478
97 0.733099880094478
98 0.733099880094478
99 0.733099880094478
};
\addlegendentry{True}
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.733101065919303
1 0.733099873047745
2 0.73309987723188
3 0.733100373263356
4 0.733099874618328
5 0.733099881787718
6 0.733099878557434
7 0.733099881541252
8 0.733099883672783
9 0.733099877071528
10 0.733099880814457
11 0.754518454411928
12 0.733099879204052
13 0.733099874272523
14 0.733099890935482
15 0.733099885768519
16 0.73309988387831
17 0.733099876003523
18 0.73309988018212
19 0.733097455796809
20 0.73309987455911
21 0.733099878395198
22 0.733099877932828
23 0.733099881634596
24 0.733099886377961
25 0.733099877263044
26 0.733367519976241
27 0.749132624647497
28 0.733099871883634
29 0.733099883701006
30 0.733099891513046
31 0.733099872324659
32 0.733099881590125
33 0.733099878729432
34 0.733099880672282
35 0.733099881723176
36 0.733099879237167
37 0.733099882454731
38 0.733099881138817
39 0.733099880615274
40 0.73308343524242
41 0.733099871080503
42 0.733099793826951
43 0.733126271223974
44 0.733099873542929
45 0.733099879041667
46 0.733099885628938
47 0.733099870708966
48 0.733099875145676
49 0.73309987839409
50 0.733099883148294
51 0.733099879084887
52 0.733099880171431
53 0.733099879412108
54 0.73309988163583
55 0.733099876590553
56 0.733099887710696
57 0.733099902865122
58 0.73944285414025
59 0.732775706621354
60 0.733099783978261
61 0.73309987304238
62 0.733099870106586
63 0.733099883648637
64 0.733099879364593
65 0.733099881125735
66 0.733100396641739
67 0.733099883846801
68 0.733099883555062
69 0.733099873622845
70 0.73309988190402
71 0.733100198562585
72 0.733099890202033
73 0.733099865243698
74 0.800622630420414
75 0.73309500351026
76 0.733099876468453
77 0.733099886157574
78 0.733099887602049
79 0.733099878375459
80 0.73309988152859
81 0.733099880388014
82 0.733099881797818
83 0.733099882195114
84 0.733099888193
85 0.733099882521454
86 0.733099882971963
87 0.729207805394307
88 0.733296064118446
89 0.733099862036143
90 0.736069121475971
91 0.733099883717454
92 0.733099891186647
93 0.733099882921368
94 0.733099877400541
95 0.73309987794165
96 0.733099882997202
97 0.733099881524456
98 0.733099882763633
99 0.733099880290168
};
\addlegendentry{Netwrok}
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.73309987783432
1 0.73309987783432
2 0.73309987783432
3 0.73309987783432
4 0.73309987783432
5 0.73309987783432
6 0.73309987783432
7 0.733099818229675
8 0.733099818229675
9 0.733099818229675
10 0.733099579811096
11 0.732907593250275
12 0.733100771903992
13 0.73309999704361
14 0.733099937438965
15 0.733099937438965
16 0.73309987783432
17 0.73309987783432
18 0.73309987783432
19 0.73309987783432
20 0.73309987783432
21 0.73309987783432
22 0.73309987783432
23 0.733099818229675
24 0.733099818229675
25 0.733099818229675
26 0.733099162578583
27 0.733222186565399
28 0.733100295066833
29 0.733099937438965
30 0.733099937438965
31 0.733099937438965
32 0.73309987783432
33 0.73309987783432
34 0.73309987783432
35 0.73309987783432
36 0.73309987783432
37 0.73309987783432
38 0.73309987783432
39 0.733099818229675
40 0.733099818229675
41 0.733099699020386
42 0.73309725522995
43 0.733105540275574
44 0.733100056648254
45 0.733099937438965
46 0.733099937438965
47 0.73309987783432
48 0.73309987783432
49 0.73309987783432
50 0.73309987783432
51 0.73309987783432
52 0.73309987783432
53 0.73309987783432
54 0.733099818229675
55 0.733099818229675
56 0.733099818229675
57 0.733099639415741
58 0.733073532581329
59 0.73310124874115
60 0.73309999704361
61 0.733099937438965
62 0.733099937438965
63 0.73309987783432
64 0.73309987783432
65 0.73309987783432
66 0.73309987783432
67 0.73309987783432
68 0.73309987783432
69 0.73309987783432
70 0.733099818229675
71 0.733099818229675
72 0.733099818229675
73 0.733099400997162
74 0.744936287403107
75 0.733100414276123
76 0.733099937438965
77 0.733099937438965
78 0.733099937438965
79 0.73309987783432
80 0.73309987783432
81 0.73309987783432
82 0.73309987783432
83 0.73309987783432
84 0.73309987783432
85 0.73309987783432
86 0.733099818229675
87 0.733099818229675
88 0.733099758625031
89 0.733098447322845
90 0.733114361763
91 0.733100175857544
92 0.733099937438965
93 0.733099937438965
94 0.733099937438965
95 0.73309987783432
96 0.73309987783432
97 0.73309987783432
98 0.73309987783432
99 0.73309987783432
};
\addlegendentry{Inverse Scattering}
%==================================== Fig 2 ==============================
% \nextgroupplot[
% width=\w cm,
% height=\h cm,
% scaled x ticks=manual:{}{\pgfmathparse{#1}},
% tick align=outside,
% tick pos=left,
% x grid style={darkgray176},
% xmin=-4.95, xmax=\xmax,
% xtick style={color=black},
% xlabel style ={color=black,font=\footnotesize},
% ylabel style ={color=black,font=\footnotesize},
% title style ={color=black,font=\footnotesize},
% y grid style={darkgray176},
% %ylabel={\(\displaystyle |\cos\phi_1(t)|\)},
% ymin=0, ymax=1.2,
% %-------- Horizantal ----
% % xtick style={color=black,font=\footnotesize},
% % xlabel = {time \(t\)},
% % title={\(\displaystyle |\cos\phi_2(t)|\)},
% %xlabel = {time \(t\)},
% %-------- Vertical ----
% ylabel={\(\displaystyle |\cos\phi_2(t)|\)},
% xtick style={color=white},
% xticklabels={},
% ]
\nextgplot{2}
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.792461900085071
1 0.897838102564357
2 0.967420333186374
3 0.998434567995651
4 0.989644367321418
5 0.941400168725476
6 0.855625316162471
7 0.735739382325891
8 0.586521841075859
9 0.413921524898832
10 0.224819463728995
11 0.0267545599991264
12 0.172376963609011
13 0.364636361645022
14 0.542358858618825
15 0.698459219411845
16 0.826714215242439
17 0.922010724158886
18 0.980549575076209
19 0.999997008738362
20 0.979577717335161
21 0.920105753578051
22 0.823952076987393
23 0.694950031218385
24 0.53824252074634
25 0.360076979494633
26 0.167556305359092
27 0.0316443099166179
28 0.229583366415347
29 0.418369658587304
30 0.590476872713188
31 0.739043637281522
32 0.858147064218503
33 0.94303887574475
34 0.990334703226316
35 0.998149011272124
36 0.966170268079864
37 0.89567336522585
38 0.789468791761032
39 0.651790588881538
40 0.488127552067482
41 0.305004410128062
42 0.10972170485391
43 0.0899352585459059
44 0.286006786994616
45 0.470676127392459
46 0.636581095895575
47 0.777107584953148
48 0.886653246903433
49 0.960850841895798
50 0.996742345961949
51 0.992896878096958
52 0.949467744969529
53 0.868186329068895
54 0.752293063948673
55 0.606408248366861
56 0.436347849554549
57 0.248891638955762
58 0.0515129041347936
59 0.14791948761566
60 0.341454796181813
61 0.521377379547116
62 0.680514292091338
63 0.812521247296909
64 0.912135544431819
65 0.975385875820392
66 0.999750650348126
67 0.984258521342095
68 0.929527111097529
69 0.837738388225924
70 0.712551679452109
71 0.558957783805391
72 0.383080005211638
73 0.191930035688959
74 0.00687157868638793
75 0.205399244904029
76 0.395738291402145
77 0.570300501046451
78 0.722126629401336
79 0.845163847844344
80 0.934507050742547
81 0.986594406535174
82 0.99934935671793
83 0.9722634016776
84 0.906416372966969
85 0.804433383828414
86 0.670380174212959
87 0.509601022558604
88 0.328505686273858
89 0.134313864937013
90 0.0652326263429608
91 0.262178498664097
92 0.44867214159559
93 0.617278642108485
94 0.761276191095912
95 0.874924060690286
96 0.953691468967469
97 0.994438207924381
98 0.995539833662581
99 0.956952427840267
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.792463165373803
1 0.897838105242104
2 0.9674203303543
3 0.998434625233116
4 0.989644367373648
5 0.941400164594114
6 0.855625304645303
7 0.735739370536748
8 0.586521827632642
9 0.41392153182515
10 0.224819462106534
11 0.0272520496208527
12 0.172376958381089
13 0.36463636185353
14 0.542358842461255
15 0.698459217726571
16 0.826714219051323
17 0.922010719258649
18 0.980549573904474
19 0.999997014419662
20 0.97957772096138
21 0.920105761928868
22 0.823952068549296
23 0.694950039408397
24 0.538242534844451
25 0.360076990085653
26 0.167600687448094
27 0.0320903129005423
28 0.229583352988995
29 0.418369671352394
30 0.590476873411624
31 0.739043633972823
32 0.858147066116717
33 0.943038876197467
34 0.990334700644263
35 0.998149012425491
36 0.966170273935097
37 0.89567336802037
38 0.789468779687885
39 0.651790591532855
40 0.488127490094392
41 0.305004424242773
42 0.109721701886574
43 0.0899832048203919
44 0.28600678944896
45 0.47067611732644
46 0.636581079172453
47 0.777107582597265
48 0.88665324780915
49 0.960850838682498
50 0.996742344887504
51 0.992896881173472
52 0.949467751339623
53 0.868186325868142
54 0.752293048578539
55 0.606408254518343
56 0.436347838736177
57 0.248891654479693
58 0.0517164364248019
59 0.147926438595479
60 0.341454810047533
61 0.521377371520394
62 0.680514277499333
63 0.812521249526961
64 0.912135547883448
65 0.975385871217521
66 0.999750660518221
67 0.984258526006793
68 0.92952711245624
69 0.837738390957492
70 0.712551673852492
71 0.558957800454544
72 0.383080014530143
73 0.191930048830556
74 0.00737851614790402
75 0.205372480964966
76 0.395738306513586
77 0.570300514555757
78 0.72212662902713
79 0.845163856001875
80 0.934507055244619
81 0.986594403377649
82 0.99934935741867
83 0.972263406731245
84 0.906416373192704
85 0.804433383302332
86 0.670380172965601
87 0.509629132025601
88 0.328506075012363
89 0.134313884798047
90 0.0653573293240359
91 0.262178486373999
92 0.448672123838798
93 0.617278632926765
94 0.761276186993732
95 0.874924061475362
96 0.953691466562881
97 0.994438206540422
98 0.995539835682736
99 0.956952434422783
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.792461931705475
1 0.897838115692139
2 0.967420339584351
3 0.998434543609619
4 0.989644348621368
5 0.941400170326233
6 0.855625331401825
7 0.735739350318909
8 0.586521863937378
9 0.413921535015106
10 0.22481943666935
11 0.0267506670206785
12 0.17237700521946
13 0.364636451005936
14 0.542358875274658
15 0.698459208011627
16 0.826714217662811
17 0.922010719776154
18 0.980549573898315
19 0.999997019767761
20 0.979577720165253
21 0.920105755329132
22 0.823952078819275
23 0.694949984550476
24 0.538242518901825
25 0.360076934099197
26 0.167556196451187
27 0.031646765768528
28 0.229583367705345
29 0.418369710445404
30 0.590476930141449
31 0.739043653011322
32 0.858147084712982
33 0.943038880825043
34 0.990334689617157
35 0.998149037361145
36 0.966170251369476
37 0.895673394203186
38 0.789468765258789
39 0.651790618896484
40 0.488127559423447
41 0.305004388093948
42 0.109721399843693
43 0.0899355262517929
44 0.28600686788559
45 0.470676124095917
46 0.636581063270569
47 0.7771075963974
48 0.886653244495392
49 0.960850834846497
50 0.996742367744446
51 0.992896854877472
52 0.949467778205872
53 0.868186354637146
54 0.752293050289154
55 0.60640823841095
56 0.436347812414169
57 0.248891532421112
58 0.0515118017792702
59 0.147919595241547
60 0.341454833745956
61 0.521377325057983
62 0.680514276027679
63 0.812521278858185
64 0.912135541439056
65 0.975385904312134
66 0.999750673770905
67 0.984258532524109
68 0.929527103900909
69 0.837738394737244
70 0.712551712989807
71 0.558957755565643
72 0.38307997584343
73 0.191929966211319
74 0.00687243696302176
75 0.205399319529533
76 0.395738303661346
77 0.5703005194664
78 0.722126662731171
79 0.845163881778717
80 0.934507071971893
81 0.986594378948212
82 0.999349355697632
83 0.972263395786285
84 0.906416356563568
85 0.804433405399323
86 0.670380175113678
87 0.50960099697113
88 0.328505605459213
89 0.134313717484474
90 0.0652332082390785
91 0.262178540229797
92 0.448672205209732
93 0.617278635501862
94 0.761276185512543
95 0.874924063682556
96 0.953691482543945
97 0.994438230991364
98 0.995539844036102
99 0.956952452659607
};

%=========================== Fig 3 ====================
\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_2(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
title style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_2(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
ylabel={\(\displaystyle |\cos\phi_3(t)|\)},
xtick style={color=white},
xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.824356457355511
1 0.824356457355511
2 0.824356457355511
3 0.824356457355511
4 0.824356457355511
5 0.824356457355511
6 0.824356457355511
7 0.824356457355511
8 0.824356457355511
9 0.824356457355511
10 0.824356457355511
11 0.824356457355511
12 0.824356457355511
13 0.824356457355511
14 0.824356457355511
15 0.824356457355511
16 0.824356457355511
17 0.824356457355511
18 0.824356457355511
19 0.824356457355511
20 0.824356457355511
21 0.824356457355511
22 0.824356457355511
23 0.824356457355511
24 0.824356457355511
25 0.824356457355511
26 0.824356457355511
27 0.824356457355511
28 0.824356457355511
29 0.824356457355511
30 0.824356457355511
31 0.824356457355511
32 0.824356457355511
33 0.824356457355511
34 0.824356457355511
35 0.824356457355511
36 0.824356457355511
37 0.824356457355511
38 0.824356457355511
39 0.824356457355511
40 0.824356457355511
41 0.824356457355511
42 0.824356457355511
43 0.824356457355511
44 0.824356457355511
45 0.824356457355511
46 0.824356457355511
47 0.824356457355511
48 0.824356457355511
49 0.824356457355511
50 0.824356457355511
51 0.824356457355511
52 0.824356457355511
53 0.824356457355511
54 0.824356457355511
55 0.824356457355511
56 0.824356457355511
57 0.824356457355511
58 0.824356457355511
59 0.824356457355511
60 0.824356457355511
61 0.824356457355511
62 0.824356457355511
63 0.824356457355511
64 0.824356457355511
65 0.824356457355511
66 0.824356457355511
67 0.824356457355511
68 0.824356457355511
69 0.824356457355511
70 0.824356457355511
71 0.824356457355511
72 0.824356457355511
73 0.824356457355511
74 0.824356457355511
75 0.824356457355511
76 0.824356457355511
77 0.824356457355511
78 0.824356457355511
79 0.824356457355511
80 0.824356457355511
81 0.824356457355511
82 0.824356457355511
83 0.824356457355511
84 0.824356457355511
85 0.824356457355511
86 0.824356457355511
87 0.824356457355511
88 0.824356457355511
89 0.824356457355511
90 0.824356457355511
91 0.824356457355511
92 0.824356457355511
93 0.824356457355511
94 0.824356457355511
95 0.824356457355511
96 0.824356457355511
97 0.824356457355511
98 0.824356457355511
99 0.824356457355511
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.824356684581715
1 0.824356460550334
2 0.82435646154057
3 0.824352560857484
4 0.824356454734182
5 0.824356454337336
6 0.824356454596882
7 0.824356454264978
8 0.824356453548249
9 0.824356459162126
10 0.824356456625465
11 0.811130258520629
12 0.824356459744575
13 0.82435646458417
14 0.824356453203859
15 0.824356453161983
16 0.824356455146422
17 0.824356457918049
18 0.824356455447375
19 0.824367018572689
20 0.824356457615877
21 0.82435646002082
22 0.824356456289758
23 0.824356452159698
24 0.824356448654149
25 0.824356463565499
26 0.824223011813665
27 0.810572408249417
28 0.824356465324795
29 0.824356451632637
30 0.824356445839962
31 0.824356460142475
32 0.824356458465808
33 0.824356457601411
34 0.824356459582758
35 0.824356459171973
36 0.82435646034012
37 0.82435645422448
38 0.824356456276984
39 0.824356459823348
40 0.82434143304376
41 0.824356465301395
42 0.824356504238204
43 0.823299187347666
44 0.824356454935444
45 0.824356461735756
46 0.824356455786399
47 0.824356461141403
48 0.824356456287914
49 0.82435645911349
50 0.824356460537117
51 0.824356458872569
52 0.824356460119883
53 0.824356455435252
54 0.82435645538197
55 0.824356464044989
56 0.824356449375692
57 0.824356503641805
58 0.821639909376592
59 0.823994220547096
60 0.824356399570305
61 0.824356464040457
62 0.82435646127466
63 0.824356456563185
64 0.824356457935846
65 0.824356455357301
66 0.824353414976913
67 0.824356456853483
68 0.824356455539513
69 0.824356455750476
70 0.824356453790243
71 0.824356767312023
72 0.824356451145187
73 0.82435646451921
74 0.768955476803036
75 0.824507547316929
76 0.824356459455618
77 0.824356450919801
78 0.824356454603311
79 0.82435645628744
80 0.824356459562516
81 0.824356457463936
82 0.82435646050388
83 0.824356461050259
84 0.824356453247149
85 0.824356459168024
86 0.824356451219748
87 0.8207953919
88 0.824513627001185
89 0.8243564687952
90 0.823428932749255
91 0.824356456677844
92 0.82435645114933
93 0.824356457142129
94 0.82435645994301
95 0.824356458674625
96 0.824356455512463
97 0.824356461609778
98 0.82435646128341
99 0.824356459142869
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.824356436729431
1 0.824356436729431
2 0.824356436729431
3 0.824356436729431
4 0.824356436729431
5 0.824356436729431
6 0.824356436729431
7 0.824356436729431
8 0.824356436729431
9 0.824356615543365
10 0.824357151985168
11 0.82469630241394
12 0.824355244636536
13 0.824356317520142
14 0.824356436729431
15 0.824356436729431
16 0.824356436729431
17 0.824356436729431
18 0.824356436729431
19 0.824356436729431
20 0.824356436729431
21 0.824356436729431
22 0.824356436729431
23 0.824356436729431
24 0.824356615543365
25 0.824356734752655
26 0.824358105659485
27 0.82415908575058
28 0.824355900287628
29 0.824356317520142
30 0.824356436729431
31 0.824356436729431
32 0.824356436729431
33 0.824356436729431
34 0.824356436729431
35 0.824356436729431
36 0.824356436729431
37 0.824356436729431
38 0.824356436729431
39 0.824356436729431
40 0.824356615543365
41 0.824356734752655
42 0.824361741542816
43 0.824347972869873
44 0.824356198310852
45 0.824356317520142
46 0.824356436729431
47 0.824356436729431
48 0.824356436729431
49 0.824356436729431
50 0.824356436729431
51 0.824356436729431
52 0.824356436729431
53 0.824356436729431
54 0.824356436729431
55 0.824356436729431
56 0.824356615543365
57 0.824356973171234
58 0.824404895305634
59 0.824354588985443
60 0.824356317520142
61 0.824356436729431
62 0.824356436729431
63 0.824356436729431
64 0.824356436729431
65 0.824356436729431
66 0.824356436729431
67 0.824356436729431
68 0.824356436729431
69 0.824356436729431
70 0.824356436729431
71 0.824356615543365
72 0.824356615543365
73 0.824357509613037
74 0.806209146976471
75 0.824355781078339
76 0.824356317520142
77 0.824356436729431
78 0.824356436729431
79 0.824356436729431
80 0.824356436729431
81 0.824356436729431
82 0.824356436729431
83 0.824356436729431
84 0.824356436729431
85 0.824356436729431
86 0.824356436729431
87 0.824356615543365
88 0.824356734752655
89 0.82435941696167
90 0.82433420419693
91 0.824356079101562
92 0.824356317520142
93 0.824356436729431
94 0.824356436729431
95 0.824356436729431
96 0.824356436729431
97 0.824356436729431
98 0.824356436729431
99 0.824356436729431
};

%=============================== Fig 4 =========================
\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_3(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_3(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
ylabel={\(\displaystyle |\cos\phi_4(t)|\)},
xtick style={color=white},
xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.753602486017811
1 0.753602486017811
2 0.753602486017811
3 0.753602486017811
4 0.753602486017811
5 0.753602486017811
6 0.753602486017811
7 0.753602486017811
8 0.753602486017811
9 0.753602486017811
10 0.753602486017811
11 0.753602486017811
12 0.753602486017811
13 0.753602486017811
14 0.753602486017811
15 0.753602486017811
16 0.753602486017811
17 0.753602486017811
18 0.753602486017811
19 0.753602486017811
20 0.753602486017811
21 0.753602486017811
22 0.753602486017811
23 0.753602486017811
24 0.753602486017811
25 0.753602486017811
26 0.753602486017811
27 0.753602486017811
28 0.753602486017811
29 0.753602486017811
30 0.753602486017811
31 0.753602486017811
32 0.753602486017811
33 0.753602486017811
34 0.753602486017811
35 0.753602486017811
36 0.753602486017811
37 0.753602486017811
38 0.753602486017811
39 0.753602486017811
40 0.753602486017811
41 0.753602486017811
42 0.753602486017811
43 0.753602486017811
44 0.753602486017811
45 0.753602486017811
46 0.753602486017811
47 0.753602486017811
48 0.753602486017811
49 0.753602486017811
50 0.753602486017811
51 0.753602486017811
52 0.753602486017811
53 0.753602486017811
54 0.753602486017811
55 0.753602486017811
56 0.753602486017811
57 0.753602486017811
58 0.753602486017811
59 0.753602486017811
60 0.753602486017811
61 0.753602486017811
62 0.753602486017811
63 0.753602486017811
64 0.753602486017811
65 0.753602486017811
66 0.753602486017811
67 0.753602486017811
68 0.753602486017811
69 0.753602486017811
70 0.753602486017811
71 0.753602486017811
72 0.753602486017811
73 0.753602486017811
74 0.753602486017811
75 0.753602486017811
76 0.753602486017811
77 0.753602486017811
78 0.753602486017811
79 0.753602486017811
80 0.753602486017811
81 0.753602486017811
82 0.753602486017811
83 0.753602486017811
84 0.753602486017811
85 0.753602486017811
86 0.753602486017811
87 0.753602486017811
88 0.753602486017811
89 0.753602486017811
90 0.753602486017811
91 0.753602486017811
92 0.753602486017811
93 0.753602486017811
94 0.753602486017811
95 0.753602486017811
96 0.753602486017811
97 0.753602486017811
98 0.753602486017811
99 0.753602486017811
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.753601860978412
1 0.75360248702962
2 0.753602485792119
3 0.753608229488729
4 0.75360248786118
5 0.753602486157098
6 0.753602478114257
7 0.75360248595987
8 0.7536024897745
9 0.753602485075069
10 0.753602490331135
11 0.754249245550176
12 0.753602482650386
13 0.753602488545377
14 0.753602484280528
15 0.753602485383323
16 0.75360248127849
17 0.753602488364951
18 0.753602488310057
19 0.753586938897364
20 0.753602484401355
21 0.753602485859687
22 0.753602483051689
23 0.753602488611355
24 0.753602496056752
25 0.753602484552583
26 0.753656386708786
27 0.752879628229071
28 0.753602487142262
29 0.753602487616418
30 0.753602475480686
31 0.753602493470149
32 0.753602483797164
33 0.75360249044555
34 0.75360249258505
35 0.753602487647648
36 0.753602487315964
37 0.753602488736368
38 0.753602487386618
39 0.753602483680748
40 0.753603792431984
41 0.753602488446975
42 0.753602477227663
43 0.753492310863899
44 0.753602491828261
45 0.753602484941857
46 0.75360248130608
47 0.753602493115866
48 0.753602491684621
49 0.753602486900135
50 0.753602488290523
51 0.753602486310432
52 0.753602491022351
53 0.753602485206323
54 0.753602482423957
55 0.753602488428474
56 0.753602485360446
57 0.753602482337782
58 0.753970945628396
59 0.753563728486934
60 0.753602474710336
61 0.753602491706553
62 0.753602497625347
63 0.7536024820297
64 0.753602487460041
65 0.753602484729139
66 0.753606983556018
67 0.753602495299466
68 0.753602489289272
69 0.753602480951333
70 0.753602486592315
71 0.753602463302244
72 0.753602489832906
73 0.753602483885619
74 0.752978931993048
75 0.753620168114944
76 0.753602486104021
77 0.753602484792582
78 0.753602483980458
79 0.753602486093143
80 0.753602485062208
81 0.753602485187496
82 0.753602493281512
83 0.753602492362775
84 0.75360249477994
85 0.75360248901856
86 0.753602487407112
87 0.754245571619691
88 0.753581853179544
89 0.753602490509905
90 0.753424358672258
91 0.753602489823254
92 0.753602480405549
93 0.753602482842772
94 0.753602488755204
95 0.753602486811941
96 0.753602483305316
97 0.753602492761204
98 0.753602492608436
99 0.753602491048327
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.753602504730225
1 0.753602504730225
2 0.753602504730225
3 0.753602504730225
4 0.753602504730225
5 0.753602504730225
6 0.753602504730225
7 0.753602504730225
8 0.75360244512558
9 0.75360244512558
10 0.753602385520935
11 0.753597259521484
12 0.753602385520935
13 0.75360244512558
14 0.753602504730225
15 0.753602504730225
16 0.753602504730225
17 0.753602504730225
18 0.753602504730225
19 0.753602504730225
20 0.753602504730225
21 0.753602504730225
22 0.753602504730225
23 0.753602504730225
24 0.75360244512558
25 0.75360244512558
26 0.75360232591629
27 0.753598928451538
28 0.753602385520935
29 0.75360244512558
30 0.753602504730225
31 0.753602504730225
32 0.753602504730225
33 0.753602504730225
34 0.753602504730225
35 0.753602504730225
36 0.753602504730225
37 0.753602504730225
38 0.753602504730225
39 0.75360244512558
40 0.75360244512558
41 0.75360244512558
42 0.753602147102356
43 0.753602027893066
44 0.75360244512558
45 0.75360244512558
46 0.753602504730225
47 0.753602504730225
48 0.753602504730225
49 0.753602504730225
50 0.753602504730225
51 0.753602504730225
52 0.753602504730225
53 0.753602504730225
54 0.753602504730225
55 0.75360244512558
56 0.75360244512558
57 0.753602385520935
58 0.753601014614105
59 0.75360232591629
60 0.75360244512558
61 0.753602504730225
62 0.753602504730225
63 0.753602504730225
64 0.753602504730225
65 0.753602504730225
66 0.753602504730225
67 0.753602504730225
68 0.753602504730225
69 0.753602504730225
70 0.753602504730225
71 0.75360244512558
72 0.75360244512558
73 0.753602385520935
74 0.753520965576172
75 0.753602385520935
76 0.75360244512558
77 0.753602504730225
78 0.753602504730225
79 0.753602504730225
80 0.753602504730225
81 0.753602504730225
82 0.753602504730225
83 0.753602504730225
84 0.753602504730225
85 0.753602504730225
86 0.753602504730225
87 0.75360244512558
88 0.75360244512558
89 0.753602266311646
90 0.753601670265198
91 0.75360244512558
92 0.75360244512558
93 0.753602504730225
94 0.753602504730225
95 0.753602504730225
96 0.753602504730225
97 0.753602504730225
98 0.753602504730225
99 0.753602504730225
};
%====================== Fig 5 ==================
\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_5(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
ylabel={\(\displaystyle |\cos\phi_5(t)|\)},
%xtick style={color=white},
%xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.935826238137458
1 0.935826238137458
2 0.935826238137458
3 0.935826238137458
4 0.935826238137458
5 0.935826238137458
6 0.935826238137458
7 0.935826238137458
8 0.935826238137458
9 0.935826238137458
10 0.935826238137458
11 0.935826238137458
12 0.935826238137458
13 0.935826238137458
14 0.935826238137458
15 0.935826238137458
16 0.935826238137458
17 0.935826238137458
18 0.935826238137458
19 0.935826238137458
20 0.935826238137458
21 0.935826238137458
22 0.935826238137458
23 0.935826238137458
24 0.935826238137458
25 0.935826238137458
26 0.935826238137458
27 0.935826238137458
28 0.935826238137458
29 0.935826238137458
30 0.935826238137458
31 0.935826238137458
32 0.935826238137458
33 0.935826238137458
34 0.935826238137458
35 0.935826238137458
36 0.935826238137458
37 0.935826238137458
38 0.935826238137458
39 0.935826238137458
40 0.935826238137458
41 0.935826238137458
42 0.935826238137458
43 0.935826238137458
44 0.935826238137458
45 0.935826238137458
46 0.935826238137458
47 0.935826238137458
48 0.935826238137458
49 0.935826238137458
50 0.935826238137458
51 0.935826238137458
52 0.935826238137458
53 0.935826238137458
54 0.935826238137458
55 0.935826238137458
56 0.935826238137458
57 0.935826238137458
58 0.935826238137458
59 0.935826238137458
60 0.935826238137458
61 0.935826238137458
62 0.935826238137458
63 0.935826238137458
64 0.935826238137458
65 0.935826238137458
66 0.935826238137458
67 0.935826238137458
68 0.935826238137458
69 0.935826238137458
70 0.935826238137458
71 0.935826238137458
72 0.935826238137458
73 0.935826238137458
74 0.935826238137458
75 0.935826238137458
76 0.935826238137458
77 0.935826238137458
78 0.935826238137458
79 0.935826238137458
80 0.935826238137458
81 0.935826238137458
82 0.935826238137458
83 0.935826238137458
84 0.935826238137458
85 0.935826238137458
86 0.935826238137458
87 0.935826238137458
88 0.935826238137458
89 0.935826238137458
90 0.935826238137458
91 0.935826238137458
92 0.935826238137458
93 0.935826238137458
94 0.935826238137458
95 0.935826238137458
96 0.935826238137458
97 0.935826238137458
98 0.935826238137458
99 0.935826238137458
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.935826374163682
1 0.93582623860673
2 0.935826237159976
3 0.935832975912941
4 0.935826238476688
5 0.935826238260904
6 0.935826239177657
7 0.935826242149338
8 0.935826239462004
9 0.935826238122567
10 0.935826237777816
11 0.935971820382555
12 0.93582623677266
13 0.935826236974713
14 0.935826237453915
15 0.935826240288223
16 0.935826236425704
17 0.935826237609176
18 0.935826239432472
19 0.935807823611657
20 0.935826236651963
21 0.935826234420418
22 0.93582623948394
23 0.93582624234565
24 0.935826242788618
25 0.93582623465526
26 0.935817201341014
27 0.93448701899358
28 0.935826236483093
29 0.93582623943538
30 0.935826241535715
31 0.935826239120077
32 0.935826237109792
33 0.935826238544288
34 0.935826236876721
35 0.935826236644293
36 0.935826234220612
37 0.935826242825184
38 0.93582624090195
39 0.935826236738829
40 0.935817329416835
41 0.935826239654223
42 0.935826231235851
43 0.935653218755263
44 0.935826240582584
45 0.935826238260209
46 0.935826239156517
47 0.935826237008734
48 0.93582623716827
49 0.935826235882759
50 0.935826235693898
51 0.935826237009005
52 0.935826236936035
53 0.935826236581521
54 0.935826241563756
55 0.935826233236029
56 0.935826239453867
57 0.935826240796271
58 0.935917556449625
59 0.93573436205412
60 0.935826218928883
61 0.935826236458451
62 0.935826236780085
63 0.935826237602797
64 0.935826239421282
65 0.935826238136101
66 0.935831448308418
67 0.935826237791061
68 0.935826239187497
69 0.93582623519935
70 0.935826238587742
71 0.935826401636181
72 0.935826238227801
73 0.935826241359985
74 0.935716590516142
75 0.935852062119065
76 0.935826236664473
77 0.935826238737005
78 0.935826237470339
79 0.935826238916012
80 0.935826238487741
81 0.93582623795852
82 0.935826235389094
83 0.935826235943038
84 0.935826239199109
85 0.935826238582199
86 0.935826241326464
87 0.934404170162014
88 0.935857749311387
89 0.935826236697473
90 0.935949747027303
91 0.935826239146829
92 0.935826235616718
93 0.935826238373954
94 0.935826236622439
95 0.935826237235317
96 0.935826238983775
97 0.935826236574367
98 0.93582623552918
99 0.935826236019876
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.935826241970062
1 0.935826241970062
2 0.935826241970062
3 0.935826241970062
4 0.935826241970062
5 0.935826241970062
6 0.935826241970062
7 0.935826241970062
8 0.935826241970062
9 0.935826241970062
10 0.935826241970062
11 0.935826003551483
12 0.935826241970062
13 0.935826241970062
14 0.935826241970062
15 0.935826241970062
16 0.935826241970062
17 0.935826241970062
18 0.935826241970062
19 0.935826241970062
20 0.935826241970062
21 0.935826241970062
22 0.935826241970062
23 0.935826241970062
24 0.935826241970062
25 0.935826241970062
26 0.935826182365417
27 0.935826480388641
28 0.935826241970062
29 0.935826241970062
30 0.935826241970062
31 0.935826241970062
32 0.935826241970062
33 0.935826241970062
34 0.935826241970062
35 0.935826241970062
36 0.935826241970062
37 0.935826241970062
38 0.935826241970062
39 0.935826241970062
40 0.935826241970062
41 0.935826241970062
42 0.935826182365417
43 0.935826301574707
44 0.935826241970062
45 0.935826241970062
46 0.935826241970062
47 0.935826241970062
48 0.935826241970062
49 0.935826241970062
50 0.935826241970062
51 0.935826241970062
52 0.935826241970062
53 0.935826241970062
54 0.935826241970062
55 0.935826241970062
56 0.935826241970062
57 0.935826241970062
58 0.935826063156128
59 0.935826301574707
60 0.935826241970062
61 0.935826241970062
62 0.935826241970062
63 0.935826241970062
64 0.935826241970062
65 0.935826241970062
66 0.935826241970062
67 0.935826241970062
68 0.935826241970062
69 0.935826241970062
70 0.935826241970062
71 0.935826241970062
72 0.935826241970062
73 0.935826182365417
74 0.935827314853668
75 0.935826241970062
76 0.935826241970062
77 0.935826241970062
78 0.935826241970062
79 0.935826241970062
80 0.935826241970062
81 0.935826241970062
82 0.935826241970062
83 0.935826241970062
84 0.935826241970062
85 0.935826241970062
86 0.935826241970062
87 0.935826241970062
88 0.935826241970062
89 0.935826182365417
90 0.935826301574707
91 0.935826241970062
92 0.935826241970062
93 0.935826241970062
94 0.935826241970062
95 0.935826241970062
96 0.935826241970062
97 0.935826241970062
98 0.935826241970062
99 0.935826241970062
};

\end{groupplot}

==> Figs/structured_phi_change/noise_0.01.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm, group name=left2 plots }]
\nextgroupplot[
anchor=north west,
at={($(left1 plots c1r1.north east) + (0.2cm,0)$)},
width=\w cm,
height=\h cm,
legend cell align={left},
legend style={at={(0,2)}, anchor=north west, legend cell align=left, align=left, font=\footnotesize, draw=white!15!black},
legend columns=3,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black,font=\footnotesize},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_0(t)|\)},
title style ={color=black,font=\footnotesize},
title = {Noise variance = $0.01$},
ymin=0, ymax=1.2,
ytick style={color=black,font=\footnotesize},
%-------- Horizantal ----
%xtick style={color=black,font=\footnotesize},
%xlabel = {time \(t\)},
%title={\(\displaystyle |\cos\phi_1(t)|\)},
%-------- Vertical ----
xtick style={color=white,font=\footnotesize},
xticklabels ={},
yticklabels={},
ytick style={color=white},
%xlabel = {time \(t\)},
%ylabel={\(\displaystyle |\cos\phi_1(t)|\)},
% xtick style={color=white},
% xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.733099880094478
1 0.733099880094478
2 0.733099880094478
3 0.733099880094478
4 0.733099880094478
5 0.733099880094478
6 0.733099880094478
7 0.733099880094478
8 0.733099880094478
9 0.733099880094478
10 0.733099880094478
11 0.733099880094478
12 0.733099880094478
13 0.733099880094478
14 0.733099880094478
15 0.733099880094478
16 0.733099880094478
17 0.733099880094478
18 0.733099880094478
19 0.733099880094478
20 0.733099880094478
21 0.733099880094478
22 0.733099880094478
23 0.733099880094478
24 0.733099880094478
25 0.733099880094478
26 0.733099880094478
27 0.733099880094478
28 0.733099880094478
29 0.733099880094478
30 0.733099880094478
31 0.733099880094478
32 0.733099880094478
33 0.733099880094478
34 0.733099880094478
35 0.733099880094478
36 0.733099880094478
37 0.733099880094478
38 0.733099880094478
39 0.733099880094478
40 0.733099880094478
41 0.733099880094478
42 0.733099880094478
43 0.733099880094478
44 0.733099880094478
45 0.733099880094478
46 0.733099880094478
47 0.733099880094478
48 0.733099880094478
49 0.733099880094478
50 0.733099880094478
51 0.733099880094478
52 0.733099880094478
53 0.733099880094478
54 0.733099880094478
55 0.733099880094478
56 0.733099880094478
57 0.733099880094478
58 0.733099880094478
59 0.733099880094478
60 0.733099880094478
61 0.733099880094478
62 0.733099880094478
63 0.733099880094478
64 0.733099880094478
65 0.733099880094478
66 0.733099880094478
67 0.733099880094478
68 0.733099880094478
69 0.733099880094478
70 0.733099880094478
71 0.733099880094478
72 0.733099880094478
73 0.733099880094478
74 0.733099880094478
75 0.733099880094478
76 0.733099880094478
77 0.733099880094478
78 0.733099880094478
79 0.733099880094478
80 0.733099880094478
81 0.733099880094478
82 0.733099880094478
83 0.733099880094478
84 0.733099880094478
85 0.733099880094478
86 0.733099880094478
87 0.733099880094478
88 0.733099880094478
89 0.733099880094478
90 0.733099880094478
91 0.733099880094478
92 0.733099880094478
93 0.733099880094478
94 0.733099880094478
95 0.733099880094478
96 0.733099880094478
97 0.733099880094478
98 0.733099880094478
99 0.733099880094478
};

\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.716221731484135
1 0.710753781055903
2 0.755954526044914
3 0.69602644766259
4 0.780401870553864
5 0.841512111148321
6 0.65646346722564
7 0.742762619180075
8 0.726077591758057
9 0.716276635475396
10 0.753867124057793
11 0.713084918640876
12 0.7410204933059
13 0.73477871512639
14 0.738030138149818
15 0.728091953385028
16 0.752628559309819
17 0.747091942332626
18 0.684188771447161
19 0.730169823074215
20 0.66963077280175
21 0.934449600542344
22 0.638514473040744
23 0.718732897178727
24 0.699382818600974
25 0.732072202727223
26 0.735245438984077
27 0.734239910312541
28 0.744090518408624
29 0.737145996003196
30 0.740739588663103
31 0.730124957787899
32 0.749438529703522
33 0.690330168526866
34 0.747954911365374
35 0.60071850832943
36 0.55332216667867
37 0.555180009107804
38 0.772523920232248
39 0.671275678212484
40 0.72731992100231
41 0.751571096026029
42 0.726044820531511
43 0.729733807804341
44 0.725861058839838
45 0.729332368520863
46 0.726564788287894
47 0.715579050008598
48 0.747370058374488
49 0.752732333594259
50 0.71388056707216
51 0.653814551475638
52 0.718972921499117
53 0.727459119848569
54 0.645863597869417
55 0.699329382597171
56 0.713588487459538
57 0.705883482454658
58 0.747105544014109
59 0.750459495575512
60 0.743371486530348
61 0.724489056450298
62 0.730170580758513
63 0.736725570071744
64 0.740916370092075
65 0.736160779426349
66 0.751838874932411
67 0.715708478653016
68 0.800836861834675
69 0.744579688359136
70 0.693795929741644
71 0.799915701918921
72 0.757788800774715
73 0.71502462910241
74 0.754634589830281
75 0.736864754018196
76 0.745655108175906
77 0.721811617478291
78 0.7336954331175
79 0.76513267756096
80 0.757838412206449
81 0.755040543698437
82 0.757074147709814
83 0.667557647384844
84 0.337716129850975
85 0.757421994500338
86 0.677480081193946
87 0.712779968718306
88 0.753048231436314
89 0.747308468177337
90 0.732065761406935
91 0.721960873923447
92 0.753621770999758
93 0.738747315477693
94 0.73082172234655
95 0.748489094234788
96 0.756216709908662
97 0.701352128597414
98 0.754599854693593
99 0.66198164968045
};

\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.71468847990036
1 0.679847955703735
2 0.781555652618408
3 0.906436204910278
4 0.750930905342102
5 0.874877750873566
6 0.98059493303299
7 0.564919531345367
8 0.830851078033447
9 0.658116817474365
10 0.83344441652298
11 0.728820025920868
12 0.740688443183899
13 0.742237091064453
14 0.741316914558411
15 0.735600590705872
16 0.774974524974823
17 0.773695528507233
18 0.699329376220703
19 0.946616291999817
20 0.740972697734833
21 0.901827216148376
22 0.954225957393646
23 0.928215861320496
24 0.845505475997925
25 0.658756256103516
26 0.720591723918915
27 0.751243948936462
28 0.733982503414154
29 0.741412162780762
30 0.74982362985611
31 0.722126007080078
32 0.737364292144775
33 0.741021573543549
34 0.648456335067749
35 0.905203700065613
36 0.880385458469391
37 0.89004784822464
38 0.928141295909882
39 0.970650672912598
40 0.753864824771881
41 0.711285412311554
42 0.747568488121033
43 0.737414479255676
44 0.71733433008194
45 0.738490998744965
46 0.738222777843475
47 0.732444703578949
48 0.731340765953064
49 0.71441787481308
50 0.919350802898407
51 0.840996921062469
52 0.876145601272583
53 0.957225263118744
54 0.909993946552277
55 0.750885248184204
56 0.853747189044952
57 0.808355629444122
58 0.764464259147644
59 0.75375360250473
60 0.743188142776489
61 0.731399834156036
62 0.722245097160339
63 0.716047942638397
64 0.765042185783386
65 0.801995754241943
66 0.654816567897797
67 0.643628835678101
68 0.884963393211365
69 0.972091436386108
70 0.778278410434723
71 0.738739192485809
72 0.7083340883255
73 0.690850079059601
74 0.771613776683807
75 0.728310108184814
76 0.753671646118164
77 0.730192959308624
78 0.741899430751801
79 0.754069626331329
80 0.816954553127289
81 0.844777286052704
82 0.887231171131134
83 0.917647659778595
84 0.952951848506927
85 0.984128952026367
86 0.770924806594849
87 0.725157976150513
88 0.765223443508148
89 0.739613473415375
90 0.723983347415924
91 0.729081094264984
92 0.756856024265289
93 0.739656507968903
94 0.751276254653931
95 0.743696391582489
96 0.72513085603714
97 0.949612975120544
98 0.606151700019836
99 0.853221952915192
};


\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
title style ={color=black,font=\footnotesize},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_1(t)|\)},
ymin=0, ymax=1.2,
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_2(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_2(t)|\)},
xtick style={color=white},
xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.880214348557974
1 0.768384900875675
2 0.625922371974234
3 0.458506293314444
4 0.272811015640486
5 0.0762396236778843
6 0.12337120149271
7 0.318063606180129
8 0.500075818596896
9 0.662151586206706
10 0.797829459614615
11 0.901700390164139
12 0.969623371637945
13 0.998890529108033
14 0.988335073363929
15 0.938377817116482
16 0.85101039852304
17 0.729715880859092
18 0.579329893776913
19 0.405847852011046
20 0.216185937112456
21 0.0179053711153667
22 0.181089025524426
23 0.372863974176026
24 0.549774012817539
25 0.704766296480238
26 0.831661771920926
27 0.925401516975611
28 0.982248423821835
29 0.999936185674426
30 0.977759647285282
31 0.916602917257865
32 0.818904121427146
33 0.688558202476517
34 0.530761640864207
35 0.351805287545853
36 0.158823567598829
37 0.0404899467916108
38 0.238189254776884
39 0.426392708823862
40 0.597597231130035
41 0.744977437658166
42 0.862657744659116
43 0.94594660965444
44 0.991523568429987
45 0.997571611465785
46 0.963849622371702
47 0.891701990437027
48 0.784005014071979
49 0.64505223186677
50 0.480383252757061
51 0.296562909296943
52 0.100919538501534
53 0.0987471758239116
54 0.294477151863991
55 0.478467253135642
56 0.643382374915504
57 0.782647871717975
58 0.890711667663229
59 0.963265600221956
60 0.997417173060214
61 0.991804870740461
62 0.946652438045543
63 0.863759959980264
64 0.746432098062747
65 0.599346343898164
66 0.428366542349119
67 0.240309118545409
68 0.0426713285245685
69 0.156667632707382
70 0.349760749816594
71 0.528910009564489
72 0.6869732963031
73 0.817649125587703
74 0.915727864476146
75 0.977299423154306
76 0.999909137877973
77 0.982655630670196
78 0.926226744416757
79 0.832872120740934
80 0.706313513891132
81 0.551596416143672
82 0.374888909947712
83 0.183235765942503
84 0.0157224098169375
85 0.21405378271191
86 0.40385150677593
87 0.57754894569192
88 0.728221330704263
89 0.849861829296724
90 0.937621018649211
91 0.988000216822378
92 0.998990964165813
93 0.970155094266243
94 0.902642202259713
95 0.799143814101274
96 0.663786083918752
97 0.501965297268506
98 0.32013273825926
99 0.125537497212892
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.859719913941957
1 0.755737588329208
2 0.643347017607994
3 0.474468593482949
4 0.287788049033217
5 0.116558935092727
6 0.126986801326773
7 0.364813682656841
8 0.488607667718298
9 0.665647782666583
10 0.791864785545156
11 0.890993430484474
12 0.976714708449954
13 0.99958973918579
14 0.981541365303902
15 0.93407505496231
16 0.848215068528733
17 0.742057089819116
18 0.601075704073858
19 0.38398859855598
20 0.250657496133863
21 0.0716267841942216
22 0.1800635711945
23 0.3464007042206
24 0.550559550060872
25 0.698732083313135
26 0.829066868266484
27 0.930288602871403
28 0.979432795585706
29 0.99999044526165
30 0.975939337885604
31 0.905560692969079
32 0.815524938574083
33 0.687002766584705
34 0.516397007049996
35 0.332648805646895
36 0.09716132034728
37 0.0784127906997064
38 0.243117971204953
39 0.395134056175823
40 0.58372558079684
41 0.75280139351839
42 0.86717882128976
43 0.935689696457238
44 0.98890114924622
45 0.997160786748449
46 0.955218017694314
47 0.888987220246017
48 0.797060186384163
49 0.616136322635336
50 0.499333480881168
51 0.251009533979221
52 0.121412811850314
53 0.0954184542322737
54 0.278711529846857
55 0.490589667009934
56 0.611877595467531
57 0.780859229068378
58 0.892714919173253
59 0.961638637869564
60 0.994905421853875
61 0.99396862310011
62 0.953072199187352
63 0.842677258100035
64 0.743933774136306
65 0.571012996506378
66 0.454949269950174
67 0.237076388448214
68 0.0419775180993033
69 0.17889683706597
70 0.393422897107346
71 0.566546753112319
72 0.66788160536353
73 0.825478208158015
74 0.920345490701357
75 0.967969174961059
76 0.999974883457671
77 0.982039953531428
78 0.924833386297212
79 0.814434759963214
80 0.715719591100061
81 0.560133147082447
82 0.338020543621799
83 0.23043166573871
84 0.0147234784035594
85 0.240654409666959
86 0.366605107660231
87 0.604712826412052
88 0.750528478801801
89 0.868565851088375
90 0.95573177100129
91 0.987850492429112
92 0.996633790294217
93 0.97175652113621
94 0.904861888299493
95 0.781351736214848
96 0.684609494822714
97 0.471662591856448
98 0.322132761269204
99 0.166745989367041
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.896112263202667
1 0.784106254577637
2 0.621050000190735
3 0.597083806991577
4 0.730338513851166
5 0.825838029384613
6 0.732579529285431
7 0.445900738239288
8 0.498706668615341
9 0.661320805549622
10 0.819013774394989
11 0.906128942966461
12 0.972504913806915
13 0.999633133411407
14 0.981501042842865
15 0.936474442481995
16 0.837105274200439
17 0.72370582818985
18 0.760472476482391
19 0.652332186698914
20 0.527234673500061
21 0.729733109474182
22 0.838299810886383
23 0.36089876294136
24 0.574885547161102
25 0.756979167461395
26 0.848868489265442
27 0.92446768283844
28 0.978242576122284
29 0.998892724514008
30 0.972406804561615
31 0.914472579956055
32 0.831008076667786
33 0.698403477668762
34 0.712594509124756
35 0.516063928604126
36 0.757163047790527
37 0.769396901130676
38 0.573079764842987
39 0.99536919593811
40 0.614116609096527
41 0.765809059143066
42 0.890622138977051
43 0.927532613277435
44 0.987555503845215
45 0.997861266136169
46 0.953752398490906
47 0.874174356460571
48 0.820500075817108
49 0.663492023944855
50 0.516298234462738
51 0.973366796970367
52 0.774484515190125
53 0.840338349342346
54 0.451351404190063
55 0.536858916282654
56 0.639322996139526
57 0.80609142780304
58 0.88707035779953
59 0.95922589302063
60 0.992377877235413
61 0.996359944343567
62 0.951028943061829
63 0.861415565013885
64 0.722747266292572
65 0.603050887584686
66 0.687308013439178
67 0.534270346164703
68 0.7501220703125
69 0.755885541439056
70 0.356185227632523
71 0.572905838489532
72 0.674728751182556
73 0.825600862503052
74 0.92787629365921
75 0.96915328502655
76 0.996412992477417
77 0.978688955307007
78 0.910427331924438
79 0.827182769775391
80 0.692267060279846
81 0.627093374729156
82 0.352682173252106
83 0.333024591207504
84 0.839948773384094
85 0.629530668258667
86 0.538595616817474
87 0.705763459205627
88 0.732646226882935
89 0.885183155536652
90 0.954160153865814
91 0.986360847949982
92 0.996669709682465
93 0.975669026374817
94 0.903982520103455
95 0.810751855373383
96 0.73068755865097
97 0.459496855735779
98 0.740352869033813
99 0.929303526878357
};

\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_2(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
title style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_2(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_3(t)|\)},
xtick style={color=white},
xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}

\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.824356457355511
1 0.824356457355511
2 0.824356457355511
3 0.824356457355511
4 0.824356457355511
5 0.824356457355511
6 0.824356457355511
7 0.824356457355511
8 0.824356457355511
9 0.824356457355511
10 0.824356457355511
11 0.824356457355511
12 0.824356457355511
13 0.824356457355511
14 0.824356457355511
15 0.824356457355511
16 0.824356457355511
17 0.824356457355511
18 0.824356457355511
19 0.824356457355511
20 0.824356457355511
21 0.824356457355511
22 0.824356457355511
23 0.824356457355511
24 0.824356457355511
25 0.824356457355511
26 0.824356457355511
27 0.824356457355511
28 0.824356457355511
29 0.824356457355511
30 0.824356457355511
31 0.824356457355511
32 0.824356457355511
33 0.824356457355511
34 0.824356457355511
35 0.824356457355511
36 0.824356457355511
37 0.824356457355511
38 0.824356457355511
39 0.824356457355511
40 0.824356457355511
41 0.824356457355511
42 0.824356457355511
43 0.824356457355511
44 0.824356457355511
45 0.824356457355511
46 0.824356457355511
47 0.824356457355511
48 0.824356457355511
49 0.824356457355511
50 0.824356457355511
51 0.824356457355511
52 0.824356457355511
53 0.824356457355511
54 0.824356457355511
55 0.824356457355511
56 0.824356457355511
57 0.824356457355511
58 0.824356457355511
59 0.824356457355511
60 0.824356457355511
61 0.824356457355511
62 0.824356457355511
63 0.824356457355511
64 0.824356457355511
65 0.824356457355511
66 0.824356457355511
67 0.824356457355511
68 0.824356457355511
69 0.824356457355511
70 0.824356457355511
71 0.824356457355511
72 0.824356457355511
73 0.824356457355511
74 0.824356457355511
75 0.824356457355511
76 0.824356457355511
77 0.824356457355511
78 0.824356457355511
79 0.824356457355511
80 0.824356457355511
81 0.824356457355511
82 0.824356457355511
83 0.824356457355511
84 0.824356457355511
85 0.824356457355511
86 0.824356457355511
87 0.824356457355511
88 0.824356457355511
89 0.824356457355511
90 0.824356457355511
91 0.824356457355511
92 0.824356457355511
93 0.824356457355511
94 0.824356457355511
95 0.824356457355511
96 0.824356457355511
97 0.824356457355511
98 0.824356457355511
99 0.824356457355511
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.826540947233242
1 0.819424773257713
2 0.804872033414668
3 0.865606062620927
4 0.777678244263585
5 0.655955416751701
6 0.848650693271306
7 0.794590157471704
8 0.821831653694203
9 0.832794235543854
10 0.798015731706111
11 0.820825223701301
12 0.828508402244903
13 0.822372902123947
14 0.836247248456819
15 0.839385190840408
16 0.851810630691211
17 0.810721598959815
18 0.825413726814964
19 0.83676119545054
20 0.824307246291034
21 0.660110892803132
22 0.850013821767565
23 0.817966357388691
24 0.837151436690736
25 0.819481975949941
26 0.830731163231527
27 0.826505268824269
28 0.83058514358132
29 0.840086844772135
30 0.822399180329911
31 0.843361574389196
32 0.802829977094809
33 0.841353445699649
34 0.807793622914511
35 0.874935037008936
36 0.904178536689817
37 0.834568502063561
38 0.836108742445472
39 0.848122081076876
40 0.817174550106403
41 0.817313820237078
42 0.820841571476794
43 0.835726879928091
44 0.812274350273978
45 0.827695839185652
46 0.828468062195397
47 0.81325039925252
48 0.828268000167049
49 0.836449926003631
50 0.805099337083494
51 0.87897812713652
52 0.680857908096823
53 0.694543675558109
54 0.8941009528934
55 0.829638591073853
56 0.845349828915478
57 0.831795983316285
58 0.845832952664838
59 0.82947501512382
60 0.831614683145904
61 0.827204657197532
62 0.808660678817778
63 0.826428318128211
64 0.824973707866826
65 0.831545782581599
66 0.801667475604147
67 0.823717081295724
68 0.834151067363765
69 0.803416172156838
70 0.798441184563678
71 0.79993008374775
72 0.813082595349754
73 0.818959790995159
74 0.82730504328271
75 0.828448022269997
76 0.84250966340216
77 0.815742319560368
78 0.861350865837705
79 0.811832849795786
80 0.79336503443531
81 0.803304354348032
82 0.812598363473114
83 0.871443239542551
84 0.977204558969898
85 0.811299441799603
86 0.825062669473339
87 0.837757120078928
88 0.804875979480896
89 0.847553601708448
90 0.829815153410605
91 0.812931347061677
92 0.822094055224205
93 0.814550603198951
94 0.827202036850577
95 0.83596320654818
96 0.808382297184837
97 0.860735088777019
98 0.838861047286953
99 0.896552210304566
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.816566526889801
1 0.868033349514008
2 0.810758054256439
3 0.532822728157043
4 0.847005844116211
5 0.542730450630188
6 0.423398226499557
7 0.825062990188599
8 0.822705209255219
9 0.857623040676117
10 0.778400063514709
11 0.784295976161957
12 0.838804423809052
13 0.826869606971741
14 0.850032985210419
15 0.824496805667877
16 0.84345805644989
17 0.799221217632294
18 0.792388439178467
19 0.493352591991425
20 0.729737401008606
21 0.684801340103149
22 0.418263763189316
23 0.712445318698883
24 0.768141150474548
25 0.851179122924805
26 0.843671202659607
27 0.780195891857147
28 0.836650431156158
29 0.852635264396667
30 0.825260579586029
31 0.839635074138641
32 0.817202746868134
33 0.767287254333496
34 0.877543270587921
35 0.635602414608002
36 0.846453189849854
37 0.872500836849213
38 0.483948528766632
39 0.363612651824951
40 0.698034524917603
41 0.834848642349243
42 0.794353127479553
43 0.827227711677551
44 0.818505227565765
45 0.812182426452637
46 0.849139988422394
47 0.816254556179047
48 0.850996375083923
49 0.891075551509857
50 0.731005668640137
51 0.29812753200531
52 0.812262654304504
53 0.257759302854538
54 0.614302396774292
55 0.884284555912018
56 0.753404915332794
57 0.774314880371094
58 0.821380198001862
59 0.829044163227081
60 0.829582929611206
61 0.840172469615936
62 0.815428853034973
63 0.867463946342468
64 0.852774977684021
65 0.720768809318542
66 0.977106213569641
67 0.73011988401413
68 0.880260944366455
69 0.61493992805481
70 0.798088312149048
71 0.803270995616913
72 0.847319900989532
73 0.834097385406494
74 0.826774656772614
75 0.83941125869751
76 0.836986184120178
77 0.799691557884216
78 0.860862910747528
79 0.827206015586853
80 0.72033154964447
81 0.656246960163116
82 0.75285404920578
83 0.523941457271576
84 0.574171185493469
85 0.711109459400177
86 0.555841743946075
87 0.764482975006104
88 0.804047048091888
89 0.855648458003998
90 0.861877620220184
91 0.800110101699829
92 0.831266522407532
93 0.814167737960815
94 0.82015997171402
95 0.840246319770813
96 0.820859551429749
97 0.707733809947968
98 0.927810490131378
99 0.156269371509552
};


\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_3(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_3(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_4(t)|\)},
xtick style={color=white},
xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.753602486017811
1 0.753602486017811
2 0.753602486017811
3 0.753602486017811
4 0.753602486017811
5 0.753602486017811
6 0.753602486017811
7 0.753602486017811
8 0.753602486017811
9 0.753602486017811
10 0.753602486017811
11 0.753602486017811
12 0.753602486017811
13 0.753602486017811
14 0.753602486017811
15 0.753602486017811
16 0.753602486017811
17 0.753602486017811
18 0.753602486017811
19 0.753602486017811
20 0.753602486017811
21 0.753602486017811
22 0.753602486017811
23 0.753602486017811
24 0.753602486017811
25 0.753602486017811
26 0.753602486017811
27 0.753602486017811
28 0.753602486017811
29 0.753602486017811
30 0.753602486017811
31 0.753602486017811
32 0.753602486017811
33 0.753602486017811
34 0.753602486017811
35 0.753602486017811
36 0.753602486017811
37 0.753602486017811
38 0.753602486017811
39 0.753602486017811
40 0.753602486017811
41 0.753602486017811
42 0.753602486017811
43 0.753602486017811
44 0.753602486017811
45 0.753602486017811
46 0.753602486017811
47 0.753602486017811
48 0.753602486017811
49 0.753602486017811
50 0.753602486017811
51 0.753602486017811
52 0.753602486017811
53 0.753602486017811
54 0.753602486017811
55 0.753602486017811
56 0.753602486017811
57 0.753602486017811
58 0.753602486017811
59 0.753602486017811
60 0.753602486017811
61 0.753602486017811
62 0.753602486017811
63 0.753602486017811
64 0.753602486017811
65 0.753602486017811
66 0.753602486017811
67 0.753602486017811
68 0.753602486017811
69 0.753602486017811
70 0.753602486017811
71 0.753602486017811
72 0.753602486017811
73 0.753602486017811
74 0.753602486017811
75 0.753602486017811
76 0.753602486017811
77 0.753602486017811
78 0.753602486017811
79 0.753602486017811
80 0.753602486017811
81 0.753602486017811
82 0.753602486017811
83 0.753602486017811
84 0.753602486017811
85 0.753602486017811
86 0.753602486017811
87 0.753602486017811
88 0.753602486017811
89 0.753602486017811
90 0.753602486017811
91 0.753602486017811
92 0.753602486017811
93 0.753602486017811
94 0.753602486017811
95 0.753602486017811
96 0.753602486017811
97 0.753602486017811
98 0.753602486017811
99 0.753602486017811
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.747436131415993
1 0.741222653010174
2 0.768491290815899
3 0.732831057940062
4 0.788968727334754
5 0.781523044354397
6 0.768464140104341
7 0.754290664012421
8 0.768002777875057
9 0.763830466720713
10 0.759304274219105
11 0.757304783825262
12 0.77174654178956
13 0.747463042364562
14 0.756593959167755
15 0.733895338906438
16 0.77149826769973
17 0.782196234290288
18 0.719282566684846
19 0.773088142181832
20 0.751805782021548
21 0.76453230811211
22 0.78305671084342
23 0.784621783550346
24 0.761632588358648
25 0.768487961878287
26 0.729445137880061
27 0.765981381572216
28 0.761286291126875
29 0.771483925619734
30 0.755179840775135
31 0.749828959579388
32 0.751613594208963
33 0.729979657382005
34 0.747132280818803
35 0.702066999684423
36 0.738111037714361
37 0.772044120315298
38 0.746415915432855
39 0.766462617556781
40 0.760264498143183
41 0.748700282094936
42 0.755902316824013
43 0.759778306267267
44 0.765184828285714
45 0.786157057961869
46 0.770330419986821
47 0.749458571435389
48 0.777978455855874
49 0.769559678304843
50 0.752524526619659
51 0.704723110738617
52 0.747454100841267
53 0.759286996955909
54 0.768755125583407
55 0.75467339568607
56 0.792784242178326
57 0.773205146766487
58 0.729622371064921
59 0.769636562099829
60 0.736180136031724
61 0.757422614078146
62 0.729894215993393
63 0.781848057588544
64 0.763983911645917
65 0.763718095015186
66 0.737446839693683
67 0.732424955937391
68 0.762921132581683
69 0.749796062806807
70 0.783149148070319
71 0.727237113588697
72 0.757158244246737
73 0.751032453780872
74 0.760242651676678
75 0.780125279488765
76 0.749878437523745
77 0.7423139821433
78 0.766679487800028
79 0.742821218968286
80 0.774510376746771
81 0.785584120109832
82 0.76296006749827
83 0.742049222001473
84 0.780708779089099
85 0.74457630103349
86 0.761821612859588
87 0.759286431698995
88 0.747003161340513
89 0.743544852904519
90 0.770955775165889
91 0.736224093370398
92 0.757521894957827
93 0.770319432628854
94 0.757657491712039
95 0.752749140442933
96 0.76539503758596
97 0.720636362081036
98 0.76862345883944
99 0.732744103555897
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.715893685817719
1 0.703742980957031
2 0.790317177772522
3 0.909020066261292
4 0.384326368570328
5 0.14362071454525
6 0.202442839741707
7 0.816742539405823
8 0.664750158786774
9 0.799162745475769
10 0.654133558273315
11 0.778363108634949
12 0.770860731601715
13 0.774044871330261
14 0.738780379295349
15 0.719707906246185
16 0.81030946969986
17 0.795972943305969
18 0.656051278114319
19 0.840979218482971
20 0.305919408798218
21 0.168176800012589
22 0.191365092992783
23 0.737352788448334
24 0.634682238101959
25 0.836254596710205
26 0.74436366558075
27 0.776040494441986
28 0.791094899177551
29 0.786548733711243
30 0.764384090900421
31 0.721013724803925
32 0.735079169273376
33 0.777189671993256
34 0.664565443992615
35 0.747229814529419
36 0.109183676540852
37 0.0963659584522247
38 0.503385663032532
39 0.678862273693085
40 0.80634731054306
41 0.781318485736847
42 0.750227570533752
43 0.750225007534027
44 0.790806412696838
45 0.764255225658417
46 0.784168720245361
47 0.77904200553894
48 0.768303096294403
49 0.733912467956543
50 0.789943277835846
51 0.548327207565308
52 0.0944150909781456
53 0.304048776626587
54 0.599563300609589
55 0.709515571594238
56 0.687747776508331
57 0.680862605571747
58 0.726064383983612
59 0.77474844455719
60 0.737335801124573
61 0.730059623718262
62 0.732712805271149
63 0.770362257957458
64 0.782949149608612
65 0.814985811710358
66 0.635097205638885
67 0.428887695074081
68 0.0824344232678413
69 0.198459610342979
70 0.739004254341125
71 0.77780419588089
72 0.784786224365234
73 0.76804780960083
74 0.727199077606201
75 0.796531319618225
76 0.77484542131424
77 0.748632848262787
78 0.779736220836639
79 0.720683336257935
80 0.817530930042267
81 0.861157357692719
82 0.798073589801788
83 0.759356260299683
84 0.138287797570229
85 0.330455899238586
86 0.825170576572418
87 0.795937120914459
88 0.737944960594177
89 0.754342257976532
90 0.798763275146484
91 0.710640668869019
92 0.779930651187897
93 0.763602614402771
94 0.802083075046539
95 0.741464078426361
96 0.740532398223877
97 0.848914325237274
98 0.556735873222351
99 0.703161537647247
};

\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_5(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_5(t)|\)},
%xtick style={color=white},
%xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.935826238137458
1 0.935826238137458
2 0.935826238137458
3 0.935826238137458
4 0.935826238137458
5 0.935826238137458
6 0.935826238137458
7 0.935826238137458
8 0.935826238137458
9 0.935826238137458
10 0.935826238137458
11 0.935826238137458
12 0.935826238137458
13 0.935826238137458
14 0.935826238137458
15 0.935826238137458
16 0.935826238137458
17 0.935826238137458
18 0.935826238137458
19 0.935826238137458
20 0.935826238137458
21 0.935826238137458
22 0.935826238137458
23 0.935826238137458
24 0.935826238137458
25 0.935826238137458
26 0.935826238137458
27 0.935826238137458
28 0.935826238137458
29 0.935826238137458
30 0.935826238137458
31 0.935826238137458
32 0.935826238137458
33 0.935826238137458
34 0.935826238137458
35 0.935826238137458
36 0.935826238137458
37 0.935826238137458
38 0.935826238137458
39 0.935826238137458
40 0.935826238137458
41 0.935826238137458
42 0.935826238137458
43 0.935826238137458
44 0.935826238137458
45 0.935826238137458
46 0.935826238137458
47 0.935826238137458
48 0.935826238137458
49 0.935826238137458
50 0.935826238137458
51 0.935826238137458
52 0.935826238137458
53 0.935826238137458
54 0.935826238137458
55 0.935826238137458
56 0.935826238137458
57 0.935826238137458
58 0.935826238137458
59 0.935826238137458
60 0.935826238137458
61 0.935826238137458
62 0.935826238137458
63 0.935826238137458
64 0.935826238137458
65 0.935826238137458
66 0.935826238137458
67 0.935826238137458
68 0.935826238137458
69 0.935826238137458
70 0.935826238137458
71 0.935826238137458
72 0.935826238137458
73 0.935826238137458
74 0.935826238137458
75 0.935826238137458
76 0.935826238137458
77 0.935826238137458
78 0.935826238137458
79 0.935826238137458
80 0.935826238137458
81 0.935826238137458
82 0.935826238137458
83 0.935826238137458
84 0.935826238137458
85 0.935826238137458
86 0.935826238137458
87 0.935826238137458
88 0.935826238137458
89 0.935826238137458
90 0.935826238137458
91 0.935826238137458
92 0.935826238137458
93 0.935826238137458
94 0.935826238137458
95 0.935826238137458
96 0.935826238137458
97 0.935826238137458
98 0.935826238137458
99 0.935826238137458
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.941184688611701
1 0.935323211748447
2 0.929059237855848
3 0.914792242653098
4 0.939254831264456
5 0.942113940536965
6 0.93857669485437
7 0.935663884946413
8 0.940983927256924
9 0.930129227779473
10 0.947499126134199
11 0.92956282634862
12 0.933671909185487
13 0.923242064488913
14 0.940009933690067
15 0.941913790565454
16 0.925801846204041
17 0.94216117473382
18 0.928239771893058
19 0.933162190160001
20 0.93144146956047
21 0.946984113332145
22 0.946243468806825
23 0.936209309993685
24 0.929210060351366
25 0.937578574982768
26 0.936062084866931
27 0.930244325804825
28 0.939008422777631
29 0.936447584736437
30 0.935640152298808
31 0.934053145218873
32 0.937809756324069
33 0.933445182616745
34 0.949408988585583
35 0.914055789999547
36 0.941574706786685
37 0.936943307475191
38 0.937972835068307
39 0.942512897797796
40 0.949761373588322
41 0.917133743011737
42 0.929006599097861
43 0.918199295356459
44 0.927204272824986
45 0.926143163367962
46 0.93605830900982
47 0.938682751572815
48 0.944466506876087
49 0.937927228685663
50 0.942919482286114
51 0.934313417068443
52 0.931297978236343
53 0.923752469445524
54 0.932603119240839
55 0.932872565011093
56 0.929423521134268
57 0.930792782697635
58 0.934807864722542
59 0.9311851597888
60 0.9329023593441
61 0.924906707382433
62 0.924110480620387
63 0.92337919934695
64 0.937510214936659
65 0.933408361908957
66 0.940396745797222
67 0.936983559289792
68 0.922714293452817
69 0.941549381646423
70 0.941284054343501
71 0.941776557586321
72 0.932617745031624
73 0.93994007703254
74 0.941290449409965
75 0.937973596751306
76 0.927782671877467
77 0.941938172483527
78 0.926794382775211
79 0.934792890193547
80 0.954713169192887
81 0.949789429749448
82 0.92243722265121
83 0.931517868870256
84 0.915949372612978
85 0.942002587921457
86 0.949791962059787
87 0.936441580446454
88 0.955636000693879
89 0.930543126599656
90 0.930072619797373
91 0.952376607821398
92 0.946771427747305
93 0.936063450487615
94 0.931788409520615
95 0.930757828786913
96 0.9416437642025
97 0.93578762122867
98 0.946081344142957
99 0.947619525178923
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.967435538768768
1 0.915039539337158
2 0.915594041347504
3 0.902722239494324
4 0.902990937232971
5 0.811268031597137
6 0.742660582065582
7 0.935555279254913
8 0.921059131622314
9 0.934231638908386
10 0.934717357158661
11 0.957887291908264
12 0.924529075622559
13 0.918757259845734
14 0.923328816890717
15 0.938842058181763
16 0.905504703521729
17 0.922539353370667
18 0.9422447681427
19 0.83099901676178
20 0.819939196109772
21 0.820312023162842
22 0.731557428836823
23 0.918813347816467
24 0.89601069688797
25 0.954703569412231
26 0.932897806167603
27 0.947239875793457
28 0.943598747253418
29 0.949932336807251
30 0.924167096614838
31 0.921399056911469
32 0.939464807510376
33 0.967154204845428
34 0.965187788009644
35 0.823184728622437
36 0.824783265590668
37 0.704344868659973
38 0.977818965911865
39 0.954363584518433
40 0.974641263484955
41 0.923281788825989
42 0.933274984359741
43 0.921399891376495
44 0.933297991752625
45 0.944844245910645
46 0.933453321456909
47 0.933178603649139
48 0.948855578899384
49 0.938444972038269
50 0.891266524791718
51 0.885418832302094
52 0.815954506397247
53 0.840871393680573
54 0.926452279090881
55 0.904199600219727
56 0.913838088512421
57 0.920070171356201
58 0.942822694778442
59 0.92988532781601
60 0.944118976593018
61 0.924587666988373
62 0.902326166629791
63 0.897426545619965
64 0.900826871395111
65 0.943975746631622
66 0.908031225204468
67 0.929252803325653
68 0.734747052192688
69 0.563104748725891
70 0.929799258708954
71 0.954916715621948
72 0.937402963638306
73 0.942984282970428
74 0.93269556760788
75 0.933507978916168
76 0.934811294078827
77 0.952864587306976
78 0.906834721565247
79 0.939145624637604
80 0.969024181365967
81 0.962307989597321
82 0.890000402927399
83 0.909395217895508
84 0.674494385719299
85 0.767891466617584
86 0.977625131607056
87 0.971144616603851
88 0.948235988616943
89 0.933611273765564
90 0.921213924884796
91 0.945073485374451
92 0.951287746429443
93 0.945690929889679
94 0.949107527732849
95 0.949279189109802
96 0.962550640106201
97 0.879135251045227
98 0.884525954723358
99 0.968007445335388
};

\end{groupplot}

==> Figs/structured_phi_change/noise_0.01_cc.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm }]
\nextgroupplot[
anchor=north west,
at={($(left plots c1r1.north east) + (0.2cm,0)$)},
width=\w cm,
height=\h cm,
legend cell align={left},
legend style={at={(0,2)}, anchor=north west, legend cell align=left, align=left, font=\footnotesize, draw=white!15!black},
legend columns=3,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black,font=\footnotesize},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_0(t)|\)},
title style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
ytick style={color=black,font=\footnotesize},
%-------- Horizantal ----
%xtick style={color=black,font=\footnotesize},
%xlabel = {time \(t\)},
%title={\(\displaystyle |\cos\phi_1(t)|\)},
%-------- Vertical ----
xtick style={color=white,font=\footnotesize},
xticklabels ={},
yticklabels={},
ytick style={color=white},
%xlabel = {time \(t\)},
%ylabel={\(\displaystyle |\cos\phi_1(t)|\)},
% xtick style={color=white},
% xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.934585425251987
1 0.934585425251987
2 0.934585425251987
3 0.934585425251987
4 0.934585425251987
5 0.934585425251987
6 0.934585425251987
7 0.934585425251987
8 0.934585425251987
9 0.934585425251987
10 0.934585425251987
11 0.934585425251987
12 0.934585425251987
13 0.934585425251987
14 0.934585425251987
15 0.934585425251987
16 0.934585425251987
17 0.934585425251987
18 0.934585425251987
19 0.934585425251987
20 0.934585425251987
21 0.934585425251987
22 0.934585425251987
23 0.934585425251987
24 0.934585425251987
25 0.934585425251987
26 0.934585425251987
27 0.934585425251987
28 0.934585425251987
29 0.934585425251987
30 0.934585425251987
31 0.934585425251987
32 0.934585425251987
33 0.934585425251987
34 0.934585425251987
35 0.934585425251987
36 0.934585425251987
37 0.934585425251987
38 0.934585425251987
39 0.934585425251987
40 0.934585425251987
41 0.934585425251987
42 0.934585425251987
43 0.934585425251987
44 0.934585425251987
45 0.934585425251987
46 0.934585425251987
47 0.934585425251987
48 0.934585425251987
49 0.934585425251987
50 0.934585425251987
51 0.934585425251987
52 0.934585425251987
53 0.934585425251987
54 0.934585425251987
55 0.934585425251987
56 0.934585425251987
57 0.934585425251987
58 0.934585425251987
59 0.934585425251987
60 0.934585425251987
61 0.934585425251987
62 0.934585425251987
63 0.934585425251987
64 0.934585425251987
65 0.934585425251987
66 0.934585425251987
67 0.934585425251987
68 0.934585425251987
69 0.934585425251987
70 0.934585425251987
71 0.934585425251987
72 0.934585425251987
73 0.934585425251987
74 0.934585425251987
75 0.934585425251987
76 0.934585425251987
77 0.934585425251987
78 0.934585425251987
79 0.934585425251987
80 0.934585425251987
81 0.934585425251987
82 0.934585425251987
83 0.934585425251987
84 0.934585425251987
85 0.934585425251987
86 0.934585425251987
87 0.934585425251987
88 0.934585425251987
89 0.934585425251987
90 0.934585425251987
91 0.934585425251987
92 0.934585425251987
93 0.934585425251987
94 0.934585425251987
95 0.934585425251987
96 0.934585425251987
97 0.934585425251987
98 0.934585425251987
99 0.934585425251987
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.934585431214913
1 0.934585426098896
2 0.934585420591209
3 0.934585418191416
4 0.93468273555785
5 0.934585425431515
6 0.934585430261045
7 0.934585433598933
8 0.9345854086599
9 0.934585437374921
10 0.934592079533547
11 0.934564346576743
12 0.944350170187034
13 0.934585521656722
14 0.934585438344548
15 0.934585433963282
16 0.934585429890294
17 0.934585424391272
18 0.934585419424479
19 0.934585418407034
20 0.934585421774201
21 0.934585426953012
22 0.934585431403827
23 0.934585434293272
24 0.934585436095802
25 0.934577341954923
26 0.934584926738341
27 0.934948977686535
28 0.934609413330012
29 0.934605507917343
30 0.934585436788302
31 0.934585432882624
32 0.934585428417369
33 0.93458542271582
34 0.934585418619935
35 0.934585419018938
36 0.934585423238394
37 0.934585428399158
38 0.934585432405049
39 0.934625113133391
40 0.934183265914122
41 0.934585439191436
42 0.934586089849711
43 0.926739274837187
44 0.934585480557661
45 0.934589370757231
46 0.934585435530227
47 0.934585431735041
48 0.934585426810531
49 0.934585421176882
50 0.934585418227902
51 0.93474892226751
52 0.934585424775264
53 0.934585429734043
54 0.934585433270172
55 0.934585917459128
56 0.934585437112986
57 0.934586606686692
58 0.934586227035272
59 0.948575458414014
60 0.934585456646936
61 0.934585439149386
62 0.934585434417992
63 0.934585430470052
64 0.934585425117415
65 0.934585419879247
66 0.934585418264797
67 0.93458542119429
68 0.934585426314134
69 0.934585430936332
70 0.934585434011777
71 0.93458543589701
72 0.934585437780284
73 0.93458945392668
74 0.934630184086129
75 0.93536901440796
76 0.934585447954218
77 0.934585437400777
78 0.934585433345607
79 0.934585429060162
80 0.934585423416156
81 0.934585418913028
82 0.934585418713982
83 0.934585422603891
84 0.934585427797518
85 0.934585431997428
86 0.932636974620937
87 0.934585436368202
88 0.934585438689854
89 0.934585512366819
90 0.933080225635529
91 0.934588044941244
92 0.93458544297225
93 0.934585436038688
94 0.934585432233761
95 0.934585427506252
96 0.934585421806168
97 0.934585418341994
98 0.934582959868959
99 0.934585424119207
};
%\addlegendentry{Netwrok}
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.934585392475128
1 0.934585452079773
2 0.934585452079773
3 0.934585452079773
4 0.934585392475128
5 0.934585392475128
6 0.934585392475128
7 0.934585392475128
8 0.934585392475128
9 0.934585392475128
10 0.934585452079773
11 0.934585571289062
12 0.93458491563797
13 0.934585332870483
14 0.934585392475128
15 0.934585392475128
16 0.934585452079773
17 0.934585452079773
18 0.934585452079773
19 0.934585452079773
20 0.934585392475128
21 0.934585392475128
22 0.934585392475128
23 0.934585392475128
24 0.934585392475128
25 0.934585392475128
26 0.934585452079773
27 0.934585630893707
28 0.934585154056549
29 0.934585332870483
30 0.934585392475128
31 0.934585392475128
32 0.934585452079773
33 0.934585452079773
34 0.934585452079773
35 0.934585452079773
36 0.934585392475128
37 0.934585392475128
38 0.934585392475128
39 0.934585392475128
40 0.934585392475128
41 0.934585392475128
42 0.934585452079773
43 0.93458616733551
44 0.934585273265839
45 0.934585332870483
46 0.934585392475128
47 0.934585392475128
48 0.934585452079773
49 0.934585452079773
50 0.934585452079773
51 0.934585392475128
52 0.934585392475128
53 0.934585392475128
54 0.934585392475128
55 0.934585392475128
56 0.934585392475128
57 0.934585452079773
58 0.934585511684418
59 0.934584498405457
60 0.934585273265839
61 0.934585392475128
62 0.934585392475128
63 0.934585392475128
64 0.934585452079773
65 0.934585452079773
66 0.934585452079773
67 0.934585392475128
68 0.934585392475128
69 0.934585392475128
70 0.934585392475128
71 0.934585392475128
72 0.934585392475128
73 0.934585452079773
74 0.934585571289062
75 0.934585094451904
76 0.934585332870483
77 0.934585392475128
78 0.934585392475128
79 0.934585452079773
80 0.934585452079773
81 0.934585452079773
82 0.934585452079773
83 0.934585392475128
84 0.934585392475128
85 0.934585392475128
86 0.934585392475128
87 0.934585392475128
88 0.934585392475128
89 0.934585452079773
90 0.934585809707642
91 0.934585213661194
92 0.934585332870483
93 0.934585392475128
94 0.934585392475128
95 0.934585452079773
96 0.934585452079773
97 0.934585452079773
98 0.934585392475128
99 0.934585392475128
};
%\addlegendentry{Inverse Scattering}

\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
title style ={color=black,font=\footnotesize},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_1(t)|\)},
ymin=0, ymax=1.2,
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_2(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_2(t)|\)},
xtick style={color=white},
xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.478643591525743
1 0.478643591525743
2 0.478643591525743
3 0.478643591525743
4 0.478643591525743
5 0.478643591525743
6 0.478643591525743
7 0.478643591525743
8 0.478643591525743
9 0.478643591525743
10 0.478643591525743
11 0.478643591525743
12 0.478643591525743
13 0.478643591525743
14 0.478643591525743
15 0.478643591525743
16 0.478643591525743
17 0.478643591525743
18 0.478643591525743
19 0.478643591525743
20 0.478643591525743
21 0.478643591525743
22 0.478643591525743
23 0.478643591525743
24 0.478643591525743
25 0.478643591525743
26 0.478643591525743
27 0.478643591525743
28 0.478643591525743
29 0.478643591525743
30 0.478643591525743
31 0.478643591525743
32 0.478643591525743
33 0.478643591525743
34 0.478643591525743
35 0.478643591525743
36 0.478643591525743
37 0.478643591525743
38 0.478643591525743
39 0.478643591525743
40 0.478643591525743
41 0.478643591525743
42 0.478643591525743
43 0.478643591525743
44 0.478643591525743
45 0.478643591525743
46 0.478643591525743
47 0.478643591525743
48 0.478643591525743
49 0.478643591525743
50 0.478643591525743
51 0.478643591525743
52 0.478643591525743
53 0.478643591525743
54 0.478643591525743
55 0.478643591525743
56 0.478643591525743
57 0.478643591525743
58 0.478643591525743
59 0.478643591525743
60 0.478643591525743
61 0.478643591525743
62 0.478643591525743
63 0.478643591525743
64 0.478643591525743
65 0.478643591525743
66 0.478643591525743
67 0.478643591525743
68 0.478643591525743
69 0.478643591525743
70 0.478643591525743
71 0.478643591525743
72 0.478643591525743
73 0.478643591525743
74 0.478643591525743
75 0.478643591525743
76 0.478643591525743
77 0.478643591525743
78 0.478643591525743
79 0.478643591525743
80 0.478643591525743
81 0.478643591525743
82 0.478643591525743
83 0.478643591525743
84 0.478643591525743
85 0.478643591525743
86 0.478643591525743
87 0.478643591525743
88 0.478643591525743
89 0.478643591525743
90 0.478643591525743
91 0.478643591525743
92 0.478643591525743
93 0.478643591525743
94 0.478643591525743
95 0.478643591525743
96 0.478643591525743
97 0.478643591525743
98 0.478643591525743
99 0.478643591525743
};

\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.478643604859884
1 0.478643601556364
2 0.478643598949989
3 0.478643595345311
4 0.478643908211273
5 0.47864358775713
6 0.478643588630897
7 0.478643593184963
8 0.478643655165411
9 0.478643615297319
10 0.478359326138315
11 0.478714176989842
12 0.468341373340253
13 0.478658753873573
14 0.478643614131715
15 0.478643607700611
16 0.478643603797501
17 0.478643600774969
18 0.478643598076528
19 0.47864359399288
20 0.478643589499054
21 0.478643587597153
22 0.478643589609184
23 0.478643595144703
24 0.478643604489337
25 0.478631530800847
26 0.478628278331347
27 0.475978696905378
28 0.478821749357796
29 0.478546487277659
30 0.47864361155792
31 0.478643606477063
32 0.478643602809805
33 0.478643600037172
34 0.478643597060102
35 0.478643592589139
36 0.478643588566257
37 0.478643587783996
38 0.478643590883058
39 0.478635289815233
40 0.478425078310208
41 0.47864363039138
42 0.478647055211818
43 0.289749793811144
44 0.478643761403312
45 0.478538916143169
46 0.478643609717391
47 0.478643605329252
48 0.478643601910634
49 0.47864359928724
50 0.478643595886634
51 0.478641185168524
52 0.478643587928772
53 0.478643588309555
54 0.478643592439971
55 0.478643826235874
56 0.478643612993025
57 0.478652135624018
58 0.47866969353922
59 0.271269103072791
60 0.478643790239428
61 0.478643615590229
62 0.478643608256107
63 0.478643604240079
64 0.478643601098506
65 0.47864359846257
66 0.478643594577242
67 0.478643589970481
68 0.47864358762265
69 0.478643589157083
70 0.478643594277765
71 0.478643603050742
72 0.478643618825187
73 0.478643478573165
74 0.478316554421764
75 0.479862988537178
76 0.478643592981795
77 0.478643612531231
78 0.478643606984477
79 0.478643603218597
80 0.478643600348082
81 0.478643597510442
82 0.478643593185786
83 0.478643588928794
84 0.478643587662624
85 0.47864359030754
86 0.478247807375585
87 0.478643606616153
88 0.47864362641326
89 0.478645760605778
90 0.452013850669736
91 0.478672557263093
92 0.478643623517547
93 0.47864361043619
94 0.478643605808852
95 0.478643602280882
96 0.478643599610919
97 0.478643596403091
98 0.478643610576511
99 0.478643588160315
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.478643625974655
1 0.478643625974655
2 0.478643625974655
3 0.478643625974655
4 0.478643625974655
5 0.478643625974655
6 0.478643625974655
7 0.478643506765366
8 0.478643506765366
9 0.478643506765366
10 0.478643506765366
11 0.478643715381622
12 0.478644758462906
13 0.478643625974655
14 0.478643625974655
15 0.478643625974655
16 0.478643625974655
17 0.478643625974655
18 0.478643625974655
19 0.478643625974655
20 0.478643625974655
21 0.478643625974655
22 0.478643625974655
23 0.478643506765366
24 0.478643506765366
25 0.478643506765366
26 0.478643506765366
27 0.478643923997879
28 0.478643834590912
29 0.478643625974655
30 0.478643625974655
31 0.478643625974655
32 0.478643625974655
33 0.478643625974655
34 0.478643625974655
35 0.478643625974655
36 0.478643625974655
37 0.478643625974655
38 0.478643506765366
39 0.478643506765366
40 0.478643506765366
41 0.478643506765366
42 0.478643625974655
43 0.478646665811539
44 0.478643625974655
45 0.478643625974655
46 0.478643625974655
47 0.478643625974655
48 0.478643625974655
49 0.478643625974655
50 0.478643625974655
51 0.478643625974655
52 0.478643625974655
53 0.478643625974655
54 0.478643506765366
55 0.478643506765366
56 0.478643506765366
57 0.478643506765366
58 0.478643625974655
59 0.478648006916046
60 0.478643625974655
61 0.478643625974655
62 0.478643625974655
63 0.478643625974655
64 0.478643625974655
65 0.478643625974655
66 0.478643625974655
67 0.478643625974655
68 0.478643625974655
69 0.478643625974655
70 0.478643506765366
71 0.478643506765366
72 0.478643506765366
73 0.478643506765366
74 0.478643715381622
75 0.478643923997879
76 0.478643625974655
77 0.478643625974655
78 0.478643625974655
79 0.478643625974655
80 0.478643625974655
81 0.478643625974655
82 0.478643625974655
83 0.478643625974655
84 0.478643625974655
85 0.478643506765366
86 0.478643506765366
87 0.478643506765366
88 0.478643506765366
89 0.478643625974655
90 0.478644549846649
91 0.478643715381622
92 0.478643625974655
93 0.478643625974655
94 0.478643625974655
95 0.478643625974655
96 0.478643625974655
97 0.478643625974655
98 0.478643625974655
99 0.478643625974655
};


\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_2(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
title style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_2(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_3(t)|\)},
xtick style={color=white},
xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.712345499463509
1 0.837577905757982
2 0.929418724079809
3 0.984206550822962
4 0.999757168228175
5 0.975450622252314
6 0.912255938179696
7 0.812692488641937
8 0.680729554181475
9 0.521628080562128
10 0.341730941463365
11 0.148210068122804
12 0.0512194729298976
13 0.248607055229278
14 0.436083458761596
15 0.606174590934022
16 0.752099455060446
17 0.868040487300687
18 0.949375484572409
19 0.992861877201816
20 0.996765999944021
21 0.960932207745464
22 0.88678908082103
23 0.777292471669031
24 0.636807664559825
25 0.47093534542741
26 0.286288320195225
27 0.090227883071894
28 0.109429655018964
29 0.304724578089461
30 0.487871093845545
31 0.651567728656271
32 0.78928841426634
33 0.895542661543233
34 0.966094448952688
35 0.998131099369728
36 0.990375412639724
37 0.943136583518115
38 0.858297875051235
39 0.739241538821632
40 0.590713975250785
41 0.418636509592434
42 0.229869327380532
43 0.0319379804805787
44 0.16726663291501
45 0.35980285349666
46 0.53799486973296
47 0.694738728253994
48 0.823785546054376
49 0.919990633739189
50 0.979518598055148
51 0.99999624691633
52 0.980607201083598
53 0.922124440628631
54 0.826879488657745
55 0.698669460843194
56 0.542605686403803
57 0.364909935538753
58 0.172666377083665
59 0.0264608449454876
60 0.224533156588688
61 0.413654039834047
62 0.586283841872031
63 0.735540357260226
64 0.855473199736278
65 0.941301025340636
66 0.98960214951182
67 0.998450958852137
68 0.96749467925722
69 0.897967439906331
70 0.792641072426497
71 0.655714606712566
72 0.492646868856104
73 0.309938854975444
74 0.114874557015529
75 0.0847694270249685
76 0.281033921515376
77 0.466094480408789
78 0.632573323214492
79 0.773833463824188
80 0.88424330620392
81 0.959401158356415
82 0.99631071389067
83 0.993500505302372
84 0.951082566739809
85 0.870747967555927
86 0.755699394709699
87 0.610523471743738
88 0.44100790457758
89 0.253910743936833
90 0.0566909631970113
91 0.142788907346795
92 0.336576234751139
93 0.516945329803683
94 0.676705445872277
95 0.809487451281465
96 0.909997746493431
97 0.974229303216653
98 0.999621411978975
99 0.985161769533474
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.712345483347109
1 0.837577891722236
2 0.929418713972539
3 0.984206546323019
4 0.999756938781126
5 0.975450619366241
6 0.912255921639039
7 0.812692452597909
8 0.680729344155453
9 0.521628010952797
10 0.341596686928427
11 0.148160843176145
12 0.0520318411267242
13 0.248607108515977
14 0.436083450367012
15 0.606174576123736
16 0.752099439200818
17 0.868040474286367
18 0.9493754759139
19 0.992861874471284
20 0.99676600038104
21 0.960932201852315
22 0.886789058883868
23 0.777292429794912
24 0.636807604776188
25 0.470933757914418
26 0.286293730071296
27 0.0910433995737748
28 0.109367530438243
29 0.304802387349099
30 0.487871083193686
31 0.651567712944403
32 0.789288399002115
33 0.895542649645423
34 0.966094441920003
35 0.998131098197071
36 0.990375412386737
37 0.943136573745747
38 0.858297847388909
39 0.739262739296754
40 0.590780238066752
41 0.418636433350377
42 0.229869533691991
43 0.0546174170580168
44 0.167266599859109
45 0.359794972144565
46 0.537994857071523
47 0.694738712155643
48 0.823785531618882
49 0.919990623068661
50 0.979518592787367
51 0.999999454902858
52 0.980607199188124
53 0.922124426234344
54 0.826879455115366
55 0.698669304570421
56 0.542605618340216
57 0.364907576183493
58 0.172666911484646
59 0.0399166976125874
60 0.224533155144106
61 0.413654032420326
62 0.586283827600302
63 0.735540341244187
64 0.855473186276571
65 0.941301016045771
66 0.989602146044819
67 0.998450959312923
68 0.967494674752212
69 0.897967420309016
70 0.792641033008717
71 0.655714548907582
72 0.492646797247192
73 0.309926511597511
74 0.114996982293107
75 0.08443358499733
76 0.281033918410885
77 0.466094470695405
78 0.632573307821267
79 0.773833448272918
80 0.884243293820641
81 0.959401150613401
82 0.996310712096323
83 0.993500505455017
84 0.951082558712253
85 0.870747942351125
86 0.756028939874838
87 0.610523409399664
88 0.441007829691753
89 0.253910512888427
90 0.0613748620827304
91 0.142789942072826
92 0.33657623035403
93 0.516945317953316
94 0.67670542987685
95 0.809487436472173
96 0.909997735286471
97 0.974229297188265
98 0.999621371882625
99 0.985161768453704
};

\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.712345540523529
1 0.837577879428864
2 0.929418683052063
3 0.984206557273865
4 0.999757170677185
5 0.97545063495636
6 0.912256002426147
7 0.812692582607269
8 0.680729627609253
9 0.521628081798553
10 0.341730892658234
11 0.148209974169731
12 0.0512192919850349
13 0.248607039451599
14 0.436083495616913
15 0.60617458820343
16 0.752099454402924
17 0.868040502071381
18 0.949375450611115
19 0.992861866950989
20 0.996766030788422
21 0.96093225479126
22 0.88678914308548
23 0.777292549610138
24 0.63680773973465
25 0.470935374498367
26 0.286288321018219
27 0.0902277082204819
28 0.109429553151131
29 0.304724633693695
30 0.487871199846268
31 0.651567757129669
32 0.789288401603699
33 0.895542681217194
34 0.966094434261322
35 0.998131096363068
36 0.990375459194183
37 0.943136632442474
38 0.858297944068909
39 0.739241600036621
40 0.590714037418365
41 0.418636471033096
42 0.229869246482849
43 0.03193748742342
44 0.167266607284546
45 0.35980287194252
46 0.537994921207428
47 0.694738745689392
48 0.823785543441772
49 0.919990599155426
50 0.979518592357635
51 0.999996244907379
52 0.980607211589813
53 0.92212450504303
54 0.826879560947418
55 0.69866955280304
56 0.542605698108673
57 0.364909946918488
58 0.172666326165199
59 0.026460375636816
60 0.224533215165138
61 0.413654148578644
62 0.58628386259079
63 0.735540390014648
64 0.855473220348358
65 0.941300988197327
66 0.989602148532867
67 0.998450994491577
68 0.96749472618103
69 0.897967517375946
70 0.792641162872314
71 0.655714690685272
72 0.492646932601929
73 0.309938788414001
74 0.114874430000782
75 0.0847693979740143
76 0.281033933162689
77 0.466094523668289
78 0.632573366165161
79 0.773833513259888
80 0.884243309497833
81 0.95940113067627
82 0.996310710906982
83 0.993500530719757
84 0.951082587242126
85 0.870748043060303
86 0.755699455738068
87 0.610523521900177
88 0.441007912158966
89 0.253910720348358
90 0.0566907562315464
91 0.142788842320442
92 0.33657631278038
93 0.516945362091064
94 0.676705479621887
95 0.809487462043762
96 0.909997701644897
97 0.974229276180267
98 0.999621391296387
99 0.985161781311035
};

\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_3(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_3(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_4(t)|\)},
xtick style={color=white},
xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.516420712893647
1 0.516420712893647
2 0.516420712893647
3 0.516420712893647
4 0.516420712893647
5 0.516420712893647
6 0.516420712893647
7 0.516420712893647
8 0.516420712893647
9 0.516420712893647
10 0.516420712893647
11 0.516420712893647
12 0.516420712893647
13 0.516420712893647
14 0.516420712893647
15 0.516420712893647
16 0.516420712893647
17 0.516420712893647
18 0.516420712893647
19 0.516420712893647
20 0.516420712893647
21 0.516420712893647
22 0.516420712893647
23 0.516420712893647
24 0.516420712893647
25 0.516420712893647
26 0.516420712893647
27 0.516420712893647
28 0.516420712893647
29 0.516420712893647
30 0.516420712893647
31 0.516420712893647
32 0.516420712893647
33 0.516420712893647
34 0.516420712893647
35 0.516420712893647
36 0.516420712893647
37 0.516420712893647
38 0.516420712893647
39 0.516420712893647
40 0.516420712893647
41 0.516420712893647
42 0.516420712893647
43 0.516420712893647
44 0.516420712893647
45 0.516420712893647
46 0.516420712893647
47 0.516420712893647
48 0.516420712893647
49 0.516420712893647
50 0.516420712893647
51 0.516420712893647
52 0.516420712893647
53 0.516420712893647
54 0.516420712893647
55 0.516420712893647
56 0.516420712893647
57 0.516420712893647
58 0.516420712893647
59 0.516420712893647
60 0.516420712893647
61 0.516420712893647
62 0.516420712893647
63 0.516420712893647
64 0.516420712893647
65 0.516420712893647
66 0.516420712893647
67 0.516420712893647
68 0.516420712893647
69 0.516420712893647
70 0.516420712893647
71 0.516420712893647
72 0.516420712893647
73 0.516420712893647
74 0.516420712893647
75 0.516420712893647
76 0.516420712893647
77 0.516420712893647
78 0.516420712893647
79 0.516420712893647
80 0.516420712893647
81 0.516420712893647
82 0.516420712893647
83 0.516420712893647
84 0.516420712893647
85 0.516420712893647
86 0.516420712893647
87 0.516420712893647
88 0.516420712893647
89 0.516420712893647
90 0.516420712893647
91 0.516420712893647
92 0.516420712893647
93 0.516420712893647
94 0.516420712893647
95 0.516420712893647
96 0.516420712893647
97 0.516420712893647
98 0.516420712893647
99 0.516420712893647
};
\addplot [semithick, red,line width=\LineWidth pt, dashed]
table {%
0 0.51642072743228
1 0.516420717103747
2 0.516420709639012
3 0.516420704500063
4 0.516420974052382
5 0.516420705957591
6 0.51642071617972
7 0.516420731356859
8 0.516420856547778
9 0.516420772528485
10 0.516804984115483
11 0.516506723753132
12 0.504203771169103
13 0.516401704524543
14 0.516420749522533
15 0.516420735839635
16 0.516420724166591
17 0.516420714626167
18 0.516420707926799
19 0.516420703457684
20 0.516420702730441
21 0.51642070829764
22 0.516420720203406
23 0.516420736421639
24 0.516420755708782
25 0.516457204569368
26 0.516430503686327
27 0.513645030512659
28 0.516613788706871
29 0.51636179136571
30 0.516420745031615
31 0.516420732305364
32 0.516420721085498
33 0.51642071240696
34 0.516420706383696
35 0.516420702725167
36 0.516420703640981
37 0.51642071119357
38 0.516420724589207
39 0.516313384611714
40 0.517802052525521
41 0.516420791882304
42 0.516410475458394
43 0.327862032226756
44 0.516420905172748
45 0.516577199339015
46 0.516420741071601
47 0.516420728860927
48 0.516420718235264
49 0.51642071042002
50 0.516420705017819
51 0.516418547507637
52 0.516420705141182
53 0.516420714596837
54 0.5164207292832
55 0.516419846657614
56 0.516420769243051
57 0.516409261872171
58 0.51636629950546
59 0.308723912361977
60 0.516420596058419
61 0.516420751708623
62 0.516420737367754
63 0.516420725532438
64 0.516420715644751
65 0.516420708632001
66 0.516420703866562
67 0.516420702515615
68 0.516420707234761
69 0.516420718448801
70 0.516420734243557
71 0.516420753120114
72 0.516420777341204
73 0.51641213016057
74 0.516067531518699
75 0.517577164851454
76 0.516420830401071
77 0.516420746848302
78 0.516420733794049
79 0.516420722366799
80 0.516420713318196
81 0.516420707017811
82 0.516420702992908
83 0.516420703183877
84 0.51642070989995
85 0.516420722688085
86 0.521324250597051
87 0.516420759351498
88 0.516420787044201
89 0.516416686847038
90 0.489245985907569
91 0.516368428899441
92 0.516420761522271
93 0.516420742708723
94 0.516420730310186
95 0.516420719413844
96 0.516420711236723
97 0.516420705573876
98 0.516420729165249
99 0.516420704431879
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.516420722007751
1 0.516420722007751
2 0.516420722007751
3 0.516420722007751
4 0.516420722007751
5 0.516420722007751
6 0.516420722007751
7 0.516420722007751
8 0.516420722007751
9 0.516420722007751
10 0.516420722007751
11 0.516420841217041
12 0.516421973705292
13 0.516420722007751
14 0.516420722007751
15 0.516420722007751
16 0.516420722007751
17 0.516420722007751
18 0.516420722007751
19 0.516420722007751
20 0.516420722007751
21 0.516420722007751
22 0.516420722007751
23 0.516420722007751
24 0.516420722007751
25 0.516420722007751
26 0.516420722007751
27 0.516421020030975
28 0.516420960426331
29 0.516420722007751
30 0.516420722007751
31 0.516420722007751
32 0.516420722007751
33 0.516420722007751
34 0.516420722007751
35 0.516420722007751
36 0.516420722007751
37 0.516420722007751
38 0.516420722007751
39 0.516420722007751
40 0.516420722007751
41 0.516420722007751
42 0.516420722007751
43 0.51642382144928
44 0.516420841217041
45 0.516420722007751
46 0.516420722007751
47 0.516420722007751
48 0.516420722007751
49 0.516420722007751
50 0.516420722007751
51 0.516420722007751
52 0.516420722007751
53 0.516420722007751
54 0.516420722007751
55 0.516420722007751
56 0.516420722007751
57 0.516420722007751
58 0.516420841217041
59 0.516425311565399
60 0.516420722007751
61 0.516420722007751
62 0.516420722007751
63 0.516420722007751
64 0.516420722007751
65 0.516420722007751
66 0.516420722007751
67 0.516420722007751
68 0.516420722007751
69 0.516420722007751
70 0.516420722007751
71 0.516420722007751
72 0.516420722007751
73 0.516420722007751
74 0.516420960426331
75 0.516421139240265
76 0.516420722007751
77 0.516420722007751
78 0.516420722007751
79 0.516420722007751
80 0.516420722007751
81 0.516420722007751
82 0.516420722007751
83 0.516420722007751
84 0.516420722007751
85 0.516420722007751
86 0.516420722007751
87 0.516420722007751
88 0.516420722007751
89 0.516420722007751
90 0.516421675682068
91 0.516420841217041
92 0.516420722007751
93 0.516420722007751
94 0.516420722007751
95 0.516420722007751
96 0.516420722007751
97 0.516420722007751
98 0.516420722007751
99 0.516420722007751
};

\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_5(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_5(t)|\)},
%xtick style={color=white},
%xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.708981512006373
1 0.708981512006373
2 0.708981512006373
3 0.708981512006373
4 0.708981512006373
5 0.708981512006373
6 0.708981512006373
7 0.708981512006373
8 0.708981512006373
9 0.708981512006373
10 0.708981512006373
11 0.708981512006373
12 0.708981512006373
13 0.708981512006373
14 0.708981512006373
15 0.708981512006373
16 0.708981512006373
17 0.708981512006373
18 0.708981512006373
19 0.708981512006373
20 0.708981512006373
21 0.708981512006373
22 0.708981512006373
23 0.708981512006373
24 0.708981512006373
25 0.708981512006373
26 0.708981512006373
27 0.708981512006373
28 0.708981512006373
29 0.708981512006373
30 0.708981512006373
31 0.708981512006373
32 0.708981512006373
33 0.708981512006373
34 0.708981512006373
35 0.708981512006373
36 0.708981512006373
37 0.708981512006373
38 0.708981512006373
39 0.708981512006373
40 0.708981512006373
41 0.708981512006373
42 0.708981512006373
43 0.708981512006373
44 0.708981512006373
45 0.708981512006373
46 0.708981512006373
47 0.708981512006373
48 0.708981512006373
49 0.708981512006373
50 0.708981512006373
51 0.708981512006373
52 0.708981512006373
53 0.708981512006373
54 0.708981512006373
55 0.708981512006373
56 0.708981512006373
57 0.708981512006373
58 0.708981512006373
59 0.708981512006373
60 0.708981512006373
61 0.708981512006373
62 0.708981512006373
63 0.708981512006373
64 0.708981512006373
65 0.708981512006373
66 0.708981512006373
67 0.708981512006373
68 0.708981512006373
69 0.708981512006373
70 0.708981512006373
71 0.708981512006373
72 0.708981512006373
73 0.708981512006373
74 0.708981512006373
75 0.708981512006373
76 0.708981512006373
77 0.708981512006373
78 0.708981512006373
79 0.708981512006373
80 0.708981512006373
81 0.708981512006373
82 0.708981512006373
83 0.708981512006373
84 0.708981512006373
85 0.708981512006373
86 0.708981512006373
87 0.708981512006373
88 0.708981512006373
89 0.708981512006373
90 0.708981512006373
91 0.708981512006373
92 0.708981512006373
93 0.708981512006373
94 0.708981512006373
95 0.708981512006373
96 0.708981512006373
97 0.708981512006373
98 0.708981512006373
99 0.708981512006373
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.708981475857687
1 0.708981477243998
2 0.708981478163875
3 0.708981482783321
4 0.708971723157385
5 0.708981510797697
6 0.7089815253972
7 0.70898153429354
8 0.708981608720986
9 0.708981533663388
10 0.708905268942433
11 0.708907663893128
12 0.694824426282846
13 0.708981862704318
14 0.708981467941727
15 0.708981473963501
16 0.708981476406794
17 0.70898147743921
18 0.708981478893019
19 0.708981485472213
20 0.708981499093238
21 0.708981515484532
22 0.708981528666963
23 0.708981535662272
24 0.708981536469992
25 0.708979653407824
26 0.708978477245989
27 0.709866706691344
28 0.709033691394597
29 0.708968730209258
30 0.708981470496728
31 0.708981474856418
32 0.70898147683348
33 0.708981477640032
34 0.70898148008117
35 0.708981488811055
36 0.708981503885661
37 0.708981519872745
38 0.708981531388145
39 0.708963673143009
40 0.709001888191165
41 0.708981528793619
42 0.708981168240736
43 0.724231889815664
44 0.708981408873761
45 0.70897279673014
46 0.70898147224717
47 0.708981475587526
48 0.708981477142914
49 0.708981477959325
50 0.708981481843218
51 0.709841220015659
52 0.708981508752217
53 0.708981523852523
54 0.708981533547006
55 0.708981538813067
56 0.70898153436381
57 0.708982019780397
58 0.708981345695295
59 0.70235334481758
60 0.708981433353536
61 0.708981466487992
62 0.708981473519183
63 0.708981476188791
64 0.708981477361022
65 0.70898147853543
66 0.708981484250266
67 0.708981497124885
68 0.708981513525281
69 0.70898152734527
70 0.708981535147899
71 0.708981536676375
72 0.708981532550602
73 0.708991327482477
74 0.709111051773059
75 0.708400130423345
76 0.708981447474241
77 0.708981469536909
78 0.708981474500572
79 0.708981476667375
80 0.708981477547667
81 0.70898147951287
82 0.708981487318247
83 0.708981501833469
84 0.708981518055371
85 0.708981530302104
86 0.708975993361814
87 0.708981536056751
88 0.708981530090792
89 0.708981498736029
90 0.717051404689412
91 0.708980273592282
92 0.708981458824707
93 0.708981471577935
94 0.708981475294303
95 0.708981477024964
96 0.708981477800911
97 0.708981481019886
98 0.708980884862658
99 0.708981506689679
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.708981513977051
1 0.708981513977051
2 0.708981513977051
3 0.708981513977051
4 0.708981513977051
5 0.708981513977051
6 0.708981454372406
7 0.708981454372406
8 0.708981394767761
9 0.708981394767761
10 0.708981335163116
11 0.708981096744537
12 0.708982527256012
13 0.708981692790985
14 0.708981573581696
15 0.708981513977051
16 0.708981513977051
17 0.708981513977051
18 0.708981513977051
19 0.708981513977051
20 0.708981513977051
21 0.708981454372406
22 0.708981454372406
23 0.708981454372406
24 0.708981394767761
25 0.708981394767761
26 0.708981335163116
27 0.708980917930603
28 0.708981931209564
29 0.70898163318634
30 0.708981573581696
31 0.708981513977051
32 0.708981513977051
33 0.708981513977051
34 0.708981513977051
35 0.708981513977051
36 0.708981513977051
37 0.708981454372406
38 0.708981454372406
39 0.708981454372406
40 0.708981394767761
41 0.708981394767761
42 0.708981215953827
43 0.708979785442352
44 0.708981812000275
45 0.70898163318634
46 0.708981573581696
47 0.708981513977051
48 0.708981513977051
49 0.708981513977051
50 0.708981513977051
51 0.708981513977051
52 0.708981513977051
53 0.708981454372406
54 0.708981454372406
55 0.708981454372406
56 0.708981394767761
57 0.708981394767761
58 0.708981215953827
59 0.708983480930328
60 0.708981692790985
61 0.70898163318634
62 0.708981573581696
63 0.708981513977051
64 0.708981513977051
65 0.708981513977051
66 0.708981513977051
67 0.708981513977051
68 0.708981454372406
69 0.708981454372406
70 0.708981454372406
71 0.708981394767761
72 0.708981394767761
73 0.708981335163116
74 0.708981037139893
75 0.708982110023499
76 0.70898163318634
77 0.708981573581696
78 0.708981513977051
79 0.708981513977051
80 0.708981513977051
81 0.708981513977051
82 0.708981513977051
83 0.708981513977051
84 0.708981454372406
85 0.708981454372406
86 0.708981454372406
87 0.708981394767761
88 0.708981394767761
89 0.708981275558472
90 0.708980560302734
91 0.708981871604919
92 0.70898163318634
93 0.708981573581696
94 0.708981513977051
95 0.708981513977051
96 0.708981513977051
97 0.708981513977051
98 0.708981513977051
99 0.708981513977051
};

\end{groupplot}

==> Figs/structured_phi_change/noise_0.05.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm, group name=left3 plots }]
\nextgroupplot[
anchor=north west,
at={($(left2 plots c1r1.north east) + (0.2cm,0)$)},
width=\w cm,
height=\h cm,
legend cell align={left},
legend style={at={(0,2)}, anchor=north west, legend cell align=left, align=left, font=\footnotesize, draw=white!15!black},
legend columns=3,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black,font=\footnotesize},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_0(t)|\)},
title style ={color=black,font=\footnotesize},
title = {Noise variance = $0.05$},
ymin=0, ymax=1.2,
ytick style={color=black,font=\footnotesize},
%-------- Horizantal ----
%xtick style={color=black,font=\footnotesize},
%xlabel = {time \(t\)},
%title={\(\displaystyle |\cos\phi_1(t)|\)},
%-------- Vertical ----
xtick style={color=white,font=\footnotesize},
xticklabels ={},
yticklabels={},
ytick style={color=white},
%xlabel = {time \(t\)},
%ylabel={\(\displaystyle |\cos\phi_1(t)|\)},
% xtick style={color=white},
% xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.733099880094478
1 0.733099880094478
2 0.733099880094478
3 0.733099880094478
4 0.733099880094478
5 0.733099880094478
6 0.733099880094478
7 0.733099880094478
8 0.733099880094478
9 0.733099880094478
10 0.733099880094478
11 0.733099880094478
12 0.733099880094478
13 0.733099880094478
14 0.733099880094478
15 0.733099880094478
16 0.733099880094478
17 0.733099880094478
18 0.733099880094478
19 0.733099880094478
20 0.733099880094478
21 0.733099880094478
22 0.733099880094478
23 0.733099880094478
24 0.733099880094478
25 0.733099880094478
26 0.733099880094478
27 0.733099880094478
28 0.733099880094478
29 0.733099880094478
30 0.733099880094478
31 0.733099880094478
32 0.733099880094478
33 0.733099880094478
34 0.733099880094478
35 0.733099880094478
36 0.733099880094478
37 0.733099880094478
38 0.733099880094478
39 0.733099880094478
40 0.733099880094478
41 0.733099880094478
42 0.733099880094478
43 0.733099880094478
44 0.733099880094478
45 0.733099880094478
46 0.733099880094478
47 0.733099880094478
48 0.733099880094478
49 0.733099880094478
50 0.733099880094478
51 0.733099880094478
52 0.733099880094478
53 0.733099880094478
54 0.733099880094478
55 0.733099880094478
56 0.733099880094478
57 0.733099880094478
58 0.733099880094478
59 0.733099880094478
60 0.733099880094478
61 0.733099880094478
62 0.733099880094478
63 0.733099880094478
64 0.733099880094478
65 0.733099880094478
66 0.733099880094478
67 0.733099880094478
68 0.733099880094478
69 0.733099880094478
70 0.733099880094478
71 0.733099880094478
72 0.733099880094478
73 0.733099880094478
74 0.733099880094478
75 0.733099880094478
76 0.733099880094478
77 0.733099880094478
78 0.733099880094478
79 0.733099880094478
80 0.733099880094478
81 0.733099880094478
82 0.733099880094478
83 0.733099880094478
84 0.733099880094478
85 0.733099880094478
86 0.733099880094478
87 0.733099880094478
88 0.733099880094478
89 0.733099880094478
90 0.733099880094478
91 0.733099880094478
92 0.733099880094478
93 0.733099880094478
94 0.733099880094478
95 0.733099880094478
96 0.733099880094478
97 0.733099880094478
98 0.733099880094478
99 0.733099880094478
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.705449451263243
1 0.70780648886028
2 0.752901080817474
3 0.757453702742735
4 0.739749724227428
5 0.800955193933919
6 0.634868996034288
7 0.406094804996195
8 0.350993375357343
9 0.178586590592082
10 0.992317158638329
11 0.481690264111032
12 0.826187104687178
13 0.754429556759063
14 0.703123243511845
15 0.701893607837774
16 0.813823693894928
17 0.687161018819927
18 0.76125937352843
19 0.685073431048856
20 0.782815141139874
21 0.806909788476786
22 0.782945325973264
23 0.573419483704425
24 0.430879391405612
25 0.942347701975966
26 0.960721327655351
27 0.707412628353419
28 0.787969172487096
29 0.748218918905527
30 0.70840603983222
31 0.775779287092837
32 0.803562288761264
33 0.699631219725349
34 0.790663923262141
35 0.791511536364425
36 0.737828503238884
37 0.76122286085398
38 0.592666587272106
39 0.791062243326072
40 0.778765700522836
41 0.964485237725255
42 0.986847122968363
43 0.807564954796184
44 0.747964453735243
45 0.749879648773811
46 0.747589236792888
47 0.742250498793204
48 0.767221924667391
49 0.775088663692744
50 0.717361935324223
51 0.67290064909187
52 0.733415960544068
53 0.785417673006935
54 0.921765663629901
55 0.908882397512999
56 0.899850871422445
57 0.914267528391876
58 0.839592199216142
59 0.536515053608613
60 0.85197463483373
61 0.777245396842899
62 0.74325128628073
63 0.744640870852575
64 0.734079673031015
65 0.710858144599377
66 0.806795605130397
67 0.806361845895034
68 0.760747847122729
69 0.646267384488348
70 0.602350088545541
71 0.680287597554312
72 0.594237741905558
73 0.960874158200694
74 0.986572751225911
75 0.787237865832901
76 0.74981820683001
77 0.697186555902099
78 0.677163731531037
79 0.765880765385155
80 0.719492643074522
81 0.743252046942932
82 0.794233322392362
83 0.740379401812532
84 0.483690509128096
85 0.0921347673373974
86 0.770814060322162
87 0.914591088465088
88 0.633550347575737
89 0.604519337491679
90 0.974053941986682
91 0.782388064053217
92 0.697146536540617
93 0.76717978190355
94 0.717893247520017
95 0.738011772632827
96 0.744251792711691
97 0.718396634222563
98 0.710992653999832
99 0.666720575280293
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.715748429298401
1 0.727001428604126
2 0.758335649967194
3 0.787291705608368
4 0.760272145271301
5 0.719063580036163
6 0.924742460250854
7 0.797281324863434
8 0.850437819957733
9 0.888111770153046
10 0.927515387535095
11 0.967481136322021
12 0.835842788219452
13 0.804965019226074
14 0.767312049865723
15 0.75270813703537
16 0.837176740169525
17 0.696782886981964
18 0.79022228717804
19 0.72990220785141
20 0.83420467376709
21 0.699352025985718
22 0.836224555969238
23 0.848310947418213
24 0.875932812690735
25 0.893964886665344
26 0.966183304786682
27 0.94939774274826
28 0.875472903251648
29 0.538789927959442
30 0.716062128543854
31 0.793020248413086
32 0.806427776813507
33 0.728005349636078
34 0.805927038192749
35 0.797088980674744
36 0.768862724304199
37 0.716497421264648
38 0.842059433460236
39 0.779142022132874
40 0.993258833885193
41 0.990423321723938
42 0.990090072154999
43 0.924749076366425
44 0.767973840236664
45 0.681883752346039
46 0.789137423038483
47 0.748453855514526
48 0.769664168357849
49 0.772410333156586
50 0.798808634281158
51 0.727815747261047
52 0.860898077487946
53 0.856183648109436
54 0.808390498161316
55 0.930647075176239
56 0.913617491722107
57 0.986675381660461
58 0.986966133117676
59 0.885740220546722
60 0.873628556728363
61 0.700572550296783
62 0.76739627122879
63 0.762033104896545
64 0.732630908489227
65 0.744288742542267
66 0.81385749578476
67 0.761268198490143
68 0.911663115024567
69 0.893416047096252
70 0.739122152328491
71 0.926448047161102
72 0.978621423244476
73 0.964094340801239
74 0.989329397678375
75 0.844403505325317
76 0.890284359455109
77 0.7380011677742
78 0.67402195930481
79 0.766106605529785
80 0.689572274684906
81 0.741807579994202
82 0.761452913284302
83 0.757104754447937
84 0.87025785446167
85 0.847599267959595
86 0.774954497814178
87 0.903329193592072
88 0.945561766624451
89 0.982495903968811
90 0.856861591339111
91 0.783368349075317
92 0.791123509407043
93 0.757449448108673
94 0.779436469078064
95 0.741792440414429
96 0.739982903003693
97 0.735295414924622
98 0.733044505119324
99 0.648916184902191
};



\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
title style ={color=black,font=\footnotesize},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_1(t)|\)},
ymin=0, ymax=1.2,
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_2(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_2(t)|\)},
xtick style={color=white},
xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.987054960926875
1 0.99924263550812
2 0.971593659504137
3 0.905210310336817
4 0.802739082652688
5 0.668265180932858
6 0.507149655281961
7 0.325815673278255
8 0.131492448551758
9 0.0680729651500804
10 0.264924524548049
11 0.451214379169969
12 0.619515740383694
13 0.763118964023292
14 0.876299042728428
15 0.954543843921521
16 0.994733994294751
17 0.99526723938009
18 0.956122320378739
19 0.878859821682345
20 0.766559955298021
21 0.623699762515788
22 0.455974628400466
23 0.270071224761965
24 0.0734009336512371
25 0.126195621054125
26 0.320761154581369
27 0.502538953095812
28 0.664282109403695
29 0.79954243427307
30 0.902927525390032
31 0.970315745422269
32 0.999020538692921
33 0.9878975356775
34 0.937390175405566
35 0.849512026945969
36 0.727766514762259
37 0.577007248235019
38 0.403244523572316
39 0.213405712266464
40 0.0150590886532155
41 0.183887893302933
42 0.375503845244898
43 0.552149643847855
44 0.706782978559558
45 0.833239106298757
46 0.926476620307876
47 0.982778435131362
48 0.999899975082854
49 0.977158658394629
50 0.915461109598673
51 0.817267015267605
52 0.686491064073022
53 0.528346880501674
54 0.34913917409972
55 0.156012390598786
56 0.0433341145897529
57 0.240953025378305
58 0.428965899416265
59 0.599877256724674
60 0.746873400829622
61 0.8640940593388
62 0.946866014508629
63 0.991889409688494
64 0.997369304192115
65 0.963087231918439
66 0.890409910905682
67 0.782234756596076
68 0.642874371025503
69 0.477884612989535
70 0.293843103485777
71 0.0980869967215749
72 0.101579529070498
73 0.297196399591272
74 0.480964987517813
75 0.645559019164806
76 0.784416649896987
77 0.892002064167656
78 0.964026171015251
79 0.997617596584969
80 0.991437156743219
81 0.945731246122985
82 0.862322015147356
83 0.74453472664228
84 0.597065188101172
85 0.425792544658625
86 0.237544896126614
87 0.0398270822023028
88 0.159478511807789
89 0.35242620081565
90 0.53132376934218
91 0.689039135874149
92 0.819284686447548
93 0.916867941974616
94 0.977898565999261
95 0.999943460134891
96 0.982123764019005
97 0.925149892702439
98 0.831293214643139
99 0.704295499413452
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.989209104706369
1 0.998309085740222
2 0.983448478174975
3 0.926853506682621
4 0.869329788517751
5 0.792281755067933
6 0.53441933057747
7 0.254719033236533
8 0.173592112724405
9 0.0462200467090269
10 0.611653941282422
11 0.426607051901515
12 0.740955739610716
13 0.765677480216294
14 0.896757110504273
15 0.961274053780863
16 0.997756204019804
17 0.983622574778797
18 0.967998857736327
19 0.932144070557955
20 0.814196506310896
21 0.640476597909895
22 0.497500911080896
23 0.324390669670884
24 0.0861124068236966
25 0.910790928967282
26 0.904510469599784
27 0.510735805747301
28 0.759934660641384
29 0.775822017118535
30 0.927869208722898
31 0.977039075455879
32 0.999487982190676
33 0.995075955967568
34 0.949425037373171
35 0.881023825584312
36 0.785520940601164
37 0.660044771471756
38 0.329895494400421
39 0.315254520329302
40 0.0375420260758235
41 0.765153338239215
42 0.828204773079
43 0.607689548225039
44 0.738790236962641
45 0.889659569814301
46 0.949939381102361
47 0.974261874388273
48 0.997251233597193
49 0.994153380916329
50 0.937664706698691
51 0.83056033143878
52 0.712384346609762
53 0.592598278126826
54 0.594987377918438
55 0.988802775483149
56 0.986532477447748
57 0.9958998838052
58 0.465366979242192
59 0.643516989971428
60 0.780659184580816
61 0.872420151228489
62 0.971564931185085
63 0.992998873157375
64 0.997054498336931
65 0.97735225597338
66 0.912963353384614
67 0.808530781347826
68 0.690254706023068
69 0.437571974967365
70 0.295507734989377
71 0.0737551609979466
72 0.0806243045795721
73 0.964640366470473
74 0.997767452979177
75 0.716068160609506
76 0.771109121697892
77 0.92005007783957
78 0.966389640169996
79 0.99938433961039
80 0.991375332580105
81 0.962264429005082
82 0.84658217231866
83 0.772637783603353
84 0.594613449057753
85 0.378035197506126
86 0.103944263912735
87 0.0887661332227556
88 0.193522245876765
89 0.351793528555831
90 0.696224826150996
91 0.740202269667564
92 0.815544044871933
93 0.938541515375247
94 0.972893940047803
95 0.999057896014496
96 0.978506039580993
97 0.914510268963181
98 0.86114786835746
99 0.807748177304879
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.986210346221924
1 0.987537503242493
2 0.960007131099701
3 0.839769423007965
4 0.853170692920685
5 0.838402092456818
6 0.618614256381989
7 0.708825886249542
8 0.942022442817688
9 0.771592199802399
10 0.538001179695129
11 0.667612254619598
12 0.75106817483902
13 0.668015122413635
14 0.792560994625092
15 0.95979517698288
16 0.992656409740448
17 0.973359525203705
18 0.949144542217255
19 0.915854215621948
20 0.716812074184418
21 0.7853884100914
22 0.521713078022003
23 0.897649466991425
24 0.709768235683441
25 0.835388779640198
26 0.945714175701141
27 0.759298026561737
28 0.685761690139771
29 0.816552698612213
30 0.86306369304657
31 0.981720864772797
32 0.99949836730957
33 0.980297088623047
34 0.945199191570282
35 0.781739294528961
36 0.772540807723999
37 0.723425805568695
38 0.784827828407288
39 0.619458615779877
40 0.568830370903015
41 0.666955053806305
42 0.566024243831635
43 0.450824111700058
44 0.707474410533905
45 0.781999468803406
46 0.925409555435181
47 0.94615775346756
48 0.979745328426361
49 0.984347343444824
50 0.870862782001495
51 0.791285216808319
52 0.607026398181915
53 0.511900186538696
54 0.443583071231842
55 0.672614932060242
56 0.686240017414093
57 0.686087906360626
58 0.695790588855743
59 0.72880631685257
60 0.73510879278183
61 0.878524303436279
62 0.966662526130676
63 0.98228794336319
64 0.990890562534332
65 0.942357182502747
66 0.90250551700592
67 0.820770919322968
68 0.623528361320496
69 0.614083886146545
70 0.766156792640686
71 0.753288149833679
72 0.779065847396851
73 0.500169157981873
74 0.772276878356934
75 0.709128379821777
76 0.829563200473785
77 0.774943768978119
78 0.977912425994873
79 0.98437887430191
80 0.971310377120972
81 0.958277344703674
82 0.87610399723053
83 0.679485380649567
84 0.666282951831818
85 0.960972428321838
86 0.884773313999176
87 0.755081474781036
88 0.781363606452942
89 0.632018089294434
90 0.486497312784195
91 0.765276253223419
92 0.816619217395782
93 0.913622617721558
94 0.938222706317902
95 0.991751611232758
96 0.962526142597198
97 0.899295687675476
98 0.844651222229004
99 0.897530972957611
};

\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_2(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
title style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_2(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_3(t)|\)},
xtick style={color=white},
xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.824356457355511
1 0.824356457355511
2 0.824356457355511
3 0.824356457355511
4 0.824356457355511
5 0.824356457355511
6 0.824356457355511
7 0.824356457355511
8 0.824356457355511
9 0.824356457355511
10 0.824356457355511
11 0.824356457355511
12 0.824356457355511
13 0.824356457355511
14 0.824356457355511
15 0.824356457355511
16 0.824356457355511
17 0.824356457355511
18 0.824356457355511
19 0.824356457355511
20 0.824356457355511
21 0.824356457355511
22 0.824356457355511
23 0.824356457355511
24 0.824356457355511
25 0.824356457355511
26 0.824356457355511
27 0.824356457355511
28 0.824356457355511
29 0.824356457355511
30 0.824356457355511
31 0.824356457355511
32 0.824356457355511
33 0.824356457355511
34 0.824356457355511
35 0.824356457355511
36 0.824356457355511
37 0.824356457355511
38 0.824356457355511
39 0.824356457355511
40 0.824356457355511
41 0.824356457355511
42 0.824356457355511
43 0.824356457355511
44 0.824356457355511
45 0.824356457355511
46 0.824356457355511
47 0.824356457355511
48 0.824356457355511
49 0.824356457355511
50 0.824356457355511
51 0.824356457355511
52 0.824356457355511
53 0.824356457355511
54 0.824356457355511
55 0.824356457355511
56 0.824356457355511
57 0.824356457355511
58 0.824356457355511
59 0.824356457355511
60 0.824356457355511
61 0.824356457355511
62 0.824356457355511
63 0.824356457355511
64 0.824356457355511
65 0.824356457355511
66 0.824356457355511
67 0.824356457355511
68 0.824356457355511
69 0.824356457355511
70 0.824356457355511
71 0.824356457355511
72 0.824356457355511
73 0.824356457355511
74 0.824356457355511
75 0.824356457355511
76 0.824356457355511
77 0.824356457355511
78 0.824356457355511
79 0.824356457355511
80 0.824356457355511
81 0.824356457355511
82 0.824356457355511
83 0.824356457355511
84 0.824356457355511
85 0.824356457355511
86 0.824356457355511
87 0.824356457355511
88 0.824356457355511
89 0.824356457355511
90 0.824356457355511
91 0.824356457355511
92 0.824356457355511
93 0.824356457355511
94 0.824356457355511
95 0.824356457355511
96 0.824356457355511
97 0.824356457355511
98 0.824356457355511
99 0.824356457355511
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.777741176352992
1 0.826880616434954
2 0.820081357862817
3 0.784080356102165
4 0.853835804332062
5 0.754046990635605
6 0.895548839406833
7 0.926410210910349
8 0.952826102794723
9 0.964865567307053
10 0.71543493251576
11 0.944155926015056
12 0.88833077029343
13 0.845073078337556
14 0.841956282693966
15 0.861341126542839
16 0.790839168252971
17 0.866681721535839
18 0.764196368377763
19 0.835216144116621
20 0.830636013206478
21 0.806503521074061
22 0.798989522761657
23 0.802238810000211
24 0.634809771451759
25 0.0163028304396104
26 0.486387653650241
27 0.820586304716797
28 0.807013605001845
29 0.802246491633202
30 0.821142779602361
31 0.819830763547846
32 0.849541139402772
33 0.813985042047051
34 0.810058353367569
35 0.786410283466968
36 0.832358708305061
37 0.765314925542495
38 0.967544611664173
39 0.82186000655255
40 0.876856968089686
41 0.886666866727089
42 0.762866411913207
43 0.784579031944092
44 0.875541847359214
45 0.794199706932898
46 0.792217139944758
47 0.806073494304684
48 0.859450618599347
49 0.844096758124404
50 0.790843573104729
51 0.837755395272357
52 0.78994017039284
53 0.855646118092188
54 0.591912419713049
55 0.0819092128952002
56 0.0250541486370604
57 0.0355467365000746
58 0.799003259624252
59 0.878878351188952
60 0.871396133306965
61 0.793603798731605
62 0.842310583480795
63 0.83053525936547
64 0.813166206842131
65 0.801330396373793
66 0.786830958399553
67 0.862542578002656
68 0.82717024118294
69 0.8772353130262
70 0.938107899662488
71 0.931674766036624
72 0.616164898260238
73 0.225688530336276
74 0.281191458978237
75 0.744271302958349
76 0.844274936773237
77 0.806286184074332
78 0.81741072448839
79 0.804445885569334
80 0.782517493787787
81 0.829814312746596
82 0.767153632321715
83 0.806968827481098
84 0.916595784870014
85 0.921494449280328
86 0.837772864770084
87 0.66302795955446
88 0.969076498822397
89 0.897501805190158
90 0.756817680012306
91 0.867132385401153
92 0.809565291269009
93 0.779568975785979
94 0.817347230552406
95 0.813142812638486
96 0.811206338680977
97 0.829873636681919
98 0.805994749744887
99 0.810948562991508
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.795847415924072
1 0.835646748542786
2 0.843309283256531
3 0.818604528903961
4 0.874941349029541
5 0.914858341217041
6 0.616875886917114
7 0.81894850730896
8 0.464543610811234
9 0.900285065174103
10 0.724129557609558
11 0.736879825592041
12 0.865055918693542
13 0.890788674354553
14 0.879723012447357
15 0.869313895702362
16 0.815618574619293
17 0.865279972553253
18 0.792193233966827
19 0.812496542930603
20 0.785797595977783
21 0.900483429431915
22 0.793516278266907
23 0.450982958078384
24 0.91160923242569
25 0.833626508712769
26 0.546811282634735
27 0.773596405982971
28 0.875149190425873
29 0.926913321018219
30 0.829065203666687
31 0.821712017059326
32 0.839934229850769
33 0.806665539741516
34 0.837931334972382
35 0.832101345062256
36 0.904763638973236
37 0.805433213710785
38 0.486137717962265
39 0.611201822757721
40 0.495334923267365
41 0.597258567810059
42 0.647011339664459
43 0.634664535522461
44 0.940984725952148
45 0.798447489738464
46 0.748800039291382
47 0.825713813304901
48 0.863249123096466
49 0.855756044387817
50 0.695877850055695
51 0.843384623527527
52 0.787289977073669
53 0.814836382865906
54 0.800449311733246
55 0.9105623960495
56 0.768921673297882
57 0.464603155851364
58 0.397525072097778
59 0.745578289031982
60 0.854524195194244
61 0.858364224433899
62 0.824028372764587
63 0.8212069272995
64 0.834083318710327
65 0.792583763599396
66 0.81264853477478
67 0.957649111747742
68 0.700846195220947
69 0.556906759738922
70 0.933107793331146
71 0.862110614776611
72 0.743948757648468
73 0.738218069076538
74 0.410824626684189
75 0.798996031284332
76 0.779343008995056
77 0.908387005329132
78 0.863043367862701
79 0.798594117164612
80 0.819489538669586
81 0.867050170898438
82 0.792926549911499
83 0.840198874473572
84 0.583245515823364
85 0.502183616161346
86 0.654987871646881
87 0.838187694549561
88 0.678929030895233
89 0.647290527820587
90 0.755810678005219
91 0.944316327571869
92 0.759844899177551
93 0.765820920467377
94 0.841296374797821
95 0.848097443580627
96 0.820915520191193
97 0.891912400722504
98 0.843626797199249
99 0.911913216114044
};


\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_3(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_3(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_4(t)|\)},
xtick style={color=white},
xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.753602486017811
1 0.753602486017811
2 0.753602486017811
3 0.753602486017811
4 0.753602486017811
5 0.753602486017811
6 0.753602486017811
7 0.753602486017811
8 0.753602486017811
9 0.753602486017811
10 0.753602486017811
11 0.753602486017811
12 0.753602486017811
13 0.753602486017811
14 0.753602486017811
15 0.753602486017811
16 0.753602486017811
17 0.753602486017811
18 0.753602486017811
19 0.753602486017811
20 0.753602486017811
21 0.753602486017811
22 0.753602486017811
23 0.753602486017811
24 0.753602486017811
25 0.753602486017811
26 0.753602486017811
27 0.753602486017811
28 0.753602486017811
29 0.753602486017811
30 0.753602486017811
31 0.753602486017811
32 0.753602486017811
33 0.753602486017811
34 0.753602486017811
35 0.753602486017811
36 0.753602486017811
37 0.753602486017811
38 0.753602486017811
39 0.753602486017811
40 0.753602486017811
41 0.753602486017811
42 0.753602486017811
43 0.753602486017811
44 0.753602486017811
45 0.753602486017811
46 0.753602486017811
47 0.753602486017811
48 0.753602486017811
49 0.753602486017811
50 0.753602486017811
51 0.753602486017811
52 0.753602486017811
53 0.753602486017811
54 0.753602486017811
55 0.753602486017811
56 0.753602486017811
57 0.753602486017811
58 0.753602486017811
59 0.753602486017811
60 0.753602486017811
61 0.753602486017811
62 0.753602486017811
63 0.753602486017811
64 0.753602486017811
65 0.753602486017811
66 0.753602486017811
67 0.753602486017811
68 0.753602486017811
69 0.753602486017811
70 0.753602486017811
71 0.753602486017811
72 0.753602486017811
73 0.753602486017811
74 0.753602486017811
75 0.753602486017811
76 0.753602486017811
77 0.753602486017811
78 0.753602486017811
79 0.753602486017811
80 0.753602486017811
81 0.753602486017811
82 0.753602486017811
83 0.753602486017811
84 0.753602486017811
85 0.753602486017811
86 0.753602486017811
87 0.753602486017811
88 0.753602486017811
89 0.753602486017811
90 0.753602486017811
91 0.753602486017811
92 0.753602486017811
93 0.753602486017811
94 0.753602486017811
95 0.753602486017811
96 0.753602486017811
97 0.753602486017811
98 0.753602486017811
99 0.753602486017811
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.747122236701847
1 0.788971814100096
2 0.761448824250579
3 0.726011441148744
4 0.756222002862557
5 0.835773161244476
6 0.704253641691227
7 0.682476449420999
8 0.721628291727775
9 0.759559989823079
10 0.448323290801656
11 0.777854184607589
12 0.752091871428761
13 0.690217150665711
14 0.775987511620368
15 0.771491192678729
16 0.789276827237198
17 0.786132336553045
18 0.768988368751339
19 0.714135971118708
20 0.788103220680777
21 0.776236316788154
22 0.776564090163467
23 0.667709708734119
24 0.767438887172314
25 0.825414478192528
26 0.420442020315553
27 0.763753769094376
28 0.731344591732967
29 0.72899326515999
30 0.726302191529251
31 0.744057210105667
32 0.782202364222163
33 0.774107145397054
34 0.729443180552045
35 0.788901033681606
36 0.748913482044052
37 0.785916588544956
38 0.700330474493921
39 0.82255539633334
40 0.738391373111507
41 0.159936165869445
42 0.284864393771192
43 0.685154110728752
44 0.766288437178713
45 0.726122015614061
46 0.799074330621188
47 0.756003148420688
48 0.733686866206859
49 0.765617121613271
50 0.748025468634572
51 0.735869149324613
52 0.74695730811819
53 0.768467403648633
54 0.89139846683815
55 0.641253644348834
56 0.698857983346604
57 0.71361609236045
58 0.649230345325841
59 0.780873211498563
60 0.724145673660828
61 0.761016370590931
62 0.756188769144601
63 0.793979237080856
64 0.718354094238357
65 0.756156328056658
66 0.815954456259942
67 0.774062265203374
68 0.76199447560871
69 0.66935270489148
70 0.722511428177373
71 0.751157880790633
72 0.684541633310266
73 0.608007580358615
74 0.619440834977845
75 0.705855792374066
76 0.79693511974418
77 0.813686608896125
78 0.787169178692099
79 0.717450198960962
80 0.802775466280511
81 0.677950315658186
82 0.762062167433413
83 0.786312414276628
84 0.675213287484027
85 0.684196467144675
86 0.754275118692274
87 0.793186389708888
88 0.733090541987735
89 0.798411068864388
90 0.47154215807281
91 0.699725762296793
92 0.763939288066078
93 0.778348394554344
94 0.789237042762381
95 0.783000194470066
96 0.77601431250001
97 0.679422419967979
98 0.744655564136607
99 0.734537550966124
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.754518449306488
1 0.744019627571106
2 0.831670999526978
3 0.769767463207245
4 0.78367280960083
5 0.677084684371948
6 0.736019134521484
7 0.510897696018219
8 0.424168348312378
9 0.106054827570915
10 0.366897791624069
11 0.366294890642166
12 0.774970710277557
13 0.920262515544891
14 0.759958982467651
15 0.699889779090881
16 0.794045567512512
17 0.804079055786133
18 0.809808135032654
19 0.785483241081238
20 0.807699799537659
21 0.604336738586426
22 0.820680201053619
23 0.545387446880341
24 0.251548677682877
25 0.284070670604706
26 0.446475446224213
27 0.432875394821167
28 0.640664458274841
29 0.8688063621521
30 0.714762151241302
31 0.760115504264832
32 0.760918140411377
33 0.671598434448242
34 0.64204615354538
35 0.8160120844841
36 0.762838363647461
37 0.721351385116577
38 0.800017535686493
39 0.668141841888428
40 0.490839272737503
41 0.368205457925797
42 0.597048819065094
43 0.779517352581024
44 0.892737746238708
45 0.856098175048828
46 0.850295424461365
47 0.772418856620789
48 0.717813372612
49 0.755223333835602
50 0.777711570262909
51 0.786048769950867
52 0.777113616466522
53 0.780845761299133
54 0.703776717185974
55 0.14546038210392
56 0.178602203726768
57 0.433094501495361
58 0.748059391975403
59 0.607266843318939
60 0.68466579914093
61 0.858319997787476
62 0.73680579662323
63 0.849512159824371
64 0.675336360931396
65 0.803158402442932
66 0.80654901266098
67 0.69241726398468
68 0.920572280883789
69 0.858915865421295
70 0.37838140130043
71 0.103895075619221
72 0.242574214935303
73 0.575861990451813
74 0.786737561225891
75 0.648310482501984
76 0.602457821369171
77 0.815465152263641
78 0.834576725959778
79 0.689410030841827
80 0.761010110378265
81 0.690102219581604
82 0.694154441356659
83 0.805976271629333
84 0.86274266242981
85 0.7013840675354
86 0.320492446422577
87 0.186358273029327
88 0.409136295318604
89 0.374019771814346
90 0.676600575447083
91 0.755732893943787
92 0.696611404418945
93 0.798762321472168
94 0.703760266304016
95 0.825084686279297
96 0.752212941646576
97 0.656877398490906
98 0.750684797763824
99 0.651942431926727
};

\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_5(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_5(t)|\)},
%xtick style={color=white},
%xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}

\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.935826238137458
1 0.935826238137458
2 0.935826238137458
3 0.935826238137458
4 0.935826238137458
5 0.935826238137458
6 0.935826238137458
7 0.935826238137458
8 0.935826238137458
9 0.935826238137458
10 0.935826238137458
11 0.935826238137458
12 0.935826238137458
13 0.935826238137458
14 0.935826238137458
15 0.935826238137458
16 0.935826238137458
17 0.935826238137458
18 0.935826238137458
19 0.935826238137458
20 0.935826238137458
21 0.935826238137458
22 0.935826238137458
23 0.935826238137458
24 0.935826238137458
25 0.935826238137458
26 0.935826238137458
27 0.935826238137458
28 0.935826238137458
29 0.935826238137458
30 0.935826238137458
31 0.935826238137458
32 0.935826238137458
33 0.935826238137458
34 0.935826238137458
35 0.935826238137458
36 0.935826238137458
37 0.935826238137458
38 0.935826238137458
39 0.935826238137458
40 0.935826238137458
41 0.935826238137458
42 0.935826238137458
43 0.935826238137458
44 0.935826238137458
45 0.935826238137458
46 0.935826238137458
47 0.935826238137458
48 0.935826238137458
49 0.935826238137458
50 0.935826238137458
51 0.935826238137458
52 0.935826238137458
53 0.935826238137458
54 0.935826238137458
55 0.935826238137458
56 0.935826238137458
57 0.935826238137458
58 0.935826238137458
59 0.935826238137458
60 0.935826238137458
61 0.935826238137458
62 0.935826238137458
63 0.935826238137458
64 0.935826238137458
65 0.935826238137458
66 0.935826238137458
67 0.935826238137458
68 0.935826238137458
69 0.935826238137458
70 0.935826238137458
71 0.935826238137458
72 0.935826238137458
73 0.935826238137458
74 0.935826238137458
75 0.935826238137458
76 0.935826238137458
77 0.935826238137458
78 0.935826238137458
79 0.935826238137458
80 0.935826238137458
81 0.935826238137458
82 0.935826238137458
83 0.935826238137458
84 0.935826238137458
85 0.935826238137458
86 0.935826238137458
87 0.935826238137458
88 0.935826238137458
89 0.935826238137458
90 0.935826238137458
91 0.935826238137458
92 0.935826238137458
93 0.935826238137458
94 0.935826238137458
95 0.935826238137458
96 0.935826238137458
97 0.935826238137458
98 0.935826238137458
99 0.935826238137458
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.958551874166055
1 0.958499553273104
2 0.929985034923385
3 0.968240281548343
4 0.913797920955819
5 0.967923701707248
6 0.888345308171027
7 0.912911399793684
8 0.875036499215917
9 0.939763633176355
10 0.649238243294882
11 0.937118726313822
12 0.848283972307682
13 0.899741253572134
14 0.902886671713852
15 0.932996192480686
16 0.971421522316662
17 0.921696465593022
18 0.951246712158347
19 0.88165164050768
20 0.948274191356788
21 0.94098680737814
22 0.95078911965871
23 0.918088852611559
24 0.963804484316459
25 0.944458167956691
26 0.996445047046216
27 0.94980255892084
28 0.91527336603312
29 0.939278643336924
30 0.942129265302411
31 0.931256913277102
32 0.930193074416856
33 0.917116365212116
34 0.918739827685217
35 0.925523244056441
36 0.933103767962521
37 0.93249132138416
38 0.967687036120637
39 0.937421337964882
40 0.928723067030868
41 0.270796911588374
42 0.430914809192934
43 0.923862066489484
44 0.948759713443823
45 0.936091357417533
46 0.963382430411413
47 0.939776640255831
48 0.938357418872922
49 0.936518990204442
50 0.927268514886373
51 0.922307661389772
52 0.948601156474088
53 0.938244859339482
54 0.938928917830823
55 0.934368819845064
56 0.93094765632019
57 0.943220148286938
58 0.942074567916706
59 0.907845355001728
60 0.885819565905774
61 0.954383011659881
62 0.927377106519813
63 0.922599298338688
64 0.946456952192713
65 0.917085747255325
66 0.953012749644611
67 0.929102487151044
68 0.888296780758787
69 0.908040035810504
70 0.925163711721656
71 0.964380077930125
72 0.919268470786305
73 0.94831192749233
74 0.946796392864282
75 0.951330093565819
76 0.860976736628945
77 0.948881463291132
78 0.940630041100824
79 0.973849469349136
80 0.942262838615673
81 0.947469937436935
82 0.955848952526678
83 0.921261239689783
84 0.920157089544871
85 0.807227433629484
86 0.922078851497244
87 0.935232516940445
88 0.929209193121351
89 0.942895772088162
90 0.721090246168421
91 0.901117279784621
92 0.959972005404697
93 0.928171461566878
94 0.935637697282971
95 0.941861426483014
96 0.958562416563046
97 0.902579598485546
98 0.963288274034698
99 0.937323813922779
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.974479734897614
1 0.941849827766418
2 0.898502349853516
3 0.937007248401642
4 0.906224727630615
5 0.913956582546234
6 0.716144323348999
7 0.620731234550476
8 0.682995975017548
9 0.443919241428375
10 0.859974563121796
11 0.859901189804077
12 0.895481288433075
13 0.901846349239349
14 0.846242785453796
15 0.896491467952728
16 0.92707371711731
17 0.899075210094452
18 0.954894661903381
19 0.871123671531677
20 0.94942319393158
21 0.936480164527893
22 0.858282029628754
23 0.661230802536011
24 0.739985466003418
25 0.759562730789185
26 0.934851825237274
27 0.792971730232239
28 0.81634259223938
29 0.925180852413177
30 0.917199611663818
31 0.951943337917328
32 0.92877334356308
33 0.917600393295288
34 0.888020277023315
35 0.876141548156738
36 0.868013799190521
37 0.944012522697449
38 0.84812206029892
39 0.880514144897461
40 0.631493449211121
41 0.67067950963974
42 0.82576060295105
43 0.828503727912903
44 0.903788089752197
45 0.932422995567322
46 0.971495807170868
47 0.893104732036591
48 0.937111973762512
49 0.90678858757019
50 0.958909511566162
51 0.936791718006134
52 0.882758796215057
53 0.90185934305191
54 0.83045893907547
55 0.308662950992584
56 0.720047235488892
57 0.794918477535248
58 0.843261659145355
59 0.945867717266083
60 0.876326858997345
61 0.960855603218079
62 0.943914234638214
63 0.90661883354187
64 0.909083724021912
65 0.884714484214783
66 0.907837748527527
67 0.873387575149536
68 0.824031054973602
69 0.877913892269135
70 0.850489616394043
71 0.21589769423008
72 0.231679022312164
73 0.766073226928711
74 0.857430100440979
75 0.910708367824554
76 0.866707503795624
77 0.868883907794952
78 0.93121725320816
79 0.973082304000854
80 0.896352291107178
81 0.929291605949402
82 0.928487181663513
83 0.920706808567047
84 0.884196043014526
85 0.695740342140198
86 0.726252198219299
87 0.649792969226837
88 0.919783473014832
89 0.801141321659088
90 0.892462372779846
91 0.881376087665558
92 0.958154320716858
93 0.926012337207794
94 0.839700222015381
95 0.942257285118103
96 0.94405460357666
97 0.763419926166534
98 0.988091051578522
99 0.933284759521484
};

\end{groupplot}

==> Figs/structured_phi_change/noise_001.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm, group name=left1 plots }]
\nextgroupplot[
anchor=north west,
at={($(left0 plots c1r1.north east) + (0.2cm,0)$)},
width=\w cm,
height=\h cm,
legend cell align={left},
legend style={at={(0,2)}, anchor=north west, legend cell align=left, align=left, font=\footnotesize, draw=white!15!black},
legend columns=3,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black,font=\footnotesize},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_0(t)|\)},
title style ={color=black,font=\footnotesize},
title = {Noise variance = $0.001$},
ymin=0, ymax=1.2,
ytick style={color=black,font=\footnotesize},
%-------- Horizantal ----
%xtick style={color=black,font=\footnotesize},
%xlabel = {time \(t\)},
%title={\(\displaystyle |\cos\phi_1(t)|\)},
%-------- Vertical ----
xtick style={color=white,font=\footnotesize},
xticklabels ={},
yticklabels={},
ytick style={color=white},
%xlabel = {time \(t\)},
%ylabel={\(\displaystyle |\cos\phi_1(t)|\)},
% xtick style={color=white},
% xticklabels={},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.733099880094478
1 0.733099880094478
2 0.733099880094478
3 0.733099880094478
4 0.733099880094478
5 0.733099880094478
6 0.733099880094478
7 0.733099880094478
8 0.733099880094478
9 0.733099880094478
10 0.733099880094478
11 0.733099880094478
12 0.733099880094478
13 0.733099880094478
14 0.733099880094478
15 0.733099880094478
16 0.733099880094478
17 0.733099880094478
18 0.733099880094478
19 0.733099880094478
20 0.733099880094478
21 0.733099880094478
22 0.733099880094478
23 0.733099880094478
24 0.733099880094478
25 0.733099880094478
26 0.733099880094478
27 0.733099880094478
28 0.733099880094478
29 0.733099880094478
30 0.733099880094478
31 0.733099880094478
32 0.733099880094478
33 0.733099880094478
34 0.733099880094478
35 0.733099880094478
36 0.733099880094478
37 0.733099880094478
38 0.733099880094478
39 0.733099880094478
40 0.733099880094478
41 0.733099880094478
42 0.733099880094478
43 0.733099880094478
44 0.733099880094478
45 0.733099880094478
46 0.733099880094478
47 0.733099880094478
48 0.733099880094478
49 0.733099880094478
50 0.733099880094478
51 0.733099880094478
52 0.733099880094478
53 0.733099880094478
54 0.733099880094478
55 0.733099880094478
56 0.733099880094478
57 0.733099880094478
58 0.733099880094478
59 0.733099880094478
60 0.733099880094478
61 0.733099880094478
62 0.733099880094478
63 0.733099880094478
64 0.733099880094478
65 0.733099880094478
66 0.733099880094478
67 0.733099880094478
68 0.733099880094478
69 0.733099880094478
70 0.733099880094478
71 0.733099880094478
72 0.733099880094478
73 0.733099880094478
74 0.733099880094478
75 0.733099880094478
76 0.733099880094478
77 0.733099880094478
78 0.733099880094478
79 0.733099880094478
80 0.733099880094478
81 0.733099880094478
82 0.733099880094478
83 0.733099880094478
84 0.733099880094478
85 0.733099880094478
86 0.733099880094478
87 0.733099880094478
88 0.733099880094478
89 0.733099880094478
90 0.733099880094478
91 0.733099880094478
92 0.733099880094478
93 0.733099880094478
94 0.733099880094478
95 0.733099880094478
96 0.733099880094478
97 0.733099880094478
98 0.733099880094478
99 0.733099880094478
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.746155038273886
1 0.740720561384845
2 0.733556164437626
3 0.737250660857035
4 0.731889463856759
5 0.745942881657928
6 0.728977768898847
7 0.730553340700521
8 0.740074826966741
9 0.73747448176667
10 0.724242264009415
11 0.723534868252313
12 0.7272582303313
13 0.728823732268844
14 0.591965012711264
15 0.761923320068695
16 0.768669953857467
17 0.744707196787255
18 0.732123583600432
19 0.734193848395567
20 0.733200625027274
21 0.736372168922433
22 0.728095002123688
23 0.73856082939716
24 0.729803839219495
25 0.727931571093373
26 0.736985264610513
27 0.724860493984099
28 0.733858310450071
29 0.726819058737039
30 0.448329799216204
31 0.726301136259262
32 0.723804601687504
33 0.725611470639846
34 0.740754291063214
35 0.741391969237483
36 0.724631727867286
37 0.728801662660091
38 0.732030654488034
39 0.734127624324629
40 0.727503267815059
41 0.746240409952406
42 0.728864244640194
43 0.738359371826639
44 0.731604431224613
45 0.73427751024242
46 0.720235200488596
47 0.722463469360794
48 0.724120220439298
49 0.741238532971529
50 0.735951960459802
51 0.735113794661088
52 0.734236583532624
53 0.726492672425206
54 0.72960700670169
55 0.73038535871907
56 0.740916214708303
57 0.72680117578574
58 0.731820311506784
59 0.73057106416622
60 0.725228432809256
61 0.623573790869677
62 0.745533776302182
63 0.735645995907504
64 0.722904560601772
65 0.72833717007482
66 0.73402706416982
67 0.733953517235423
68 0.729169177243327
69 0.728180015762852
70 0.731264028580377
71 0.735647779903931
72 0.736665848278586
73 0.739910203716718
74 0.725550772435737
75 0.736935265582278
76 0.658062603490029
77 0.753242238129341
78 0.689333628687203
79 0.715301307073224
80 0.742614634739746
81 0.72803899962307
82 0.739063002538563
83 0.730408566993567
84 0.729516133735303
85 0.728698594165538
86 0.731161156060174
87 0.731957153583952
88 0.728175476002976
89 0.736391545432526
90 0.724167370390104
91 0.743639917842209
92 0.742783417373776
93 0.715464662246327
94 0.720773419499927
95 0.737850968748702
96 0.739643556537811
97 0.725464551553908
98 0.739163232576734
99 0.720485515277916
};
%\addlegendentry{Netwrok}
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.796050548553467
1 0.725427687168121
2 0.66753351688385
3 0.765453100204468
4 0.74944669008255
5 0.73720371723175
6 0.730496764183044
7 0.73031610250473
8 0.737953782081604
9 0.733441472053528
10 0.734692335128784
11 0.739787101745605
12 0.806178689002991
13 0.994518935680389
14 0.898239493370056
15 0.740832686424255
16 0.779820084571838
17 0.714400172233582
18 0.724559009075165
19 0.758156299591064
20 0.721947491168976
21 0.736289978027344
22 0.72825688123703
23 0.738456666469574
24 0.730540037155151
25 0.721539855003357
26 0.742448687553406
27 0.732049167156219
28 0.752329468727112
29 0.745687067508698
30 0.914401531219482
31 0.994732141494751
32 0.7888343334198
33 0.670533657073975
34 0.720998704433441
35 0.750436902046204
36 0.723499238491058
37 0.729397118091583
38 0.730352640151978
39 0.738314986228943
40 0.727119624614716
41 0.751337170600891
42 0.734556972980499
43 0.73209273815155
44 0.766308665275574
45 0.900850355625153
46 0.944329142570496
47 0.8546342253685
48 0.75591504573822
49 0.653264701366425
50 0.690347671508789
51 0.729555428028107
52 0.728111267089844
53 0.726102352142334
54 0.727729618549347
55 0.729261100292206
56 0.743011057376862
57 0.737688958644867
58 0.736982464790344
59 0.680168509483337
60 0.951314926147461
61 0.894824743270874
62 0.953924596309662
63 0.934486567974091
64 0.73470151424408
65 0.718769609928131
66 0.739253640174866
67 0.729987442493439
68 0.735311448574066
69 0.731400072574615
70 0.730961680412292
71 0.734667301177979
72 0.733575522899628
73 0.754327297210693
74 0.700806617736816
75 0.741483569145203
76 0.738081157207489
77 0.897917032241821
78 0.94080001115799
79 0.818570673465729
80 0.594665944576263
81 0.700905561447144
82 0.746045649051666
83 0.724375605583191
84 0.729912459850311
85 0.72965794801712
86 0.732190907001495
87 0.732643067836761
88 0.727584004402161
89 0.740147709846497
90 0.773060202598572
91 0.601854026317596
92 0.716010928153992
93 0.918971240520477
94 0.95186460018158
95 0.763828933238983
96 0.760358870029449
97 0.678735733032227
98 0.747771143913269
99 0.723706841468811
};
%\addlegendentry{Inverse Scattering}

\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
title style ={color=black,font=\footnotesize},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_1(t)|\)},
ymin=0, ymax=1.2,
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_2(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_2(t)|\)},
xtick style={color=white},
xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.264924524548049
1 0.451214379169969
2 0.619515740383694
3 0.763118964023292
4 0.876299042728428
5 0.954543843921521
6 0.994733994294751
7 0.99526723938009
8 0.956122320378739
9 0.878859821682345
10 0.766559955298021
11 0.623699762515788
12 0.455974628400466
13 0.270071224761965
14 0.0734009336512371
15 0.126195621054125
16 0.320761154581369
17 0.502538953095812
18 0.664282109403695
19 0.79954243427307
20 0.902927525390032
21 0.970315745422269
22 0.999020538692921
23 0.9878975356775
24 0.937390175405566
25 0.849512026945969
26 0.727766514762259
27 0.577007248235019
28 0.403244523572316
29 0.213405712266464
30 0.0150590886532155
31 0.183887893302933
32 0.375503845244898
33 0.552149643847855
34 0.706782978559558
35 0.833239106298757
36 0.926476620307876
37 0.982778435131362
38 0.999899975082854
39 0.977158658394629
40 0.915461109598673
41 0.817267015267605
42 0.686491064073022
43 0.528346880501674
44 0.34913917409972
45 0.156012390598786
46 0.0433341145897529
47 0.240953025378305
48 0.428965899416265
49 0.599877256724674
50 0.746873400829622
51 0.8640940593388
52 0.946866014508629
53 0.991889409688494
54 0.997369304192115
55 0.963087231918439
56 0.890409910905682
57 0.782234756596076
58 0.642874371025503
59 0.477884612989535
60 0.293843103485777
61 0.0980869967215749
62 0.101579529070498
63 0.297196399591272
64 0.480964987517813
65 0.645559019164806
66 0.784416649896987
67 0.892002064167656
68 0.964026171015251
69 0.997617596584969
70 0.991437156743219
71 0.945731246122985
72 0.862322015147356
73 0.74453472664228
74 0.597065188101172
75 0.425792544658625
76 0.237544896126614
77 0.0398270822023028
78 0.159478511807789
79 0.35242620081565
80 0.53132376934218
81 0.689039135874149
82 0.819284686447548
83 0.916867941974616
84 0.977898565999261
85 0.999943460134891
86 0.982123764019005
87 0.925149892702439
88 0.831293214643139
89 0.704295499413452
90 0.549219745155122
91 0.372248332820587
92 0.180436554154038
93 0.018568660526159
94 0.216833601307975
95 0.406454070663639
96 0.579870498861935
97 0.730169320157782
98 0.851358594841471
99 0.938606888966237
};

\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.26215365096214
1 0.44402870730442
2 0.630172075133476
3 0.77581698194705
4 0.879688948282845
5 0.95648547455055
6 0.992843562016613
7 0.995637098956235
8 0.954249118803595
9 0.875549177181915
10 0.754911565153484
11 0.615623789720245
12 0.472715827631814
13 0.268231847768953
14 0.0633453291423598
15 0.139821401183342
16 0.330789736099938
17 0.503371779012841
18 0.673031168353177
19 0.796507662562902
20 0.905031812153014
21 0.972855352586919
22 0.99794303761264
23 0.989882125856531
24 0.939222638385526
25 0.846866389121592
26 0.737641973557678
27 0.560131568002221
28 0.39999163667294
29 0.19995488389906
30 0.00276190722701836
31 0.179821110710052
32 0.372572306589538
33 0.541857995295831
34 0.714560770705934
35 0.836069223118536
36 0.926470750915584
37 0.980389278767036
38 0.999978121221369
39 0.97926065255223
40 0.918041787432778
41 0.817170467127331
42 0.679306379947925
43 0.523111898107596
44 0.350258904293992
45 0.166162270614509
46 0.046683359509139
47 0.240134215124744
48 0.411434264123858
49 0.614915542981966
50 0.747742506640598
51 0.859215126397073
52 0.946667889913271
53 0.991208998904703
54 0.997060929622719
55 0.962159167210236
56 0.896497180640589
57 0.778129140516676
58 0.652144209726061
59 0.4829212255075
60 0.291413644629424
61 0.0940677522550399
62 0.107397907122777
63 0.307702615056638
64 0.476337889380012
65 0.642298115872285
66 0.791454600762107
67 0.893982017074009
68 0.964288667247667
69 0.996923869173791
70 0.991857726700159
71 0.944873691097505
72 0.865509595283389
73 0.742978711790185
74 0.601730961194925
75 0.430184238668617
76 0.228360630836829
77 0.0497347095397406
78 0.169500465096632
79 0.357696881404744
80 0.526929089921743
81 0.684186570303627
82 0.820549837820333
83 0.917137614409493
84 0.976549791681397
85 0.999684755463254
86 0.981109735595153
87 0.921800686679578
88 0.829884521004684
89 0.702537211473512
90 0.556217592580598
91 0.376071543051614
92 0.177964545536996
93 0.0115881706664362
94 0.204099937541821
95 0.415714623395902
96 0.577125907229196
97 0.730290553781436
98 0.858392269519039
99 0.9314409951996
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.524381279945374
1 0.46993425488472
2 0.681766033172607
3 0.788087904453278
4 0.874465644359589
5 0.956118822097778
6 0.994589626789093
7 0.995819449424744
8 0.958897113800049
9 0.877552628517151
10 0.740665674209595
11 0.601971745491028
12 0.441980212926865
13 0.41279935836792
14 0.519153952598572
15 0.248592257499695
16 0.418171226978302
17 0.490001201629639
18 0.681772708892822
19 0.792608380317688
20 0.912953197956085
21 0.972328126430511
22 0.996742129325867
23 0.989606440067291
24 0.93711245059967
25 0.851084530353546
26 0.729838073253632
27 0.570555746555328
28 0.385120272636414
29 0.368839770555496
30 0.754378020763397
31 0.264809429645538
32 0.38036322593689
33 0.549627602100372
34 0.707969963550568
35 0.836037516593933
36 0.926060318946838
37 0.97879558801651
38 0.999859035015106
39 0.976682901382446
40 0.921471118927002
41 0.82278972864151
42 0.670283436775208
43 0.526529371738434
44 0.375643730163574
45 0.807274639606476
46 0.60038161277771
47 0.308734089136124
48 0.425106018781662
49 0.633775651454926
50 0.74635249376297
51 0.864430785179138
52 0.944239437580109
53 0.99219673871994
54 0.997497320175171
55 0.964586079120636
56 0.893740117549896
57 0.765503764152527
58 0.650707185268402
59 0.511546432971954
60 0.294795840978622
61 0.880691349506378
62 0.681731760501862
63 0.393409848213196
64 0.487861007452011
65 0.658761620521545
66 0.793470442295074
67 0.89649885892868
68 0.961875259876251
69 0.995250642299652
70 0.992921054363251
71 0.94759339094162
72 0.861551523208618
73 0.732615768909454
74 0.630138158798218
75 0.459205985069275
76 0.592876732349396
77 0.819554209709167
78 0.795200705528259
79 0.409529805183411
80 0.582560539245605
81 0.699526131153107
82 0.814694344997406
83 0.916626572608948
84 0.977693736553192
85 0.999737024307251
86 0.980761647224426
87 0.919997036457062
88 0.828481495380402
89 0.705772221088409
90 0.523739099502563
91 0.498372673988342
92 0.472347438335419
93 0.75702029466629
94 0.429539829492569
95 0.392536848783493
96 0.560312390327454
97 0.728354811668396
98 0.861783921718597
99 0.929997980594635
};


\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
xtick style={color=black},
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_2(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
title style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_2(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_3(t)|\)},
xtick style={color=white},
xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.824356457355511
1 0.824356457355511
2 0.824356457355511
3 0.824356457355511
4 0.824356457355511
5 0.824356457355511
6 0.824356457355511
7 0.824356457355511
8 0.824356457355511
9 0.824356457355511
10 0.824356457355511
11 0.824356457355511
12 0.824356457355511
13 0.824356457355511
14 0.824356457355511
15 0.824356457355511
16 0.824356457355511
17 0.824356457355511
18 0.824356457355511
19 0.824356457355511
20 0.824356457355511
21 0.824356457355511
22 0.824356457355511
23 0.824356457355511
24 0.824356457355511
25 0.824356457355511
26 0.824356457355511
27 0.824356457355511
28 0.824356457355511
29 0.824356457355511
30 0.824356457355511
31 0.824356457355511
32 0.824356457355511
33 0.824356457355511
34 0.824356457355511
35 0.824356457355511
36 0.824356457355511
37 0.824356457355511
38 0.824356457355511
39 0.824356457355511
40 0.824356457355511
41 0.824356457355511
42 0.824356457355511
43 0.824356457355511
44 0.824356457355511
45 0.824356457355511
46 0.824356457355511
47 0.824356457355511
48 0.824356457355511
49 0.824356457355511
50 0.824356457355511
51 0.824356457355511
52 0.824356457355511
53 0.824356457355511
54 0.824356457355511
55 0.824356457355511
56 0.824356457355511
57 0.824356457355511
58 0.824356457355511
59 0.824356457355511
60 0.824356457355511
61 0.824356457355511
62 0.824356457355511
63 0.824356457355511
64 0.824356457355511
65 0.824356457355511
66 0.824356457355511
67 0.824356457355511
68 0.824356457355511
69 0.824356457355511
70 0.824356457355511
71 0.824356457355511
72 0.824356457355511
73 0.824356457355511
74 0.824356457355511
75 0.824356457355511
76 0.824356457355511
77 0.824356457355511
78 0.824356457355511
79 0.824356457355511
80 0.824356457355511
81 0.824356457355511
82 0.824356457355511
83 0.824356457355511
84 0.824356457355511
85 0.824356457355511
86 0.824356457355511
87 0.824356457355511
88 0.824356457355511
89 0.824356457355511
90 0.824356457355511
91 0.824356457355511
92 0.824356457355511
93 0.824356457355511
94 0.824356457355511
95 0.824356457355511
96 0.824356457355511
97 0.824356457355511
98 0.824356457355511
99 0.824356457355511
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.81496184653319
1 0.827773303658108
2 0.820850588776564
3 0.827626398260177
4 0.830162230200413
5 0.820206460419273
6 0.821659288935205
7 0.828244269323175
8 0.818524381292753
9 0.824824033193426
10 0.830713179153323
11 0.827175648442562
12 0.830293595777284
13 0.826973382592154
14 0.945217791069408
15 0.809515269951409
16 0.79624986416221
17 0.821493050116147
18 0.81865074196844
19 0.818357729289645
20 0.822619609755926
21 0.822775959999128
22 0.824859001320004
23 0.825732525286909
24 0.826612743917276
25 0.83110640959623
26 0.821049203221553
27 0.82569035757941
28 0.835644220684464
29 0.830095461534994
30 0.995475126304917
31 0.827240423973909
32 0.831249069847202
33 0.824146328752078
34 0.823142133538622
35 0.819418967207859
36 0.820201686717625
37 0.818044693355596
38 0.819840879561811
39 0.824729508901318
40 0.826682022810027
41 0.824283448005367
42 0.826357267198654
43 0.822452918418737
44 0.823666668554083
45 0.807346461979422
46 0.787577514244272
47 0.840825619955964
48 0.840730256338528
49 0.821908408465021
50 0.829365512226764
51 0.827250741608583
52 0.821276522961762
53 0.828450213579928
54 0.823731559928741
55 0.83107668672188
56 0.83131737818337
57 0.836377107671482
58 0.822894467138872
59 0.826305631740284
60 0.828563773941682
61 0.854962425944362
62 0.740601486240018
63 0.811804393151771
64 0.837970481157164
65 0.822586158998555
66 0.827298494412292
67 0.819311744571756
68 0.813313862189825
69 0.82395483244899
70 0.820388229444996
71 0.832437217189864
72 0.822975983993556
73 0.831705789505634
74 0.831662110316162
75 0.826358464649759
76 0.868232640428202
77 0.827173081583811
78 0.831947780073461
79 0.833512106141414
80 0.824587953728211
81 0.818943027336997
82 0.820640414919042
83 0.821784058286994
84 0.822043781099701
85 0.81513891266092
86 0.824206798926259
87 0.821398060774491
88 0.824048555567065
89 0.817205134940377
90 0.829280009057454
91 0.828270136539932
92 0.82670595892061
93 0.872020113013928
94 0.859563301843965
95 0.813724938217462
96 0.831174553243274
97 0.821721747787421
98 0.826668644777224
99 0.814312314470351
};

\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.38791635632515
1 0.809663593769073
2 0.811363875865936
3 0.80935674905777
4 0.830630660057068
5 0.826349437236786
6 0.820511758327484
7 0.829760372638702
8 0.825872778892517
9 0.828033566474915
10 0.829770982265472
11 0.820557117462158
12 0.767916083335876
13 0.415938258171082
14 0.17235654592514
15 0.30888643860817
16 0.600125789642334
17 0.8580561876297
18 0.802439451217651
19 0.816631376743317
20 0.819722294807434
21 0.81808876991272
22 0.839973449707031
23 0.830553770065308
24 0.820995688438416
25 0.83802056312561
26 0.822195827960968
27 0.801854908466339
28 0.855909705162048
29 0.527463555335999
30 0.935936689376831
31 0.503949284553528
32 0.807916343212128
33 0.860178649425507
34 0.838254034519196
35 0.808788239955902
36 0.823217451572418
37 0.818634927272797
38 0.829017877578735
39 0.811773419380188
40 0.831569373607635
41 0.814422488212585
42 0.828739941120148
43 0.859415471553802
44 0.738388359546661
45 0.149847507476807
46 0.217756524682045
47 0.613010466098785
48 0.816859602928162
49 0.905339419841766
50 0.876816093921661
51 0.832728803157806
52 0.836308777332306
53 0.827017366886139
54 0.830262064933777
55 0.839296281337738
56 0.831186473369598
57 0.835998594760895
58 0.814124822616577
59 0.878619134426117
60 0.663001656532288
61 0.19840981066227
62 0.293882548809052
63 0.553405702114105
64 0.841938376426697
65 0.791566729545593
66 0.822006464004517
67 0.808370530605316
68 0.814030528068542
69 0.821397304534912
70 0.816991329193115
71 0.84095823764801
72 0.831969738006592
73 0.824436366558075
74 0.853964686393738
75 0.770241022109985
76 0.667362093925476
77 0.334358781576157
78 0.136207416653633
79 0.700898051261902
80 0.940162599086761
81 0.809885263442993
82 0.807765603065491
83 0.821919679641724
84 0.821602582931519
85 0.814516127109528
86 0.825706005096436
87 0.819207668304443
88 0.826983869075775
89 0.811128318309784
90 0.801678955554962
91 0.943620800971985
92 0.46420282125473
93 0.743762373924255
94 0.271379321813583
95 0.896448016166687
96 0.816296458244324
97 0.851639568805695
98 0.817529618740082
99 0.823586404323578
};

\nextgroupplot[
width=\w cm,
height=\h cm,
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_3(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_3(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_4(t)|\)},
xtick style={color=white},
xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.753602486017811
1 0.753602486017811
2 0.753602486017811
3 0.753602486017811
4 0.753602486017811
5 0.753602486017811
6 0.753602486017811
7 0.753602486017811
8 0.753602486017811
9 0.753602486017811
10 0.753602486017811
11 0.753602486017811
12 0.753602486017811
13 0.753602486017811
14 0.753602486017811
15 0.753602486017811
16 0.753602486017811
17 0.753602486017811
18 0.753602486017811
19 0.753602486017811
20 0.753602486017811
21 0.753602486017811
22 0.753602486017811
23 0.753602486017811
24 0.753602486017811
25 0.753602486017811
26 0.753602486017811
27 0.753602486017811
28 0.753602486017811
29 0.753602486017811
30 0.753602486017811
31 0.753602486017811
32 0.753602486017811
33 0.753602486017811
34 0.753602486017811
35 0.753602486017811
36 0.753602486017811
37 0.753602486017811
38 0.753602486017811
39 0.753602486017811
40 0.753602486017811
41 0.753602486017811
42 0.753602486017811
43 0.753602486017811
44 0.753602486017811
45 0.753602486017811
46 0.753602486017811
47 0.753602486017811
48 0.753602486017811
49 0.753602486017811
50 0.753602486017811
51 0.753602486017811
52 0.753602486017811
53 0.753602486017811
54 0.753602486017811
55 0.753602486017811
56 0.753602486017811
57 0.753602486017811
58 0.753602486017811
59 0.753602486017811
60 0.753602486017811
61 0.753602486017811
62 0.753602486017811
63 0.753602486017811
64 0.753602486017811
65 0.753602486017811
66 0.753602486017811
67 0.753602486017811
68 0.753602486017811
69 0.753602486017811
70 0.753602486017811
71 0.753602486017811
72 0.753602486017811
73 0.753602486017811
74 0.753602486017811
75 0.753602486017811
76 0.753602486017811
77 0.753602486017811
78 0.753602486017811
79 0.753602486017811
80 0.753602486017811
81 0.753602486017811
82 0.753602486017811
83 0.753602486017811
84 0.753602486017811
85 0.753602486017811
86 0.753602486017811
87 0.753602486017811
88 0.753602486017811
89 0.753602486017811
90 0.753602486017811
91 0.753602486017811
92 0.753602486017811
93 0.753602486017811
94 0.753602486017811
95 0.753602486017811
96 0.753602486017811
97 0.753602486017811
98 0.753602486017811
99 0.753602486017811
};
\addplot [semithick, red,line width=\LineWidth pt, dashed]
table {%
0 0.744312885445358
1 0.750145302976525
2 0.749372505673031
3 0.756830826840838
4 0.748954109833765
5 0.75718645880117
6 0.762101387654458
7 0.74649277714792
8 0.753602442755578
9 0.75929758276741
10 0.740730585447671
11 0.749457785503976
12 0.754379657614837
13 0.759675529300396
14 0.745336696207046
15 0.742459731771324
16 0.735150583683766
17 0.748989912358059
18 0.750810762767991
19 0.744921630586411
20 0.75616180183063
21 0.750085327793229
22 0.753802038295956
23 0.752136638653569
24 0.755192798032651
25 0.750825519412615
26 0.751127224312082
27 0.740538069622995
28 0.762066440052782
29 0.748666707363959
30 0.752288006323508
31 0.751753973595254
32 0.753185377279395
33 0.755345039796396
34 0.746195852943536
35 0.746208541237575
36 0.749602301675725
37 0.754914710511251
38 0.749375321783963
39 0.749656682933103
40 0.753887813854902
41 0.758932400237673
42 0.748278504785143
43 0.75688291733854
44 0.752898287591649
45 0.751506679910491
46 0.7605239708646
47 0.746409608204736
48 0.760514882492448
49 0.746009689406713
50 0.749472130232735
51 0.754854758619252
52 0.746047522628315
53 0.757950271441173
54 0.746271405673436
55 0.75463722491097
56 0.757187801857191
57 0.750349429714616
58 0.755874918052498
59 0.755895160202646
60 0.746690953238923
61 0.742176830180024
62 0.757953045956879
63 0.753103126064889
64 0.762249193142054
65 0.758509044739513
66 0.75929606188031
67 0.754493640341368
68 0.759448746958087
69 0.756224318738386
70 0.753670848571637
71 0.7518422007279
72 0.755301626285992
73 0.75537288645068
74 0.745334819341235
75 0.7511516065497
76 0.743105813338925
77 0.759309565683203
78 0.762848423538424
79 0.761514663483381
80 0.74224528906373
81 0.74594464758368
82 0.757244391653364
83 0.75267480436799
84 0.756120425685906
85 0.745611311160968
86 0.756288385784629
87 0.75711088201433
88 0.755686748346984
89 0.749852444157929
90 0.749650914703587
91 0.755607551430982
92 0.751133432682657
93 0.752274788276908
94 0.760244566285533
95 0.753193649647226
96 0.754808820205393
97 0.762573739904946
98 0.758326231221221
99 0.760016263558548
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.923561275005341
1 0.758681774139404
2 0.812664747238159
3 0.728205680847168
4 0.726023435592651
5 0.771603345870972
6 0.773307740688324
7 0.745272278785706
8 0.743736326694489
9 0.754860520362854
10 0.754252552986145
11 0.758989989757538
12 0.787811279296875
13 0.890000224113464
14 0.457785844802856
15 0.895297288894653
16 0.773442447185516
17 0.762913703918457
18 0.761586129665375
19 0.720979928970337
20 0.778913080692291
21 0.747560739517212
22 0.75444632768631
23 0.754404962062836
24 0.752886831760406
25 0.740675330162048
26 0.756522536277771
27 0.743163883686066
28 0.770288646221161
29 0.691148281097412
30 0.0184182990342379
31 0.636222004890442
32 0.719721555709839
33 0.78613942861557
34 0.758181989192963
35 0.73831832408905
36 0.750155866146088
37 0.749254643917084
38 0.752664983272552
39 0.757528960704803
40 0.755178391933441
41 0.767184853553772
42 0.750407993793488
43 0.742161870002747
44 0.771335542201996
45 0.777085661888123
46 0.234231367707253
47 0.818614780902863
48 0.742025971412659
49 0.791922032833099
50 0.782577037811279
51 0.765272617340088
52 0.751100361347198
53 0.766118288040161
54 0.755999982357025
55 0.749653816223145
56 0.760315954685211
57 0.763567328453064
58 0.765497624874115
59 0.734116733074188
60 0.806763231754303
61 0.258817225694656
62 0.210253402590752
63 0.815788984298706
64 0.756227791309357
65 0.776630043983459
66 0.754565358161926
67 0.762407243251801
68 0.749622404575348
69 0.741739571094513
70 0.748193025588989
71 0.75121545791626
72 0.756034851074219
73 0.768006920814514
74 0.725206673145294
75 0.750736951828003
76 0.423705905675888
77 0.121831580996513
78 0.878886699676514
79 0.712534844875336
80 0.808556318283081
81 0.773256659507751
82 0.756121456623077
83 0.759470462799072
84 0.758029460906982
85 0.74524861574173
86 0.764563083648682
87 0.756761193275452
88 0.753634989261627
89 0.754580616950989
90 0.77182924747467
91 0.697900116443634
92 0.585890173912048
93 0.0266057606786489
94 0.85356467962265
95 0.764797449111938
96 0.744692206382751
97 0.790704309940338
98 0.749305665493011
99 0.753730475902557
};

\nextgroupplot[
width=\w cm,
height=\h cm,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.95, xmax=\xmax,
y grid style={darkgray176},
%ylabel={\(\displaystyle |\cos\phi_5(t)|\)},
xlabel style ={color=black,font=\footnotesize},
ylabel style ={color=black,font=\footnotesize},
ymin=0, ymax=1.2,
title style ={color=black,font=\footnotesize},
%-------- Horizantal ----
% xtick style={color=black,font=\footnotesize},
% xlabel = {time \(t\)},
% title={\(\displaystyle |\cos\phi_5(t)|\)},
%xlabel = {time \(t\)},
%-------- Vertical ----
%ylabel={\(\displaystyle |\cos\phi_5(t)|\)},
%xtick style={color=white},
%xticklabels={},
yticklabels={},
ytick style={color=white},
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\addplot [semithick, blue,line width=\LineWidth pt]
table {%
0 0.935826238137458
1 0.935826238137458
2 0.935826238137458
3 0.935826238137458
4 0.935826238137458
5 0.935826238137458
6 0.935826238137458
7 0.935826238137458
8 0.935826238137458
9 0.935826238137458
10 0.935826238137458
11 0.935826238137458
12 0.935826238137458
13 0.935826238137458
14 0.935826238137458
15 0.935826238137458
16 0.935826238137458
17 0.935826238137458
18 0.935826238137458
19 0.935826238137458
20 0.935826238137458
21 0.935826238137458
22 0.935826238137458
23 0.935826238137458
24 0.935826238137458
25 0.935826238137458
26 0.935826238137458
27 0.935826238137458
28 0.935826238137458
29 0.935826238137458
30 0.935826238137458
31 0.935826238137458
32 0.935826238137458
33 0.935826238137458
34 0.935826238137458
35 0.935826238137458
36 0.935826238137458
37 0.935826238137458
38 0.935826238137458
39 0.935826238137458
40 0.935826238137458
41 0.935826238137458
42 0.935826238137458
43 0.935826238137458
44 0.935826238137458
45 0.935826238137458
46 0.935826238137458
47 0.935826238137458
48 0.935826238137458
49 0.935826238137458
50 0.935826238137458
51 0.935826238137458
52 0.935826238137458
53 0.935826238137458
54 0.935826238137458
55 0.935826238137458
56 0.935826238137458
57 0.935826238137458
58 0.935826238137458
59 0.935826238137458
60 0.935826238137458
61 0.935826238137458
62 0.935826238137458
63 0.935826238137458
64 0.935826238137458
65 0.935826238137458
66 0.935826238137458
67 0.935826238137458
68 0.935826238137458
69 0.935826238137458
70 0.935826238137458
71 0.935826238137458
72 0.935826238137458
73 0.935826238137458
74 0.935826238137458
75 0.935826238137458
76 0.935826238137458
77 0.935826238137458
78 0.935826238137458
79 0.935826238137458
80 0.935826238137458
81 0.935826238137458
82 0.935826238137458
83 0.935826238137458
84 0.935826238137458
85 0.935826238137458
86 0.935826238137458
87 0.935826238137458
88 0.935826238137458
89 0.935826238137458
90 0.935826238137458
91 0.935826238137458
92 0.935826238137458
93 0.935826238137458
94 0.935826238137458
95 0.935826238137458
96 0.935826238137458
97 0.935826238137458
98 0.935826238137458
99 0.935826238137458
};
\addplot [semithick, red,line width=\LineWidth pt,dashed]
table {%
0 0.935726150173863
1 0.93243961841364
2 0.93921734782486
3 0.934797838242867
4 0.934765878335273
5 0.93116336813743
6 0.937557542129138
7 0.93333039329831
8 0.936135503235224
9 0.937702836400306
10 0.933920674411142
11 0.934487840204236
12 0.939852244628269
13 0.936551655188784
14 0.935280800881848
15 0.933642891716116
16 0.93698737136278
17 0.933408334829361
18 0.934978084903416
19 0.93689682400204
20 0.936761243538514
21 0.938060523437731
22 0.936462998883943
23 0.931816892830289
24 0.936615468509104
25 0.935888691459032
26 0.939788832354102
27 0.93445003697207
28 0.932602630817031
29 0.935329173542147
30 0.939415932670573
31 0.936969050208336
32 0.937496888298838
33 0.934723380185841
34 0.931876702750954
35 0.937384734118943
36 0.933716970854448
37 0.938239744821582
38 0.932015780842149
39 0.937017888852623
40 0.928551957877256
41 0.937102010854516
42 0.937553474190904
43 0.937602283929877
44 0.93411419070571
45 0.931241922509268
46 0.934052503535191
47 0.937175587365241
48 0.93418306357709
49 0.937874784170481
50 0.930990253432719
51 0.935977730103398
52 0.942296162232066
53 0.932367639435983
54 0.938751936541214
55 0.933863075299372
56 0.93604556530815
57 0.932692904108187
58 0.938251062517302
59 0.9402160948667
60 0.939254328657195
61 0.932503610850312
62 0.931681560011444
63 0.9383239476249
64 0.929706718707422
65 0.937300298820287
66 0.935641950369204
67 0.940221224524749
68 0.938693786806183
69 0.935283896637598
70 0.935090177755212
71 0.939155665690211
72 0.934488163732142
73 0.940061692342151
74 0.932410525252131
75 0.933154713774036
76 0.926617127257696
77 0.935827726713862
78 0.940743859049868
79 0.937287733433823
80 0.932138572114068
81 0.934128504702678
82 0.936266506581613
83 0.936101693048245
84 0.940762464769514
85 0.938845608550584
86 0.932478616623485
87 0.937598107831344
88 0.939808418156011
89 0.937886122124791
90 0.929393581048477
91 0.940424598257889
92 0.932107200515594
93 0.936507359456714
94 0.931334659571307
95 0.93385197265234
96 0.934801914164692
97 0.937521232116435
98 0.937746276714059
99 0.939103663165208
};
\addplot [semithick, green,line width=\LineWidth pt, dotted]
table {%
0 0.956074178218842
1 0.938155770301819
2 0.952183961868286
3 0.936433434486389
4 0.926474153995514
5 0.930754661560059
6 0.941973268985748
7 0.93296205997467
8 0.936621308326721
9 0.939718842506409
10 0.920438766479492
11 0.931900084018707
12 0.933652639389038
13 0.903177201747894
14 0.923016965389252
15 0.938697814941406
16 0.954071223735809
17 0.929714679718018
18 0.944002449512482
19 0.93270069360733
20 0.945581912994385
21 0.941534280776978
22 0.928662478923798
23 0.924749553203583
24 0.939432501792908
25 0.929706215858459
26 0.940755665302277
27 0.939660131931305
28 0.933214664459229
29 0.94721257686615
30 0.639336407184601
31 0.924092233181
32 0.933331549167633
33 0.939467430114746
34 0.930497527122498
35 0.9411700963974
36 0.932563364505768
37 0.937459528446198
38 0.927198112010956
39 0.943719625473022
40 0.926074266433716
41 0.943654000759125
42 0.931573629379272
43 0.919138491153717
44 0.93605375289917
45 0.872532784938812
46 0.885390043258667
47 0.924163162708282
48 0.931880712509155
49 0.928919434547424
50 0.926474511623383
51 0.935193717479706
52 0.934517085552216
53 0.939999043941498
54 0.93684047460556
55 0.933618724346161
56 0.940797209739685
57 0.926825761795044
58 0.940532982349396
59 0.946876764297485
60 0.914888978004456
61 0.907902240753174
62 0.805208086967468
63 0.913837313652039
64 0.92917937040329
65 0.949209988117218
66 0.940537512302399
67 0.947905898094177
68 0.935285747051239
69 0.93757039308548
70 0.940599322319031
71 0.932528853416443
72 0.928886890411377
73 0.931137919425964
74 0.93419337272644
75 0.941826343536377
76 0.922441601753235
77 0.892448663711548
78 0.927221775054932
79 0.941948413848877
80 0.925938367843628
81 0.944169104099274
82 0.939713001251221
83 0.93705677986145
84 0.944431483745575
85 0.935272574424744
86 0.929677367210388
87 0.936905860900879
88 0.936744689941406
89 0.93546324968338
90 0.921470642089844
91 0.944058358669281
92 0.96014940738678
93 0.789682805538177
94 0.916668653488159
95 0.911668419837952
96 0.935774385929108
97 0.932552754878998
98 0.938856244087219
99 0.933424353599548
};

\end{groupplot}

==> Figs/temp.tex <==
\begin{groupplot}[group style={group size=1 by 5,horizontal sep=0.2cm,
vertical sep=0.1cm, group name=left3 plots }]

%================= Fig1 ===============
\firstgplot{1}

%================= Fig2 ===============
\nextgplot{2}
%================= Fig3 ===============
\nextgplot{3}
%================= Fig4 ===============
\nextgplot{4}
%================= Fig5 ===============
\lastgplot{5}

\end{groupplot}

==> Figs/time_freq.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
width=4cm,
height= 3cm,
%legend cell align={left},
% %legend style={
%   fill opacity=0.8,
%   draw opacity=1,
%   text opacity=1,
%   at={(0,0)},
%   %anchor=south,
%   draw=lightgray204
% },
log basis y={10},
%tick align=outside,
tick pos=left,
ylabel={\footnotesize{\(|\mr{H}_{0,0}(t)|\)}},
%ylabel={\(|H_{0,0}(t)|\)},
x grid style={darkgray176},
xlabel={\footnotesize{$t (time)$}},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={darkgray176},
ymin=0.000189809486832061, ymax=1.40467801843624,
ymode=log,
ytick style={color=black},
ytick={1e-05,0.0001,0.001,0.01,0.1,1,10,100},
xtick={0,1,2,3,4,5},
yticklabels={
  \(\displaystyle {10^{-5}}\),
  \(\displaystyle {10^{-4}}\),
  \(\displaystyle {10^{-3}}\),
  \(\displaystyle {10^{-2}}\),
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\)
},
xticklabels={
  \({0}\),
  \({\tau}\),
  \({2\tau}\),
  \({3\tau}\),
  \({4\tau}\),
  \({5\tau}\)
}
]
\pgfplotsset{every tick label/.append style={font=\footnotesize},}
\path [draw=blue, semithick]
(axis cs:0,0.000485968333161077)
--(axis cs:0,1e-5);

\path [draw=blue, semithick]
(axis cs:1,0.249815545648551)
--(axis cs:1,1e-5);

\path [draw=blue, semithick]
(axis cs:2,0.579393678101871)
--(axis cs:2,1e-05);

\path [draw=blue, semithick]
(axis cs:3,0.936917569338035)
--(axis cs:3,1e-5);

\path [draw=blue, semithick]
(axis cs:4,0.167854977552195)
--(axis cs:4,1e-5);

\path [draw=blue, semithick]
(axis cs:5,0.000284572754924465)
--(axis cs:5,1e-5);

\addplot [semithick, blue, mark=*, mark size=3, mark options={solid}, only marks, forget plot]
table {%
0 0.000485968333161077
1 0.249815545648551
2 0.579393678101871
3 0.936917569338035
4 0.167854977552195
5 0.000284572754924465
};
% \addplot [semithick, crimson2143940, forget plot]
% table {%
% 0 0
% 5 0
% };
\end{axis}

\end{tikzpicture}

